Confidence Interval and Uncertainty Propagation Analysis of SAFT-type Equations of State

Thermodynamic models and, in particular, SAFT-type equations are vital in characterizing complex systems. This paper presents a framework for sampling parameter distributions in PC-SAFT and SAFT-VR Mie equations of state to understand parameter confidence intervals and correlations. We identify conserved quantities contributing to significant correlations. Comparing the equations of state, we find that additional parameters introduced in the SAFT-VR Mie equation increase relative uncertainties (1\%-2\% to 3\%-4\%) and introduce more correlations. When incorporating association through additional parameters, relative uncertainties increase, but correlations slightly decrease. We investigate how uncertainties propagate to derived properties and observe small uncertainties for that data with which the parameters were regressed, especially for saturated-liquid volumes. However, extrapolating to saturated-vapour volumes yields larger uncertainties due to the larger isothermal compressibility. Near the critical point, uncertainties in saturated volumes diverge due to increased sensitivity of the isothermal compressibility to parameter uncertainties. This effect significantly impacts bulk properties, particularly isobaric heat capacity, where uncertainties near the critical point become extremely large, even when these uncertainties are small. We emphasize that even small uncertainties near the critical point lead to divergences in predicted properties.

==> references <==

@article{rehner_surfactant_2021,
	title = {Surfactant {Modeling} {Using} {Classical} {Density} {Functional} {Theory} and a {Group} {Contribution} {PC}-{SAFT} {Approach}},
	volume = {60},
	issn = {0888-5885},
	url = {https://doi.org/10.1021/acs.iecr.1c00169},
	doi = {10.1021/acs.iecr.1c00169},
	abstract = {Models for surfactants need to incorporate the amphiphilic character of the molecules to describe key properties such as the adsorption at interfaces and the reduction of interfacial tensions. One possibility is to model the surfactant molecules as heteronuclear chains. Therefore, we revisit the heterosegmented density functional theory and present a theory consistent with the group contribution perturbed-chain statistical associating fluid theory equation of state. The model is used to study water/surfactant and water/surfactant/octane systems with surfactants from the group of polyethylene glycol alkyl ethers, a commonly used group of nonionic surfactants. The model parameters are obtained by fitting to pure component data of small surfactants. Binary interaction parameters are required to model the water/alkane subsystem and to account for the polarity of the head groups of the surfactant. The model is able to reproduce the significant enrichment of surfactant molecules at both vapor–liquid surfaces and liquid–liquid interfaces and the corresponding reduction of interfacial tensions. For liquid–liquid interfaces, the competing solubility of the surfactant in both phases has to be taken into account when searching for an optimal surfactant molecule.},
	number = {19},
	urldate = {2022-12-09},
	journal = {Industrial \& Engineering Chemistry Research},
	author = {Rehner, Philipp and Bursik, Benjamin and Gross, Joachim},
	month = may,
	year = {2021},
	note = {Publisher: American Chemical Society},
	pages = {7111--7123},
}

@article{sauer_comparison_2014,
	title = {Comparison between a {Homo}- and a {Heterosegmented} {Group} {Contribution} {Approach} {Based} on the {Perturbed}-{Chain} {Polar} {Statistical} {Associating} {Fluid} {Theory} {Equation} of {State}},
	volume = {53},
	issn = {0888-5885},
	url = {https://doi.org/10.1021/ie502203w},
	doi = {10.1021/ie502203w},
	abstract = {Depending on the molecular model, group contribution (GC) approaches based on the statistical associating fluid theory (SAFT) can be classified in homosegmented and heterosegmented GC approaches. In homosegmented GC approaches, molecules are modeled as chains composed of identical segments. Heterosegmented GC approaches, on the other hand, consider molecular chains composed of different segment types and thus maintain a more detailed picture of real molecules. Therefore, heterosegmented GC approaches are arguably more physically realistic and ought to give more accurate descriptions of thermodynamic properties. In this work, we evaluate the performance of a homosegmented and a heterosegmented GC approach based on the perturbed-chain polar SAFT (PCP-SAFT) equation of state (EoS). To ensure a meaningful comparison between both GC approaches, a dipole term for the heterosegmented GC approach is formulated. Group parameters of 22 functional groups were adjusted to pure component property data. The comparison between both GC approaches shows that the heterosegmented GC approach leads to significantly better agreement with experimental data for various chemical families.},
	number = {38},
	urldate = {2022-12-09},
	journal = {Industrial \& Engineering Chemistry Research},
	author = {Sauer, Elmar and Stavrou, Marina and Gross, Joachim},
	month = sep,
	year = {2014},
	note = {Publisher: American Chemical Society},
	pages = {14854--14864},
}

@article{xu_density-functional_2012,
	title = {Density-{Functional} {Theory} for {Polymer}–{Carbon} {Dioxide} {Mixtures}},
	volume = {51},
	issn = {0888-5885},
	url = {https://doi.org/10.1021/ie2029267},
	doi = {10.1021/ie2029267},
	abstract = {We propose a new density-functional theory (DFT) describing inhomogeneous polymer–carbon dioxide (CO2) mixtures. The theory is constructed by combining the bulk Peng–Robinson equation of state (PR-EOS) with the statistical associating fluid theory (SAFT) and the fundamental measure theory (FMT). The weight density functions from FMT are used to extend the bulk excess Helmholtz free energy of PR-EOS to the inhomogeneous case, while the SAFT is used to describe correlations due to polymer chain connectivity and short-range forces due to weakly polar or association interactions. The additional long-range dispersion contributions are included using a mean-field approach. We apply our DFT to the interfacial properties of polystyrene–CO2 and poly(methyl methacrylate)–CO2 systems. The calculated interfacial tension values are in good agreement with experimental data at low to intermediate pressures. The inclusion of association energy for CO2 is shown to have a significant effect. We also point out the limitation of the PR-EOS for describing polymer–CO2 mixtures at high pressures (P {\textgreater} 35 MPa).},
	number = {9},
	urldate = {2022-12-01},
	journal = {Industrial \& Engineering Chemistry Research},
	author = {Xu, Xiaofei and Cristancho, Diego E. and Costeux, Stéphane and Wang, Zhen-Gang},
	month = mar,
	year = {2012},
	pages = {3832--3840},
}

@misc{noauthor_rigorous_nodate,
	title = {Rigorous {Phase} {Equilibrium} {Calculation} {Methods} for {Strong} {Electrolyte} {Solutions}: {The} {Isothermal} {Flash} {\textbar} {Elsevier} {Enhanced} {Reader}},
	shorttitle = {Rigorous {Phase} {Equilibrium} {Calculation} {Methods} for {Strong} {Electrolyte} {Solutions}},
	url = {https://reader.elsevier.com/reader/sd/pii/S0378381222000668?token=0EB50FD26CF9288251E91F1B634BF2E22BC350EFFBA6FCFBCC7FB5255FF811F40D755B26EC86CC5F3C646E0CCBB75FD2&originRegion=us-east-1&originCreation=20221201011847},
	language = {en},
	urldate = {2022-12-01},
	doi = {10.1016/j.fluid.2022.113441},
}

@misc{noauthor_rigorous_nodate-1,
	title = {Rigorous {Phase} {Equilibrium} {Calculation} {Methods} for {Strong} {Electrolyte} {Solutions}: {The} {Isothermal} {Flash} {\textbar} {Elsevier} {Enhanced} {Reader}},
	shorttitle = {Rigorous {Phase} {Equilibrium} {Calculation} {Methods} for {Strong} {Electrolyte} {Solutions}},
	url = {https://reader.elsevier.com/reader/sd/pii/S0378381222000668?token=0EB50FD26CF9288251E91F1B634BF2E22BC350EFFBA6FCFBCC7FB5255FF811F40D755B26EC86CC5F3C646E0CCBB75FD2&originRegion=us-east-1&originCreation=20221201011847},
	language = {en},
	urldate = {2022-12-01},
	doi = {10.1016/j.fluid.2022.113441},
}

@article{jiang_thermodynamic_2001,
	title = {Thermodynamic properties and phase equilibria of charged hard sphere chain model for polyelectrolyte solutions},
	volume = {99},
	issn = {0026-8976},
	url = {https://doi.org/10.1080/00268970110043414},
	doi = {10.1080/00268970110043414},
	abstract = {A recent thermodynamic perturbation theory for flexible polyelectrolyte solutions is extended to study thermodynamic properties and phase equilibria for polyelectrolyte solutions with different polyion, chain lengths. Osmotic pressure, activity coefficient of an individual ion (polyion or counterion) and average activity coefficient are calculated. Except for the activity coefficient of the polyion, the chain length dependence of the properties is small. Also presented are vapour-liquid equilibrium coexisting curves, vapour pressures and critical points. As the polyion chain length approaches infinity the critical properties (temperature, pressure and density) become constants.},
	number = {13},
	urldate = {2022-11-29},
	journal = {Molecular Physics},
	author = {JIANG, J. W. and BLUM, L. and BERNARD, O. and PRAUSNITZ, J. M.},
	month = jul,
	year = {2001},
	note = {Publisher: Taylor \& Francis
\_eprint: https://doi.org/10.1080/00268970110043414},
	pages = {1121--1128},
}

@article{stockmayer_theory_1944,
	title = {Theory of {Molecular} {Size} {Distribution} and {Gel} {Formation} in {Branched} {Polymers} {II}. {General} {Cross} {Linking}},
	volume = {12},
	issn = {0021-9606},
	url = {https://aip.scitation.org/doi/10.1063/1.1723922},
	doi = {10.1063/1.1723922},
	number = {4},
	urldate = {2022-11-29},
	journal = {The Journal of Chemical Physics},
	author = {Stockmayer, Walter H.},
	month = apr,
	year = {1944},
	note = {Publisher: American Institute of Physics},
	pages = {125--131},
}

@article{stockmayer_theory_1944-1,
	title = {Theory of {Molecular} {Size} {Distribution} and {Gel} {Formation} in {Branched} {Polymers} {II}. {General} {Cross} {Linking}},
	volume = {12},
	issn = {0021-9606, 1089-7690},
	url = {http://aip.scitation.org/doi/10.1063/1.1723922},
	doi = {10.1063/1.1723922},
	language = {en},
	number = {4},
	urldate = {2022-11-29},
	journal = {The Journal of Chemical Physics},
	author = {Stockmayer, Walter H.},
	month = apr,
	year = {1944},
	pages = {125--131},
}

@article{xu_density-functional_2012-1,
	title = {Density-functional theory for polymer-carbon dioxide mixtures: {A} perturbed-chain {SAFT} approach},
	volume = {137},
	issn = {0021-9606},
	shorttitle = {Density-functional theory for polymer-carbon dioxide mixtures},
	url = {https://aip.scitation.org/doi/full/10.1063/1.4742346},
	doi = {10.1063/1.4742346},
	abstract = {We propose a density-functional theory (DFT) describing inhomogeneous polymer-carbon dioxide mixtures based on a perturbed-chain statistical associating fluid theory equation of state (PC-SAFT EOS). The weight density functions from fundamental measure theory are used to extend the bulk excess Helmholtz free energy to the inhomogeneous case. The additional long-range dispersion contributions are included using a mean-field approach. We apply our DFT to the interfacial properties of polystyrene-CO2 and poly(methyl methacrylate) CO2 systems. Calculated values for both solubility and interfacial tension are in good agreement with experimental data. In comparison with our earlier DFT based on the Peng-Robinson-SAFT EOS, the current DFT produces quantitatively superior agreement with experimental data and is free of the unphysical behavior at high pressures ({\textgreater}35 MPa) in the earlier theory.},
	number = {5},
	urldate = {2022-11-23},
	journal = {The Journal of Chemical Physics},
	author = {Xu, Xiaofei and Cristancho, Diego E. and Costeux, Stéphane and Wang, Zhen-Gang},
	month = aug,
	year = {2012},
	note = {Publisher: American Institute of Physics},
	pages = {054902},
}

@article{ermoshkin_polyelectrolytes_2003,
	title = {Polyelectrolytes in the {Presence} of {Multivalent} {Ions}: {Gelation} {Versus} {Segregation}},
	volume = {90},
	shorttitle = {Polyelectrolytes in the {Presence} of {Multivalent} {Ions}},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.90.125504},
	doi = {10.1103/PhysRevLett.90.125504},
	abstract = {We analyze solutions of strongly charged chains bridged by linkers such as multivalent ions. The gelation induced by the strong short range electrostatic attractions is dramatically suppressed by the long range electrostatic correlations due to the charge along the non-cross-linked monomers and ions. A modified Debye-Hückel approach of cross-linked clusters of charged chains is used to determine the mean field gelation transition self-consistently. Highly dilute polyelectrolyte solutions tend to segregate macroscopically. Semidilute solutions can form gels if the Bjerrum length lB and the distance between neighboring charged monomers along the chain b are both greater than the ion size a.},
	number = {12},
	urldate = {2022-11-22},
	journal = {Physical Review Letters},
	author = {Ermoshkin, A. V. and Olvera de la Cruz, M.},
	month = mar,
	year = {2003},
	note = {Publisher: American Physical Society},
	pages = {125504},
}

@article{ermoshkin_thermoreversible_2004,
	title = {Thermoreversible crosslinking of polyelectrolyte chains},
	volume = {120},
	issn = {0021-9606},
	url = {https://aip.scitation.org/doi/abs/10.1063/1.1753573},
	doi = {10.1063/1.1753573},
	number = {24},
	urldate = {2022-11-22},
	journal = {The Journal of Chemical Physics},
	author = {Ermoshkin, A. V. and Kudlay, A. N. and Olvera de la Cruz, M.},
	month = jun,
	year = {2004},
	note = {Publisher: American Institute of Physics},
	pages = {11930--11940},
}

@article{jacobs_quantifying_2021,
	title = {Quantifying the {Effect} of {Multivalent} {Ions} in {Polyelectrolyte} {Solutions}},
	volume = {54},
	issn = {0024-9297},
	url = {https://doi.org/10.1021/acs.macromol.1c01326},
	doi = {10.1021/acs.macromol.1c01326},
	abstract = {We implemented a scaling approach, based on the relationship between the solution correlation length ξ = lgν/B and the number of repeat units per correlation blob g for polymers with repeat unit projection length l, to quantify properties of solutions of carboxymethylcellulose and polystyrene sulfonate with monovalent and divalent counterions. The parameter B is equal to Bpe, Bg, Bth, and 1, and the exponent v = 1, 0.588, 0.5, and 1 in semidilute polyelectrolyte solutions, solutions of overlapping electrostatic and thermal blobs, and concentrated polymer solutions, which are separated by crossover concentrations cD, cth, and c**, respectively. The values of the B-parameters are obtained using the linear relationship between the specific viscosity ηsp(c) in the unentangled solution regime and the number of correlation blobs Nw/g per chain, with the weight-average degree of polymerization, Nw, and g = B3/(3ν–1)(cl3)1/(1–3ν) as a function of the repeat unit concentration, c, and the B-parameters in different solution regimes. This analysis shows that (i) there is only a small fraction of free counterions, f* {\textless} 12\%; (ii) divalent ions have a strong effect on the renormalization of the excluded volume, reducing it by a factor of 2; and (iii) the effect of divalent counterions is much weaker on the renormalization of the Kuhn length, accounting for an increase of up to 10\%. In combination, these effects significantly reduce chain stretching, increase the number of repeat units per solution correlation length, and promote chain disentanglement in polyelectrolyte solutions with divalent ions in comparison with that in solutions with monovalent counterions. There is an indication of chain bridging by Ca2+ ions in concentrated solutions of carboxymethylcellulose, manifested as an increase in solution viscosity. The concentration dependence of the solution correlation length ξ calculated using the set of B-parameters is in good agreement with that obtained from the peak position of the scattering function for concentrations c {\textless} cD.},
	number = {20},
	urldate = {2022-11-22},
	journal = {Macromolecules},
	author = {Jacobs, Michael and Lopez, Carlos G. and Dobrynin, Andrey V.},
	month = oct,
	year = {2021},
	note = {Publisher: American Chemical Society},
	pages = {9577--9586},
}

@misc{noauthor_gelation_nodate,
	title = {Gelation in strongly charged polyelectrolytes - {Ermoshkin} - 2004 - {Journal} of {Polymer} {Science} {Part} {B}: {Polymer} {Physics} - {Wiley} {Online} {Library}},
	url = {https://onlinelibrary.wiley.com/doi/full/10.1002/polb.10752},
	urldate = {2022-11-22},
}

@article{wilcox_fundamentals_2021,
	title = {Fundamentals and mechanics of polyelectrolyte gels: {Thermodynamics}, swelling, scattering, and elasticity},
	volume = {2},
	copyright = {© 2021 Author(s).},
	shorttitle = {Fundamentals and mechanics of polyelectrolyte gels},
	url = {https://aip.scitation.org/doi/abs/10.1063/5.0048152},
	doi = {10.1063/5.0048152},
	abstract = {Polyelectrolyte gels are ionizable, crosslinked polymer networks swollen in a solvent. These materials are prevalent in biological and synthetic applications ranging from the extracellular matrix to personal care products because they swell and deswell according to changes in the solution environment and internal structure. These environmental and internal factors include temperature, solvent, salt, pH, polymer volume fraction, and crosslink density. In order to predict useful properties like swelling and modulus, 70+ years of effort have been taken to understand the thermodynamic driving forces that affect polyelectrolyte gels. Here, we consider the current thermodynamic model of polyelectrolyte gel behavior, which includes balancing the mixing, electrostatic, Donnan, and elastic osmotic pressures, and we present current experimental results in the context of this model. Since the internal free energy of polyelectrolyte gels results in structural and modulus changes, we also review how thermodynamics are linked to rheological and scattering studies. Due to the complex nature of polyelectrolyte gels, the influence of the solution environment on gel behavior and structure has been investigated; however, the current findings are convoluted with multiple equilibrium states and there is a need for greater understanding of the influence of counterion condensation, interfaces, and inhomogeneities. By describing the current state of the thermodynamic model for polyelectrolyte behavior, we emphasize the complexity and tunability of polyelectrolyte gels for future applications. We propose the future direction of polyelectrolyte gel research to focus on gels at interfaces, in human biology, and on gel inhomogeneities. However, these future directions require an understanding of polyelectrolyte gel mechanical properties, structure, and complex nature that can be understood using the current thermodynamic model.},
	language = {en},
	number = {4},
	urldate = {2022-11-22},
	journal = {Chemical Physics Reviews},
	author = {Wilcox, Kathryn G. and Kozawa, Susan K. and Morozova, Svetlana},
	month = dec,
	year = {2021},
	note = {Publisher: AIP Publishing LLCAIP Publishing},
	pages = {041309},
}

@article{ermoshkin_polyelectrolytes_2003-1,
	title = {Polyelectrolytes in the {Presence} of {Multivalent} {Ions}: {Gelation} {Versus} {Segregation}},
	volume = {90},
	shorttitle = {Polyelectrolytes in the {Presence} of {Multivalent} {Ions}},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.90.125504},
	doi = {10.1103/PhysRevLett.90.125504},
	abstract = {We analyze solutions of strongly charged chains bridged by linkers such as multivalent ions. The gelation induced by the strong short range electrostatic attractions is dramatically suppressed by the long range electrostatic correlations due to the charge along the non-cross-linked monomers and ions. A modified Debye-Hückel approach of cross-linked clusters of charged chains is used to determine the mean field gelation transition self-consistently. Highly dilute polyelectrolyte solutions tend to segregate macroscopically. Semidilute solutions can form gels if the Bjerrum length lB and the distance between neighboring charged monomers along the chain b are both greater than the ion size a.},
	number = {12},
	urldate = {2022-11-22},
	journal = {Physical Review Letters},
	author = {Ermoshkin, A. V. and Olvera de la Cruz, M.},
	month = mar,
	year = {2003},
	note = {Publisher: American Physical Society},
	pages = {125504},
}

@article{yu_structures_2002,
	title = {Structures of hard-sphere fluids from a modified fundamental-measure theory},
	volume = {117},
	issn = {0021-9606},
	url = {https://aip.scitation.org/doi/10.1063/1.1520530},
	doi = {10.1063/1.1520530},
	number = {22},
	urldate = {2022-11-19},
	journal = {The Journal of Chemical Physics},
	author = {Yu, Yang-Xin and Wu, Jianzhong},
	month = dec,
	year = {2002},
	note = {Publisher: American Institute of Physics},
	pages = {10156--10164},
}

@article{sauer_classical_2017,
	title = {Classical {Density} {Functional} {Theory} for {Liquid}–{Fluid} {Interfaces} and {Confined} {Systems}: {A} {Functional} for the {Perturbed}-{Chain} {Polar} {Statistical} {Associating} {Fluid} {Theory} {Equation} of {State}},
	volume = {56},
	issn = {0888-5885},
	shorttitle = {Classical {Density} {Functional} {Theory} for {Liquid}–{Fluid} {Interfaces} and {Confined} {Systems}},
	url = {https://doi.org/10.1021/acs.iecr.6b04551},
	doi = {10.1021/acs.iecr.6b04551},
	abstract = {A Helmholtz energy functional based on the Perturbed-Chain Polar Statistical Associating Fluid Theory Equation of State is proposed. A weighted density approximation is used to develop two variants of dispersion functionals. We conduct molecular simulations (Monte Carlo) in order to assess both models. The structure of thin liquid adsorbed layers of a few molecular diameters thickness are shown to be particularly meaningful to detect deficiencies of Helmholtz energy functionals and thus discriminate between models. We further compare the model to experimental data of interfacial tensions for pure components and for binary mixtures exhibiting vapor–liquid equilibria and liquid–liquid equilibria. The proposed Helmholtz energy functional is in good agreement with experimental data of pure (organic) substances and mixtures and compares well with molecular simulation data of fluids adsorbing at solid interfaces.},
	number = {14},
	urldate = {2022-11-19},
	journal = {Industrial \& Engineering Chemistry Research},
	author = {Sauer, Elmar and Gross, Joachim},
	month = apr,
	year = {2017},
	note = {Publisher: American Chemical Society},
	pages = {4119--4135},
}

@article{camacho_vergara_study_2020,
	title = {On the study of the vapor-liquid interface of associating fluids with classical density functional theory},
	volume = {522},
	issn = {0378-3812},
	url = {https://www.sciencedirect.com/science/article/pii/S0378381220302910},
	doi = {10.1016/j.fluid.2020.112744},
	abstract = {Classical density functional theory (DFT) is applied to study the vapor-liquid interface of associating fluids. Our classical DFT implementation uses a Helmholtz free energy functional that reduces to the perturbed-chain statistical associating fluid theory (PC-SAFT) equation of state in the bulk limit. We apply a new association functional, presented in one of our previous works, based on the weighted density approximation to calculate the interfacial tension of associating fluids and compare them with two of the most used association functionals from literature. It is found that classical DFT with the three association functionals and the current molecular parameters of PC-SAFT is not able to predict satisfactorily the interfacial tension of alkanols. Therefore, the experimental interfacial tension of alkanols and some associating fluids is included in the determination of the pure molecular parameters of PC-SAFT. With this approach the determination of interfacial tension of pure associating fluids can be greatly improved with the new parameters, but at the expense of slightly higher deviations in the vapor pressure. The new parameters are tested for the determination of vapor-liquid equilibria (VLE) and the prediction of interfacial tension of binary mixtures containing at least one associating compound. Good agreement is found between experimental data of VLE and interfacial tension of the binary mixtures and the three association functionals. Furthermore, we discuss about the limitations and capabilities of the current classical DFT implementation in the study of the vapor-liquid interface of associating fluids.},
	language = {en},
	urldate = {2022-11-19},
	journal = {Fluid Phase Equilibria},
	author = {Camacho Vergara, Edgar L. and Kontogeorgis, Georgios M. and Liang, Xiaodong},
	month = nov,
	year = {2020},
	keywords = {Associating fluids, Classical density functional theory, Interfacial tension},
	pages = {112744},
}

@article{sauer_classical_2017-1,
	title = {Classical {Density} {Functional} {Theory} for {Liquid}–{Fluid} {Interfaces} and {Confined} {Systems}: {A} {Functional} for the {Perturbed}-{Chain} {Polar} {Statistical} {Associating} {Fluid} {Theory} {Equation} of {State}},
	volume = {56},
	issn = {0888-5885, 1520-5045},
	shorttitle = {Classical {Density} {Functional} {Theory} for {Liquid}–{Fluid} {Interfaces} and {Confined} {Systems}},
	url = {https://pubs.acs.org/doi/10.1021/acs.iecr.6b04551},
	doi = {10.1021/acs.iecr.6b04551},
	abstract = {A Helmholtz energy functional based on the Perturbed-Chain Polar Statistical Associating Fluid Theory Equation of State is proposed. A weighted density approximation is used to develop two variants of dispersion functionals. We conduct molecular simulations (Monte Carlo) in order to assess both models. The structure of thin liquid adsorbed layers of a few molecular diameters thickness are shown to be particularly meaningful to detect deﬁciencies of Helmholtz energy functionals and thus discriminate between models. We further compare the model to experimental data of interfacial tensions for pure components and for binary mixtures exhibiting vapor−liquid equilibria and liquid−liquid equilibria. The proposed Helmholtz energy functional is in good agreement with experimental data of pure (organic) substances and mixtures and compares well with molecular simulation data of ﬂuids adsorbing at solid interfaces.},
	language = {en},
	number = {14},
	urldate = {2022-11-19},
	journal = {Industrial \& Engineering Chemistry Research},
	author = {Sauer, Elmar and Gross, Joachim},
	month = apr,
	year = {2017},
	pages = {4119--4135},
}

@article{klink_density_2014,
	title = {A {Density} {Functional} {Theory} for {Vapor}–{Liquid} {Interfaces} of {Mixtures} {Using} the {Perturbed}-{Chain} {Polar} {Statistical} {Associating} {Fluid} {Theory} {Equation} of {State}},
	volume = {53},
	issn = {0888-5885},
	url = {https://doi.org/10.1021/ie4029895},
	doi = {10.1021/ie4029895},
	abstract = {A density functional theory based on the perturbed-chain polar statistical associating fluid theory (PCP-SAFT) is extended to mixtures. The Helmholtz energy functional is suitable for inhomogeneous fluid phases and is here applied to vapor–liquid systems. The attractive branch of the van der Waals attractions are treated with a perturbation theory of first order in a nonmean field approach. The radial distribution function is considered in the Percus–Yevick closure for chain fluids with a three-fluid theory approach. This perturbation term is brought to consistency with the PCP-SAFT equation of state using the approach of Gloor et al. [Gloor, G. J.; Jackson, G.; Blas, F. J.; del Rio, E. M.; de Miguel, E. J. Chem. Phys. 2004, 121, 12740]. The approach is applied to vapor–liquid interfaces of mixtures and the resulting surface tension is compared to experimental data. Binary mixtures with two subcritical components as well as mixtures with one species above its critical point, for the considered temperature, are considered. The density functional theory is applied to these systems with unaltered pure component parameters of the PC-SAFT or PCP-SAFT model. The binary interaction parameter was determined to bulk-phase vapor–liquid data (temperature, pressure, composition) only. Excellent agreement was found for the surface tension of mixtures without any model parameter adjusted to interfacial properties.},
	number = {14},
	urldate = {2022-11-19},
	journal = {Industrial \& Engineering Chemistry Research},
	author = {Klink, Christoph and Gross, Joachim},
	month = apr,
	year = {2014},
	note = {Publisher: American Chemical Society},
	pages = {6169--6178},
}

@misc{noauthor_density_nodate,
	title = {A density functional theory for vapor-liquid interfaces using the {PCP}-{SAFT} equation of state: {The} {Journal} of {Chemical} {Physics}: {Vol} 131, {No} 20},
	url = {https://aip.scitation.org/doi/10.1063/1.3263124},
	urldate = {2022-11-19},
}

@article{noauthor_numerical_2017,
	title = {Numerical aspects of classical density functional theory for one-dimensional vapor-liquid interfaces},
	volume = {444},
	issn = {0378-3812},
	url = {https://www.sciencedirect.com/science/article/pii/S0378381217301231},
	doi = {10.1016/j.fluid.2017.03.023},
	abstract = {This study compares different algorithms for solving the equations of classical density functional theory for the one-dimensional vapor-liquid interfa…},
	language = {en},
	urldate = {2022-11-19},
	journal = {Fluid Phase Equilibria},
	month = jul,
	year = {2017},
	note = {Publisher: Elsevier},
	pages = {1--12},
}

@article{lazarou_development_nodate,
	title = {Development of the {SAFT}-γ {Mie} equation of state for predicting the thermodynamic behaviour of strong and weak electrolyte solutions},
	language = {en},
	author = {Lazarou, Georgia},
	pages = {294},
}

@article{lazarou_development_2017,
	title = {Development of the {SAFT}-γ {Mie} equation of state for predicting the thermodynamic behaviour of strong and weak electrolyte solutions},
	url = {http://spiral.imperial.ac.uk/handle/10044/1/60588},
	doi = {10.25560/60588},
	abstract = {The thermodynamic modelling of fluid mixtures containing electrolytes using the SAFT-γ 
Mie equation of state is addressed in detail in this thesis. The SAFT-γ Mie approach 
allows the implementation of heteronuclear molecules using a group-contribution formalism, 
and offers a versatile framework for developing models to describe molecules of varying 
chemical functionality for a broad range of physical properties. In the present work, the 
SAFT-γ Mie equation of state is extended to electrolyte mixtures with the incorporation 
of the primitive unrestricted mean spherical approximation (MSA-PM) for describing the 
Coulombic ion–ion interactions, and the Born solvation free energy to implicitly treat ion– 
solvent polar interactions. Novel reformulations of the MSA-PM and Born theories within a 
group-contribution framework are proposed in order to enable ionic species of any size and 
chemical structure to be modelled, from small inorganic ions to large non-spherical charged 
molecules. Taking carboxylate anions in linear alkyl chain molecules as an illustrative case 
study, the proposed theory is shown to effectively account for localised charge effects arising 
from the structural topology of the charged species. A holistic description of electrolyte 
solutions is employed in this work; in addition to the short-range dispersion forces and 
the long-range Coulombic interactions which are pertinent to such mixtures, the models 
developed here also account for the formation of hydrogen bonds, ion-pairing phenomena, 
and electrolyte dissociation equilibria. The proposed SAFT-γ Mie equation of state is used to 
model aqueous solutions of strong electrolytes including alkali halide salts, hydrogen halide 
acids, and alkali hydroxide bases. Aqueous solutions of sulphuric acid and nitric acid are 
studied in detail by modelling these as speciating weak electrolytes. Finally, the treatment of 
ion-pairing phenomena is investigated through a consideration of aqueous alkali nitrate salt 
solutions. This work presents a new theoretical formulation and SAFT-γ Mie group models 
for twenty species in total.},
	language = {en-US-GB},
	urldate = {2022-11-17},
	author = {Lazarou, Georgia},
	month = sep,
	year = {2017},
	note = {Accepted: 2018-07-05T10:46:39Z
Publisher: Imperial College London},
}

@article{weidlich_modified_1987,
	title = {A modified {UNIFAC} model. 1. {Prediction} of {VLE}, hᴱ, and γ᪲},
	volume = {26},
	issn = {0888-5885},
	url = {https://pubs.acs.org/doi/abs/10.1021/ie00067a018},
	doi = {10.1021/ie00067a018},
	number = {7},
	journal = {Ind. Eng. Chem. Res.},
	author = {Weidlich, Ulrich and Gmehling, Juergen},
	month = jul,
	year = {1987},
	pages = {1372--1381},
}

@article{lange_predicting_2016,
	title = {Predicting the {Aqueous} {Solubility} of {Pharmaceutical} {Cocrystals} {As} a {Function} of {pH} and {Temperature}},
	volume = {16},
	issn = {1528-7483},
	url = {https://doi.org/10.1021/acs.cgd.6b00024},
	doi = {10.1021/acs.cgd.6b00024},
	abstract = {The solubility of pharmaceutical cocrystals in aqueous solution is influenced by pH-dependent dissociation and salt formation which complicates the design of cocrystal formation and purification processes. To increase the efficiency of those processes, the aqueous solubility of pharmaceutical cocrystals was predicted in this work using perturbed-chain statistical associating fluid theory (PC-SAFT). Modeling results and experimental data of pH-dependent solubilities were compared for the weak base nicotinamide, the weak acid succinic acid, their 2:1 cocrystal, as well as for all occurring salts at 298.15 and 310.15 K. It was found that the pH-dependent acid–base equilibria of nicotinamide and succinic acid directly influence the solubility of their cocrystal and their salts. By accounting for the thermodynamic nonideality of the components in the cocrystal system, PC-SAFT is able to predict the solubility behavior of all above-mentioned components in good agreement with the experimental data.},
	number = {5},
	urldate = {2022-11-11},
	journal = {Cryst. Growth Des.},
	author = {Lange, Linda and Lehmkemper, Kristin and Sadowski, Gabriele},
	month = may,
	year = {2016},
	note = {Publisher: American Chemical Society},
	pages = {2726--2740},
}

@article{rashid_effect_2014,
	title = {Effect of {Solvent} {Composition} and {Temperature} on the {Solubility} of {Ibuprofen} in {Aqueous} {Ethanol}},
	volume = {59},
	issn = {0021-9568, 1520-5134},
	url = {https://pubs.acs.org/doi/10.1021/je400819z},
	doi = {10.1021/je400819z},
	abstract = {The solubilities of ibuprofen [(R,S)-2-(4-(2-methylpropyl)phenyl)propanoic acid] in absolute ethanol and in water−ethanol mixtures were measured at temperatures from 10 °C to 40 °C, the expected range relevant to its industrial crystallization. The solubility studies were carried out by dissolution of ibuprofen crystals in stirred Schott bottles kept in a constant temperature bath. The ibuprofen concentration in the clear supernatant at equilibrium was determined by vacuum drying. An allowance was made for the small amount of sublimation from dried ibuprofen. In absolute ethanol, the experimental results showed that the solubility increased as a square law with temperature, from 0.59 g of ibuprofen/g ethanol at 10.0 °C to 2.15 g/g at 40.0 °C. The results are considered to be accurate to within ±1\% (as 95\% conﬁdence). In water−ethanol mixtures, the solubility of ibuprofen (expressed as w/w ibuprofen/solvent) generally decreased with increasing water addition. At 40 °C and possibly at 25 °C, the solubility initially increased slightly to a maximum level as a small amount of water was added before then decreasing. At 40 °C, phase separation into two immiscible liquid layers was observed for solvent concentrations from 34 to 64\% ethanol on an ibuprofen-free basis.},
	language = {en},
	number = {9},
	urldate = {2022-08-01},
	journal = {J. Chem. Eng. Data},
	author = {Rashid, Abdur and White, Edward T. and Howes, Tony and Litster, James D. and Marziano, Ivan},
	month = sep,
	year = {2014},
	pages = {2699--2703},
}

@article{alessi_liquid-liquid_1989,
	title = {Liquid-liquid equilibrium of cyclohexane-n-hexane-methanol mixtures: effect of water content},
	volume = {34},
	issn = {0021-9568},
	shorttitle = {Liquid-liquid equilibrium of cyclohexane-n-hexane-methanol mixtures},
	url = {https://doi.org/10.1021/je00056a026},
	doi = {10.1021/je00056a026},
	number = {2},
	urldate = {2022-11-11},
	journal = {J. Chem. Eng. Data},
	author = {Alessi, Paolo and Fermeglia, Maurizio and Kikic, Ireneo},
	month = apr,
	year = {1989},
	note = {Publisher: American Chemical Society},
	pages = {236--240},
}

@article{bell_application_2019,
	title = {Application of the group contribution volume translated {Peng}–{Robinson} equation of state to new commercial refrigerant mixtures},
	volume = {103},
	issn = {0140-7007},
	url = {https://www.sciencedirect.com/science/article/pii/S0140700719301707},
	doi = {10.1016/j.ijrefrig.2019.04.014},
	abstract = {This work evaluates the performance of the group contribution volume translated Peng–Robinson model when predicting the vapor–liquid equilibrium and single phase densities of 28 refrigerant mixtures with low global warming potential and zero ozone depletion potential. Cubic equations of state, and particularly the Peng–Robinson equation of state, are widely used in the refrigeration industry due to their easy applicability for new substances, and their low computational time, although generally lower prediction accuracies must be expected compared to multiparameter equations of state. The group contribution volume translated Peng–Robinson equation of state combines the Peng–Robinson equation of state with a new attraction term, improved mixing rules using a group contribution approach, and volume translation. The results are compared with the estimates obtained using the non-volume-translated Peng–Robinson equation of state, and a multiparameter equation of state.},
	language = {en},
	urldate = {2022-11-10},
	journal = {Int. J. Refrig.},
	author = {Bell, I. H. and Welliquet, J. and Mondejar, M. E. and Bazyleva, A. and Quoilin, S. and Haglind, F.},
	month = jul,
	year = {2019},
	keywords = {Cubic equation of state, GC-VTPR, Mélanges de frigorigènes, Peng-Robinson, Peng–Robinson, Refrigerant mixtures, UNIFAC, Équation d’état cubique},
	pages = {316--328},
}

@article{schmid_extension_2014,
	title = {Extension of the {VTPR} {Group} {Contribution} {Equation} of {State}: {Group} {Interaction} {Parameters} for {Additional} 192 {Group} {Combinations} and {Typical} {Results}},
	volume = {53},
	issn = {0888-5885},
	shorttitle = {Extension of the {VTPR} {Group} {Contribution} {Equation} of {State}},
	url = {https://doi.org/10.1021/ie404118f},
	doi = {10.1021/ie404118f},
	abstract = {Today development, design, and optimization of the various processes is carried out with the help of process simulators. The reliability of the results mainly depends on the quality of the thermodynamic model and the model parameters used. While gE models can be applied for calculation of the phase equilibrium behavior of multicomponent systems using only binary experimental data, group contribution methods like UNIFAC or modified UNIFAC Dortmund allow prediction of the required thermophysical properties using only a limited number of group interaction parameters. For systems containing supercritical components equations of state like Soave–Redlich–Kwong or Peng–Robinson or group contribution equations of state (GCEOS) like the predictive Soave–Redlich–Kwong (PSRK) or the volume-translated Peng–Robinson group contribution equations of state (VTPR) can be applied. In different papers it was already shown that VTPR is a very powerful thermodynamic model. In this paper new group interaction parameters for 192 group combinations are presented, so that the actual matrix now contains group interaction parameters for 252 group combinations. In this paper predicted results of the VTPR group contribution equation of state are compared with the results obtained using modified UNIFAC Dortmund or the PSRK method.},
	number = {8},
	urldate = {2022-11-10},
	journal = {Ind. Eng. Chem. Res.},
	author = {Schmid, Bastian and Schedemann, Andre and Gmehling, Jürgen},
	month = feb,
	year = {2014},
	note = {Publisher: American Chemical Society},
	pages = {3393--3405},
}

@article{polishuk_estimation_2004,
	title = {Estimation of {Liquid}--{Liquid}--{Vapor} {Equilibria} in {Binary} {Mixtures} of n-{Alkanes}},
	volume = {43},
	issn = {0888-5885},
	url = {https://doi.org/10.1021/ie049797j},
	doi = {10.1021/ie049797j},
	abstract = {This study tests the ability of the best presently available semipredictive models, namely, predictive Soave−Redlich−Kwong (PSRK), linear combination of Vidal mixing rules (LCVM), and the novel global phase diagram approach (GPDA), to estimate the three-phase liquid−liquid−vapor equilibrium (LLVE) in the homologous series methane−n-alkanes, ethane−n-alkanes, propane−n-alkanes, and n-butane−n-alkanes. It is demonstrated that at high pressures GE mixing rules predict the wrong shape of the liquid−liquid critical curves, which involves fictitious closed loops of liquid−liquid equilibrium. Such a behavior is responsible for predicting nonrealistic three-phase LLVE behavior along the homologous series under consideration. In addition, both PSRK and LCVM fail in estimating the lower critical end-point curve. The results presented here for the GE-based models under consideration are probably characteristic for them. In contrast, GPDA is consistent in the entire thermodynamic phase space and does not predict nonphysical results. Although GPDA tends to underestimate the temperatures of the end points and to overestimate the double critical end points, its results are at least qualitatively accurate.},
	number = {18},
	urldate = {2022-11-10},
	journal = {Ind. Eng. Chem. Res.},
	author = {Polishuk, Ilya and Wisniak, Jaime and Segura, Hugo},
	month = sep,
	year = {2004},
	note = {Publisher: American Chemical Society},
	pages = {5957--5964},
}

@article{polishuk_standardized_2014,
	title = {Standardized {Critical} {Point}-{Based} {Numerical} {Solution} of {Statistical} {Association} {Fluid} {Theory} {Parameters}: {The} {Perturbed} {Chain}-{Statistical} {Association} {Fluid} {Theory} {Equation} of {State} {Revisited}},
	volume = {53},
	issn = {0888-5885},
	shorttitle = {Standardized {Critical} {Point}-{Based} {Numerical} {Solution} of {Statistical} {Association} {Fluid} {Theory} {Parameters}},
	url = {https://doi.org/10.1021/ie502633e},
	doi = {10.1021/ie502633e},
	abstract = {The current study has aimed at developing an approach replacing the lists of the compound-specific molecular parameters attached to perturbed chain-statistical association fluid theory (PC-SAFT) by the entirely transparent and universal method for their derivation. The proposed approach requires limited data for the numerical solution of the PC-SAFT parameters, namely, the critical constants and the triple point liquid density. Its implementation has necessitated a careful re-evaluation of part of the PC-SAFT universal parameters matrix and some additional revisions. The resulting model appears to be virtually free of several undesired numerical pitfalls characteristic for PC-SAFT. The proposed equation of state (EoS) has been implemented for modeling data of nonpolar substances such as the light compounds, n-alkanes, and 1-alkenes and their mixtures. Using a large experimental database (more than 6000 points) it has been demonstrated that it exhibits remarkable precision in predicting the high-pressure liquid phase densities and sound velocities, with AAD hardly exceeding 3\% even in the cases of complex asymmetric mixtures. However, a major drawback of the proposed model is a poor accuracy of predicting the vacuum vapor pressures of heavy compounds away from their critical points.},
	number = {36},
	urldate = {2022-11-10},
	journal = {Ind. Eng. Chem. Res.},
	author = {Polishuk, Ilya},
	month = sep,
	year = {2014},
	note = {Publisher: American Chemical Society},
	pages = {14127--14141},
}

@article{moine_i-pc-saft_2019,
	title = {I-{PC}-{SAFT}: {An} {Industrialized} {Version} of the {Volume}-{Translated} {PC}-{SAFT} {Equation} of {State} for {Pure} {Components}, {Resulting} from {Experience} {Acquired} {All} through the {Years} on the {Parameterization} of {SAFT}-{Type} and {Cubic} {Models}},
	volume = {58},
	issn = {0888-5885},
	shorttitle = {I-{PC}-{SAFT}},
	url = {https://doi.org/10.1021/acs.iecr.9b04660},
	doi = {10.1021/acs.iecr.9b04660},
	abstract = {The SAFT and cubic models are often compared in the open literature. Usually, limitations and strengths of both types of equations of state (EoSs) are ascribed to their theoretical foundations. Little attention has been paid until now to the influence of parameterization choices on the performance of these EoSs. By parameterization, it is here meant the way or method used to attribute values to EoS component-dependent parameters. SAFT-type and cubic EoSs for pure compounds use two different parameterization methods: SAFT parameters are generally regressed on vapor pressure and liquid density data, whereas cubic models use as input parameters experimental values of the critical temperature, pressure, and acentric factor and are generally parameterized to exactly reproduce these three properties. As a consequence of these parameterization methods, SAFT EoSs overestimate critical pressures, whereas cubic EoSs fail in reproducing accurately liquid density data. To discuss the influence of parameterization methods on EoS performances, three different parameterization methods are considered and applied to both SAFT and cubic models. It is shown that by application of the same parameterization method, SAFT and cubic EoSs are equivalent as they exhibit similar accuracies for the correlation of vapor pressure, enthalpy of vaporization, heat capacity, and liquid density data. This study led us to conclude that EoSs requiring three component-dependent parameters cannot provide a simultaneous accurate prediction for all of the properties of a pure fluid. It is highlighted that the key point to get high accuracy (for nonassociating pure compounds) is to work with an EoS equivalent to a four-parameter corresponding-states principle, i.e., that requires the specification of four macroscopic properties for a given pure compound. Eventually, we have considered a volume-translated PC-SAFT EoS version involving four input parameters: the three classical ones (m, σ, and ε) and a volume-translation parameter (c). Such an EoS shows excellent performances: for no less than 587 nonassociating compounds, vapor pressure data are predicted with an error of 1.5\%, liquid heat capacity and enthalpy of vaporization are predicted with an error of 3\%, and liquid density data are predicted with an error of 4\%; critical temperatures and pressures are exactly reproduced.},
	number = {45},
	urldate = {2022-11-10},
	journal = {Ind. Eng. Chem. Res.},
	author = {Moine, Edouard and Piña-Martinez, Andrés and Jaubert, Jean-Noël and Sirjean, Baptiste and Privat, Romain},
	month = nov,
	year = {2019},
	note = {Publisher: American Chemical Society},
	pages = {20815--20827},
}

@article{fingerhut_comprehensive_2017,
	title = {Comprehensive {Assessment} of {COSMO}-{SAC} {Models} for {Predictions} of {Fluid}-{Phase} {Equilibria}},
	volume = {56},
	issn = {0888-5885},
	url = {https://doi.org/10.1021/acs.iecr.7b01360},
	doi = {10.1021/acs.iecr.7b01360},
	abstract = {Two recent and fully open source COSMO-SAC models are assessed for the first time on the basis of very large experimental data sets. The model performance of COSMO-SAC 2010 and COSMO-SAC-dsp (2013) is studied for vapor–liquid equilibrium (VLE) and infinite dilution activity coefficient (γi∞) predictions, and it is benchmarked with respect to the group contribution models UNIFAC and mod. UNIFAC(DO). For this purpose, binary mixture combinations of 2 295 components are investigated. This leads to 10 897 γi∞ and 6 940 VLE mixtures, which correspond to 29 173 γi∞ and 139 921 VLE data points. The model performance is analyzed in terms of chemical families. A MATLAB program is provided for the interested reader to study the models in detail. The comprehensive assessment shows that there is a clear improvement from COSMO-SAC 2010 to COSMO-SAC-dsp and from UNIFAC to mod. UNIFAC(DO). The mean absolute deviation of γi∞ predictions is reduced from 95\% to 86\% (COSMO-SAC 2010 to COSMO-SAC-dsp) and from 73\% to 58\% (UNIFAC to mod. UNIFAC(DO)). A combined mean absolute deviation is introduced to study the temperature, pressure, and vapor mole fraction errors of VLE predictions, and it is reduced from 4.77\% to 4.63\% (COSMO-SAC 2010 to COSMO-SAC-dsp) and from 4.47\% to 3.51\% (UNIFAC to mod. UNIFAC(DO)). Detailed error analyses show that the accuracy of COSMO-SAC models mainly depends on chemical family types, but not on the molecular size asymmetry or polarity. The present results may serve as a reference for the reliability of predictions with COSMO-SAC methods and provide direction for future developments.},
	number = {35},
	urldate = {2022-11-11},
	journal = {Ind. Eng. Chem. Res.},
	author = {Fingerhut, Robin and Chen, Wei-Lin and Schedemann, Andre and Cordes, Wilfried and Rarey, Jürgen and Hsieh, Chieh-Ming and Vrabec, Jadran and Lin, Shiang-Tai},
	month = sep,
	year = {2017},
	note = {Publisher: American Chemical Society},
	pages = {9868--9884},
}

@article{schmid_revised_2012,
	title = {Revised parameters and typical results of the {VTPR} group contribution equation of state},
	volume = {317},
	issn = {0378-3812},
	url = {https://www.sciencedirect.com/science/article/pii/S0378381212000076},
	doi = {10.1016/j.fluid.2012.01.006},
	abstract = {Group contribution methods like UNIFAC or modified UNIFAC and group contribution equations of state such as PSRK and VTPR are ideal tools for the development of the different processes in chemical industry, where the latter methods have the advantage that they can be applied for supercritical compounds. With the development of VTPR the weaknesses of the PSRK model (poor results for activity coefficients at infinite dilution, excess enthalpies, asymmetric systems, liquid densities) were as far as possible removed. With the application for systems with strongly polar compounds, such as water, alcohols, etc., the VTPR model had to be revised. For example new fragmentation rules and van der Waals surfaces had to be used, and further thermophysical properties and a sophisticated procedure had to be applied for the simultaneous fit of the temperature-dependent group interaction parameters to a comprehensive data base. In this paper the required parameters for different group combinations are given. Furthermore the quality of the results of the group contribution equation of state VTPR is demonstrated on various examples of industrial interest.},
	language = {en},
	urldate = {2022-11-10},
	journal = {Fluid Phase Equilib},
	author = {Schmid, Bastian and Gmehling, Jürgen},
	month = mar,
	year = {2012},
	keywords = {Group contribution equation of state, Revised fragmentation rules, Revised group interaction parameters, Revised van der Waals surface areas, VTPR},
	pages = {110--126},
}

@article{jager_combination_2018,
	title = {A combination of multi-fluid mixture models with {COSMO}-{SAC}},
	volume = {476},
	issn = {0378-3812},
	url = {https://www.sciencedirect.com/science/article/pii/S0378381218303108},
	doi = {10.1016/j.fluid.2018.08.004},
	abstract = {Recently, a new theoretically based departure function for multi-fluid mixture models has been proposed, which allows for the combination of the multi-fluid mixture model with a model for the excess Gibbs energy [A. Jäger, I.H. Bell, C. Breitkopf, Fluid Phase Equilibria 469 (2018) 56–69]. In the aforementioned article, it is demonstrated that the combination of a multi-fluid mixture model with UNIFAC yields comparable or better results for phase equilibrium calculations than using standard mixing rules, i.e., linear mixing rules or Lorentz-Berthelot combining rules, for the binary mixtures of the components ethanol, ethane, carbon dioxide, propene, and benzene. In this work, this multi-fluid mixture model is combined with the predictive excess Gibbs energy model COSMO-SAC for the first time. Results for all binary mixtures of the components ethanol, ethane, carbon dioxide, propene, and benzene are compared to experimental data as well as to results of the multi-fluid mixture model with standard mixing rules. The combination of COSMO-SAC and the multi-fluid mixture model yields comparable or better results than the multi-fluid mixture model with standard mixing rules for the binary mixtures considered. One of the main advantages of multi-fluid mixture models in general is that any thermal equation of state can be used to model a component in the mixture. Multiparameter equations of state, the Soave-Redlich-Kwong equation of state, and the Peng-Robinson equation of state are employed for modeling the components in the mixtures. It is demonstrated that the mixture model also yields good results if instead of multiparameter equations of state cubic equations of state are used.},
	language = {en},
	urldate = {2022-11-10},
	journal = {Fluid Phase Equilib.},
	author = {Jäger, Andreas and Mickoleit, Erik and Breitkopf, Cornelia},
	month = nov,
	year = {2018},
	keywords = {COSMO-SAC, Excess Gibbs energy, Excess Helmholtz energy, Multi-fluid mixture model, Reference equations of state, Theoretically based departure function, Vapor-liquid equilibria},
	pages = {147--156},
}

@article{jager_theoretically_2018,
	title = {A theoretically based departure function for multi-fluid mixture models},
	volume = {469},
	issn = {0378-3812},
	url = {https://www.sciencedirect.com/science/article/pii/S0378381218301626},
	doi = {10.1016/j.fluid.2018.04.015},
	abstract = {Multi-fluid mixture models for highly accurate multiparameter equations of state have been applied very successfully in the past years in order to accurately model thermophysical properties of mixtures. The multi-fluid mixture model mainly relies on empirical reducing functions and for some mixtures also on departure functions, for which the mathematical structure is a priori unknown and thus must be determined during the fitting procedure. By applying standard mixing rules for the reducing functions and by omitting the departure function, the mixture model can also be used predictively. However, it is demonstrated in this work that the predictive capability of this type of mixture model is rather limited. Therefore, a new model is proposed, which is a combination of the multi-fluid model with excess Gibbs energy models. This new approach results in a theoretically based formulation for the departure function of the multi-fluid model. It is shown that the new model yields very good results for the description of binary mixtures of the components ethanol, ethane, carbon dioxide, propene, and benzene. While the state-of-the-art multi-fluid model with either predictive linear mixing rules or Lorentz-Berthelot combining rules for the parameters of the reducing functions does not represent the phase equilibria for the investigated binary mixtures well, and in case of the azeotropes predicts qualitatively wrong mixture behavior, the new model is capable of accurately representing the phase equilibria of all binary mixtures investigated.},
	language = {en},
	urldate = {2022-11-10},
	journal = {Fluid Phase Equilib.},
	author = {Jäger, Andreas and Bell, Ian H. and Breitkopf, Cornelia},
	month = aug,
	year = {2018},
	keywords = {Excess Gibbs energy, Excess Helmholtz energy, Multi-fluid mixture model, Reference equations of state, Theoretically based departure function, UNIFAC, Vapor-liquid equilibria},
	pages = {56--69},
}

@article{hradetzky_phase_1991,
	title = {Phase equilibria in binary and higher systems methanol + hydrocarbon(s): {Part} {I}. {Experimental} determination of liquid-liquid equilibrium data and their representation using the {NRTL} equation},
	volume = {69},
	issn = {0378-3812},
	shorttitle = {Phase equilibria in binary and higher systems methanol + hydrocarbon(s)},
	url = {https://www.sciencedirect.com/science/article/pii/037838129190040E},
	doi = {10.1016/0378-3812(91)90040-E},
	abstract = {Hradetzky, G. and Lempe, D.A., 1991. Phase equilibria in binary and higher systems methanol + hydrocarbon(s). Part I. Experimental determination of liquid-liquid equilibrium data and their representation using the NRTL equation. Fluid Phase Equilibria, 69: 285-301. New measurements of the liquid-liquid equilibrium were carried out in the binary system methanol + hexane in the temperature range from 293 K up to the critical solution temperature, and in the ternary system methanol + hexane + cyclohexane in the temperature range 293–313 K. A double-plait point appearing in the ternary system could be determined exactly with the help of a special ampoule technique. This system shows a remarkably strong temperature dependence of the LLE. The LLE data were correlated using the NRTL equation with temperature-dependent parameters. Reliable results were obtained for the LLE data of the binary and ternary systems. Systematic deviations arise if the modelling of the VLE data is additionally included.},
	language = {en},
	urldate = {2022-11-11},
	journal = {Fluid Phase Equilib.},
	author = {Hradetzky, G. and Lempe, D. A.},
	month = dec,
	year = {1991},
	pages = {285--301},
}

@article{doz_influence_2011,
	title = {Influence of temperature on the (liquid+liquid) equilibria of \{methanol+benzene+hexane\} ternary system},
	volume = {305},
	issn = {0378-3812},
	url = {https://www.sciencedirect.com/science/article/pii/S0378381211001087},
	doi = {10.1016/j.fluid.2011.02.022},
	abstract = {In order to show the influence of temperature on the liquid–liquid equilibria (LLE) of \{methanol(1)+benzene(2)+hexane(3)\} ternary system, equilibrium data at T=(278.15, 283.15, and 293.15)K are reported. The effect of the temperature on liquid–liquid equilibrium is determined and discussed. Ternary system is available from the literature at T=298K. All chemicals were quantified by gas chromatography using a thermal conductivity detector. The solubility data for methanol+hexane and the upper critical temperature (UCST) at 308.3K was reported. The tie line data for the ternary system were satisfactorily correlated by the Othmer and Tobias method, and the plait point coordinates for the three temperatures were estimated. Experimental data for the ternary system are compared with values calculated by the NRTL and UNIQUAC equations, and predicted by means of the UNIFAC group contribution method. It is found that the UNIQUAC and NRTL models provide similar good correlations of the equilibrium data at these three temperatures. Finally, the UNIFAC model predicts an immiscibility region larger than the experimental observed. Distribution coefficients were also analysed through distribution curves.},
	language = {en},
	number = {1},
	urldate = {2022-11-14},
	journal = {Fluid Phase Equilib.},
	author = {Doz, Mónica B. Gramajo de and Bonatti, Carlos M. and Lucena, María C. and González, Diego A. and Mancilla, Marcos E.},
	month = jun,
	year = {2011},
	keywords = {Benzene, Data, Hexane, Liquid–liquid equilibria, Methanol, Ternary system},
	pages = {34--38},
}

@article{held_epc-saft_2014,
	title = {{ePC}-{SAFT} revised},
	volume = {92},
	issn = {02638762},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0263876214002469},
	doi = {10.1016/j.cherd.2014.05.017},
	language = {en},
	number = {12},
	urldate = {2022-01-04},
	journal = {Chem. Eng. Res. Des.},
	author = {Held, Christoph and Reschke, Thomas and Mohammad, Sultan and Luza, Armando and Sadowski, Gabriele},
	month = dec,
	year = {2014},
	pages = {2884--2897},
}

@article{bhargava_modelling_2008,
	title = {Modelling room temperature ionic liquids},
	issn = {1359-7345, 1364-548X},
	url = {http://xlink.rsc.org/?DOI=b805384g},
	doi = {10.1039/b805384g},
	language = {en},
	number = {29},
	urldate = {2022-02-02},
	journal = {Chem. Commun.},
	author = {Bhargava, B. L. and Balasubramanian, Sundaram and Klein, Michael L.},
	year = {2008},
	pages = {3339},
}

@article{hao_nonrandom_2021,
	title = {Nonrandom two-liquid activity coefficient model with association theory},
	volume = {67},
	issn = {1547-5905},
	doi = {10.1002/aic.17061},
	abstract = {Considered one of the most versatile and widely used classical thermodynamic models to correlate phase equilibria behavior of nonideal systems, the nonrandom two-liquid (NRTL) theory does not explicitly account for specific chemical associations such as hydrogen bonding. This deficiency has been recognized as the cause for unsatisfactory representation of association systems like methanol–alkanes binaries. This work presents a practical approach to integrate Wertheim's perturbation theory for association contribution with the classical NRTL model. Specifically, the association contribution is calculated from pre-determined molecule-specific association strengths while the physical interaction contribution is captured with NRTL binary interaction parameters. The resulting association NRTL model correlates fluid phase equilibria of association systems with few adjustable parameters and offers improved predictive capability for higher order systems.},
	language = {en},
	number = {1},
	urldate = {2022-09-24},
	journal = {AIChE J.},
	author = {Hao, Yifan and Chen, Chau-Chyun},
	year = {2021},
	keywords = {phase equilibrium, thermodynamics/classical},
	pages = {e17061},
}

@article{specovius_tricritical_1981,
	title = {Tricritical phenomena in quasi-binary mixtures of hydrocarbons. 2. {Binary} ethane systems},
	volume = {85},
	issn = {0022-3654},
	url = {https://doi.org/10.1021/j150616a003},
	doi = {10.1021/j150616a003},
	number = {16},
	urldate = {2022-11-14},
	journal = {The Journal of Physical Chemistry},
	author = {Specovius, Juergen and Leiva, Miguel A. and Scott, Robert L. and Knobler, Charles M.},
	month = aug,
	year = {1981},
	note = {Publisher: American Chemical Society},
	pages = {2313--2316},
}

@book{michelsen_thermodynamic_2020,
	edition = {2nd},
	title = {Thermodynamic {Models}: {Fundamentals} and {Computational} {Aspects}},
	url = {https://tie-tech.com/new-book-release/},
	language = {en-US},
	urldate = {2022-11-14},
	publisher = {Tie-Line Publications},
	author = {Michelsen, Michael L. and Mollerup, Jorgen},
	month = oct,
	year = {2020},
}

@article{van_konynenburg_critical_1980,
	title = {Critical lines and phase equilibria in binary van der {Waals} mixtures},
	volume = {298},
	url = {https://royalsocietypublishing.org/doi/10.1098/rsta.1980.0266},
	doi = {10.1098/rsta.1980.0266},
	abstract = {The study of phase equilibria is historically one of the most important sources of information about the nature of intermolecular forces in non-electrolyte liquids and their mixtures. Many of the main features of vapour-liquid and liquid-liquid phase behaviour were already well characterized experimentally during the early part of this century, but the theoretical explanation of phase equilibria for a wide variety of substances and over a large range of pressures and temperatures has lagged far behind. This paper presents theoretical studies of phase equilibria in binary mixtures obeying the van der Waals equation, especially liquid-liquid equilibria that can occur at high pressures. The variety of fluid phase behaviour that occurs in binary mixtures can be qualitatively discussed in terms of the changes in thermodynamic properties near critical points. Upper critical solution temperatures (UCSTs) occur when a heterogeneous (two-phase) system becomes a homogeneous (one-phase) system when the temperature is raised. The maximum temperature along the temperature-mole fraction (T, x) coexistence curve for constant pressure is the UCST at this pressure. Lower critical solution temperatures (LCSTs) occur when a homogeneous system becomes a two-phase system when the temperature is increased. The LCST is at the minimum of the T, x coexistence curve. Thermodynamic considerations of critical points yield requirements for the curvature of the mixing functions plotted against x.},
	number = {1442},
	urldate = {2022-11-12},
	journal = {Philosophical Transactions of the Royal Society of London. Series A, Mathematical and Physical Sciences},
	author = {van Konynenburg, P. H. and Scott, R. L. and Rowlinson, John Shipley},
	month = dec,
	year = {1980},
	note = {Publisher: Royal Society},
	pages = {495--540},
}

@misc{noauthor_predicting_nodate,
	title = {Predicting the {Aqueous} {Solubility} of {Pharmaceutical} {Cocrystals} {As} a {Function} of {pH} and {Temperature} {\textbar} {Crystal} {Growth} \& {Design}},
	url = {https://pubs.acs.org/doi/10.1021/acs.cgd.6b00024},
	urldate = {2022-11-11},
}

@misc{noauthor_pii_nodate,
	title = {{PII}: 0378-3812(91)90040-{E} {\textbar} {Elsevier} {Enhanced} {Reader}},
	shorttitle = {{PII}},
	url = {https://reader.elsevier.com/reader/sd/pii/037838129190040E?token=A42791C384F9EC0BDD00083BB1C724F734D7E78EC7968422949F2FD8FFAE28A8F57527A3F576DF50847C4F951D9D1757&originRegion=us-east-1&originCreation=20221111014038},
	language = {en},
	urldate = {2022-11-11},
	doi = {10.1016/0378-3812(91)90040-E},
	note = {ISSN: 0378-3812},
}

@article{hradetzky_phase_1986,
	title = {Phase {Equilibria} in {Methanol} + {Hexane} or + {Heptane} ({Liquid}-{Liquid}) and {Methanol} + {Cyclohexane} ({Solid}-{Liquid}-{Liquid})},
	number = {3},
	journal = {Int. Data Ser. Sel. Data Mixtures Ser. A},
	author = {Hradetzky, G and Bittrich, H.J.},
	year = {1986},
	pages = {216--218},
}

@article{chung_group_2022,
	title = {Group {Contribution} and {Machine} {Learning} {Approaches} to {Predict} {Abraham} {Solute} {Parameters}, {Solvation} {Free} {Energy}, and {Solvation} {Enthalpy}},
	volume = {62},
	copyright = {All rights reserved},
	issn = {1549-9596, 1549-960X},
	url = {https://pubs.acs.org/doi/10.1021/acs.jcim.1c01103},
	doi = {10.1021/acs.jcim.1c01103},
	abstract = {We present a group contribution method (SoluteGC) and a machine learning model (SoluteML) to predict the Abraham solute parameters, as well as a machine learning model (DirectML) to predict solvation free energy and enthalpy at 298 K. The proposed group contribution method uses atom-centered functional groups with corrections for ring and polycyclic strain while the machine learning models adopt a directed message passing neural network. The solute parameters predicted from SoluteGC and SoluteML are used to calculate solvation energy and enthalpy via linear free energy relationships. Extensive data sets containing 8366 solute parameters, 20,253 solvation free energies, and 6322 solvation enthalpies are compiled in this work to train the models. The three models are each evaluated on the same test sets using both random and substructure-based solute splits for solvation energy and enthalpy predictions. The results show that the DirectML model is superior to the SoluteML and SoluteGC models for both predictions and can provide accuracy comparable to that of advanced quantum chemistry methods. Yet, even though the DirectML model performs better in general, all three models are useful for various purposes. Uncertain predicted values can be identiﬁed by comparing the three models, and when the 3 models are combined together, they can provide even more accurate predictions than any one of them individually. Finally, we present our compiled solute parameter, solvation energy, and solvation enthalpy databases (SoluteDB, dGsolvDBx, dHsolvDB) and provide public access to our ﬁnal prediction models through a simple web-based tool, software packages, and source code.},
	language = {en},
	number = {3},
	urldate = {2022-01-22},
	journal = {J. Chem. Inf. Model.},
	author = {Chung, Yunsie and Vermeire, Florence H. and Wu, Haoyang and Walker, Pierre and Abraham, Michael H. and Green, William H.},
	month = jan,
	year = {2022},
	pages = {433--446},
}

@misc{noauthor_gproms_2022,
	title = {{gPROMS}},
	url = {www.psenterprise.com/products/gproms},
	urldate = {2022-03-15},
	month = oct,
	year = {2022},
}

@article{vilcu_isothermal_2004,
	title = {Isothermal {Liquid}-{Vapor} {Equilibrium} in {Acetonitrile}-{Water} {System}},
	volume = {2},
	language = {en},
	journal = {Analele Universitii Bucuresti Chimie},
	author = {Vilcu, Rodica and Cenuse, Zoica},
	year = {2004},
	pages = {6},
}

@article{binous_calculation_2021,
	title = {Calculation of ternary liquid-liquid equilibrium data using arc-length continuation},
	volume = {3},
	issn = {2577-8196},
	url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/eng2.12296},
	doi = {10.1002/eng2.12296},
	abstract = {Liquid-liquid extraction is an important separation technique used in several chemical engineering processes. When experimental data are unavailable, reliable prediction of liquid-liquid equilibrium (LLE) data is essential for the optimal design of these processes. This paper describes a new methodology based on the application of the arc-length continuation numerical technique in order to compute LLE data using non-random two liquid or universal quasi-chemical activity coefficient models. This technique is straightforward to implement in Mathematica©. In addition, the arc-length method avoids the main disadvantage of root finding methods, such as Newton's method, for which the convergence often depends on the proper choice of an initial guess. Another advantage of the proposed approach, based on arc-length continuation, is that all LLE data are generated in one single calculation. Several case studies, involving the three main types of ternary systems (ie, Type I, II and 0), illustrate the proposed method. For type I, we study the following three ternary systems: (1) water-ethanol-benzene, (2) 5-hydroxymethylfurfural-1-butanol-water, and (3) methanol-benzene-water. We have selected, for type II systems, the following mixtures: (1) isobutyl alcohol-cyclohexane-water, (2) methanol-cyclohexane-water, and (3) 4-methyl-2-pentanone-2-butanol-water. For type 0 systems, we have chosen a mixture composed of DMSO-THF-water. Finally, for each case, our predicted results are benchmarked against the corresponding experimental data.},
	language = {en},
	number = {2},
	urldate = {2022-11-09},
	journal = {Engineering Reports},
	author = {Binous, Housam and Bellagi, Ahmed},
	year = {2021},
	note = {\_eprint: https://onlinelibrary.wiley.com/doi/pdf/10.1002/eng2.12296},
	keywords = {Mathematica©, NRTL and UNIQUAC models, arc-length continuation, liquid-liquid equilibrium data},
	pages = {e12296},
}

@article{binous_calculation_2021-1,
	title = {Calculation of ternary liquid-liquid equilibrium data using arc-length continuation},
	volume = {3},
	issn = {2577-8196},
	url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/eng2.12296},
	doi = {10.1002/eng2.12296},
	abstract = {Liquid-liquid extraction is an important separation technique used in several chemical engineering processes. When experimental data are unavailable, reliable prediction of liquid-liquid equilibrium (LLE) data is essential for the optimal design of these processes. This paper describes a new methodology based on the application of the arc-length continuation numerical technique in order to compute LLE data using non-random two liquid or universal quasi-chemical activity coefficient models. This technique is straightforward to implement in Mathematica©. In addition, the arc-length method avoids the main disadvantage of root finding methods, such as Newton's method, for which the convergence often depends on the proper choice of an initial guess. Another advantage of the proposed approach, based on arc-length continuation, is that all LLE data are generated in one single calculation. Several case studies, involving the three main types of ternary systems (ie, Type I, II and 0), illustrate the proposed method. For type I, we study the following three ternary systems: (1) water-ethanol-benzene, (2) 5-hydroxymethylfurfural-1-butanol-water, and (3) methanol-benzene-water. We have selected, for type II systems, the following mixtures: (1) isobutyl alcohol-cyclohexane-water, (2) methanol-cyclohexane-water, and (3) 4-methyl-2-pentanone-2-butanol-water. For type 0 systems, we have chosen a mixture composed of DMSO-THF-water. Finally, for each case, our predicted results are benchmarked against the corresponding experimental data.},
	language = {en},
	number = {2},
	urldate = {2022-11-09},
	journal = {Engineering Reports},
	author = {Binous, Housam and Bellagi, Ahmed},
	year = {2021},
	note = {\_eprint: https://onlinelibrary.wiley.com/doi/pdf/10.1002/eng2.12296},
	keywords = {Mathematica©, NRTL and UNIQUAC models, arc-length continuation, liquid-liquid equilibrium data},
	pages = {e12296},
}

@article{lhamblin_selective_2022,
	title = {Selective solvent conditions influence sequence development and supramolecular assembly in step-growth copolymerization},
	volume = {18},
	url = {https://pubs.rsc.org/en/content/articlelanding/2022/sm/d1sm01571k},
	doi = {10.1039/D1SM01571K},
	language = {en},
	number = {5},
	urldate = {2022-10-19},
	journal = {Soft Matter},
	author = {L. Hamblin, Ryan and Q. Nguyen, Nhu and H. DuBay, Kateri},
	year = {2022},
	note = {Publisher: Royal Society of Chemistry},
	pages = {943--955},
}

@article{nguyen_emergent_2022,
	title = {Emergent {Sequence} {Biasing} in {Step}-{Growth} {Copolymerization}: {Influence} of {Non}-{Bonded} {Interactions} and {Comonomer} {Reactivities}},
	volume = {126},
	issn = {1520-6106},
	shorttitle = {Emergent {Sequence} {Biasing} in {Step}-{Growth} {Copolymerization}},
	url = {https://doi.org/10.1021/acs.jpcb.2c04092},
	doi = {10.1021/acs.jpcb.2c04092},
	abstract = {The phase behavior and material properties of copolymers are intrinsically dependent on their primary comonomer sequences. Achieving precise control over monomer sequence in synthetic copolymerizations is challenging, as sequence determination is influenced not only by the reaction conditions and the properties of the reactants but also by the statistical nature of the copolymerization process itself. Mayo–Lewis reactivity ratios are often used to predict copolymer composition and sequence and are based on ratios of static reactivity constants. However, prior results have demonstrated that in a generic, solution-based step-growth A,B-copolymerization, relatively weak non-bonded attractions between certain monomer pairs induce emergent microphase separations. Such polymerization-driven separations lead to deviations from standard kinetics due to the emergent heterogeneities in reactant concentrations, which can also cause significant shifts in the resulting copolymer sequences. Previously, these effects were observed in systems where the activation energies were equal for all reaction pathways, that is, between all monomer pair combinations. In this work, we explore the combined effects on copolymerization kinetics of differences in both activation energies and non-bonded attractions between monomers and examine the sequences produced within this same step-growth copolymerization model. Our results indicate that altering activation energies influences the kinetics and sequences in a manner that also depends on the non-bonded attractions, showing that these effects may work in concert or in opposition to one another to bias the sequences formed. Non-standard kinetic behaviors and long-range sequence biasing are observed under certain conditions, and the extent of each clearly shifts as the reaction proceeds. These findings provide insight into the complex interplay between sequence and nascent oligomer phase behavior, highlighting the potential for exploiting emergent phase properties in the informed design of advanced sequence-biased materials.},
	number = {34},
	urldate = {2022-10-19},
	journal = {The Journal of Physical Chemistry B},
	author = {Nguyen, Nhu Q. and Hamblin, Ryan L. and DuBay, Kateri H.},
	month = sep,
	year = {2022},
	note = {Publisher: American Chemical Society},
	pages = {6585--6597},
}

@article{witman_lattice_2006,
	title = {A {Lattice} {Model} of {Vitrification} and {Gelation}},
	volume = {110},
	issn = {1520-6106},
	url = {https://doi.org/10.1021/jp051365e},
	doi = {10.1021/jp051365e},
	abstract = {In this work we introduce a simple lattice model with T-shaped molecules in two dimensions that exhibits a rich range of morphological behaviors. Depending on the volume fraction and quench path, this system can adopt uniform liquid, solution, and phase-separated states, as well as inhomogeneous glass or gel-like states, as revealed by dynamic mean-field simulations. An important characteristic of this system is the existence of a large number of degenerate low-energy states with small barriers that leads to a broad, kinetically explored landscape. The mean-field stability and phase diagram of this model is constructed and provides a useful guide for understanding the complex behaviors of the system. One striking feature is that there is a cascade of instabilities that converge to mark the onset of what we identify as the glass transition. Both dynamic mean-field and Monte Carlo simulations reveal glass-like relaxation dynamics. Our results lead to a picture of gelation as a continuation of the glass transition into the two-phase region, or equivalently, as an incomplete phase separation arrested by the onset of the glass transition.},
	number = {12},
	urldate = {2022-10-19},
	journal = {The Journal of Physical Chemistry B},
	author = {Witman, Jennifer E. and Wang, Zhen-Gang},
	month = mar,
	year = {2006},
	note = {Publisher: American Chemical Society},
	pages = {6312--6324},
}

@article{zheng_morphology_1995,
	title = {Morphology of {ABC} {Triblock} {Copolymers}},
	volume = {28},
	issn = {0024-9297, 1520-5835},
	url = {https://pubs.acs.org/doi/abs/10.1021/ma00125a026},
	doi = {10.1021/ma00125a026},
	abstract = {We present results from theoretical calculations of the morphological phase diagrams for ABC triblock copolymers in the strong segregation limit. The chain conformation free energy is approximated following an approach proposed by Ohta and Kawasaki. Our study focuses on two unique features of the ABC triblock copolymers, namely, the dependence of the morphology on the sequence of the triblock chain and the relative strength of the various interaction parameters. Our results compare favorably with experimental observations. In addition, we predict the existence of some new structures that have yet to be observed experimentally.},
	language = {en},
	number = {21},
	urldate = {2022-10-19},
	journal = {Macromolecules},
	author = {Zheng, Wei and Wang, Zhen-Gang},
	month = oct,
	year = {1995},
	pages = {7215--7223},
}

@article{kumar_gelation_2001,
	title = {Gelation in {Physically} {Associating} {Polymer} {Solutions}},
	volume = {87},
	issn = {0031-9007, 1079-7114},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.87.188301},
	doi = {10.1103/PhysRevLett.87.188301},
	language = {en},
	number = {18},
	urldate = {2022-10-19},
	journal = {Physical Review Letters},
	author = {Kumar, Sanat K. and Douglas, Jack F.},
	month = oct,
	year = {2001},
	pages = {188301},
}

@article{kumar_gelation_2001-1,
	title = {Gelation in {Physically} {Associating} {Polymer} {Solutions}},
	volume = {87},
	issn = {0031-9007, 1079-7114},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.87.188301},
	doi = {10.1103/PhysRevLett.87.188301},
	language = {en},
	number = {18},
	urldate = {2022-10-19},
	journal = {Physical Review Letters},
	author = {Kumar, Sanat K. and Douglas, Jack F.},
	month = oct,
	year = {2001},
	pages = {188301},
}

@article{omar_shear-induced_2017,
	title = {Shear-{Induced} {Heterogeneity} in {Associating} {Polymer} {Gels}: {Role} of {Network} {Structure} and {Dilatancy}},
	volume = {119},
	shorttitle = {Shear-{Induced} {Heterogeneity} in {Associating} {Polymer} {Gels}},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.119.117801},
	doi = {10.1103/PhysRevLett.119.117801},
	abstract = {We study associating polymer gels under steady shear using Brownian dynamics simulation to explore the interplay between the network structure, dynamics, and rheology. For a wide range of flow rates, we observe the formation of shear bands with a pronounced difference in shear rate, concentration, and structure. A striking increase in the polymer pressure in the gradient direction with shear, along with the inherently large compressibility of the gels, is shown to be a crucial factor in destabilizing homogeneous flow through shear-gradient concentration coupling. We find that shear has only a modest influence on the degree of association, but induces marked spatial heterogeneity in the network connectivity. We attribute the increase in the polymer pressure (and polymer mobility) to this structural reorganization.},
	number = {11},
	urldate = {2022-09-30},
	journal = {Physical Review Letters},
	author = {Omar, Ahmad K. and Wang, Zhen-Gang},
	month = sep,
	year = {2017},
	note = {Publisher: American Physical Society},
	pages = {117801},
}

@article{rubinstein_thermoreversible_1998,
	title = {Thermoreversible {Gelation} in {Solutions} of {Associating} {Polymers}. 2. {Linear} {Dynamics}},
	volume = {31},
	issn = {0024-9297, 1520-5835},
	url = {https://pubs.acs.org/doi/10.1021/ma970617%2B},
	doi = {10.1021/ma970617+},
	abstract = {Viscoelastic properties of reversible networks formed in solutions of associating polymers are considered theoretically in the Rouse-Zimm (unentangled) regime. It is shown that the dynamics is governed primarily by the network strand size and by the effective lifetime of reversible junctions. Both frequency and concentration dependencies of viscosity and dynamical moduli are considered. A novel model taking into account the possibility of multiple dissociation and recombination of the same pair of stickers is developed. It is shown that this effect gives rise to an increase of the apparent activation energy which is predicted to be substantially larger than the priming activation energy for dissociation of two stickers.},
	language = {en},
	number = {4},
	urldate = {2022-10-19},
	journal = {Macromolecules},
	author = {Rubinstein, Michael and Semenov, Alexander N.},
	month = feb,
	year = {1998},
	pages = {1386--1397},
}

@article{semenov_thermoreversible_1998,
	title = {Thermoreversible {Gelation} in {Solutions} of {Associative} {Polymers}. 1. {Statics}},
	volume = {31},
	issn = {0024-9297, 1520-5835},
	url = {https://pubs.acs.org/doi/10.1021/ma970616h},
	doi = {10.1021/ma970616h},
	abstract = {An equilibrium mean-field theory for reversible network formation in solutions of associative polymers is presented. We study polymer solutions with many associating groups per chain and consider pairwise association of these groups. A simple analytical expression for the free energy of these systems is derived and is shown to be consistent with the classical gelation picture developed by Flory and Stockmayer. It is shown that association and formation of a reversible network is always accompanied by a tendency for phase separation which might occur even under marginal solvent conditions. The mean-field theory is also generalized to take into account the effect of local intrachain loops as well as excluded volume interactions (partial swelling of polymer chains). It is shown that phase separation might be suppressed by the excluded volume interactions.},
	language = {en},
	number = {4},
	urldate = {2022-10-19},
	journal = {Macromolecules},
	author = {Semenov, Alexander N. and Rubinstein, Michael},
	month = feb,
	year = {1998},
	pages = {1373--1385},
}

@article{binous_application_2021,
	title = {Application of graduate-level numerical tools to teach phase equilibria of liquid ternary systems},
	volume = {29},
	issn = {1099-0542},
	url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/cae.22411},
	doi = {10.1002/cae.22411},
	abstract = {The present paper describes a numerical technique to compute phase equilibria of ternary liquid systems. First, particle swarm optimization is used to estimate the binary interaction parameters of the NRTL (Non-Random Two Liquid) and UNIQUAC (Universal Quasi-Chemical) models. We show how the arc-length continuation method allows the calculation of the liquid–liquid equilibrium diagram for any ternary system. A total of seven case studies of industrially important mixtures are described. Both Type I systems (oleic acid–water–ethanol, water–1-propanol–toluene, DEC–ethanol–water, water–propionic acid–n-hexane, and water–TMA–benzene) and Type II mixtures (water–1-butanol–n-hexane) are discussed. In addition, a system with temperature-dependent behavior (n-hexane–methyl cyclopentane–aniline) is studied. The numerical techniques and the thermodynamic problem involved in this paper are suitable for a first-year graduate-level course in chemical engineering. All computer coding is based either on Mathematica© or Matlab®. This is an ideal opportunity to introduce graduate students to advanced commands and programming syntax of state-of-the-art mathematical software.},
	language = {en},
	number = {6},
	urldate = {2022-10-01},
	journal = {Computer Applications in Engineering Education},
	author = {Binous, Housam and Mejbri, Khalifa and Bellagi, Ahmed},
	year = {2021},
	note = {\_eprint: https://onlinelibrary.wiley.com/doi/pdf/10.1002/cae.22411},
	keywords = {Mathematica© and Matlab®, NRTL and UNIQUAC models, arc-length continuation, graduate chemical engineering thermodynamics, liquid–liquid equilibrium data},
	pages = {1589--1601},
}

@article{li_measurement_2019,
	title = {Measurement and correlation of isobaric vapour-liquid equilibrium for the (acetonitrile + water) system containing different ionic liquids at atmospheric pressure},
	volume = {138},
	issn = {00219614},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0021961419301016},
	doi = {10.1016/j.jct.2019.07.006},
	abstract = {Isobaric vapour-liquid equilibrium (VLE) for the (acetonitrile + water) system containing 1-hexyl-3methylimidazolium chloride ([HMIM][Cl]), 1-butyl-3-methylimidazolium chloride ([BMIM][Cl]), 1-allyl-3-methylimidazolium chloride ([AMIM][Cl]) and 1-butyl-3-methylimidazolium acetate ([BMIM] [OAC]) are measured at atmospheric pressure (101.30 kPa). The experimental results show that the addition of ionic liquids (ILs) can improve the separation of acetonitrile and water and eliminate the azeotrope when the content of ILs reaches a certain value. The separation ability of ILs is [BMIM] [OAC] {\textgreater} [AMIM][Cl] {\textgreater} [BMIM][Cl] \% [HMIM][Cl]. A crossover effect of salting-in and -out of acetonitrile in different concentration ranges is observed. The experimental VLE data are satisfactorily correlated with the non-random two liquid (NRTL) model. Additionally, COSMO-SAC is employed to predict the phase behaviours of the investigated systems and good trends are obtained.},
	language = {en},
	urldate = {2022-01-04},
	journal = {J. Chem. Thermodyn.},
	author = {Li, Jinlong and Li, Jiashu and Zheng, Yeling and Peng, Changjun and Liu, Honglai},
	month = nov,
	year = {2019},
	keywords = {Acetonitrile, COSMO-SAC, Ionic liquid, NRTL model, Vapour-liquid equilibrium, Water},
	pages = {366--373},
}

@article{aucejo_densities_1995,
	title = {Densities, {Viscosities}, and {Refractive} {Indices} of {Some} n-{Alkane} {Binary} {Liquid} {Systems} at 298.15 {K}},
	volume = {40},
	issn = {0021-9568},
	url = {https://doi.org/10.1021/je00017a032},
	doi = {10.1021/je00017a032},
	number = {1},
	urldate = {2022-09-19},
	journal = {J. Chem. Eng. Data},
	author = {Aucejo, Antonio and Burguet, M. Cruz and Munoz, Rosa and Marques, Jose L.},
	month = jan,
	year = {1995},
	note = {Publisher: American Chemical Society},
	pages = {141--147},
}

@article{grambow_accurate_2019,
	title = {Accurate {Thermochemistry} with {Small} {Data} {Sets}: {A} {Bond} {Additivity} {Correction} and {Transfer} {Learning} {Approach}},
	volume = {123},
	issn = {1089-5639},
	shorttitle = {Accurate {Thermochemistry} with {Small} {Data} {Sets}},
	url = {https://doi.org/10.1021/acs.jpca.9b04195},
	doi = {10.1021/acs.jpca.9b04195},
	abstract = {Machine learning provides promising new methods for accurate yet rapid prediction of molecular properties, including thermochemistry, which is an integral component of many computer simulations, particularly automated reaction mechanism generation. Often, very large data sets with tens of thousands of molecules are required for training the models, but most data sets of experimental or high-accuracy quantum mechanical quality are much smaller. To overcome these limitations, we calculate new high-level data sets and derive bond additivity corrections to significantly improve enthalpies of formation. We adopt a transfer learning technique to train neural network models that achieve good performance even with a relatively small set of high-accuracy data. The training data for the entropy model are carefully selected so that important conformational effects are captured. The resulting models are generally applicable thermochemistry predictors for organic compounds with oxygen and nitrogen heteroatoms that approach experimental and coupled cluster accuracy while only requiring molecular graph inputs. Due to their versatility and the ease of adding new training data, they are poised to replace conventional estimation methods for thermochemical parameters in reaction mechanism generation. Since high-accuracy data are often sparse, similar transfer learning approaches are expected to be useful for estimating many other molecular properties.},
	number = {27},
	urldate = {2022-09-24},
	journal = {J. Phys. Chem. A},
	author = {Grambow, Colin A. and Li, Yi-Pei and Green, William H.},
	month = jul,
	year = {2019},
	note = {Publisher: American Chemical Society},
	pages = {5826--5835},
}

@article{zhu_excess_1993,
	title = {Excess enthalpies of (ethanol or propan-1-ol + cyclohexane + decane) at the temperature 298.15 {K}},
	volume = {25},
	issn = {0021-9614},
	url = {https://www.sciencedirect.com/science/article/pii/S0021961483710888},
	doi = {10.1006/jcht.1993.1088},
	abstract = {Excess molar enthalpies, measured at 298.15 K in a flow-microcalorimeter are reported for the ternary mixtures \{x1CH3(CH2)vOH + x2c -C6H12 + (1-x1-x2)CH3(CH2)8CH3\} with v = 1 and 2. Smooth representations of the results are described and used to construct constant-enthalpy contours on a Roozeboom diagram.},
	language = {en},
	number = {7},
	urldate = {2022-09-19},
	journal = {J. Chem. Thermodyn.},
	author = {Zhu, Shemin and Shen, Shubao and Benson, George C. and Lu, Benjamin C. -Y.},
	month = jul,
	year = {1993},
	pages = {909--917},
}

@article{walker_ab_2022,
	title = {\textit{{Ab} initio} development of generalized {Lennard}-{Jones} ({Mie}) force fields for predictions of thermodynamic properties in advanced molecular-based {SAFT} equations of state},
	volume = {156},
	copyright = {All rights reserved},
	issn = {0021-9606, 1089-7690},
	url = {https://aip.scitation.org/doi/10.1063/5.0087125},
	doi = {10.1063/5.0087125},
	abstract = {A methodology for obtaining molecular parameters of a modified statistical associating fluid theory for variable-range interactions of Mie form (SAFT-VR Mie) equation of state (EoS) from ab initio calculations is proposed for non-associative species that can be modeled as single spherical segments. The methodology provides a strategy to map interatomic or intermolecular potentials obtained from ab initio quantumchemistry calculations to the corresponding Mie potentials that can be used within the SAFT-VR Mie EoS. The inclusion of corrections for quantum and many-body effects allows for an excellent, fully predictive description of the vapor–liquid envelope and other bulk thermodynamic properties of noble gases; this description is of similar or superior quality to that obtained using SAFT-VR Mie with parameters regressed in the traditional way using experimental thermodynamic-property data. The methodology is extended to an anisotropic species, methane, where similar levels of accuracy are obtained. The efficacy of using less-accurate quantum-chemistry methods in this methodology is explored, showing that these methods do not provide satisfactory results, although we note that the description is nevertheless substantially better than those obtained using the conductor-like screening model for describing real solvents (COSMO-RS), the only other fully predictive ab initio method currently available. Overall, the reliance on thermophysical data is completely dispensed with, providing the first extensible, wholly predictive SAFT-type EoSs.},
	language = {en},
	number = {15},
	urldate = {2022-04-18},
	journal = {J. Chem. Phys.},
	author = {Walker, Pierre J. and Zhao, Tianpu and Haslam, Andrew J. and Jackson, George},
	month = apr,
	year = {2022},
	pages = {154106},
}

@article{van_westen_perturbation_2022,
	title = {Perturbation theories for fluids with short-ranged attractive forces: {A} case study of the {Lennard}-{Jones} spline fluid},
	volume = {156},
	issn = {0021-9606, 1089-7690},
	shorttitle = {Perturbation theories for fluids with short-ranged attractive forces},
	url = {https://aip.scitation.org/doi/10.1063/5.0082690},
	doi = {10.1063/5.0082690},
	abstract = {It is generally not straightforward to apply molecular-thermodynamic theories to fluids with short-ranged attractive forces between their constituent molecules (or particles). This especially applies to perturbation theories, which, for short-ranged attractive fluids, typically must be extended to high order or may not converge at all. Here, we show that a recent first-order perturbation theory, the uv-theory, holds promise for describing such fluids. As a case study, we apply the uv-theory to a fluid with pair interactions defined by the Lennard-Jones spline potential, which is a short-ranged version of the LJ potential that is known to provide a challenge for equation-of-state development. The results of the uv-theory are compared to those of third-order Barker–Henderson and fourth-order Weeks–Chandler–Andersen perturbation theories, which are implemented using Monte Carlo simulation results for the respective perturbation terms. Theoretical predictions are compared to an extensive dataset of molecular simulation results from this (and previous) work, including vapor–liquid equilibria, firstand second-order derivative properties, the critical region, and metastable states. The uv-theory proves superior for all properties examined. An especially accurate description of metastable vapor and liquid states is obtained, which might prove valuable for future applications of the equation-of-state model to inhomogeneous phases or nucleation processes. Although the uv-theory is analytic, it accurately describes molecular simulation results for both the critical point and the binodal up to at least 99\% of the critical temperature. This suggests that the difficulties typically encountered in describing the vapor–liquid critical region are only to a small extent caused by non-analyticity.},
	language = {en},
	number = {10},
	urldate = {2022-08-01},
	journal = {J. Chem. Phys.},
	author = {van Westen, Thijs and Hammer, Morten and Hafskjold, Bjørn and Aasen, Ailo and Gross, Joachim and Wilhelmsen, Øivind},
	month = mar,
	year = {2022},
	pages = {104504},
}

@article{van_westen_accurate_2021,
	title = {Accurate thermodynamics of simple fluids and chain fluids based on first-order perturbation theory and second virial coefficients: \textit{uv} -theory},
	volume = {155},
	issn = {0021-9606, 1089-7690},
	shorttitle = {Accurate thermodynamics of simple fluids and chain fluids based on first-order perturbation theory and second virial coefficients},
	url = {https://aip.scitation.org/doi/10.1063/5.0073572},
	doi = {10.1063/5.0073572},
	abstract = {We develop a simplification of our recently proposed uf -theory for describing the thermodynamics of simple fluids and fluids comprising short chain molecules. In its original form, the uf -theory interpolates the Helmholtz energy between a first-order f -expansion and first-order u-expansion as (effective) lower and upper bounds. We here replace the f -bound by a new, tighter (effective) lower bound. The resulting equation of state interpolates between a first-order u-expansion at high densities and another first-order u-expansion that is modified to recover the exact second virial coefficient at low densities. The theory merely requires the Helmholtz energy of the reference fluid, the firstorder u-perturbation term, and the total perturbation contribution to the second virial coefficient as input. The revised theory—referred to as uv-theory—is thus simpler than the uf -theory but leads to similar accuracy, as we show for fluids with intermolecular pair interactions governed by a Mie potential. The uv-theory is thereby easier to extend to fluid mixtures and provides more flexibility in extending the model to non-spherical or chain-like molecules. The usefulness of the uv-theory for developing equation-of-state models of non-spherical molecules is here exemplified by developing an equation of state for Lennard-Jones dimers.},
	language = {en},
	number = {24},
	urldate = {2022-08-01},
	journal = {J. Chem. Phys.},
	author = {van Westen, Thijs and Gross, Joachim},
	month = dec,
	year = {2021},
	pages = {244501},
}

@article{van_westen_accurate_2021-1,
	title = {Accurate first-order perturbation theory for fluids: \textit{uf} -theory},
	volume = {154},
	issn = {0021-9606, 1089-7690},
	shorttitle = {Accurate first-order perturbation theory for fluids},
	url = {http://aip.scitation.org/doi/10.1063/5.0031545},
	doi = {10.1063/5.0031545},
	abstract = {We propose a new first-order perturbation theory that provides a near-quantitative description of the thermodynamics of simple fluids. The theory is based on the ansatz that the Helmholtz free energy is bounded below by a first-order Mayer-f expansion. Together with the rigorous upper bound provided by a first-order u-expansion, this brackets the actual free energy between an upper and (effective) lower bound that can both be calculated based on first-order perturbation theory. This is of great practical use. Here, the two bounds are combined into an interpolation scheme for the free energy. The scheme exploits the fact that a first-order Mayer-f perturbation theory is exact in the lowdensity limit, whereas the accuracy of a first-order u-expansion grows when density increases. This allows an interpolation between the lower “f ”-bound at low densities and the upper “u” bound at higher liquid-like densities. The resulting theory is particularly well behaved. Using a density-dependent interpolating function of only two adjustable parameters, we obtain a very accurate representation of the full fluid-phase behavior of a Lennard-Jones fluid. The interpolating function is transferable to other intermolecular potential types, which is here shown for the Mie m-6 family of fluids. The extension to mixtures is simple and accurate without requiring any dependence of the interpolating function on the composition of the mixture.},
	language = {en},
	number = {4},
	urldate = {2022-08-01},
	journal = {J. Chem. Phys.},
	author = {van Westen, Thijs and Gross, Joachim},
	month = jan,
	year = {2021},
	pages = {041102},
}

@article{mansoori_equilibrium_1971,
	title = {Equilibrium {Thermodynamic} {Properties} of the {Mixture} of {Hard} {Spheres}},
	volume = {54},
	issn = {0021-9606, 1089-7690},
	url = {http://aip.scitation.org/doi/10.1063/1.1675048},
	doi = {10.1063/1.1675048},
	language = {en},
	number = {4},
	urldate = {2022-01-04},
	journal = {J. Chem. Phys.},
	author = {Mansoori, G. A. and Carnahan, N. F. and Starling, K. E. and Leland, T. W.},
	month = feb,
	year = {1971},
	pages = {1523--1525},
}

@article{lafitte_accurate_2013,
	title = {Accurate statistical associating fluid theory for chain molecules formed from {Mie} segments},
	volume = {139},
	issn = {0021-9606, 1089-7690},
	url = {http://aip.scitation.org/doi/10.1063/1.4819786},
	doi = {10.1063/1.4819786},
	language = {en},
	number = {15},
	urldate = {2022-01-04},
	journal = {J. Chem. Phys.},
	author = {Lafitte, Thomas and Apostolakou, Anastasia and Avendaño, Carlos and Galindo, Amparo and Adjiman, Claire S. and Müller, Erich A. and Jackson, George},
	month = oct,
	year = {2013},
	pages = {154504},
}

@article{boublik_hardsphere_1970,
	title = {Hard‐{Sphere} {Equation} of {State}},
	volume = {53},
	issn = {0021-9606, 1089-7690},
	url = {http://aip.scitation.org/doi/10.1063/1.1673824},
	doi = {10.1063/1.1673824},
	language = {en},
	number = {1},
	urldate = {2022-01-04},
	journal = {J. Chem. Phys.},
	author = {Boublík, Tomáš},
	month = jul,
	year = {1970},
	pages = {471--472},
}

@article{gopi_acetonitrilewater_2015,
	title = {Acetonitrile–water hydrogen-bonded interaction: {Matrix}-isolation infrared and ab initio computation},
	volume = {1094},
	issn = {00222860},
	shorttitle = {Acetonitrile–water hydrogen-bonded interaction},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0022286015002811},
	doi = {10.1016/j.molstruc.2015.03.046},
	abstract = {The 1:1 hydrogen-bonded complex of acetonitrile (CH3CN) and water (H2O) was trapped in Ar and N2 matrices and studied using infrared technique. Ab initio computations showed two types of complexes formed between CH3CN and H2O, a linear complex A with a C„NÁ Á ÁH interaction between nitrogen of CH3CN and hydrogen of H2O and a cyclic complex B, in which the interactions are between the hydrogen of CH3CN with oxygen of H2O and hydrogen of H2O with p cloud of AC„N of CH3CN. Vibrational wavenumber calculations revealed that both the complexes A and B were minima on the potential energy surface. Interaction energies computed at B3LYP/6-311++G(d,p) showed that linear complex A is more stable than cyclic complex B. Computations identiﬁed a blue shift of \$11.5 cmÀ1 and a red shift of \$6.5 cmÀ1 in the CN stretching mode for the complexes A and B, respectively. Experimentally, we observed a blue shift of \$15.0 and \$8.3 cmÀ1 in N2 and Ar matrices, respectively, in the CN stretching mode of CH3CN, which supports the formation of complex A. The Onsager Self Consistent Reaction Field (SCRF) model was used to explain the inﬂuence of matrices on the complexes A and B. To understand the nature of the interactions, Atoms in Molecules (AIM) and Natural Bond Orbital (NBO) analyses were carried out for the complexes A and B.},
	language = {en},
	urldate = {2021-10-12},
	journal = {J. Mol. Struct.},
	author = {Gopi, R. and Ramanathan, N. and Sundararajan, K.},
	month = aug,
	year = {2015},
	pages = {118--129},
}

@article{basdogan_machine_2020,
	title = {Machine {Learning}-{Guided} {Approach} for {Studying} {Solvation} {Environments}},
	volume = {16},
	issn = {1549-9618},
	url = {https://doi.org/10.1021/acs.jctc.9b00605},
	doi = {10.1021/acs.jctc.9b00605},
	abstract = {Molecular-level understanding and characterization of solvation environments are often needed across chemistry, biology, and engineering. Toward practical modeling of local solvation effects of any solute in any solvent, we report a static and all-quantum mechanics-based cluster-continuum approach for calculating single-ion solvation free energies. This approach uses a global optimization procedure to identify low-energy molecular clusters with different numbers of explicit solvent molecules and then employs the smooth overlap for atomic positions learning kernel to quantify the similarity between different low-energy solute environments. From these data, we use sketch maps, a nonlinear dimensionality reduction algorithm, to obtain a two-dimensional visual representation of the similarity between solute environments in differently sized microsolvated clusters. After testing this approach on different ions having charges 2+, 1+, 1–, and 2–, we find that the solvation environment around each ion can be seen to usually become more similar in hand with its calculated single-ion solvation free energy. Without needing either dynamics simulations or an a priori knowledge of local solvation structure of the ions, this approach can be used to calculate solvation free energies within 5\% of experimental measurements for most cases, and it should be transferable for the study of other systems where dynamics simulations are not easily carried out.},
	number = {1},
	urldate = {2022-09-20},
	journal = {J. Chem. Theory Comput.},
	author = {Basdogan, Yasemin and Groenenboom, Mitchell C. and Henderson, Ethan and De, Sandip and Rempe, Susan B. and Keith, John A.},
	month = jan,
	year = {2020},
	note = {Publisher: American Chemical Society},
	pages = {633--642},
}

@article{walker_new_2020,
	title = {A {New} {Predictive} {Group}-{Contribution} {Ideal}-{Heat}-{Capacity} {Model} and {Its} {Influence} on {Second}-{Derivative} {Properties} {Calculated} {Using} a {Free}-{Energy} {Equation} of {State}},
	volume = {65},
	copyright = {All rights reserved},
	issn = {0021-9568, 1520-5134},
	url = {https://pubs.acs.org/doi/10.1021/acs.jced.0c00723},
	doi = {10.1021/acs.jced.0c00723},
	abstract = {A statistical-thermodynamics-based group contribution (GC) method, commensurate with the GC methodology used in SAFT-γ Mie, is proposed to model ideal heat capacities. Special treatment of halogenated groups allows many halogenated molecules to be modeled with few parameters. Parameters for small, single-group species agree well with experimental vibrational temperatures. Parameters corresponding to groups used for larger species highlight eﬀects such as anharmonicity and torsional modes. The proposed correlation consistently demonstrates higher accuracy than that of Joback and Reid. Ideal heat capacities are seldom used in isolation, but contribute to other properties that may be used to assess the quality of an equation of state. The importance of the ideal free energy to various second-derivative properties, as calculated using the SAFT-γ Mie equation of state, is examined. In the majority of cases, using the proposed correlation to calculate the ideal free energy results in more-accurately estimated second-derivative propertiessometimes substantially so. Further studies of the contribution of the ideal free energy are carried out revealing interesting behavior near the critical point that may relate to the Widom-Fisher and Widom lines.},
	language = {en},
	number = {12},
	urldate = {2021-09-27},
	journal = {J. Chem. Eng. Data},
	author = {Walker, Pierre J. and Haslam, Andrew J.},
	month = dec,
	year = {2020},
	pages = {5809--5829},
}

@article{reamer_phase_1966,
	title = {Phase {Equilibria} in {Hydrocarbon} {Systems}. {Volumetric} and {Phase} {Behavior} of the {Propane}-n-{Decane} {System}.},
	volume = {11},
	issn = {0021-9568},
	url = {https://doi.org/10.1021/je60028a004},
	doi = {10.1021/je60028a004},
	number = {1},
	urldate = {2022-09-19},
	journal = {J. Chem. Eng. Data},
	author = {Reamer, H. H. and Sage, B. H.},
	month = jan,
	year = {1966},
	note = {Publisher: American Chemical Society},
	pages = {17--24},
}

@article{raal_examination_1972,
	title = {Examination of ethanol-n-heptane, methanol-n-hexane systems using new vapor-liquid equilibrium still},
	volume = {17},
	issn = {0021-9568},
	url = {https://doi.org/10.1021/je60053a019},
	doi = {10.1021/je60053a019},
	number = {2},
	urldate = {2022-09-19},
	journal = {J. Chem. Eng. Data},
	author = {Raal, J. David and Code, Russel K. and Best, Donald A.},
	month = apr,
	year = {1972},
	note = {Publisher: American Chemical Society},
	pages = {211--216},
}

@article{di_cave_liquid-liquid_1991,
	title = {Liquid-liquid equilibria for ternary systems formed by acetonitrile, water, and aromatic hydrocarbons},
	volume = {36},
	issn = {0021-9568, 1520-5134},
	url = {https://pubs.acs.org/doi/abs/10.1021/je00003a012},
	doi = {10.1021/je00003a012},
	language = {en},
	number = {3},
	urldate = {2022-09-08},
	journal = {J. Chem. Eng. Data},
	author = {Di Cave, Sergio and Mazzarotta, Barbara},
	month = jul,
	year = {1991},
	pages = {298--303},
}

@article{ylitalo_competition_2022,
	title = {Competition between {CO} $_{\textrm{2}}$ -philicity and {Mixing} {Entropy} {Leads} to {CO} $_{\textrm{2}}$ {Solubility} {Maximum} in {Polyether} {Polyols}},
	copyright = {All rights reserved},
	issn = {0888-5885, 1520-5045},
	url = {https://pubs.acs.org/doi/10.1021/acs.iecr.2c02396},
	doi = {10.1021/acs.iecr.2c02396},
	abstract = {In carbon dioxide-blown polymer foams, the solubility of carbon dioxide (CO2) in the polymer profoundly shapes the structure and, consequently, the physical properties of the foam. One such foam is polyurethane�commonly used for thermal insulation, acoustic insulation, and cushioning�which increasingly relies on CO2 to replace environmentally harmful blowing agents. Polyurethane is produced through the reaction of isocyanate and polyol, of which the polyol has the higher capacity for dissolving CO2. While previous studies have suggested the importance of the effect of hydroxyl end groups on CO2 solubility in short polyols ({\textless}1000 g/mol), their effect in polyols with higher molecular weight (≥1000 g/mol) and higher functionality ({\textgreater}2 hydroxyls per chain)�as are commonly used in polyurethane foams�has not been reported. Here, we show that the solubility of CO2 in polyether polyols decreases with molecular weight above 1000 g/mol and decreases with functionality using measurements performed by gravimetry-axisymmetric drop-shape analysis. The nonmonotonic effect of molecular weight on CO2 solubility results from the competition between effects that reduce CO2 solubility (lower mixing entropy) and effects that increase CO2 solubility (lower ratio of hydroxyl end groups to ether backbone groups). To generalize our measurements, we modeled the CO2 solubility using a perturbed chain-statistical associating fluid theory (PC-SAFT) model, which we validated by showing that a density functional theory model based on the PC-SAFT free energy accurately predicted the interfacial tension.},
	language = {en},
	urldate = {2022-08-18},
	journal = {Ind. Eng. Chem. Res.},
	author = {Ylitalo, Andrew S. and Chao, Huikuan and Walker, Pierre J. and Crosthwaite, Jacob and Fitzgibbons, Thomas C. and Ginzburg, Valeriy G. and Zhou, Weijun and Wang, Zhen-Gang and Di Maio, Ernesto and Kornfield, Julia A.},
	month = aug,
	year = {2022},
	pages = {acs.iecr.2c02396},
}

@article{walker_clapeyronjl_2022,
	title = {Clapeyron.jl: {An} {Extensible}, {Open}-{Source} {Fluid} {Thermodynamics} {Toolkit}},
	volume = {61},
	copyright = {All rights reserved},
	issn = {0888-5885, 1520-5045},
	shorttitle = {Clapeyron.jl},
	url = {https://pubs.acs.org/doi/10.1021/acs.iecr.2c00326},
	doi = {10.1021/acs.iecr.2c00326},
	abstract = {Thermodynamic models are often vital when characterizing complex systems, particularly natural gas, electrolyte, polymer, pharmaceutical, and biological systems. However, their implementations have historically been abstruse and cumbersome, and as such, the only options available were black box commercial tools. In this article, we present Clapeyron.jl: a pioneering attempt at an open-source ﬂuid thermodynamics toolkit to build and make use of thermodynamic models. This toolkit is built using Julia, a modern language for scientiﬁc computing known for its ease of use, extensibility, and ﬁrst-class support for diﬀerentiable programming. We currently support more models than any package available, including standard cubic (SRK, PR, PSRK, etc.), activity coeﬃcient (NRTL, UNIFAC, etc.), COSMO-based, and the venerable SAFT equations. The property estimation methods supported are extensive, including bulk, VLE, LLE, VLLE, and critical properties. With Clapeyron.jl, researchers and enthusiasts alike will be able to focus on the application and worry less about the implementation.},
	language = {en},
	number = {20},
	urldate = {2022-05-27},
	journal = {Ind. Eng. Chem. Res.},
	author = {Walker, Pierre J. and Yew, Hon-Wa and Riedemann, Andrés},
	month = may,
	year = {2022},
	pages = {7130--7153},
}

@article{sauer_comparison_2014-1,
	title = {Comparison between a {Homo}- and a {Heterosegmented} {Group} {Contribution} {Approach} {Based} on the {Perturbed}-{Chain} {Polar} {Statistical} {Associating} {Fluid} {Theory} {Equation} of {State}},
	volume = {53},
	issn = {0888-5885, 1520-5045},
	url = {https://pubs.acs.org/doi/10.1021/ie502203w},
	doi = {10.1021/ie502203w},
	abstract = {Depending on the molecular model, group contribution (GC) approaches based on the statistical associating ﬂuid theory (SAFT) can be classiﬁed in homosegmented and heterosegmented GC approaches. In homosegmented GC approaches, molecules are modeled as chains composed of identical segments. Heterosegmented GC approaches, on the other hand, consider molecular chains composed of diﬀerent segment types and thus maintain a more detailed picture of real molecules. Therefore, heterosegmented GC approaches are arguably more physically realistic and ought to give more accurate descriptions of thermodynamic properties. In this work, we evaluate the performance of a homosegmented and a heterosegmented GC approach based on the perturbed-chain polar SAFT (PCP-SAFT) equation of state (EoS). To ensure a meaningful comparison between both GC approaches, a dipole term for the heterosegmented GC approach is formulated. Group parameters of 22 functional groups were adjusted to pure component property data. The comparison between both GC approaches shows that the heterosegmented GC approach leads to signiﬁcantly better agreement with experimental data for various chemical families.},
	language = {en},
	number = {38},
	urldate = {2022-08-01},
	journal = {Ind. Eng. Chem. Res.},
	author = {Sauer, Elmar and Stavrou, Marina and Gross, Joachim},
	month = sep,
	year = {2014},
	pages = {14854--14864},
}

@article{ramdin_state---art_2012,
	title = {State-of-the-{Art} of {CO} $_{\textrm{2}}$ {Capture} with {Ionic} {Liquids}},
	volume = {51},
	issn = {0888-5885, 1520-5045},
	url = {https://pubs.acs.org/doi/10.1021/ie3003705},
	doi = {10.1021/ie3003705},
	abstract = {Economical and environmental aspects are the main motivation for research on energy eﬃcient processes and the search for environment friendly materials for CO2 capture. Currently, CO2 capture is dominated by amine-based (e.g., monoethanolamine) technologies, which are very energy intensive and less attractive from an environmental point of view due to emissions of the used volatile solvent components. Ionic liquids have been proposed as a promising alternative to the conventional volatile solvents, because of their low volatility and other interesting properties. This remarkable interest has led to a rapid growth of literature on this speciﬁc subject. The aim of the present review paper is to provide a detailed overview of the achievements and diﬃculties that has been encountered in ﬁnding a suitable ionic liquid for CO2 capture from ﬂue-gas streams. A major part of this review includes an overview of the experimental data of CO2 solubility, selectivity, and diﬀusivity in diﬀerent ionic liquids. The eﬀect of anions, cations, and functional groups on the CO2 solubility, biodegradability, and toxicity of the ionic liquids are highlighted. Recent developments on task-speciﬁc ionic liquids and supported ionic liquid membranes are also discussed. Scarcely available results of molecular simulations, which is a valuable tool in designing and evaluating ionic liquids, are also reviewed. The trends highlighted here can be used by solvent designers to navigate through the massive amount of theoretically possible ILs.},
	language = {en},
	number = {24},
	urldate = {2022-04-18},
	journal = {Ind. Eng. Chem. Res.},
	author = {Ramdin, Mahinder and de Loos, Theo W. and Vlugt, Thijs J.H.},
	month = jun,
	year = {2012},
	pages = {8149--8177},
}

@article{quinteros-lama_second-order_2019,
	title = {Second-{Order} {Differential} {Accelerators} {Based} on the {Geometry} of {Equilibrium} for {Thermodynamic} {Calculations}. {Part} {I}. {Pure} {Fluids}},
	volume = {58},
	issn = {0888-5885},
	url = {https://pubs.acs.org/doi/10.1021/acs.iecr.9b04771},
	doi = {10.1021/acs.iecr.9b04771},
	number = {45},
	journal = {Ind. Eng. Chem. Res.},
	author = {Quinteros-Lama, Héctor and Garrido, José Matías and Polishuk, Ilya},
	month = nov,
	year = {2019},
	pages = {20838--20846},
}

@article{naseri_boroujeni_comparison_2022,
	title = {Comparison of {Models} for the {Prediction} of the {Electrical} {Conductivity} of {Electrolyte} {Solutions}},
	volume = {61},
	issn = {0888-5885, 1520-5045},
	url = {https://pubs.acs.org/doi/10.1021/acs.iecr.1c04365},
	doi = {10.1021/acs.iecr.1c04365},
	abstract = {It has been almost one century since Onsager developed the limiting law of equivalent conductivity of electrolyte solutions. Thenceforth, many models have been developed; however, they have not been assessed thoroughly and systematically. This paper comprehensively investigates the accuracy and reliability of six equivalent conductivity models, namely, the Debye−Hückel−Onsager limiting law (DHOLL), extended law (DHOEE), smaller ion shell (DHOSiS), along with the simpliﬁed and full mean spherical approximation (MSA, MSA-Simple), and Quint−Viallard (QV). To this aim, we have prepared a database of experimental data for 126 electrolytes. The accuracy of the models is examined with the help of graphical methods and error analysis over a wide range of concentrations ([0, 18] mol/L) and temperatures ([0, 100] °C). Moreover, the origin of possible errors of models is inspected with a term-by-term analysis of relaxation and electrophoretic eﬀects. It is shown that the absolute average deviation of models depends highly on the electrolyte type, and it is generally smaller for 1:1 salts, especially at low concentrations (less than 5\%). The error evolution with concentration also reveals that MSA-Simple and DHOEE are more reliable over a wide range of concentration and electrolyte types. It is concluded that MSA-Simple predicts the equivalent conductivity at lower temperatures and the trend of Λ versus T more satisfactorily than the other models.},
	language = {en},
	number = {8},
	urldate = {2022-06-22},
	journal = {Ind. Eng. Chem. Res.},
	author = {Naseri Boroujeni, Saman and Liang, Xiaodong and Maribo-Mogensen, Bjørn and Kontogeorgis, Georgios M.},
	month = mar,
	year = {2022},
	pages = {3168--3185},
}

@article{lee_priori_2015,
	title = {A {Priori} {Prediction} of {Dissociation} {Phenomena} and {Phase} {Behaviors} of {Ionic} {Liquids}},
	volume = {54},
	issn = {0888-5885, 1520-5045},
	url = {https://pubs.acs.org/doi/10.1021/acs.iecr.5b01762},
	doi = {10.1021/acs.iecr.5b01762},
	abstract = {Many unique properties of ionic liquids (ILs) are closely related to the extent of dissociation (α) in solution. However, most of the existing models for ILs assume either full dissociation or full nondissociation regardless of mixture compositions. In this work, the dissociation of ILs (CA = C+ + A−) is described as a chemical reaction. Together with the predictive COSMO-SAC model, the dissociation constant can be determined based on the value of α in the pure state. Our results show that the predicted composition dependence of α is in good agreement with experiment over the entire concentration range. We further examine the prediction of a variety of thermodynamic properties and phase behaviors of IL solutions, covering high (inﬁnite dilution activity coeﬃcient of solvent), medium (vapor−liquid and liquid−liquid), and low (osmotic coeﬃcient and mean ionic activity coeﬃcient) IL concentrations (a total of 9857 data points). Our results show that the composition dependence of IL dissociation has a signiﬁcant impact on the phase behaviors of IL solutions. The dominating factors for the solution nonideality changes from short-range ion-pair interactions at high IL concentrations to long-range ion−ion interactions at low IL concentrations.},
	language = {en},
	number = {36},
	urldate = {2022-01-22},
	journal = {Ind. Eng. Chem. Res.},
	author = {Lee, Bong-Seop and Lin, Shiang-Tai},
	month = sep,
	year = {2015},
	pages = {9005--9012},
}

@article{gross_application_2002,
	title = {Application of the {Perturbed}-{Chain} {SAFT} {Equation} of {State} to {Associating} {Systems}},
	volume = {41},
	issn = {0888-5885, 1520-5045},
	url = {https://pubs.acs.org/doi/10.1021/ie010954d},
	doi = {10.1021/ie010954d},
	language = {en},
	number = {22},
	urldate = {2022-01-04},
	journal = {Ind. Eng. Chem. Res.},
	author = {Gross, Joachim and Sadowski, Gabriele},
	month = oct,
	year = {2002},
	pages = {5510--5515},
}

@article{gross_perturbed-chain_2001,
	title = {Perturbed-{Chain} {SAFT}: {An} {Equation} of {State} {Based} on a {Perturbation} {Theory} for {Chain} {Molecules}},
	volume = {40},
	issn = {0888-5885, 1520-5045},
	shorttitle = {Perturbed-{Chain} {SAFT}},
	url = {https://pubs.acs.org/doi/10.1021/ie0003887},
	doi = {10.1021/ie0003887},
	language = {en},
	number = {4},
	urldate = {2022-01-04},
	journal = {Ind. Eng. Chem. Res.},
	author = {Gross, Joachim and Sadowski, Gabriele},
	month = feb,
	year = {2001},
	pages = {1244--1260},
}

@article{bell_algorithm_2022,
	title = {Algorithm to {Identify} {Vapor}–{Liquid}–{Liquid} {Equilibria} of {Binary} {Mixtures} from {Vapor}–{Liquid} {Equilibria}},
	volume = {61},
	issn = {0888-5885},
	url = {https://pubs.acs.org/doi/10.1021/acs.iecr.1c04703},
	doi = {10.1021/acs.iecr.1c04703},
	number = {6},
	journal = {Ind. Eng. Chem. Res.},
	author = {Bell, Ian H. and Deiters, Ulrich K. and Jäger, Andreas},
	month = feb,
	year = {2022},
	pages = {2592--2599},
}

@article{bakhtazma_second-order_2019,
	title = {Second-{Order} {Thermodynamic} {Derivative} {Properties} of {Ionic} {Liquids} from {ePC}-{SAFT}: {The} {Effect} of {Partial} {Ionic} {Dissociation}},
	volume = {58},
	issn = {0888-5885, 1520-5045},
	shorttitle = {Second-{Order} {Thermodynamic} {Derivative} {Properties} of {Ionic} {Liquids} from {ePC}-{SAFT}},
	url = {https://pubs.acs.org/doi/10.1021/acs.iecr.9b05593},
	doi = {10.1021/acs.iecr.9b05593},
	abstract = {Ionic liquids (ILs) are potentially suitable compounds as replacements for organic solvents in chemical processes and play an important role in reducing the production of toxic compounds. In this work, the electrolyte Perturbed-Chain Statistical Associating Fluid Theory (ePCSAFT) equation of state (EoS) was utilized to predict the second-order thermodynamic derivative properties including isothermal compressibility coeﬃcient, thermal expansion coeﬃcient, heat capacities, thermal pressure coeﬃcient, isentropic compressibility coeﬃcient, and speed of sound of imidazolium-based ionic liquids with [BF4]−, [Tf2N]−, and [PF6]− anions. Two ionic dissociation models were considered. The ﬁrst model assumes a complete dissociation of IL molecule into ions (full dissociation), while the second model considers partial dissociation of molecules into ions where molecules, anions, and cations coexist in the liquid phase. The ﬁrst model is convenient when applying ePC-SAFT to ILs. The second model, however, is new within ePC-SAFT. The secondorder thermodynamic derivative properties of pure ILs were predicted with partially and fully ionic dissociation approaches and compared to available experimental data from the literature. The parameters of ePC-SAFT with the partial dissociation approach were estimated by ﬁtting the experimental liquid density from the literature. The comparison of results from the two methods with experimental data showed that the predictions by the partial dissociation approach were more accurate than those by the full dissociation approach. The improved accuracy might be a result of better approximation of the real ionic liquid systems by the partial dissociation assumption.},
	language = {en},
	number = {49},
	urldate = {2022-01-22},
	journal = {Ind. Eng. Chem. Res.},
	author = {Bakhtazma, Farnoosh and Alavi, Farzad},
	month = dec,
	year = {2019},
	pages = {22408--22417},
}

@article{thomas_prediction_1984,
	title = {Prediction of limiting activity coefficients by a modified separation of cohesive energy density model and {UNIFAC}},
	volume = {23},
	issn = {0196-4305, 1541-5716},
	url = {https://pubs.acs.org/doi/abs/10.1021/i200025a002},
	doi = {10.1021/i200025a002},
	language = {en},
	number = {2},
	urldate = {2022-09-11},
	journal = {Ind. Eng. Chem. Proc. Des. Dev.},
	author = {Thomas, Eugene R. and Eckert, Charles A.},
	month = apr,
	year = {1984},
	pages = {194--209},
}

@article{glanville_volumetric_1950,
	title = {Volumetric and {Phase} {Behavior} of {Propane}-{Benzene} {System}},
	volume = {42},
	issn = {0019-7866},
	url = {https://doi.org/10.1021/ie50483a030},
	doi = {10.1021/ie50483a030},
	number = {3},
	urldate = {2022-09-19},
	journal = {Ind. Eng. Chem. Res.},
	author = {Glanville, J. W. and Sage, B. H. and Lacey, W. N.},
	month = mar,
	year = {1950},
	note = {Publisher: American Chemical Society},
	pages = {508--513},
}

@article{walker_importance_2022,
	title = {Importance of the {Relative} {Static} {Permittivity} in electrolyte {SAFT}-{VR} {Mie} {Equations} of {State}},
	volume = {551},
	copyright = {All rights reserved},
	issn = {03783812},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0378381221003198},
	doi = {10.1016/j.fluid.2021.113256},
	language = {en},
	urldate = {2022-01-04},
	journal = {Fluid Phase Equilib.},
	author = {Walker, Pierre J. and Liang, Xiaodong and Kontogeorgis, Georgios M.},
	month = jan,
	year = {2022},
	keywords = {Debye-Hückel, Dielectric Constant, Electrolytes, MSA, SAFT},
	pages = {113256},
}

@article{spyriouni_thermodynamics_2011,
	title = {Thermodynamics of pharmaceuticals: {Prediction} of solubility in pure and mixed solvents with {PC}-{SAFT}},
	volume = {302},
	issn = {03783812},
	shorttitle = {Thermodynamics of pharmaceuticals},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0378381210004565},
	doi = {10.1016/j.fluid.2010.08.029},
	abstract = {A new scheme is presented for the parameterization of pharmaceuticals in the context of the perturbedchain statistical associating ﬂuid theory (PC-SAFT). The pharmaceutical parameters are ﬁtted to experimental solubility values in three different solvents, i.e., a hydrophilic, a polar, and a hydrophobic solvent. Subsequently, the solubility of the pharmaceuticals in other solvents is predicted without the need for additional interaction parameters. The approach is presented for six commonly used pharmaceutical compounds (paracetamol, naproxen, ibuprofen, ﬂurbiprofen, ketoprofen, and lovastatin) in numerous pure and mixed solvents, and in different temperatures.},
	language = {en},
	number = {1-2},
	urldate = {2022-08-01},
	journal = {Fluid Phase Equilib.},
	author = {Spyriouni, Theodora and Krokidis, Xenophon and Economou, Ioannis G.},
	month = mar,
	year = {2011},
	pages = {331--337},
}

@article{singh_excess_1996,
	title = {Excess molar enthalpies of mixing of 1-propanol or 2-propanol with aromatic hydrocarbons at 308.15 {K} in terms of an association model},
	volume = {119},
	issn = {0378-3812},
	url = {https://www.sciencedirect.com/science/article/pii/037838129502865X},
	doi = {10.1016/0378-3812(95)02865-X},
	abstract = {Heat of mixing data for 1-propanol or 2-propanol with benzene, toluene, o-xylene, m-xylene and p-xylene at 308.15 K have been reported. The analysis in terms of the Mecke-Kempter association model with a Flory contribution term and generalized quasi-lattice model by Barker is described.},
	language = {en},
	number = {1},
	urldate = {2022-09-19},
	journal = {Fluid Phase Equilib.},
	author = {Singh, K. C. and Kalra, K. C. and Maken, Sanjeev and Gupta, Vibha},
	month = may,
	year = {1996},
	keywords = {Associated, Excess enthalpy, Excess volume, Flory theory, MK model},
	pages = {175--190},
}

@article{pereira_duality-based_2010,
	title = {A duality-based optimisation approach for the reliable solution of ({P}, {T}) phase equilibrium in volume-composition space},
	volume = {299},
	issn = {03783812},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0378381210004048},
	doi = {10.1016/j.fluid.2010.08.001},
	abstract = {A reliable algorithm for the solution of ﬂuid phase equilibrium at constant pressure and temperature (P, T ﬂash) is presented. The approach is applicable to multi-component mixtures described with general equations of state and is based on a formulation of P, T phase equilibrium as a dual optimisation problem in volume-composition space, translated away from the Gibbs free energy to the Helmholtz free energy. This formulation facilitates the use of guaranteed solution algorithms, particularly in the case of sophisticated equations of state (EOSs) such as SAFT (statistical associating ﬂuid theory), because such representations are higher-than-cubic functions in volume and are formulated in the Helmholtz free energy. With the proposed algorithm (which is based on a combination of local and global optimisation, where the number of subproblems to be solved globally is kept at a minimum) one is guaranteed to identify the number of stable phases present at equilibrium, along with their properties, without any need for initial guesses, or indeed any a priori knowledge about the behaviour of the system. The method is applicable to the calculation of any kind of ﬂuid phase behaviour (e.g., vapour–liquid (VLE), liquid–liquid (LLE), vapour–liquid–liquid (VLLE), etc.). Several algorithmic options are investigated and their computational performance compared. A prototype implementation is used to determine the ﬂuid phase equilibria of a number of binary and ternary systems, where the thermodynamic properties are calculated through a molecular-based EOS. Examples are shown for the VLE and VLLE for mixtures modelled with an augmented van der Waals EOS, a non-cubic EOS that incorporates the Carnahan and Starling representation of the repulsive interactions. Further examples are presented for VLE and VLLE in polymer systems, modelled with an EOS of the generic SAFT form. Fluid phase equilibrium calculations for polymer systems are notoriously difﬁcult, and convergence problems are often encountered, even with good initial guesses. The proposed method is found to be reliable in all cases examined.},
	language = {en},
	number = {1},
	urldate = {2022-04-25},
	journal = {Fluid Phase Equilib.},
	author = {Pereira, Frances E. and Jackson, George and Galindo, Amparo and Adjiman, Claire S.},
	month = dec,
	year = {2010},
	pages = {1--23},
}

@article{oakley_first_2010,
	title = {First principles models of the interactions of methane and carbon dioxide},
	volume = {290},
	issn = {03783812},
	doi = {10.1016/j.fluid.2009.11.011},
	abstract = {We present ab initio calculations on the CH4-CH4 and CH4-CO2 dimer potential energy surfaces. We show that the fit to these surfaces is improved over the Lennard-Jones potential by changing the form of the repulsive wall. Ab initio calculations are also performed on trimers to evaluate the strength of nonadditive interactions. The experimental CH4 phase properties are reproduced in simulations that include correction for nonadditive dispersion. The phase-coexistence curve of mixtures of CH4 and CO2 is also improved by including this nonadditive dispersion term. © 2009 Elsevier B.V. All rights reserved.},
	number = {1-2},
	journal = {Fluid Phase Equilib.},
	author = {Oakley, Mark T. and Do, Hainam and Wheatley, Richard J.},
	month = mar,
	year = {2010},
	keywords = {Ab initio calculations, Gibbs ensemble, Potential energy surface, Vapor-liquid equilibrium},
	pages = {48--54},
}

@article{naeem_pepc-saft_2011,
	title = {{pePC}-{SAFT}: {Modeling} of polyelectrolyte systems 2. {Aqueous} two-phase systems},
	volume = {306},
	issn = {03783812},
	shorttitle = {{pePC}-{SAFT}},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0378381211001105},
	doi = {10.1016/j.fluid.2011.02.024},
	language = {en},
	number = {1},
	urldate = {2022-04-19},
	journal = {Fluid Phase Equilib.},
	author = {Naeem, Shahbaz and Sadowski, Gabriele},
	month = jul,
	year = {2011},
	pages = {67--75},
}

@article{naeem_pepc-saft_2010,
	title = {{pePC}-{SAFT}: {Modeling} of polyelectrolyte systems},
	volume = {299},
	issn = {03783812},
	shorttitle = {{pePC}-{SAFT}},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0378381210004590},
	doi = {10.1016/j.fluid.2010.09.004},
	abstract = {A molecular thermodynamic model for polyelectrolyte systems—called pePC-SAFT—is proposed. The effect of charged monomers within the polyelectrolyte chain is explicitly taken into account in the reference term by replacing the hard-chain contribution of the PC-SAFT model by a charged-hard-chain contribution. Moreover, counterion condensation is accounted for to determine the effective number of charges along the polyion as well as of free counterions. The electrostatic contribution of the free counterions is described by a Debye–Hückel term.},
	language = {en},
	number = {1},
	urldate = {2022-04-19},
	journal = {Fluid Phase Equilib.},
	author = {Naeem, Shahbaz and Sadowski, Gabriele},
	month = dec,
	year = {2010},
	pages = {84--93},
}

@article{ji_modeling_2012,
	title = {Modeling imidazolium-based ionic liquids with {ePC}-{SAFT}},
	volume = {335},
	issn = {03783812},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0378381212003846},
	doi = {10.1016/j.fluid.2012.05.029},
	language = {en},
	urldate = {2022-01-04},
	journal = {Fluid Phase Equilib.},
	author = {Ji, Xiaoyan and Held, Christoph and Sadowski, Gabriele},
	month = dec,
	year = {2012},
	pages = {64--73},
}

@article{jaubert_impressive_2022,
	title = {The impressive impact of including enthalpy and heat capacity of mixing data when parameterising equations of state. {Application} to the development of the {E}-{PPR78} ({Enhanced}-{Predictive}-{Peng}-{Robinson}-78) model.},
	issn = {03783812},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0378381222000814},
	doi = {10.1016/j.fluid.2022.113456},
	journal = {Fluid Phase Equilib.},
	author = {Jaubert, Jean-Noël and Qian, Jun-Wei and Lasala, Silvia and Privat, Romain},
	month = mar,
	year = {2022},
	pages = {113456},
}

@article{held_modeling_2008,
	title = {Modeling aqueous electrolyte solutions {Part} 1. {Fully} dissociated electrolytes},
	abstract = {Liquid densities (pvT), vapor pressures (VLE), and mean ionic activity coefﬁcients (MIAC) at 25 ◦C of 115 single-salt electrolyte solutions containing univalent up to trivalent ions are modeled with the ePC-SAFT equation of state proposed by Cameretti et al. [L.F. Cameretti, G. Sadowski, J.M. Mollerup, Ind. Eng. Chem. Res. 44 (2005) 3355–3362; ibid., 8944]. For each ion, only two model parameters were adjusted to experimental density and MIAC data. Without using any additional binary parameters, ePC-SAFT is able to reproduce experimental data of the respective salt solutions up to high electrolyte molalities. Moreover, it is even able to describe the reversed MIAC series for alkali hydroxides and ﬂuorides.},
	language = {en},
	journal = {Fluid Phase Equilib.},
	author = {Held, Christoph and Cameretti, Luca F and Sadowski, Gabriele},
	year = {2008},
	pages = {10},
}

@article{guerrero-zarate_calculation_2017,
	title = {Calculation of critical points for natural gas mixtures with the {GERG}-2008 equation of state},
	volume = {437},
	issn = {03783812},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0378381217300213},
	doi = {10.1016/j.fluid.2017.01.012},
	journal = {Fluid Phase Equilib.},
	author = {Guerrero-Zárate, David and Estrada-Baltazar, Alejandro and Iglesias-Silva, Gustavo A.},
	month = apr,
	year = {2017},
	pages = {69--82},
}

@article{gross_application_2000,
	title = {Application of perturbation theory to a hard-chain reference fluid: an equation of state for square-well chains},
	volume = {168},
	issn = {03783812},
	shorttitle = {Application of perturbation theory to a hard-chain reference fluid},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0378381200003022},
	doi = {10.1016/S0378-3812(00)00302-2},
	abstract = {An equation of state for square-well chain fluids is developed applying the second-order perturbation theory of Barker and Henderson to a hard-chain reference fluid. The structural information required in the perturbation theory is incorporated using an expression for the radial distribution function of the reference chain fluid proposed by Chiew. The equation of state is simplified by fitting polynomials in density and simple functions of segment number to the original perturbation expressions of first-and second-order. The equation of state is extended to mixtures by applying one-fluid mixing rules and is tested against molecular simulation data of homonuclear chain molecules and mixtures from the literature. q 2000 Elsevier Science B.V. All rights reserved.},
	language = {en},
	number = {2},
	urldate = {2022-01-04},
	journal = {Fluid Phase Equilib.},
	author = {Gross, Joachim and Sadowski, Gabriele},
	month = feb,
	year = {2000},
	pages = {183--199},
}

@article{gloor_saftdft_2002,
	title = {A {SAFT}–{DFT} approach for the vapour–liquid interface of associating fluids},
	volume = {194-197},
	issn = {03783812},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0378381201007749},
	doi = {10.1016/S0378-3812(01)00774-9},
	abstract = {We present a density functional theory (DFT) based on the statistical associating ﬂuid theory (SAFT) bulk free energy to describe the behaviour of inhomogeneous associating molecular ﬂuids, with a special emphasis on the vapour–liquid interface. The molecules are described in terms of hard-sphere (HS) segments which interact through an arbitrary intermolecular potential. Off-centre square-well bonding sites are incorporated to mediate the association between molecules. The approach presented here is based on a perturbation theory about a HS reference ﬂuid under the local density approximation (LDA); the contributions due to chain formation and association are also considered at the local density level. The Helmholtz free energy functional due to the dispersive attractive interactions is treated at the mean-ﬁeld level by ignoring the correlations. This description is essentially a ‘van der Waals’ theory of non-uniform ﬂuids. The incorporation of a SAFT free energy of the bulk associating ﬂuid represents the simplest extension of the theory to deal with inhomogeneous associating systems (SAFT–DFT). The resulting functional is used to investigate the effect of the range of the attractive interactions on the interfacial properties, such as the density proﬁle and surface tension, for two different intermolecular potential models, namely the Yukawa and square-well. This simple SAFT–DFT approach is also used to make quantitative comparisons with the experimental surface tension for water. © 2002 Elsevier Science B.V. All rights reserved.},
	language = {en},
	urldate = {2022-06-22},
	journal = {Fluid Phase Equilib.},
	author = {Gloor, Guy J. and Blas, Felipe J. and del Rı́o, Elvira Martı́n and de Miguel, Enrique and Jackson, George},
	month = mar,
	year = {2002},
	pages = {521--530},
}

@article{feroiu_computation_1990,
	title = {Computation of vapour—liquid equilibrium in {N2} + {CO2} + {CH4} system by a general cubic equation of state},
	volume = {55},
	issn = {03783812},
	url = {https://linkinghub.elsevier.com/retrieve/pii/0378381290850223},
	doi = {10.1016/0378-3812(90)85022-3},
	language = {en},
	number = {3},
	urldate = {2022-08-01},
	journal = {Fluid Phase Equilib.},
	author = {Feroiu, Viorel and Geana, Dan},
	month = dec,
	year = {1990},
	pages = {263--270},
}

@article{deiters_differential_2016,
	title = {Differential equations for the calculation of fluid phase equilibria},
	volume = {428},
	issn = {03783812},
	url = {http://dx.doi.org/10.1016/j.fluid.2016.04.014},
	doi = {10.1016/j.fluid.2016.04.014},
	abstract = {The thermodynamic conditions for isothermal or isobaric two-phase boundaries of fluid mixtures are expressed as sets of first-order ordinary differential equations. In contrast to the Gibbs–Konovalov equations, the new equations use molar densities instead of mole fractions. The resulting formalism is applicable to multicomponent mixtures, well-suited for machine calculations, and allows a very rapid calculation of phase diagrams.},
	journal = {Fluid Phase Equilib.},
	author = {Deiters, Ulrich K.},
	year = {2016},
	note = {Publisher: Elsevier Ltd},
	keywords = {Algorithm, Fluid phase equilibria, Gibbs–Konovalov equations, Multicomponent mixtures},
	pages = {164--173},
}

@article{das_saft-vrequation_2016,
	title = {A {SAFT}-{VR}+{DE} equation of state based approach for the study of mixed dipolar solvent electrolytes},
	volume = {416},
	issn = {03783812},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0378381215302326},
	doi = {10.1016/j.fluid.2015.11.027},
	abstract = {The SAFT-VRþDE approach was developed by combining the statistical associating ﬂuid theory for potentials of variable range (SAFT-VR) with integral equation theory and the generalized mean spherical approximation using a non-primitive model, in order to explicitly describe the solvent in electrolyte solutions. Subsequently, the theory was applied to study nineteen different aqueous electrolyte solutions and a range of thermodynamic properties across different temperatures and salt concentrations were successfully predicted. Here, the theory is applied to study several model mixed dipolar solvent electrolytes in order to validate a simple one-ﬂuid-like approximation that is proposed to describe the interactions between ions and dipolar solvents of arbitrary size and dipole moment. Before application to real ﬂuids the approach is extensively tested through comparison with isothermal-isobaric ensemble (NPT) Monte Carlo simulations for a number of model mixed dipolar solvent electrolyte systems. Simulations have been performed for different ionic concentrations, solvent compositions, cation, anion, and solvent segment diameters, and solvent polarity. The results show that the SAFT-VRþDE equation provides a good description of the PVT behavior of the model mixed solvent electrolyte systems studied, with some over-prediction of the PVT behavior observed only at higher ionic concentrations. Additionally, comparisons are made between predictions from the non-primitive and primitive models for electrolytes and the importance of capturing the effect of ions on the solvent dielectric is demonstrated. © 2015 Elsevier B.V. All rights reserved.},
	language = {en},
	urldate = {2021-09-30},
	journal = {Fluid Phase Equilib.},
	author = {Das, Gaurav and Hlushak, Stepan and McCabe, Clare},
	month = may,
	year = {2016},
	pages = {72--82},
}



@article{abdollahi-demneh_comparison_2010,
	title = {Comparison of the prediction power of 23 generalized equations of state: {Part} {I}. {Saturated} thermodynamic properties of 102 pure substances},
	volume = {288},
	issn = {03783812},
	shorttitle = {Comparison of the prediction power of 23 generalized equations of state},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0378381209004075},
	doi = {10.1016/j.fluid.2009.10.006},
	abstract = {Accurate representation of the thermodynamic properties of pure compounds is required to increase the robustness of an equation of state (EOS) when predicting phase equilibria for mixtures. With this purpose, 23 generalized equations of state (EOSs) have been applied to predict the thermodynamic properties of 102 pure substances (16,107 data points) and to report the average absolute deviations of these properties from experimental values. Investigated thermodynamic properties are: vapor pressure, saturated vapor and liquid molar volume, molar enthalpy and entropy of vaporization and saturated liquid molar isobaric heat capacity. Furthermore, behavior of the cubic and non-cubic EOSs in the vicinity of the critical point has been elucidated. Pure compounds which have been used in this study can be classiﬁed as elements (monatomic and diatomic), oxides, alkanes, naphthenes, halogenated alkanes, alkenes, cyclic aliphatics, alkynes, dienes, alcohols, aromatics, ethers and miscellaneous groups (consisting of acetone, ethyl acetate and ammonia). Based on obtained average absolute deviations, it can be concluded that LKP (Lee–Kesler–Plöcker et al.), TBS (Trebble–Bishnoi–Salim), TB (Trebble–Bishnoi), MNM (modiﬁed Nasrifar–Moshfeghian), MMM (Mohsen-Nia–Modarres–Mansoori), PT (Patel–Teja) and PRGGPR (Gasem–Gao–Pan–Robinson modiﬁcation to the Peng–Robinson EOS) EOSs, respectively have the most accurate predictions among the 23 studied generalized EOSs for the above-mentioned saturated thermodynamic properties of the 102 pure components investigated.},
	language = {en},
	number = {1-2},
	urldate = {2022-08-01},
	journal = {Fluid Phase Equilib.},
	author = {Abdollahi-Demneh, F. and Moosavian, M.A. and Montazer-Rahmati, M.M. and Omidkhah, M.R. and Bahmaniar, H.},
	month = jan,
	year = {2010},
	pages = {67--82},
}

@article{aasen_accurate_2020,
	title = {Accurate quantum-corrected cubic equations of state for helium, neon, hydrogen, deuterium and their mixtures},
	volume = {524},
	issn = {03783812},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0378381220303381},
	doi = {10.1016/j.fluid.2020.112790},
	journal = {Fluid Phase Equilib.},
	author = {Aasen, Ailo and Hammer, Morten and Lasala, Silvia and Jaubert, Jean-Noël and Wilhelmsen, Øivind},
	month = dec,
	year = {2020},
	pages = {112790},
}

@article{dong_span_2022,
	title = {{\textless}span style="font-variant:small-caps;"{\textgreater}{SAFT}{\textless}/span{\textgreater} ‐γ {Mie} model for ionic liquids},
	issn = {0001-1541, 1547-5905},
	shorttitle = {{\textless}span style="font-variant},
	url = {https://onlinelibrary.wiley.com/doi/10.1002/aic.17697},
	doi = {10.1002/aic.17697},
	abstract = {The SAFT-γ Mie model is a recent version of statistical associating fluid theory (SAFT), which uses a group contribution approach to obtain a high-quality equation of state. In this work, this model is, for the first time, extended to ionic liquids (ILs). The SAFT-γ Mie calculated values agree well with the experimental data for onecomponent, binary and ternary systems that contain ILs, thus indicating the versatility and accuracy of this extension.},
	language = {en},
	urldate = {2022-04-18},
	journal = {AIChE J.},
	author = {Dong, Yichun and Warsahartana, Hubertus Gilbert and Hammad, Faisal and Masters, Andrew},
	month = apr,
	year = {2022},
}

@article{deiters_calculation_2019,
	title = {Calculation of phase envelopes of fluid mixtures through parametric marching},
	volume = {65},
	issn = {0001-1541},
	url = {https://onlinelibrary.wiley.com/doi/10.1002/aic.16730},
	doi = {10.1002/aic.16730},
	number = {11},
	journal = {AIChE J.},
	author = {Deiters, Ulrich K. and Bell, Ian H.},
	month = nov,
	year = {2019},
}

@article{butcher_thermodynamic_2007,
	title = {Thermodynamic properties of methanol-benzene mixtures at elevated temperatures},
	volume = {18},
	issn = {00218871},
	url = {https://onlinelibrary.wiley.com/doi/10.1002/jctb.5010180402},
	doi = {10.1002/jctb.5010180402},
	number = {4},
	journal = {J. Appl. Chem.},
	author = {Butcher, K. L. and Medani, M. S.},
	month = may,
	year = {2007},
	pages = {100--107},
}

@misc{winter_spt-nrtl_2022,
	title = {{SPT}-{NRTL}: {A} physics-guided machine learning model to predict thermodynamically consistent activity coefficients},
	shorttitle = {{SPT}-{NRTL}},
	url = {http://arxiv.org/abs/2209.04135},
	doi = {10.48550/arXiv.2209.04135},
	abstract = {The availability of property data is one of the major bottlenecks in the development of chemical processes, often requiring time-consuming and expensive experiments or limiting the design space to a small number of known molecules. This bottleneck has been the motivation behind the continuing development of predictive property models. For the property prediction of novel molecules, group contribution methods have been groundbreaking. In recent times, machine learning has joined the more established property prediction models. However, even with recent successes, the integration of physical constraints into machine learning models remains challenging. Physical constraints are vital to many thermodynamic properties, such as the Gibbs-Dunham relation, introducing an additional layer of complexity into the prediction. Here, we introduce SPT-NRTL, a machine learning model to predict thermodynamically consistent activity coefficients and provide NRTL parameters for easy use in process simulations. The results show that SPT-NRTL achieves higher accuracy than UNIFAC in the prediction of activity coefficients across all functional groups and is able to predict many vapor-liquid-equilibria with near experimental accuracy, as illustrated for the exemplary mixtures water/ethanol and chloroform/n-hexane. To ease the application of SPT-NRTL, NRTL-parameters of 100 000 000 mixtures are calculated with SPT-NRTL and provided online.},
	urldate = {2022-09-20},
	publisher = {arXiv},
	author = {Winter, Benedikt and Winter, Clemens and Esper, Timm and Schilling, Johannes and Bardow, André},
	month = sep,
	year = {2022},
	note = {arXiv:2209.04135 [physics]},
	keywords = {Computer Science - Machine Learning, Physics - Chemical Physics},
}

@article{turq_conductance_1995,
	title = {Conductance in {Associated} {Electrolytes} {Using} the {Mean} {Spherical} {Approximation}},
	volume = {99},
	issn = {0022-3654, 1541-5740},
	url = {https://pubs.acs.org/doi/abs/10.1021/j100002a053},
	doi = {10.1021/j100002a053},
	language = {en},
	number = {2},
	urldate = {2022-06-04},
	journal = {The Journal of Physical Chemistry},
	author = {Turq, Pierre and Blum, Lesser and Bernard, Olivier and Kunz, Werner},
	month = jan,
	year = {1995},
	pages = {822--827},
}

@article{cameretti_statistical_2005,
	title = {Statistical {Associated} {Fluid} {Theory}},
	doi = {10.1021/ie0488142},
	author = {Cameretti, Luca F and Sadowski, Gabriele},
	year = {2005},
	pages = {3355--3362},
}

@article{gupta_molar_1996,
	title = {Molar excess volumes of 1-propanol or 2-propanol + cyclohexane or aromatic hydrocarbons at 303.15 {K}},
	volume = {35},
	number = {6},
	journal = {Indian J. Chem. Sect. A},
	author = {Gupta, V. and Maken, S and Kalra, K.},
	year = {1996},
	pages = {508--512},
}

@article{udovenko_liquid-vapor_1967,
	title = {Liquid-{Vapor} {Equilibrium} in the {Propan}-2-ol - {Water} and {Propan}-2-ol - {Benzene} {Systems}},
	volume = {41},
	number = {7},
	journal = {Zh. Fiz. Khim.},
	author = {Udovenko, V.V. and Mazanko, T.F.},
	year = {1967},
	pages = {1615--1618},
}

@article{son_ion_2020,
	title = {Ion transport in small-molecule and polymer electrolytes},
	volume = {153},
	issn = {0021-9606, 1089-7690},
	url = {http://aip.scitation.org/doi/10.1063/5.0016163},
	doi = {10.1063/5.0016163},
	abstract = {Solid-state polymer electrolytes and high-concentration liquid electrolytes, such as water-in-salt electrolytes and ionic liquids, are emerging materials to replace the flammable organic electrolytes widely used in industrial lithium-ion batteries. Extensive efforts have been made to understand the ion transport mechanisms and optimize the ion transport properties. This perspective reviews the current understanding of the ion transport and polymer dynamics in liquid and polymer electrolytes, comparing the similarities and differences in the two types of electrolytes. Combining recent experimental and theoretical findings, we attempt to connect and explain ion transport mechanisms in different types of small-molecule and polymer electrolytes from a theoretical perspective, linking the macroscopic transport coefficients to the microscopic, molecular properties such as the solvation environment of the ions, salt concentration, solvent/polymer molecular weight, ion pairing, and correlated ion motion. We emphasize universal features in the ion transport and polymer dynamics by highlighting the relevant time and length scales. Several outstanding questions and anticipated developments for electrolyte design are discussed, including the negative transference number, control of ion transport through precision synthesis, and development of predictive multiscale modeling approaches.},
	language = {en},
	number = {10},
	urldate = {2022-09-14},
	journal = {The Journal of Chemical Physics},
	author = {Son, Chang Yun and Wang, Zhen-Gang},
	month = sep,
	year = {2020},
	pages = {100903},
}

@article{sha_dilute_2015,
	title = {Dilute or {Concentrated} {Electrolyte} {Solutions}? {Insight} from {Ionic} {Liquid}/{Water} {Electrolytes}},
	volume = {6},
	issn = {1948-7185, 1948-7185},
	shorttitle = {Dilute or {Concentrated} {Electrolyte} {Solutions}?},
	url = {https://pubs.acs.org/doi/10.1021/acs.jpclett.5b01513},
	doi = {10.1021/acs.jpclett.5b01513},
	abstract = {When room-temperature ionic liquids (IL) are used as an electrolyte, their transport behaviors are still under heavy debate due to their complicated ion-associations. In this article, we conducted molecular dynamics simulations to study the molecular scale ion associations from the very dilute 1butyl-3-methylimidazolium iodide/water solution to the pure IL. It revealed that ions are localized in a multicoordinated ion cage structure with nanoseconds in concentrated IL solutions. Dynamics analyses indicate that the transport of this solution can be depicted by the Debye−Hückel model only in dilute IL/water electrolyte. The velocity and rotational correlation functions showed that the lifetime of translational and rotational motions are at the level of picoseconds and nanoseconds, respectively, because of the ion cage eﬀect. The lifetime of ion association demonstrated that the recombination of association ions was prevalent in IL solutions. It means that the dipolar or stable contact ion-pairs model may not be suitable for depicting the IL transport.},
	language = {en},
	number = {18},
	urldate = {2022-09-14},
	journal = {The Journal of Physical Chemistry Letters},
	author = {Sha, Maolin and Dong, Huaze and Luo, Fabao and Tang, Zhongfeng and Zhu, Guanglai and Wu, Guozhong},
	month = sep,
	year = {2015},
	pages = {3713--3720},
}

@article{bekker_prediction_1987,
	title = {Prediction of solvent activities using the {UNIFAC}-{FV} model},
	volume = {16},
	issn = {0095-9782, 1572-8927},
	url = {http://link.springer.com/10.1007/BF00649090},
	doi = {10.1007/BF00649090},
	language = {en},
	number = {8},
	urldate = {2022-09-08},
	journal = {Journal of Solution Chemistry},
	author = {Bekker, Alex Y. and Knox, Dana E. and Sund, Steven E.},
	month = aug,
	year = {1987},
	pages = {635--639},
}

@article{tai_mathematical_1994,
	title = {A {Mathematical} {Model} for the {Determination} of {Total} {Area} {Under} {Glucose} {Tolerance} and {Other} {Metabolic} {Curves}},
	volume = {17},
	issn = {0149-5992},
	url = {https://doi.org/10.2337/diacare.17.2.152},
	doi = {10.2337/diacare.17.2.152},
	abstract = {To develop a mathematical model for the determination of total areas under curves from various metabolic studies.In Tai's Model, the total area under a curve is computed by dividing the area under the curve between two designated values on the X-axis (abscissas) into small segments (rectangles and triangles) whose areas can be accurately calculated from their respective geometrical formulas. The total sum of these individual areas thus represents the total area under the curve. Validity of the model is established by comparing total areas obtained from this model to these same areas obtained from graphic method Gess than ±0.4\%). Other formulas widely applied by researchers under- or overestimated total area under a metabolic curve by a great margin.Tai's model proves to be able to 1) determine total area under a curve with precision; 2) calculate area with varied shapes that may or may not intercept on one or both X/Y axes; 3) estimate total area under a curve plotted against varied time intervals (abscissas), whereas other formulas only allow the same time interval; and 4) compare total areas of metabolic curves produced by different studies.The Tai model allows flexibility in experimental conditions, which means, in the case of the glucose-response curve, samples can be taken with differing time intervals and total area under the curve can still be determined with precision.},
	number = {2},
	urldate = {2022-09-04},
	journal = {Diabetes Care},
	author = {Tai, Mary M},
	month = feb,
	year = {1994},
	pages = {152--154},
}

@article{tanaka_general_2000,
	title = {General view of a liquid-liquid phase transition},
	volume = {62},
	issn = {1063-651X, 1095-3787},
	url = {https://link.aps.org/doi/10.1103/PhysRevE.62.6968},
	doi = {10.1103/PhysRevE.62.6968},
	language = {en},
	number = {5},
	urldate = {2022-09-02},
	journal = {Physical Review E},
	author = {Tanaka, Hajime},
	month = nov,
	year = {2000},
	pages = {6968--6976},
}

@article{tanaka_two-order-parameter_1999,
	title = {Two-order-parameter description of liquids: critical phenomena and phase separation of supercooled liquids},
	volume = {11},
	issn = {0953-8984, 1361-648X},
	shorttitle = {Two-order-parameter description of liquids},
	url = {https://iopscience.iop.org/article/10.1088/0953-8984/11/15/005},
	doi = {10.1088/0953-8984/11/15/005},
	abstract = {Because of the isotropic and disordered nature of liquids, anisotropy hidden in manybody intermolecular interactions is usually neglected. Thus, it has been believed so far that the only order parameter required to describe a simple liquid is the density. Not accepting this common-sense view, we argue that a new additional order parameter, which represents the spontaneous formation of locally favoured structures, is necessary for the physical description of liquids near the lower stability limit. This model explains well two mysterious phenomena of supercooled liquids: (i) the large-scale density ﬂuctuations known as ‘Fischer clusters’ and (ii) the phase separation of a onecomponent liquid into two phases.},
	language = {en},
	number = {15},
	urldate = {2022-09-02},
	journal = {Journal of Physics: Condensed Matter},
	author = {Tanaka, Hajime},
	month = apr,
	year = {1999},
	pages = {L159--L168},
}

@article{rybinska-fryca_prediction_2018,
	title = {Prediction of dielectric constant of ionic liquids},
	volume = {260},
	issn = {0167-7322},
	url = {https://www.sciencedirect.com/science/article/pii/S016773221735660X},
	doi = {10.1016/j.molliq.2018.03.080},
	abstract = {Ionic liquids are compounds commonly used as solvents in many fields of chemistry such as electrochemistry or separation techniques. One of the crucial properties for accommodation of the appropriate solvent to the specific process, is the solvation power of the solvent. It is usually expressed by the polarity and could be measured by the dielectric constant value (ε). Unfortunately, in case of ionic liquids there is a lack of available experimental data for dielectric constant. For that reason, this work presents a new approach that allows to find relationship between structural features and dielectric constant value. Our approach is based on the quantitative structure–property relationship (QSPR) method, therefore no additional experimental data is required. In this study, we found that both the ions have impact on the modeled value. Structural features like size, branching and polarizability play the main role in case of cation. However, the mass and shape of the anion are also important. Additionally, predictive ability of our approach was tested by using external data set. Moreover, the developed QSPR model have been additionally applied for estimating dielectric constant for new computationally designed 15,000 ionic liquids.},
	language = {en},
	urldate = {2022-08-26},
	journal = {Journal of Molecular Liquids},
	author = {Rybinska-Fryca, Anna and Sosnowska, Anita and Puzyn, Tomasz},
	month = jun,
	year = {2018},
	keywords = {Dielectric constant, Ionic liquids, QSPR},
	pages = {57--64},
}

@article{zheng_hydrogen-bonding_2014,
	title = {Hydrogen-bonding interactions between [{BMIM}][{BF4}] and dimethyl sulfoxide},
	volume = {1069},
	issn = {00222860},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0022286014000441},
	doi = {10.1016/j.molstruc.2014.01.013},
	abstract = {Mixtures of Ionic liquids and small polar organic solvent are potential green solvents for cellulose dissolution under mild conditions. In this work, the interactions between a representative imidazolium-based ionic liquid 1-butyl-3-methylimidazolium tetraﬂuoroborate ([BMIM][BF4]) and dimethyl sulfoxide (DMSO) were investigated in detail by attenuated total reﬂection infrared spectroscopy (ATR-IR) and density functional theory calculations (DFT). The main conclusions are: (1) C2–H is the main interaction site in forming cation–anion, cation–DMSO, and [BMIM][BF4]–DMSO complexes. (2) The two turning points of the wavenumber shift changes of C2–H may indicate that the dilution process can be divided into several stages: from larger ion clusters to smaller ion clusters, then to ion pairs, and ﬁnally to individual ions. The solvent molecules cannot break apart the strong Coulombic interaction between [BMIM]+ and [BF4]À but can break apart the ion clusters into ion pairs when the mole fraction of DMSO is less than 0.9. When the mole fraction of DMSO is greater than 0.9, ion pairs can be broke into ions. (3) The hydrogen-bonds of the aromatic C–Hs in [BMIM]+ are strengthened in the dilution process while those of the alkyl C–Hs of [BMIM]+ are weakened. (4) The aromatic C–Hs of the [BMIM]+ cation strength before the weakening of the alkyl C–Hs. These in-depth studies on the properties of the ionic liquid-DMSO mixed solvents may shed light on exploring their applications as mixed solvents in cellulose dissolution and other practices. Ó 2014 Elsevier B.V. All rights reserved.},
	language = {en},
	urldate = {2022-06-22},
	journal = {Journal of Molecular Structure},
	author = {Zheng, Yan-Zhen and He, Hong-Yan and Zhou, Yu and Yu, Zhi-Wu},
	month = jul,
	year = {2014},
	pages = {140--146},
}

@article{wu_densities_2014,
	title = {The densities and viscosities of a binary liquid mixture of 1-n-butyl-3-methylimidazolium tetrafluoroborate, ([{Bmim}][{BF4}]) with acetone, methyl ethyl ketone and {N},{N}-dimethylformamide, at 303.15 to 333.{15K}},
	volume = {45},
	issn = {18761070},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S1876107014001175},
	doi = {10.1016/j.jtice.2014.04.012},
	language = {en},
	number = {5},
	urldate = {2022-06-22},
	journal = {Journal of the Taiwan Institute of Chemical Engineers},
	author = {Wu, Jheng-Yu and Chen, Yan-Ping and Su, Chie-Shaan},
	month = sep,
	year = {2014},
	pages = {2205--2211},
}

@article{chaudhary_thermophysical_2014,
	title = {Thermophysical and {Spectroscopic} {Studies} of {Pure} 1-{Butyl}-3-methylimidazolium {Tetrafluoroborate} and {Its} {Aqueous} {Mixtures}},
	volume = {43},
	issn = {0095-9782, 1572-8927},
	url = {http://link.springer.com/10.1007/s10953-014-0137-8},
	doi = {10.1007/s10953-014-0137-8},
	abstract = {Intermolecular interactions in the aqueous mixtures of the room temperature ionic liquid, 1-butyl-3-methylimidazolium tetraﬂuoroborate ([BMIM][BF4]), have been studied. The thermophysical properties: density q, speed of sound u, speciﬁc conductivity j and refractive index nD have been measured over the whole composition range at different temperatures (293.15–323.15 K) and are discussed. The results from thermophysical measurements are explained with the help of spectroscopy. In order to interpret the nature of molecular interactions occurring between [BMIM][BF4] and water molecules, as well as to identify the moieties in which interactions are taking place, 1H, 13C NMR and FT-IR spectra of the solutions have been studied. Excess molar volume VE, excess molar isentropic compressibility KSE, partial molar excess volume ViE, partial molar excess isentropic compressibility KSE;i, deviation in speciﬁc conductivity Dj, and deviation in refractive index DR have also been determined and analyzed to have a better understanding of the interactions taking place between the different components. Additionally, the excess ultrasonic speed uE and excess isentropic compressibility kSE, in terms of volume fractions, have been calculated and analyzed. It has been observed that temperature has a signiﬁcant effect on the thermophysical properties of the studied system. Spectroscopic measurements conﬁrm the disruption of ion-pair interactions of [BMIM][BF4] and hydrogen-bonded network of water in the aqueous mixture of [BMIM][BF4].},
	language = {en},
	number = {2},
	urldate = {2022-04-18},
	journal = {Journal of Solution Chemistry},
	author = {Chaudhary, Ganga Ram and Bansal, Shafila and Mehta, S. K. and Ahluwalia, A. S.},
	month = feb,
	year = {2014},
	pages = {340--359},
}

@article{nyamapfene_does_2010,
	title = {Does class attendance still matter?},
	volume = {5},
	issn = {1750-0052, 1750-0044},
	url = {https://www.tandfonline.com/doi/full/10.11120/ened.2010.05010064},
	doi = {10.11120/ened.2010.05010064},
	abstract = {This paper presents a study on the impact of class attendance on academic performance in a second year Electronics Engineering course module with online notes and no mandatory class attendance policy. The study shows that class attendance is highly correlated to academic performance, despite the availability of online class notes. In addition, there is significant correlation between class attendance and non-class contact with the lecturer and between student performance in the first year of university study and current academic performance and class attendance. However, there is no correlation between pre-university academic performance and current class attendance and academic performance. The study finds no gender bias in either class attendance or academic performance. Lastly, this being a course module open to students following different degree programmes, the study finds that a student’s choice of degree programme has no impact on class attendance and academic performance in this particular course module.},
	language = {en},
	number = {1},
	urldate = {2022-08-01},
	journal = {Engineering Education},
	author = {Nyamapfene, Abel},
	month = jun,
	year = {2010},
	pages = {64--74},
}

@article{bouillot_solubility_2017,
	title = {Solubility of pharmaceuticals: {A} comparison between {SciPharma}, a {PC}-{SAFT}-based approach, and {NRTL}-{SAC}},
	volume = {226},
	issn = {1951-6355, 1951-6401},
	shorttitle = {Solubility of pharmaceuticals},
	url = {http://link.springer.com/10.1140/epjst/e2016-60225-5},
	doi = {10.1140/epjst/e2016-60225-5},
	abstract = {The solubility of seven pharmaceutical compounds (paracetamol, benzoic acid, 4-aminobenzoic acid, salicylic acid, ibuprofen, naproxen and temazepam) in pure and mixed solvents as a function of temperature is calculated with SciPharma, a semi-empirical approach based on PC-SAFT, and the NRTL-SAC model. To conduct a fair comparison between the approaches, the parameters of the compounds were regressed against the same solubility data, chosen to account for hydrophilic, polar and hydrophobic interactions. Only these solubility data were used by both models for predicting solubility in other pure and mixed solvents for which experimental data were available for comparison. A total of 386 pure solvent data points were used for the comparison comprising one or more temperatures per solvent. SciPharma is found to be more accurate than NRTL-SAC on the pure solvent data used especially in the description of the temperature dependence. This is due to the appropriate parameterization of the pharmaceuticals and the temperature-dependent description of the activity coeﬃcient in PC-SAFT. The solubility in mixed solvents is predicted satisfactorily with SciPharma. NRTL-SAC tends to overestimate the solubility in aqueous solutions of alcohols or shows invariable solubility with composition in other cases.},
	language = {en},
	number = {5},
	urldate = {2022-08-01},
	journal = {The European Physical Journal Special Topics},
	author = {Bouillot, Baptiste and Spyriouni, Theodora and Teychené, Sébastien and Biscans, Béatrice},
	month = apr,
	year = {2017},
	pages = {913--929},
}

@article{shao_role_2020,
	title = {Role of {Viscosity} in {Deviations} from the {Nernst}–{Einstein} {Relation}},
	volume = {124},
	issn = {1520-6106, 1520-5207},
	url = {https://pubs.acs.org/doi/10.1021/acs.jpcb.0c02544},
	doi = {10.1021/acs.jpcb.0c02544},
	abstract = {Deviations from the Nernst−Einstein relation are commonly attributed to ion−ion correlation and ion pairing. Despite the fact that these deviations can be quantiﬁed by either experimental measurements or molecular dynamics simulations, there is no rule of thumb to tell the extent of deviations. Here, we show that deviations from the Nernst−Einstein relation are proportional to the inverse viscosity by exploring the ﬁnite-size eﬀect on transport properties under periodic boundary conditions. This conclusion is in accord with the established experimental results of ionic liquids.},
	language = {en},
	number = {23},
	urldate = {2022-08-01},
	journal = {The Journal of Physical Chemistry B},
	author = {Shao, Yunqi and Shigenobu, Keisuke and Watanabe, Masayoshi and Zhang, Chao},
	month = jun,
	year = {2020},
	pages = {4774--4780},
}

@article{crede_class_2010,
	title = {Class {Attendance} in {College}: {A} {Meta}-{Analytic} {Review} of the {Relationship} of {Class} {Attendance} {With} {Grades} and {Student} {Characteristics}},
	volume = {80},
	issn = {0034-6543, 1935-1046},
	shorttitle = {Class {Attendance} in {College}},
	url = {http://journals.sagepub.com/doi/10.3102/0034654310362998},
	doi = {10.3102/0034654310362998},
	abstract = {A meta-analysis of the relationship between class attendance in college and college grades reveals that attendance has strong relationships with both class grades ( k = 69, N = 21,195, ρ = .44) and GPA ( k = 33, N = 9,243, ρ = .41). These relationships make class attendance a better predictor of college grades than any other known predictor of academic performance, including scores on standardized admissions tests such as the SAT, high school GPA, study habits, and study skills. Results also show that class attendance explains large amounts of unique variance in college grades because of its relative independence from SAT scores and high school GPA and weak relationship with student characteristics such as conscientiousness and motivation. Mandatory attendance policies appear to have a small positive impact on average grades ( k = 3, N = 1,421, d = .21). Implications for theoretical frameworks of student academic performance and educational policy are discussed.},
	language = {en},
	number = {2},
	urldate = {2022-08-01},
	journal = {Review of Educational Research},
	author = {Credé, Marcus and Roch, Sylvia G. and Kieszczynka, Urszula M.},
	month = jun,
	year = {2010},
	pages = {272--295},
}

@article{biasutti_using_2012,
	title = {Using {Wiki} in teacher education: {Impact} on knowledge management processes and student satisfaction},
	volume = {59},
	issn = {03601315},
	shorttitle = {Using {Wiki} in teacher education},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0360131512000930},
	doi = {10.1016/j.compedu.2012.04.009},
	abstract = {The current study reports on the use of Wiki as an online didactic tool to develop knowledge management (KM) processes in higher education. This study integrates social constructivist principles to learning where learners are pro-active and collaborative through higher order cognitive processes. The study was administered in two countries, namely Egypt and Italy, to close a gap in the literature with an aim to introduce KM processes in teacher educational programmes. These processes are seen as necessary for teachers’ professional skills. Such processes are claimed to enable teachers and therefore schools to evolve in a networked information-driven global society, especially as the complexity of subject knowledge is increasing. It is also a learning experience where teachers learn how to provide their students with educational settings where technology is enabled.},
	language = {en},
	number = {3},
	urldate = {2022-07-25},
	journal = {Computers \& Education},
	author = {Biasutti, Michele and EL-Deghaidy, Heba},
	month = nov,
	year = {2012},
	pages = {861--872},
}

@inproceedings{johnson_benefits_2020,
	address = {Virtual Event USA},
	title = {Benefits and {Pitfalls} of {Jupyter} {Notebooks} in the {Classroom}},
	isbn = {978-1-4503-7045-5},
	url = {https://dl.acm.org/doi/10.1145/3368308.3415397},
	doi = {10.1145/3368308.3415397},
	abstract = {Jupyter notebooks are widely used in industry and in academic research, but have only begun to make inroads into the classroom. The design of the Jupyter notebook is in many ways well suited for teaching subjects in information technology and computer science, but it is a tool that departs significantly from a standard text editor or integrated development environment, and thus carries with it several unique advantages as well as several surprising potential pitfalls. As use of Jupyter notebooks has grown, so has criticism of the notebook, for varied reasons: notebooks can behave in unexpected ways, they can be difficult to reproduce, they open up potential security issues, and they may encourage poor coding practices. A set of best practices to guide instructors and help addressing these concerns when using Jupyter notebooks in the classroom is currently lacking. This paper addresses the strengths and weaknesses of the Jupyter notebook for education, drawing on existing literature as well as the author’s experience teaching a range of courses with Jupyter notebooks for over five years, and recommends a set of best practices for teaching with the Jupyter notebook.},
	language = {en},
	urldate = {2022-07-25},
	booktitle = {Proceedings of the 21st {Annual} {Conference} on {Information} {Technology} {Education}},
	publisher = {ACM},
	author = {Johnson, Jeremiah W.},
	month = oct,
	year = {2020},
	pages = {32--37},
}

@article{kalogeropoulos_facilitating_2020,
	title = {Facilitating {Independent} {Learning}: {Student} {Perspectives} on the {Value} of {Student}-{Led} {Maker} {Spaces} in {Engineering} {Education}},
	volume = {36},
	copyright = {All rights reserved},
	language = {en},
	number = {4},
	journal = {IJEE},
	author = {Kalogeropoulos, Nikolaos and Walker, Pierre and Hale, Colin and Hellgardt, Klaus and Macey, Andrew and Shah, Umang V and Maraj, Marsha P},
	year = {2020},
	pages = {14},
}

@article{yue_comparison_2022,
	title = {Comparison between {Ab} {Initio} {Molecular} {Dynamics} and {OPLS}-{Based} {Force} {Fields} for {Ionic} {Liquid} {Solvent} {Organization}},
	volume = {126},
	issn = {1520-6106, 1520-5207},
	url = {https://pubs.acs.org/doi/10.1021/acs.jpcb.2c01636},
	doi = {10.1021/acs.jpcb.2c01636},
	abstract = {OPLS-based force ﬁelds (FFs) have been shown to provide accurate bulk-phase properties for a wide variety of imidazolium-based ionic liquids (ILs). However, the ability of OPLS to reproduce an IL solvent structure is not as well-validated given the relative lack of high-level theoretical or experimental data available for comparison. In this study, ab initio molecular dynamics (AIMD) simulations were performed for three widely used ILs: the 1-butyl-3methylimidazolium cation with chloride, tetraﬂuoroborate, or hexaﬂuorophosphate anions, that is, [BMIM][Cl], [BMIM][BF4], and [BMIM][PF6], respectively, as a basis for further assessment of two unique IL FFs: the ±0.8 charge-scaled OPLS-2009IL FF and the OPLS-VSIL FF. The OPLS-2009IL FF employs a traditional allatom functional form, whereas the OPLS-VSIL FF was developed using a virtual site that oﬄoads negative charge to inside the plane of the ring with careful attention given to reproducing hydrogen bonding. Detailed comparisons between AIMD and the OPLS FFs were made based on radial distribution functions (RDFs), combined distribution functions (CDFs), and spatial distribution functions (SDFs) to examine cation−anion interactions and π+−π+ stacking between the imidazolium rings. While both FFs were able to correctly capture the general solvent structure of these popular ILs, the OPLS-VSIL FF quantitatively reproduced interaction distances more accurately. In addition, this work provides further insights into the diﬀerent short- and long-range structure patterns of these popular ILs.},
	language = {en},
	number = {21},
	urldate = {2022-06-03},
	journal = {The Journal of Physical Chemistry B},
	author = {Yue, Kun and Doherty, Brian and Acevedo, Orlando},
	month = jun,
	year = {2022},
	pages = {3908--3919},
}

@article{thompson_scalable_2019,
	title = {Scalable {Screening} of {Soft} {Matter}: {A} {Case} {Study} of {Mixtures} of {Ionic} {Liquids} and {Organic} {Solvents}},
	volume = {123},
	issn = {1520-6106, 1520-5207},
	shorttitle = {Scalable {Screening} of {Soft} {Matter}},
	url = {https://pubs.acs.org/doi/10.1021/acs.jpcb.8b11527},
	doi = {10.1021/acs.jpcb.8b11527},
	abstract = {Room-temperature ionic liquids (RTILs) are a class of organic salts that are liquid at room temperature. Their physiochemical properties, including low vapor pressure and wide electrochemical stability window, have driven their use as electrolytes in many electrochemical applications; however, the slow transport properties of many RTILs have limited their utility in some applications. This issue is often mitigated by solvating ionic liquids in neutral organic solvents. To date, however, solvent interactions have only been explored for a small number of solvents, particularly acetonitrile and propylene carbonate, at only a few compositions. In this work, we use molecular dynamics simulations in the context of a computational screening approach to study mixtures of ionic liquids in many diﬀerent solvents at a range of concentrations. Building on prior work, we again ﬁnd that ionic liquid diﬀusivity increases monotonically with greater solvent concentration. In contrast to prior work, we ﬁnd that pure solvent diﬀusivity, not polarity, is the most inﬂuential solvent property on mixture behavior. We also explore the concentration dependence of ionic conductivity and ﬁnd maxima at intermediate concentrations. Experimental conductivity measurements, inspired by the computational screening study, support this observation with qualitatively consistent results. These results can further guide the selection of solvents for electrochemical applications of RTILs.},
	language = {en},
	number = {6},
	urldate = {2022-06-03},
	journal = {The Journal of Physical Chemistry B},
	author = {Thompson, Matthew W. and Matsumoto, Ray and Sacci, Robert L. and Sanders, Nicolette C. and Cummings, Peter T.},
	month = feb,
	year = {2019},
	pages = {1340--1347},
}

@article{sese_feynman-hibbs_1995,
	title = {Feynman-{Hibbs} potentials and path integrals for quantum {Lennard}-{Jones} systems: {Theory} and {Monte} {Carlo} simulations},
	volume = {85},
	issn = {13623028},
	doi = {10.1080/00268979500101571},
	abstract = {This paper addresses unexplored aspects of the Feynman-Hibbs Gaussian picture and the ħ2- and ħ4-effective potentials obtainable from that model. Thermodynamic and structural properties are compared with their path-integral counterparts. In particular, a closed formula for the self-correlation (intranecklace) radial distribution function is derived from the Feynman-Hibbs model in view of, first, its importance in determining quantum structure factors and, second, the great difficulty in computing it accurately via path-integral calculations. In order to assess the reliability of the ħ2- and ħ4-potentials, neon liquid and helium-4 gas are studied for new state points with the corresponding semiclassical and ‘exact' path-integral Monte Carlo simulations. As regards thermodynamics, energies, pressures and also specific heats at constant volume are reported. Structural results cover necklace radii of gyration, and instantaneous, linear response and self-correlation radial distribution functions. Comparison with experiment is made wherever possible, and the results indicate better performances for the ħ2-potential. © 1995 Taylor \& Francis Ltd.},
	number = {5},
	journal = {Mol. Phys.},
	author = {Sesé, Luis M.},
	month = aug,
	year = {1995},
	pages = {931--947},
}

@article{sese_study_1994,
	title = {Study of the {Feynman}-{Hibbs} effective potential against the path-integral formalism for {Monte} {Carlo} simulations of quantum many-body {Lennard}-{Jones} systems},
	volume = {81},
	issn = {0026-8976},
	url = {http://www.tandfonline.com/doi/abs/10.1080/00268979400100891},
	doi = {10.1080/00268979400100891},
	abstract = {Approximate quantum pair radial correlation functions and thermodynamic quantities for Lennard-Jones systems can be computed with Monte Carlo simulation involving Feynman-Hibbs potentials. A convolution approach to produce the quantum pair radial function from the direct Monte Carlo structural results is presented by analysing its connection with the path-integral instantaneous and linear response pair radial functions. Several Lennard-Jones systems with substantial quantum behaviour:Methane, argon, neon, deuterium and helium-4 (eighteen state points) are studied. For the sake of comparison, new path-integral simulations of helium-4 and improved path-integral results for methane are also reported. The effective potential results are in close agreement with experimental and exact path-integral data over a wide range of de Broglie wavelengths, densities and temperatures. © 1994 Taylor and Francis Group, LLC.},
	number = {6},
	journal = {Mol. Phys.},
	author = {Sesé, Luis M.},
	month = apr,
	year = {1994},
	pages = {1297--1312},
}

@article{mceldrew_salt--ionic-liquid_2021,
	title = {Salt-in-{Ionic}-{Liquid} {Electrolytes}: {Ion} {Network} {Formation} and {Negative} {Effective} {Charges} of {Alkali} {Metal} {Cations}},
	volume = {125},
	issn = {1520-6106, 1520-5207},
	shorttitle = {Salt-in-{Ionic}-{Liquid} {Electrolytes}},
	url = {https://pubs.acs.org/doi/10.1021/acs.jpcb.1c05546},
	doi = {10.1021/acs.jpcb.1c05546},
	abstract = {Salt-in-ionic liquid electrolytes have attracted signiﬁcant attention as potential electrolytes for next generation batteries largely due to their safety enhancements over typical organic electrolytes. However, recent experimental and computational studies have shown that under certain conditions alkali cations can migrate in electric ﬁelds as if they carried a net negative eﬀective charge. In particular, alkali cations were observed to have negative transference numbers at small mole fractions of alkalimetal salt that revert to the expected net positive transference numbers at large mole fractions. Simulations have provided some insights into these observations, where the formation of asymmetric ionic clusters, as well as a percolating ion network, could largely explain the anomalous transport of alkali cations. However, a thermodynamic theory that captures such phenomena has not been developed, as ionic associations were typically treated via the formation of ion pairs. The theory presented herein, based on the classical polymer theories, describes thermoreversible associations between alkali cations and anions, where the formation of large, asymmetric ionic clusters and a percolating ionic network are a natural result of the theory. Furthermore, we present several general methods to calculate the eﬀective charge of alkali cations in ionic liquids. We note that the negative eﬀective charge is a robust prediction with respect to the parameters of the theory and that the formation of a percolating ionic network leads to the restoration of net positive charges of the cations at large mole fractions of alkali metal salt. Overall, we ﬁnd excellent qualitative agreement between our theory and molecular simulations in terms of ionic cluster statistics and the eﬀective charges of the alkali cations.},
	language = {en},
	number = {50},
	urldate = {2022-01-22},
	journal = {The Journal of Physical Chemistry B},
	author = {McEldrew, Michael and Goodwin, Zachary A. H. and Molinari, Nicola and Kozinsky, Boris and Kornyshev, Alexei A. and Bazant, Martin Z.},
	month = dec,
	year = {2021},
	pages = {13752--13766},
}

@article{jorgensen_development_1996,
	title = {Development and {Testing} of the {OPLS} {All}-{Atom} {Force} {Field} on {Conformational} {Energetics} and {Properties} of {Organic} {Liquids}},
	volume = {118},
	issn = {0002-7863, 1520-5126},
	url = {https://pubs.acs.org/doi/10.1021/ja9621760},
	doi = {10.1021/ja9621760},
	abstract = {The parametrization and testing of the OPLS all-atom force field for organic molecules and peptides are described. Parameters for both torsional and nonbonded energetics have been derived, while the bond stretching and angle bending parameters have been adopted mostly from the AMBER all-atom force field. The torsional parameters were determined by fitting to rotational energy profiles obtained from ab initio molecular orbital calculations at the RHF/6-31G*//RHF/6-31G* level for more than 50 organic molecules and ions. The quality of the fits was high with average errors for conformational energies of less than 0.2 kcal/mol. The force-field results for molecular structures are also demonstrated to closely match the ab initio predictions. The nonbonded parameters were developed in conjunction with Monte Carlo statistical mechanics simulations by computing thermodynamic and structural properties for 34 pure organic liquids including alkanes, alkenes, alcohols, ethers, acetals, thiols, sulfides, disulfides, aldehydes, ketones, and amides. Average errors in comparison with experimental data are 2\% for heats of vaporization and densities. The Monte Carlo simulations included sampling all internal and intermolecular degrees of freedom. It is found that such non-polar and monofunctional systems do not show significant condensed-phase effects on internal energies in going from the gas phase to the pure liquids.},
	language = {en},
	number = {45},
	urldate = {2022-06-03},
	journal = {Journal of the American Chemical Society},
	author = {Jorgensen, William L. and Maxwell, David S. and Tirado-Rives, Julian},
	month = nov,
	year = {1996},
	pages = {11225--11236},
}

@article{hellmann_state---art_2017,
	title = {State-of-the-art ab initio potential energy curve for the xenon atom pair and related spectroscopic and thermophysical properties},
	volume = {147},
	issn = {00219606},
	doi = {10.1063/1.4994267},
	abstract = {A new ab initio interatomic potential energy curve for two ground-state xenon atoms is presented. It is based on supermolecular calculations at the coupled-cluster level with single, double, and perturbative triple excitations [CCSD(T)] employing basis sets up to sextuple-zeta quality, which were developed as part of this work. In addition, corrections were determined for higher coupled-cluster levels up to CCSDTQ as well as for scalar and spin-orbit relativistic effects at the CCSD(T) level. A physically motivated analytical function was fitted to the calculated interaction energies and used to compute the vibrational spectrum of the dimer, the second virial coefficient, and the dilute gas transport properties. The agreement with the best available experimental data for the investigated properties is excellent; the new potential function is superior not only to previous ab initio potentials but also to the most popular empirical ones.},
	number = {3},
	journal = {J. Chem. Phys.},
	author = {Hellmann, Robert and Jäger, Benjamin and Bich, Eckard},
	month = jul,
	year = {2017},
	pmid = {28734299},
	note = {Publisher: American Institute of Physics Inc.},
	pages = {034304},
}

@article{galindo_saft-vre_1999,
	title = {{SAFT}-{VRE}: {Phase} {Behavior} of {Electrolyte} {Solutions} with the {Statistical} {Associating} {Fluid} {Theory} for {Potentials} of {Variable} {Range}},
	volume = {103},
	issn = {1520-6106, 1520-5207},
	shorttitle = {{SAFT}-{VRE}},
	url = {https://pubs.acs.org/doi/10.1021/jp991959f},
	doi = {10.1021/jp991959f},
	language = {en},
	number = {46},
	urldate = {2022-06-04},
	journal = {The Journal of Physical Chemistry B},
	author = {Galindo, Amparo and Gil-Villegas, Alejandro and Jackson, George and Burgess, Andrew N.},
	month = nov,
	year = {1999},
	pages = {10272--10281},
}

@article{dong_hydrogen_2006,
	title = {Hydrogen {Bonds} in {Imidazolium} {Ionic} {Liquids}},
	volume = {110},
	issn = {1089-5639, 1520-5215},
	url = {https://pubs.acs.org/doi/10.1021/jp054054c},
	doi = {10.1021/jp054054c},
	language = {en},
	number = {31},
	urldate = {2022-06-04},
	journal = {The Journal of Physical Chemistry A},
	author = {Dong, Kun and Zhang, Suojiang and Wang, Daxi and Yao, Xiaoqian},
	month = aug,
	year = {2006},
	pages = {9775--9782},
}

@article{chang_structure_2021,
	title = {Structure, {Molecular} {Interactions}, and {Dynamics} of {Aqueous} [{BMIM}][{BF} $_{\textrm{4}}$ ] {Mixtures}: {A} {Molecular} {Dynamics} {Study}},
	volume = {125},
	issn = {1520-6106, 1520-5207},
	shorttitle = {Structure, {Molecular} {Interactions}, and {Dynamics} of {Aqueous} [{BMIM}][{BF} $_{\textrm{4}}$ ] {Mixtures}},
	url = {https://pubs.acs.org/doi/10.1021/acs.jpcb.0c09731},
	doi = {10.1021/acs.jpcb.0c09731},
	language = {en},
	number = {4},
	urldate = {2022-06-04},
	journal = {The Journal of Physical Chemistry B},
	author = {Chang, Tsun-Mei and Billeck, Stephanie E.},
	month = feb,
	year = {2021},
	pages = {1227--1240},
}

@article{bich_ab_2008,
	title = {Ab initio potential energy curve for the neon atom pair and thermophysical properties for the dilute neon gas. {II}. {Thermophysical} properties for low-density neon},
	volume = {106},
	issn = {00268976},
	doi = {10.1080/00268970801964207},
	abstract = {A neon-neon interatomic potential energy curve determined from quantum-mechanical ab initio calculations and described with an analytical representation (R. Hellmann, E. Bich, and E. Vogel, Molec. Phys. 106, 133 (2008)) was used in the framework of the quantum-statistical mechanics and of the corresponding kinetic theory to calculate the most important thermophysical properties of neon governed by two-body and three-body interactions. The second and third pressure virial coefficients as well as the viscosity and thermal conductivity coefficients, the last two in the so-called limit of zero density, were calculated for natural Ne from 25 to 10,000 K. Comparison of the calculated viscosity and thermal conductivity with the most accurate experimental data at ambient temperature shows that these values are accurate enough to be applied as standard values for the complete temperature range of the calculations characterized by an uncertainty of about 0.1\% except at the lowest temperatures.},
	number = {6},
	journal = {Mol. Phys.},
	author = {Bich, Eckard and Hellmann, Robert and Vogel, Eckhard},
	month = mar,
	year = {2008},
	keywords = {Neon gas property standards, Neon pair potential, Second and third pressure virial coefficients, Thermal conductivity, Viscosity},
	pages = {813--825},
}

@article{bester-rogac_molar_2010,
	title = {Molar {Conductivities} and {Association} {Constants} of 1-{Butyl}-3-methylimidazolium {Chloride} and 1-{Butyl}-3-methylimidazolium {Tetrafluoroborate} in {Methanol} and {DMSO}},
	volume = {55},
	issn = {0021-9568, 1520-5134},
	url = {https://pubs.acs.org/doi/10.1021/je900531b},
	doi = {10.1021/je900531b},
	language = {en},
	number = {5},
	urldate = {2022-05-27},
	journal = {Journal of Chemical \& Engineering Data},
	author = {Bešter-Rogač, Marija and Hunger, Johannes and Stoppa, Alexander and Buchner, Richard},
	month = may,
	year = {2010},
	pages = {1799--1803},
}

@article{wu_density_2015,
	title = {Density and {Viscosity} of {Ionic} {Liquid} {Binary} {Mixtures} of 1-n-{Butyl}-3-methylimidazolium {Tetrafluoroborate} with {Acetonitrile}, {N},{N}-{Dimethylacetamide}, {Methanol}, and {N}-{Methyl}-2-pyrrolidone},
	volume = {44},
	issn = {0095-9782, 1572-8927},
	url = {http://link.springer.com/10.1007/s10953-014-0273-1},
	doi = {10.1007/s10953-014-0273-1},
	abstract = {In this study, thermodynamic properties of the binary mixtures of ionic liquid with an organic compound, as potential solvent systems in pharmaceutical industry applications, are studied. The densities and viscosities of the binary mixtures of 1-butyl-3methylimidazolium tetraﬂuoroborate ([C4mim][BF4]) with acetonitrile, N,N-dimethylacetamide, methanol, and N-methyl-2-pyrrolidone were measured at atmospheric pressure over the [C4mim][BF4] mole fraction range from 0.1 to 0.9 and at temperatures from 303.15 to 333.15 K at intervals of 10 K. The densities were measured using a vibratingtube digital density meter and the viscosities were measured using a capillary viscometer. The excess molar volumes (VE) and viscosity deviations (Dg) were calculated from densities and viscosities of mixture, respectively, and ﬁtted to the Redlich–Kister polynomial. The optimally ﬁtted parameters are also determined and the correlation results are in satisfactory agreement with the experimental data. In addition, the excess molar volumes of binary mixtures of ionic liquid with different organic compounds are compared and discussed using the Hansen solubility parameter.},
	language = {en},
	number = {3-4},
	urldate = {2022-06-22},
	journal = {Journal of Solution Chemistry},
	author = {Wu, Jheng-Yu and Chen, Yan-Ping and Su, Chie-Shaan},
	month = apr,
	year = {2015},
	pages = {395--412},
}

@article{feng_free_2019,
	title = {Free and {Bound} {States} of {Ions} in {Ionic} {Liquids}, {Conductivity}, and {Underscreening} {Paradox}},
	volume = {9},
	issn = {2160-3308},
	url = {https://link.aps.org/doi/10.1103/PhysRevX.9.021024},
	doi = {10.1103/PhysRevX.9.021024},
	language = {en},
	number = {2},
	urldate = {2022-06-22},
	journal = {Physical Review X},
	author = {Feng, Guang and Chen, Ming and Bi, Sheng and Goodwin, Zachary A. H. and Postnikov, Eugene B. and Brilliantov, Nikolai and Urbakh, Michael and Kornyshev, Alexei A.},
	month = may,
	year = {2019},
	pages = {021024},
}

@article{mceldrew_ion_2021,
	title = {Ion {Clusters} and {Networks} in {Water}-in-{Salt} {Electrolytes}},
	volume = {168},
	issn = {0013-4651, 1945-7111},
	url = {https://iopscience.iop.org/article/10.1149/1945-7111/abf975},
	doi = {10.1149/1945-7111/abf975},
	abstract = {Water-in-salt electrolytes (WiSEs) are a class of super-concentrated electrolytes that have shown much promise in replacing organic electrolytes in lithium-ion batteries. At the extremely high salt concentrations of WiSEs, ionic association is more complicated than the simple ion pair description. In fact, large branched clusters can be present in WiSEs, and past a critical salt concentration, an infinite percolating ionic network can form spontaneously. In this work, we simplify our recently developed thermodynamic model of reversible ionic aggregation and gelation, tailoring it specifically for WiSEs. Our simplified theory only has a handful of parameters, all of which can be readily determined from simulations. Our model is able to quantitatively reproduce the populations of ionic clusters of different sizes as a function of salt concentration, the critical salt concentration for ionic gelation, and the fraction of ions incorporated into the ionic gel, as observed from molecular simulations of three different lithium-based WiSEs. The extent of ionic association and gelation greatly affects the effective ionic strength of solution, the coordination environment of active cations that is known to govern the chemistry of the solid-electrolyte interface, and the thermodynamic activity of all species in the electrolyte.},
	language = {en},
	number = {5},
	urldate = {2022-06-22},
	journal = {Journal of The Electrochemical Society},
	author = {McEldrew, Michael and Goodwin, Zachary A. H. and Bi, Sheng and Kornyshev, Alexei A. and Bazant, Martin Z.},
	month = may,
	year = {2021},
	pages = {050514},
}

@article{rilo_electrical_2010,
	title = {Electrical {Conductivity} and {Viscosity} of {Aqueous} {Binary} {Mixtures} of 1-{Alkyl}-3-methyl {Imidazolium} {Tetrafluoroborate} at {Four} {Temperatures}},
	volume = {55},
	issn = {0021-9568, 1520-5134},
	url = {https://pubs.acs.org/doi/10.1021/je900600c},
	doi = {10.1021/je900600c},
	language = {en},
	number = {2},
	urldate = {2022-06-22},
	journal = {Journal of Chemical \& Engineering Data},
	author = {Rilo, Esther and Vila, Juan and Pico, José and García-Garabal, Sandra and Segade, Luisa and Varela, Luis M. and Cabeza, Oscar},
	month = feb,
	year = {2010},
	pages = {639--644},
}

@article{kalugin_conductometric_2013,
	title = {Conductometric study of binary systems based on ionic liquids and acetonitrile in a wide concentration range},
	volume = {105},
	issn = {00134686},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0013468613008475},
	doi = {10.1016/j.electacta.2013.04.140},
	language = {en},
	urldate = {2022-06-22},
	journal = {Electrochimica Acta},
	author = {Kalugin, Oleg N. and Voroshylova, Iuliia V. and Riabchunova, Anastasiia V. and Lukinova, Elena V. and Chaban, Vitaly V.},
	month = aug,
	year = {2013},
	pages = {188--199},
}

@article{dufal_development_nodate,
	title = {Development and application of advanced thermodynamic molecular description for complex reservoir ﬂuids containing carbon dioxide and brines},
	language = {en},
	author = {Dufal, Simon},
	pages = {263},
}

@article{zheng_hydrogen-bonding_2013,
	title = {Hydrogen-bonding interactions between [{BMIM}][{BF4}] and acetonitrile},
	volume = {15},
	issn = {1463-9076, 1463-9084},
	url = {http://xlink.rsc.org/?DOI=c3cp53356e},
	doi = {10.1039/c3cp53356e},
	language = {en},
	number = {41},
	urldate = {2022-06-22},
	journal = {Physical Chemistry Chemical Physics},
	author = {Zheng, Yan-Zhen and Wang, Nan-Nan and Luo, Jun-Jie and Zhou, Yu and Yu, Zhi-Wu},
	year = {2013},
	pages = {18055},
}

@article{mceldrew_correlated_2021,
	title = {Correlated {Ion} {Transport} and the {Gel} {Phase} in {Room} {Temperature} {Ionic} {Liquids}},
	volume = {125},
	issn = {1520-6106, 1520-5207},
	url = {https://pubs.acs.org/doi/10.1021/acs.jpcb.0c09050},
	doi = {10.1021/acs.jpcb.0c09050},
	abstract = {Here we present a theory of ion aggregation and gelation of room temperature ionic liquids (RTILs). Based on it, we investigate the eﬀect of ion aggregation on correlated ion transportionic conductivity and transference numbersobtaining closed-form expressions for these quantities. The theory depends on the maximum number of associations a cation and anion can form and the strength of their association. To validate the presented theory, we perform molecular dynamics simulations on several RTILs and a range of temperatures for one RTIL. The simulations indicate the formation of large clusters, even percolating through the system under certain circumstances, thus forming a gel, with the theory accurately describing the obtained cluster distributions in all cases. However, based on the strength and lifetime of associations in the simulated RTILs, we expect free ions to dominate ionic conductivity despite the presence of clusters, and we do not expect the percolating cluster to trigger structural arrest in the RTIL.},
	language = {en},
	number = {10},
	urldate = {2022-06-22},
	journal = {The Journal of Physical Chemistry B},
	author = {McEldrew, Michael and Goodwin, Zachary A. H. and Zhao, Hongbo and Bazant, Martin Z. and Kornyshev, Alexei A.},
	month = mar,
	year = {2021},
	pages = {2677--2689},
}

@article{fan_density_2016,
	title = {Density and {Viscosity} {Measurements} for {Binary} {Mixtures} of 1-{Ethyl}-3-methylimidazolium {Tetrafluoroborate} ([{Emim}][{BF} $_{\textrm{4}}$ ]) with {Dimethylacetamide}, {Dimethylformamide}, and {Dimethyl} {Sulfoxide}},
	volume = {61},
	issn = {0021-9568, 1520-5134},
	url = {https://pubs.acs.org/doi/10.1021/acs.jced.5b00753},
	doi = {10.1021/acs.jced.5b00753},
	abstract = {The density and viscosity data of three binary liquid mixtures containing the ionic liquid (IL) 1-ethyl-3methylimidazolium tetraﬂuoroborate and organic solvents, dimethylacetamide (DMAC), dimethylformamide (DMF), and dimethyl sulfoxide (DMSO) were obtained under atmospheric pressure, at temperatures of 303.15 to 333.15 K over the entire composition range. A vibrating-tube digital density meter and a capillary viscometer were used for density and viscosity measurements, respectively. Excess molar volumes (VE) and viscosity deviations (Δη) for the binary mixture system were calculated from the experimental data and were satisfactorily ﬁtted with the Redlich−Kister equation. Adding DMAC, DMF, and DMSO led to negative values of VE and Δη. This ﬁnding revealed that the packing of the constituents was more eﬃcient, and the anion−cation interaction of IL was decreased in the binary liquid mixtures. The sequences of VE and Δη for the three binary liquid mixtures in this study are also discussed using intermolecular interactions.},
	language = {en},
	number = {2},
	urldate = {2022-06-22},
	journal = {Journal of Chemical \& Engineering Data},
	author = {Fan, Xian-Heng and Chen, Yan-Ping and Su, Chie-Shaan},
	month = feb,
	year = {2016},
	pages = {920--927},
}

@article{neumann_dipole_1983,
	title = {Dipole moment fluctuation formulas in computer simulations of polar systems},
	volume = {50},
	issn = {0026-8976, 1362-3028},
	url = {http://www.tandfonline.com/doi/abs/10.1080/00268978300102721},
	doi = {10.1080/00268978300102721},
	language = {en},
	number = {4},
	urldate = {2022-06-22},
	journal = {Molecular Physics},
	author = {Neumann, Martin},
	month = nov,
	year = {1983},
	pages = {841--858},
}

@article{simonin_full_2021,
	title = {Full solution to the mean spherical approximation ({MSA}) for an arbitrary mixture of ions in a dipolar solvent},
	volume = {155},
	issn = {0021-9606, 1089-7690},
	url = {https://aip.scitation.org/doi/10.1063/5.0064188},
	doi = {10.1063/5.0064188},
	abstract = {The complete solution to the mean-spherical approximation is given for an arbitrary mixture of ions in a dipolar solvent. The calculation is done for an overall neutral collection of charged hard spheres (ions) and dipoles (solvent) that bear a central point dipole. Previous solutions to this problem were not consistent because they did not include the solvent particles as a (neutral) solute in the mixture. The present solution accounts for this peculiar counterintuitive feature, fully and consistently. Complete expressions for the chemical potentials of the ions and solvent are provided for the first time. To illustrate, a binary 1-1 asymmetric electrolyte solution in a water-like dipolar solvent is considered, and some numerical results are examined. In particular, it is verified that a set of thermodynamic consistency relations are accurately fulfilled.},
	language = {en},
	number = {11},
	urldate = {2022-06-22},
	journal = {The Journal of Chemical Physics},
	author = {Simonin, Jean-Pierre and Høye, Johan S.},
	month = sep,
	year = {2021},
	pages = {114502},
}

@article{simonin_solution_2020,
	title = {On the solution of the mean-spherical approximation ({MSA}) for ions in a dipolar solvent in the general case},
	volume = {10},
	issn = {2158-3226},
	url = {http://aip.scitation.org/doi/10.1063/5.0022864},
	doi = {10.1063/5.0022864},
	abstract = {This paper deals with the problem of a mixture of hard spherical ions and central point dipoles, described within the mean-spherical approximation. In this non-primitive model, the species have different diameters (unrestricted case). The first purpose of this work is to establish clear and valid equations for this problem and present a method to solve them. Formulas for the pressure, the internal and Helmholtz energies, and the chemical potentials of the species are given and discussed. The results are illustrated by considering a binary 1–1 electrolyte solution in a water-like dipolar solvent.},
	language = {en},
	number = {9},
	urldate = {2022-06-22},
	journal = {AIP Advances},
	author = {Simonin, Jean-Pierre},
	month = sep,
	year = {2020},
	pages = {095213},
}

@article{hess_determining_2002,
	title = {Determining the shear viscosity of model liquids from molecular dynamics simulations},
	volume = {116},
	issn = {00219606},
	url = {http://scitation.aip.org/content/aip/journal/jcp/116/1/10.1063/1.1421362},
	doi = {10.1063/1.1421362},
	language = {en},
	number = {1},
	urldate = {2022-06-22},
	journal = {The Journal of Chemical Physics},
	author = {Hess, Berk},
	year = {2002},
	pages = {209},
}

@article{krienke_association_1998,
	title = {Association concepts in electrolyte solutions},
	volume = {78},
	issn = {01677322},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0167732298000877},
	doi = {10.1016/S0167-7322(98)00087-7},
	abstract = {Association in electrolyte solutions is investigated as a part of the thermodynamic and transport excess functions in the framework of different theoretical approaches, and the influence of solvent-averaged short range interactions between ions on the association constant is discussed. The low concentration chemical model (lcCM) is compared with results of the MSA theory for equilibrium and nonequilibrium situations for models which include interactions with ion pairs. At the limit of strong electrostatic association a parameter-free theory is derived for ion pairs made up by ions of different diameters. The limitations of the models, and the inherent approximations of the theories are discussed. © 1998Elsevier Science B.V. All rights reserved.},
	language = {en},
	number = {1-2},
	urldate = {2022-06-22},
	journal = {Journal of Molecular Liquids},
	author = {Krienke, H. and Barthel, J.},
	month = aug,
	year = {1998},
	pages = {123--138},
}

@article{reddy_reciprocity_2020,
	title = {Reciprocity between ion-dipole and hydrogen bond interactions in the binary mixtures of {N},{N}-{Dimethylformamide} with ionic liquids},
	volume = {301},
	issn = {01677322},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0167732219346732},
	doi = {10.1016/j.molliq.2020.112487},
	abstract = {In this work, classical molecular dynamics (MD) simulations were carried out to investigate the structure and dynamics of binary mixtures of N, N-dimethylformamide (DMF) and ionic liquids (ILs), diethylammonium acetate (DEAA) and triethylammonium acetate (TEAA), with the change in mole fraction of ILs. The hydrogen bonding, dipole-dipole, and ion-dipole interactions were exclusively studied to explore the structural as well as dynamical evolution produced by the number of ionic entities in the mixtures. We have calculated the structural properties such as radial distribution functions (RDFs), spatial distribution functions (SDFs), and coordination numbers. These calculations were followed by studies involving dynamic properties like diffusion coefﬁcients, hydrogen bond relaxation, and residence times. RDFs indicate the long-range correlations between ions in pure ILs. Structural properties also reveal an increase in ion-dipole interactions between DMF and ILs at high mole fractions of IL. These binary mixtures show high ion mobility at lower concentrations of ILs. Overall, the acetate anions show slightly higher diffusion than ammonium cations in pure ILs, and these two ions exhibit enhanced dynamics in the mixtures rich in DMF.},
	language = {en},
	urldate = {2022-06-22},
	journal = {Journal of Molecular Liquids},
	author = {Reddy, Th. Dhileep N. and Mallik, Bhabani S.},
	month = mar,
	year = {2020},
	pages = {112487},
}

@article{tsanas_calculation_2022,
	title = {Calculation of phase and chemical equilibrium for multiple ion-containing phases including stability analysis},
	volume = {248},
	issn = {00092509},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0009250921007399},
	doi = {10.1016/j.ces.2021.117174},
	abstract = {A reactive ﬂash algorithm based on the work of Gautam, Seider, White (Gautam and Seider, 1979a, 1979b, 1979c; White and Seider, 1981) and Barreau et al. (2006) is presented. The original algorithm minimizes the total Gibbs energy of the system with respect to an elemental material balance constraint and the overall system electroneutrality. In our approach, we perform the minimization taking into account the charge/electric potential contribution to the Gibbs energy to allow application to multiple electrolyte phases. Moreover, the composition derivatives of fugacity coefﬁcients are not ignored in the derivation of the working equations. Finally, the need of the overall electroneutrality equation is discussed. The algorithm is applied to a demixing amine system (water/DEEA/MAPA) with carbon dioxide, modeled with eNRTL for both phases (Mouhoubi et al., 2020). In LLE conditions, both phases are electroneutral, chemical reaction equilibrium is satisﬁed and phase equilibrium of each molecule and ion individually has been established. Stability analysis based on the electrochemical potential allows the determination of an electroneutral ion-containing phase. Although calculations are compared with experimental data, the purpose of the work was not the parameterization of the model, and therefore its accuracy is not addressed. Since our implementation of eNRTL did not satisfy the Gibbs-Duhem equation, its composition derivatives were incompatible with the algorithm and certain terms had to be ignored. Even though the algorithm is generally expected to converge quadratically, convergence in this work resembles the one of a partial Newton method due to the omitted derivative terms.},
	language = {en},
	urldate = {2022-06-22},
	journal = {Chemical Engineering Science},
	author = {Tsanas, Christos and de Hemptinne, Jean-Charles and Mougin, Pascal},
	month = feb,
	year = {2022},
	pages = {117174},
}

@article{wertheim_fluids_1986,
	title = {Fluids with highly directional attractive forces. {III}. {Multiple} attraction sites},
	volume = {42},
	issn = {0022-4715, 1572-9613},
	url = {http://link.springer.com/10.1007/BF01127721},
	doi = {10.1007/BF01127721},
	language = {en},
	number = {3-4},
	urldate = {2022-06-04},
	journal = {Journal of Statistical Physics},
	author = {Wertheim, M. S.},
	month = feb,
	year = {1986},
	pages = {459--476},
}

@article{wertheim_fluids_1986-1,
	title = {Fluids with highly directional attractive forces. {IV}. {Equilibrium} polymerization},
	volume = {42},
	issn = {0022-4715, 1572-9613},
	url = {http://link.springer.com/10.1007/BF01127722},
	doi = {10.1007/BF01127722},
	language = {en},
	number = {3-4},
	urldate = {2022-06-04},
	journal = {Journal of Statistical Physics},
	author = {Wertheim, M. S.},
	month = feb,
	year = {1986},
	pages = {477--492},
}

@article{wertheim_fluids_1984,
	title = {Fluids with highly directional attractive forces. {I}. {Statistical} thermodynamics},
	volume = {35},
	issn = {0022-4715, 1572-9613},
	url = {http://link.springer.com/10.1007/BF01017362},
	doi = {10.1007/BF01017362},
	language = {en},
	number = {1-2},
	urldate = {2022-06-04},
	journal = {Journal of Statistical Physics},
	author = {Wertheim, M. S.},
	month = apr,
	year = {1984},
	pages = {19--34},
}

@article{wertheim_fluids_1984-1,
	title = {Fluids with highly directional attractive forces. {II}. {Thermodynamic} perturbation theory and integral equations},
	volume = {35},
	issn = {0022-4715, 1572-9613},
	url = {http://link.springer.com/10.1007/BF01017363},
	doi = {10.1007/BF01017363},
	language = {en},
	number = {1-2},
	urldate = {2022-06-04},
	journal = {Journal of Statistical Physics},
	author = {Wertheim, M. S.},
	month = apr,
	year = {1984},
	pages = {35--47},
}

@article{noauthor_gromacs_nodate,
	title = {{GROMACS} {Documentation}},
	pages = {670},
}

@article{brehm_travisfree_2020,
	title = {{TRAVIS}—{A} free analyzer for trajectories from molecular simulation},
	volume = {152},
	issn = {0021-9606, 1089-7690},
	url = {http://aip.scitation.org/doi/10.1063/5.0005078},
	doi = {10.1063/5.0005078},
	abstract = {TRAVIS (“Trajectory Analyzer and Visualizer”) is a program package for post-processing and analyzing trajectories from molecular dynamics and Monte Carlo simulations, mostly focused on molecular condensed phase systems. It is an open source free software licensed under the GNU GPL, is platform independent, and does not require any external libraries. Nine years after the original publication of TRAVIS, we highlight some of the recent new functions and features in this article. At the same time, we shortly present some of the underlying algorithms in TRAVIS, which contribute to make trajectory analysis more efficient. Some modern visualization techniques such as Sankey diagrams are also demonstrated. Many analysis functions are implemented, covering structural analyses, dynamical analyses, and functions for predicting vibrational spectra from molecular dynamics simulations. While some of the analyses are known since several decades, others are very recent. For example, TRAVIS has been used to compute the first ab initio predictions in the literature of bulk phase vibrational circular dichroism spectra, bulk phase Raman optical activity spectra, and bulk phase resonance Raman spectra within the last few years.},
	language = {en},
	number = {16},
	urldate = {2022-06-04},
	journal = {The Journal of Chemical Physics},
	author = {Brehm, M. and Thomas, M. and Gehrke, S. and Kirchner, B.},
	month = apr,
	year = {2020},
	pages = {164105},
}

@article{michaud-agrawal_mdanalysis_2011,
	title = {{MDAnalysis}: {A} toolkit for the analysis of molecular dynamics simulations},
	volume = {32},
	issn = {01928651},
	shorttitle = {{MDAnalysis}},
	url = {https://onlinelibrary.wiley.com/doi/10.1002/jcc.21787},
	doi = {10.1002/jcc.21787},
	abstract = {MDAnalysis is an object-oriented library for structural and temporal analysis of molecular dynamics (MD) simulation trajectories and individual protein structures. It is written in the Python language with some performance-critical code in C. It uses the powerful NumPy package to expose trajectory data as fast and efﬁcient NumPy arrays. It has been tested on systems of millions of particles. Many common ﬁle formats of simulation packages including CHARMM, Gromacs, Amber, and NAMD and the Protein Data Bank format can be read and written. Atoms can be selected with a syntax similar to CHARMM’s powerful selection commands. MDAnalysis enables both novice and experienced programmers to rapidly write their own analytical tools and access data stored in trajectories in an easily accessible manner that facilitates interactive explorative analysis. MDAnalysis has been tested on and works for most Unix-based platforms such as Linux and Mac OS X. It is freely available under the GNU General Public License from http://mdanalysis.googlecode.com.},
	language = {en},
	number = {10},
	urldate = {2022-06-03},
	journal = {Journal of Computational Chemistry},
	author = {Michaud-Agrawal, Naveen and Denning, Elizabeth J. and Woolf, Thomas B. and Beckstein, Oliver},
	month = jul,
	year = {2011},
	pages = {2319--2327},
}

@article{rog_n_2003,
	title = {\textit{n} {Moldyn}: {A} program package for a neutron scattering oriented analysis of molecular dynamics simulations: \textit{n} {Moldyn}},
	volume = {24},
	issn = {01928651},
	shorttitle = {\textit{n} {Moldyn}},
	url = {https://onlinelibrary.wiley.com/doi/10.1002/jcc.10243},
	doi = {10.1002/jcc.10243},
	abstract = {We present a new implementation of the program nMoldyn, which has been developed for the computation and decomposition of neutron scattering intensities from Molecular Dynamics trajectories (Comp. Phys. Commun 1995, 91, 191–214). The new implementation extends the functionality of the original version, provides a much more convenient user interface (both graphical/interactive and batch), and can be used as a tool set for implementing new analysis modules. This was made possible by the use of a high-level language, Python, and of modern object-oriented programming techniques. The quantities that can be calculated by nMoldyn are the mean-square displacement, the velocity autocorrelation function as well as its Fourier transform (the density of states) and its memory function, the angular velocity autocorrelation function and its Fourier transform, the reorientational correlation function, and several functions speciﬁc to neutron scattering: the coherent and incoherent intermediate scattering functions with their Fourier transforms, the memory function of the coherent scattering function, and the elastic incoherent structure factor. The possibility to compute memory function is a new and powerful feature that allows to relate simulation results to theoretical studies.},
	language = {en},
	number = {5},
	urldate = {2022-06-03},
	journal = {Journal of Computational Chemistry},
	author = {Róg, T. and Murzyn, K. and Hinsen, K. and Kneller, G. R.},
	month = apr,
	year = {2003},
	pages = {657--667},
}

@article{martinez_packmol_2009,
	title = {{PACKMOL}: {A} package for building initial configurations for molecular dynamics simulations},
	volume = {30},
	issn = {01928651, 1096987X},
	shorttitle = {{PACKMOL}},
	url = {https://onlinelibrary.wiley.com/doi/10.1002/jcc.21224},
	doi = {10.1002/jcc.21224},
	abstract = {Adequate initial conﬁgurations for molecular dynamics simulations consist of arrangements of molecules distributed in space in such a way to approximately represent the system’s overall structure. In order that the simulations are not disrupted by large van der Waals repulsive interactions, atoms from different molecules must keep safe pairwise distances. Obtaining such a molecular arrangement can be considered a packing problem: Each type molecule must satisfy spatial constraints related to the geometry of the system, and the distance between atoms of different molecules must be greater than some speciﬁed tolerance. We have developed a code able to pack millions of atoms, grouped in arbitrarily complex molecules, inside a variety of three-dimensional regions. The regions may be intersections of spheres, ellipses, cylinders, planes, or boxes. The user must provide only the structure of one molecule of each type and the geometrical constraints that each type of molecule must satisfy. Building complex mixtures, interfaces, solvating biomolecules in water, other solvents, or mixtures of solvents, is straightforward. In addition, different atoms belonging to the same molecule may also be restricted to different spatial regions, in such a way that more ordered molecular arrangements can be built, as micelles, lipid double-layers, etc. The packing time for state-of-the-art molecular dynamics systems varies from a few seconds to a few minutes in a personal computer. The input ﬁles are simple and currently compatible with PDB, Tinker, Molden, or Moldy coordinate ﬁles. The package is distributed as free software and can be downloaded from http://www.ime.unicamp.br/∼martinez/packmol/.},
	language = {en},
	number = {13},
	urldate = {2022-06-03},
	journal = {Journal of Computational Chemistry},
	author = {Martínez, L. and Andrade, R. and Birgin, E. G. and Martínez, J. M.},
	month = oct,
	year = {2009},
	pages = {2157--2164},
}

@article{berendsen_missing_1987,
	title = {The missing term in effective pair potentials},
	volume = {91},
	issn = {0022-3654, 1541-5740},
	url = {https://pubs.acs.org/doi/10.1021/j100308a038},
	doi = {10.1021/j100308a038},
	language = {en},
	number = {24},
	urldate = {2022-06-03},
	journal = {The Journal of Physical Chemistry},
	author = {Berendsen, H. J. C. and Grigera, J. R. and Straatsma, T. P.},
	month = nov,
	year = {1987},
	pages = {6269--6271},
}

@article{wang_multiscale_2015,
	title = {Multiscale modeling of the trihexyltetradecylphosphonium chloride ionic liquid},
	volume = {17},
	issn = {1463-9076, 1463-9084},
	url = {http://xlink.rsc.org/?DOI=C5CP02586A},
	doi = {10.1039/C5CP02586A},
	abstract = {Hierarchical trihexyltetradecylphosphonium cationic and chloride anionic models.
          , 
            
              A multiscale modeling protocol was sketched for the trihexyltetradecylphosphonium chloride ([P
              6,6,6,14
              ]Cl) ionic liquid (IL). The optimized molecular geometries of an isolated [P
              6,6,6,14
              ] cation and a tightly bound [P
              6,6,6,14
              ]Cl ion pair structure were obtained from quantum chemistry
              ab initio
              calculations. A cost-effective united-atom model was proposed for the [P
              6,6,6,14
              ] cation based on the corresponding atomistic model. Atomistic and coarse-grained molecular dynamics simulations were performed over a wide temperature range to validate the proposed united-atom [P
              6,6,6,14
              ] model against the available experimental data. Through a systemic analysis of volumetric quantities, microscopic structures, and transport properties of the bulk [P
              6,6,6,14
              ]Cl IL under varied thermodynamic conditions, it was identified that the proposed united-atom [P
              6,6,6,14
              ] cationic model could essentially capture the local intermolecular structures and the nonlocal experimental thermodynamics, including liquid density, volume expansivity and isothermal compressibility, and transport properties, such as zero-shear viscosity, of the bulk [P
              6,6,6,14
              ]Cl IL within a wide temperature range.},
	language = {en},
	number = {34},
	urldate = {2022-05-27},
	journal = {Physical Chemistry Chemical Physics},
	author = {Wang, Yong-Lei and Sarman, Sten and Li, Bin and Laaksonen, Aatto},
	year = {2015},
	pages = {22125--22135},
}

@article{sharma_pressure-dependent_2016,
	title = {Pressure-dependent morphology of trihexyl(tetradecyl)phosphonium ionic liquids: {A} molecular dynamics study},
	volume = {145},
	issn = {0021-9606, 1089-7690},
	shorttitle = {Pressure-dependent morphology of trihexyl(tetradecyl)phosphonium ionic liquids},
	url = {http://aip.scitation.org/doi/10.1063/1.4963271},
	doi = {10.1063/1.4963271},
	language = {en},
	number = {13},
	urldate = {2022-05-27},
	journal = {The Journal of Chemical Physics},
	author = {Sharma, Shobha and Gupta, Aditya and Dhabal, Debdas and Kashyap, Hemant K.},
	month = oct,
	year = {2016},
	pages = {134506},
}

@article{hettige_communication_2014,
	title = {Communication: {Anomalous} temperature dependence of the intermediate range order in phosphonium ionic liquids},
	volume = {140},
	issn = {0021-9606, 1089-7690},
	shorttitle = {Communication},
	url = {http://aip.scitation.org/doi/10.1063/1.4867900},
	doi = {10.1063/1.4867900},
	language = {en},
	number = {11},
	urldate = {2022-05-27},
	journal = {The Journal of Chemical Physics},
	author = {Hettige, Jeevapani J. and Kashyap, Hemant K. and Margulis, Claudio J.},
	month = mar,
	year = {2014},
	pages = {111102},
}

@article{yang_influence_2021,
	title = {Influence of {Ionic} {Interaction} {Strength} on {Glass} {Formation} of an {Ion}-{Containing} {Polymer} {Melt}},
	volume = {54},
	issn = {0024-9297, 1520-5835},
	url = {https://pubs.acs.org/doi/10.1021/acs.macromol.1c01719},
	doi = {10.1021/acs.macromol.1c01719},
	abstract = {A deep understanding of the glass formation of ion-containing polymers is crucial for applications of high technological relevance, but it remains a signiﬁcant challenge to develop a molecular theory to predict thermodynamic and dynamic properties of these materials. Here, we perform extensive molecular dynamics simulations of an ion-containing polymer melt having variable ionic interaction strength to address the essential phenomenology of thermodynamic and dynamic properties upon approaching the glass-transition temperature. Both thermodynamic and dynamic properties are shown to be strongly inﬂuenced by ionic interaction strength. The characteristic temperatures of glass formation increase with increasing ionic interaction strength in a nearly linear fashion, a trend that can be rationalized based on changes in the cohesive energy density induced by ionic interactions. The growth of fragility with increasing ionic interaction strength is found to be somewhat nonlinear. Moreover, we demonstrate that the string model of glass formation provides an excellent description of the relationship between the structural relaxation time and the string length in our ion-containing polymer melt having variable ionic interaction strength, implying that the entropy theory provides a promising tool for investigating the glass formation of ion-containing polymers if ionic interactions are incorporated properly. The string model also allows us to establish the general trends of the enthalpy and entropy of high temperature activation in variation with ionic interaction strength, fundamental energetic parameters that play a key role in the entropy theory of glass formation. Our simulation results should be helpful for developing a general framework to understand the glass formation of ion-containing polymers.},
	language = {en},
	number = {20},
	urldate = {2022-05-25},
	journal = {Macromolecules},
	author = {Yang, Zhenyue and Xu, Xiaolei and Xu, Wen-Sheng},
	month = oct,
	year = {2021},
	pages = {9587--9601},
}

@article{mcdaniel_polarization_2018,
	title = {Polarization {Effects} in {Binary} [{BMIM} $^{\textrm{+}}$ ][{BF} $_{\textrm{4}}$ $^{\textrm{–}}$ ]/1,2-{Dichloroethane}, {Acetone}, {Acetonitrile}, and {Water} {Electrolytes}},
	volume = {122},
	issn = {1520-6106, 1520-5207},
	url = {https://pubs.acs.org/doi/10.1021/acs.jpcb.8b01714},
	doi = {10.1021/acs.jpcb.8b01714},
	abstract = {Organic electrolytes are unique in that their constituent solvents may be of much lower dielectric strength than water. This is because the ions of organic electrolytes are often those that comprise room-temperature ionic liquids, which are surprisingly miscible with many diﬀerent organic solvents of low dielectric strength. Strong ion correlation results from the relatively low dielectric screening of the solvent, resulting in properties that can substantially deviate from Debye−Huckel descriptions; in addition remains the fundamental question of why the ionic liquids and low dielectric solvents are even miscible in the ﬁrst place. In this work, we study electrolyte mixtures composed of the roomtemperature ionic liquid 1-butyl-3-methylimidazolium tetraﬂuoroborate [BMIM+][BF4−] mixed with four solvents of systematically varying dielectric strength, 1,2-dichloroethane, acetone, acetonitrile, and water. We show that miscibility with the lowest dielectric solvent, dichloroethane, is directly attributed to ion solvation enhancement mediated by both electronic and conformational polarization of the solvent molecules. A strong dielectric enhancement results from the ∼70−80\% increase in solvent dipole moments at high ion content, providing signiﬁcantly better solvation than predicted by the bulk solvent dielectric strength. This implies a general mechanism for miscibility of ionic liquids with low dielectric solvents, through which ions eﬀectly create their own solvation dipoles by polarizing the local environment. From a purely computational perspective, our results imply that explicitly polarizable force ﬁelds are essential for modeling many of the organic electrolytes that are used in electrochemical applications.},
	language = {en},
	number = {15},
	urldate = {2022-05-25},
	journal = {The Journal of Physical Chemistry B},
	author = {McDaniel, Jesse G.},
	month = apr,
	year = {2018},
	pages = {4345--4355},
}

@article{mukherjee_gelation_2020,
	title = {Gelation {Impairs} {Phase} {Separation} and {Small} {Molecule} {Migration} in {Polymer} {Mixtures}},
	volume = {12},
	issn = {2073-4360},
	url = {https://www.mdpi.com/2073-4360/12/7/1576},
	doi = {10.3390/polym12071576},
	abstract = {Surface segregation of the low molecular weight component of a polymeric mixture is a ubiquitous phenomenon that leads to degradation of industrial formulations. We report a simultaneous phase separation and surface migration phenomena in oligomer–polymer (OP) and oligomer–gel (OG) systems following a temperature quench that induces demixing of components. We compute equilibrium and time varying migrant (oligomer) density proﬁles and wetting layer thickness in these systems using coarse grained molecular dynamics (CGMD) and mesoscale hydrodynamics (MH) simulations. Such multiscale methods quantitatively describe the phenomena over a wide range of length and time scales. We show that surface migration in gel–oligomer systems is signiﬁcantly reduced on account of network elasticity. Furthermore, the phase separation processes are signiﬁcantly slowed in gels leading to the modiﬁcation of the well known Lifshitz–Slyozov–Wagner (LSW) law (τ) ∼ τ1/3. Our work allows for rational design of polymer/gel–oligomer mixtures with predictable surface segregation characteristics that can be compared against experiments.},
	language = {en},
	number = {7},
	urldate = {2022-05-25},
	journal = {Polymers},
	author = {Mukherjee, Biswaroop and Chakrabarti, Buddhapriya},
	month = jul,
	year = {2020},
	pages = {1576},
}

@article{duering_relaxation_1991,
	title = {Relaxation of randomly cross-linked polymer melts},
	volume = {67},
	issn = {0031-9007},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.67.3531},
	doi = {10.1103/PhysRevLett.67.3531},
	language = {en},
	number = {25},
	urldate = {2022-05-25},
	journal = {Physical Review Letters},
	author = {Duering, Edgardo R. and Kremer, Kurt and Grest, Gary S.},
	month = dec,
	year = {1991},
	pages = {3531--3534},
}

@article{goswami_computer_2007,
	title = {Computer {Simulations} of {Ionomer} {Self}-{Assembly} and {Dynamics}},
	volume = {40},
	issn = {0024-9297, 1520-5835},
	url = {https://pubs.acs.org/doi/10.1021/ma070074w},
	doi = {10.1021/ma070074w},
	language = {en},
	number = {12},
	urldate = {2022-05-25},
	journal = {Macromolecules},
	author = {Goswami, Monojoy and Kumar, Sanat K. and Bhattacharya, Aniket and Douglas, Jack F.},
	month = jun,
	year = {2007},
	pages = {4113--4118},
}

@article{hall_ionic_2012,
	title = {Ionic {Aggregate} {Structure} in {Ionomer} {Melts}: {Effect} of {Molecular} {Architecture} on {Aggregates} and the {Ionomer} {Peak}},
	volume = {134},
	issn = {0002-7863, 1520-5126},
	shorttitle = {Ionic {Aggregate} {Structure} in {Ionomer} {Melts}},
	url = {https://pubs.acs.org/doi/10.1021/ja209142b},
	doi = {10.1021/ja209142b},
	abstract = {We perform a comprehensive set of coarse-grained molecular dynamics simulations of ionomer melts with varying polymer architectures and compare the results to experiments in order to understand ionic aggregation on a molecular level. The model ionomers contain periodically or randomly spaced charged beads, placed either within or pendant to the polymer backbone, with the counterions treated explicitly. The ionic aggregate structure was determined as a function of the spacing of charged beads and also depends on whether the charged beads are in the polymer backbone or pendant to the backbone. The low wavevector ionomer peak in the counterion scattering is observed for all systems, and it is sharpest for ionomers with periodically spaced pendant charged beads with a large spacing between charged beads. Changing to a random or a shorter spacing moves the peak to lower wavevector. We present new experimental X-ray scattering data on Na+-neutralized poly(ethylene-co-acrylic acid) ionomers that show the same two trends in the ionomer peak, for similarly structured ionomers. The order within and between aggregates, and how this relates to various models used to fit the ionomer peak, is quantified and discussed.},
	language = {en},
	number = {1},
	urldate = {2022-05-25},
	journal = {Journal of the American Chemical Society},
	author = {Hall, Lisa M. and Seitz, Michelle E. and Winey, Karen I. and Opper, Kathleen L. and Wagener, Kenneth B. and Stevens, Mark J. and Frischknecht, Amalie L.},
	month = jan,
	year = {2012},
	pages = {574--587},
}

@article{abbott_effects_2019,
	title = {Effects of {Side} {Chain} {Length} on {Ionic} {Aggregation} and {Dynamics} in {Polymer} {Single}-{Ion} {Conductors}},
	volume = {52},
	issn = {0024-9297, 1520-5835},
	url = {https://pubs.acs.org/doi/10.1021/acs.macromol.9b00415},
	doi = {10.1021/acs.macromol.9b00415},
	abstract = {We employed bead-spring models of polymer single-ion conductors to study the impact of chain architecture on ionic aggregation and dynamics. In most simulations, the ionic aggregates were ordered amorphously, but layered ionic structures were also formed in two cases. Here, we focus on the amorphous systems. The local aggregate structure was determined primarily by the ionic interaction strength, with strong interactions yielding blocky aggregates and weak interactions yielding stringy aggregates. Long side chains increased the conformational freedom of the polymer-bound anions, encouraging greater ionic aggregation. Correspondingly, percolated networks of ionic aggregates were common in the long-side-chain systems, while discrete aggregates were more typical of the short-side-chain systems. The aggregates formed physical crosslinks within the system and, therefore, strongly inﬂuenced the dynamics. With strong ionic interactions, cations moved more quickly via a shuttling mechanism through percolated aggregates instead of relying solely on the slow rearrangement of discrete aggregates. However, with weaker ionic interactions, the aggregate morphologies were less important, since the lifetimes of ion association were signiﬁcantly reduced.},
	language = {en},
	number = {19},
	urldate = {2022-05-25},
	journal = {Macromolecules},
	author = {Abbott, Lauren J. and Lawson, John W.},
	month = oct,
	year = {2019},
	pages = {7456--7467},
}

@article{shen_molecular_2021,
	title = {Molecular {Dynamics} {Simulations} of {Ion}-{Containing} {Polymers} {Using} {Generic} {Coarse}-{Grained} {Models}},
	volume = {54},
	issn = {0024-9297, 1520-5835},
	url = {https://pubs.acs.org/doi/10.1021/acs.macromol.0c02557},
	doi = {10.1021/acs.macromol.0c02557},
	abstract = {Molecular dynamics simulations with generic bead−spring models have been instrumental in revealing the molecular-scale behavior that underlies structure−property relationships of various types of polymeric systems. The generic, coarse-grained modeling approach does not include atomistic detail and is not focused on quantitatively matching the properties of a particular chemical system, though typically several parameters are included that can be tuned to consider diﬀerent types of chemistries. Besides allowing access to longer length and time scales due to computational eﬃciency, this type of approach is advantageous in that the physical insight gained is often relevant across the entire class of related materials. The connectivity and number of beads in a generic bead−spring models can be adjusted in an obvious manner to describe the most basic homopolymer features (e.g., to consider diﬀerent chain lengths and linear versus branched architectures). In uncharged copolymers or solventcontaining systems, the chemical interactions between components are considered by adjusting the strength of the various pairwise interparticle potentials (usually without changing their form). However, ions can have stronger and longer-ranged interactions with each other, with solvents, and with monomers that can require additional complexity be added to appropriately describe relevant phenomena in ion-containing polymeric systems. Recent eﬀorts are pushing the boundaries of the generic coarse-grained approach by including additional ion−ion or ion−polymer interactions to more closely capture and analyze such phenomena, while still avoiding detailed and speciﬁc empirical adjustments that would make the model only apply to a single chemical system. In this perspective, we highlight a variety of recent molecular dynamics work that applies generic coarse-grained models to study ioncontaining polymeric materials. We also discuss possible future directions and challenges of the generic coarse-graining approach in this area.},
	language = {en},
	number = {5},
	urldate = {2022-05-25},
	journal = {Macromolecules},
	author = {Shen, Kuan-Hsuan and Fan, Mengdi and Hall, Lisa M.},
	month = mar,
	year = {2021},
	pages = {2031--2052},
}

@article{sampath_impact_2017,
	title = {Impact of ionic aggregate structure on ionomer mechanical properties from coarse-grained molecular dynamics simulations},
	volume = {147},
	issn = {0021-9606, 1089-7690},
	url = {http://aip.scitation.org/doi/10.1063/1.4985904},
	doi = {10.1063/1.4985904},
	language = {en},
	number = {13},
	urldate = {2022-05-25},
	journal = {The Journal of Chemical Physics},
	author = {Sampath, Janani and Hall, Lisa M.},
	month = oct,
	year = {2017},
	pages = {134901},
}

@article{chremos_influence_2016,
	title = {Influence of higher valent ions on flexible polyelectrolyte stiffness and counter-ion distribution},
	volume = {144},
	issn = {0021-9606, 1089-7690},
	url = {http://aip.scitation.org/doi/10.1063/1.4947221},
	doi = {10.1063/1.4947221},
	language = {en},
	number = {16},
	urldate = {2022-05-25},
	journal = {The Journal of Chemical Physics},
	author = {Chremos, Alexandros and Douglas, Jack F.},
	month = apr,
	year = {2016},
	pages = {164904},
}

@article{wong_molecular_2002,
	title = {Molecular dynamics simulation of microstructure and counterion transport in dry ionic heteropolymers},
	volume = {116},
	issn = {0021-9606, 1089-7690},
	url = {http://aip.scitation.org/doi/10.1063/1.1461356},
	doi = {10.1063/1.1461356},
	language = {en},
	number = {15},
	urldate = {2022-05-25},
	journal = {The Journal of Chemical Physics},
	author = {Wong, Chee and Clarke, Julian H. R.},
	month = apr,
	year = {2002},
	pages = {6795--6802},
}

@misc{noauthor_httpspubsacsorgdoipdf101021acsjpcb8b01714_nodate,
	title = {https://pubs.acs.org/doi/pdf/10.1021/acs.jpcb.8b01714},
	url = {https://pubs.acs.org/doi/pdf/10.1021/acs.jpcb.8b01714},
	urldate = {2022-05-23},
}

@article{wang_microstructures_2017,
	title = {Microstructures and dynamics of tetraalkylphosphonium chloride ionic liquids},
	volume = {147},
	issn = {0021-9606, 1089-7690},
	url = {http://aip.scitation.org/doi/10.1063/1.4995003},
	doi = {10.1063/1.4995003},
	language = {en},
	number = {22},
	urldate = {2022-05-19},
	journal = {The Journal of Chemical Physics},
	author = {Wang, Yong-Lei and Li, Bin and Sarman, Sten and Laaksonen, Aatto},
	month = dec,
	year = {2017},
	pages = {224502},
}

@article{kremer_dynamics_1990,
	title = {Dynamics of entangled linear polymer melts: {A} molecular‐dynamics simulation},
	volume = {92},
	issn = {0021-9606, 1089-7690},
	shorttitle = {Dynamics of entangled linear polymer melts},
	url = {http://aip.scitation.org/doi/10.1063/1.458541},
	doi = {10.1063/1.458541},
	language = {en},
	number = {8},
	urldate = {2022-05-16},
	journal = {The Journal of Chemical Physics},
	author = {Kremer, Kurt and Grest, Gary S.},
	month = apr,
	year = {1990},
	pages = {5057--5086},
}

@article{everaers_kremergrest_2020,
	title = {Kremer–{Grest} {Models} for {Commodity} {Polymer} {Melts}: {Linking} {Theory}, {Experiment}, and {Simulation} at the {Kuhn} {Scale}},
	volume = {53},
	issn = {0024-9297, 1520-5835},
	shorttitle = {Kremer–{Grest} {Models} for {Commodity} {Polymer} {Melts}},
	url = {https://pubs.acs.org/doi/10.1021/acs.macromol.9b02428},
	doi = {10.1021/acs.macromol.9b02428},
	abstract = {The Kremer−Grest (KG) polymer model is a standard model for studying generic polymer properties in molecular dynamics simulations. It owes its popularity to its simplicity and computational eﬃciency, rather than its ability to represent speciﬁc polymers species and conditions. Here we show that by tuning the chain stiﬀness it is possible to adapt the KG model to model melts of real polymers. In particular, we provide mapping relations from KG to SI units for a wide range of commodity polymers. The connection between the experimental and the KG melts is made at the Kuhn scale, i.e., at the crossover from the chemistry-speciﬁc small scale to the universal large scale behavior. We expect Kuhn scale-mapped KG models to faithfully represent universal properties dominated by the large scale conformational statistics and dynamics of ﬂexible polymers. In particular, we observe very good agreement between entanglement moduli of our KG models and the experimental moduli of the target polymers.},
	language = {en},
	number = {6},
	urldate = {2022-05-16},
	journal = {Macromolecules},
	author = {Everaers, Ralf and Karimi-Varzaneh, Hossein Ali and Fleck, Frank and Hojdis, Nils and Svaneborg, Carsten},
	month = mar,
	year = {2020},
	pages = {1901--1916},
}

@article{canongia_lopes_modeling_2004,
	title = {Modeling {Ionic} {Liquids} {Using} a {Systematic} {All}-{Atom} {Force} {Field}},
	volume = {108},
	issn = {1520-6106, 1520-5207},
	url = {https://pubs.acs.org/doi/10.1021/jp0362133},
	doi = {10.1021/jp0362133},
	language = {en},
	number = {6},
	urldate = {2022-05-12},
	journal = {The Journal of Physical Chemistry B},
	author = {Canongia Lopes, José N. and Deschamps, Johnny and Pádua, Agílio A. H.},
	month = feb,
	year = {2004},
	pages = {2038--2047},
}

@article{canongia_lopes_molecular_2006,
	title = {Molecular {Force} {Field} for {Ionic} {Liquids} {III}: {Imidazolium}, {Pyridinium}, and {Phosphonium} {Cations}; {Chloride}, {Bromide}, and {Dicyanamide} {Anions}},
	volume = {110},
	issn = {1520-6106, 1520-5207},
	shorttitle = {Molecular {Force} {Field} for {Ionic} {Liquids} {III}},
	url = {https://pubs.acs.org/doi/10.1021/jp063901o},
	doi = {10.1021/jp063901o},
	language = {en},
	number = {39},
	urldate = {2022-05-12},
	journal = {The Journal of Physical Chemistry B},
	author = {Canongia Lopes, José N. and Pádua, Agílio A. H.},
	month = oct,
	year = {2006},
	pages = {19586--19592},
}

@article{vogel_ab_2010,
	title = {Ab initio pair potential energy curve for the argon atom pair and thermophysical properties for the dilute argon gas. {II}. {Thermophysical} properties for low-density argon},
	volume = {108},
	issn = {00268976},
	doi = {10.1080/00268976.2010.507557},
	abstract = {A recent argon-argon interatomic potential energy curve determined from quantum-mechanical ab initio calculations and described with an analytical representation [B. Jager, R. Hellmann, E. Bich, and E. Vogel, Mol. Phys. 107, 2181 (2009); 108, 105 (2010)] was used to calculate the most important thermophysical properties of argon governed by two-body interactions. Second pressure, acoustic, and dielectric virial coefficients as well as viscosity and thermal conductivity in the limit of zero density were computed for natural argon from 83 to 10,000 K. The calculated values for the different thermophysical properties are compared with available experimental data and values computed for other argon-argon potentials. This extensive analysis shows that the proposed potential is superior to all previous ones and that the calculated thermophysical property values are accurate enough to be applied as standard values for the complete temperature range of the calculations. © 2010 Taylor \& Francis.},
	number = {24},
	journal = {Molecular Physics},
	author = {Vogel, Eckhard and Jager, Benjamin and Hellmann, Robert and Bich, Eckard},
	year = {2010},
	keywords = {argon gas property standards, second acoustic virial coefficient, second dielectric virial coefficient, second pressure virial coefficient, viscosity and thermal conductivity},
	pages = {3335--3352},
}

@article{kowalczyk_static_2009,
	title = {Static and thermodynamic properties of low-density supercritical {4He} - {Breakdown} of the {Feynman}-{Hibbs} approximation},
	volume = {11},
	issn = {14639076},
	doi = {10.1039/b907165b},
	abstract = {We study the applicability of the semiclassical Feynman and Hibbs (FH) (second-order or fourth-order) effective potentials to the description of the thermodynamic properties of quantum fluids at finite temperatures. First, we use path integral Monte Carlo (PIMC) simulations to estimate the thermodynamic/static properties of our model quantum fluid, i.e. low-density 4He at 10 K. With PIMC we obtain the experimental equation of state, the single-particle mean kinetic energy, the single-particle density matrix and the single-particle momentum distribution of this system at low densities. We show that our PIMC results are in full agreement with experimental data obtained with deep inelastic neutron scattering at high momentum transfers (D. Colognesi, C. Andreani, R. Senesi, Europhys. Lett., 2000, 50, 202). As expected, in this region of the 4He phase diagram, quantum effects modify the width of the single-particle momentum distribution but do not alter its Gaussian shape. Knowing the exact values of density, pressure and single-particle mean kinetic energy for our model quantum fluid, we investigate the limitations of the semiclassical FH effective potentials. We show that commonly used 'short-time' approximations to the high-temperature density matrix due to Feynman and Hibbs can only be applied in a very limited range of the 4He phase diagram. We found that FH effective potentials reproduce the experimental densities of 4He at 10 K for Λ/a {\textless} 0.45 (Λ = 2.73 denotes the thermal de Broglie wavelength, a = ρ-1/3 is the mean nearest-neighbor distance in the fluid and ρ denotes fluid density). Moreover, semiclassical FH effective potentials are able to correctly predict the single-particle mean kinetic energy of 4He at 10 K in a very limited range of fluid densities, i.e.Λ/a {\textless} 0.17. We show that the ad hoc application of the semiclassical FH effective potentials for the calculation of the thermodynamic properties of dense liquid-like para-hydrogen (para-H2) adsorbed in nanoporous materials below 72 K is questionable. © the Owner Societies 2009.},
	number = {40},
	journal = {Physical Chemistry Chemical Physics},
	author = {Kowalczyk, Piotr and Brualla, Lorenzo and Gauden, Piotr A. and Terzyk, Artur P.},
	year = {2009},
	pages = {9182--9187},
}

@article{tchouar_computation_2004,
	title = {Computation of the properties of liquid neon, methane, and gas helium at low temperature by the {Feynman}-{Hibbs} approach},
	volume = {121},
	issn = {00219606},
	doi = {10.1063/1.1794651},
	number = {15},
	journal = {Journal of Chemical Physics},
	author = {Tchouar, N. and Ould-Kaddour, F. and Levesque, D.},
	year = {2004},
	pages = {7326--7331},
}

@misc{yew_clapeyronjl_2021,
	title = {Clapeyron.jl},
	url = {https://github.com/ypaul21/Clapeyron.jl},
	author = {Yew, Hon-Wa and Walker, Pierre J. and Riedeman, Andrés},
	year = {2021},
	doi = {10.5281/zenodo.4059343},
}

@article{tihic_predictive_2008,
	title = {A predictive group-contribution simplified {PC}-{SAFT} equation of state: {Application} to polymer systems},
	volume = {47},
	issn = {08885885},
	doi = {10.1021/ie0710768},
	abstract = {A group-contribution (GC) method is coupled with the molecular-based perturbed-chain statistical associating fluid theory (PC-SAFT) equation of state (EoS) to predict its characteristic pure compound parameters. The estimation of group contributions for the parameters is based on a parameter database of 400 low-molecularweight compounds estimated by fitting experimental vapor pressures and liquid densities. The method has been successfully used for estimating the PC-SAFT parameters for common polymers. Specifically, using the new polymer parameters as calculated from the proposed GC scheme, the simplified PC-SAFT yields rather good predictions of polymer densities and gives promising modeling results of various binary polymer mixtures exhibiting both vapor - liquid and liquid-liquid phase equilibria. In summary, the data required for calculating polymer phase equilibria with the proposed method are the molecular structure of the polymer of interest in terms of functional groups and a single binary interaction parameter for accurate mixture calculations. © 2008 American Chemical Society.},
	number = {15},
	journal = {Ind. Eng. Chem. Res.},
	author = {Tihic, Amra and Kontogeorgis, Georgios M. and Von Solms, Nicolas and Michelsen, Michael L.},
	year = {2008},
	pages = {5092--5101},
}

@article{rushbrooke_statistical_1940,
	title = {On the statistical mechanics of assemblies whose energy-levels depend on the temperature},
	volume = {36},
	issn = {0014-7672},
	doi = {10.1039/tf9403601055},
	journal = {Trans. Faraday Soc.},
	author = {Rushbrooke, G. S.},
	year = {1940},
	pages = {1055},
}

@article{pereira_held_2012,
	title = {The {HELD} algorithm for multicomponent, multiphase equilibrium calculations with generic equations of state},
	volume = {36},
	issn = {00981354},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0098135411002365},
	doi = {10.1016/j.compchemeng.2011.07.009},
	language = {en},
	urldate = {2022-04-25},
	journal = {Computers \& Chemical Engineering},
	author = {Pereira, Frances E. and Jackson, George and Galindo, Amparo and Adjiman, Claire S.},
	month = jan,
	year = {2012},
	pages = {99--118},
}

@article{peng_new_1976,
	title = {A {New} {Two}-{Constant} {Equation} of {State}},
	volume = {15},
	issn = {01964313},
	doi = {10.1021/i160057a011},
	abstract = {The development of a new two-constant equation of state in which the attractive pressure term of the semiempirical van der Waals equation has been modified is outlined. Examples of the use of the equation for predicting the vapor pressure and volumetric behavior of single-component systems, and the phase behavior and volumetric behavior of binary, ternary, and multicomponent systems are given. The proposed equation combines simplicity and accuracy. It performs as well as or better than the Soave-Redlich-Kwong equation in all cases tested and shows its greatest advantages in the prediction of liquid phase densities. © 1976, American Chemical Society. All rights reserved.},
	number = {1},
	journal = {Ind. Eng. Chem. Fundam.},
	author = {Peng, Ding Yu and Robinson, Donald B.},
	year = {1976},
	pages = {59--64},
}

@article{papaioannou_group_2014,
	title = {Group contribution methodology based on the statistical associating fluid theory for heteronuclear molecules formed from {Mie} segments},
	volume = {140},
	issn = {00219606},
	doi = {10.1063/1.4851455},
	abstract = {A generalization of the recent version of the statistical associating fluid theory for variable range Mie potentials [Lafitte et al., J. Chem. Phys. 139, 154504 (2013)] is formulated within the framework of a group contribution approach (SAFT-γ Mie). Molecules are represented as comprising distinct functional (chemical) groups based on a fused heteronuclear molecular model, where the interactions between segments are described with the Mie (generalized Lennard-Jonesium) potential of variable attractive and repulsive range. A key feature of the new theory is the accurate description of the monomeric group-group interactions by application of a high-temperature perturbation expansion up to third order. The capabilities of the SAFT-γ Mie approach are exemplified by studying the thermodynamic properties of two chemical families, the n-alkanes and the n-alkyl esters, by developing parameters for the methyl, methylene, and carboxylate functional groups (CH3, CH 2, and COO). The approach is shown to describe accurately the fluid-phase behavior of the compounds considered with absolute average deviations of 1.20\% and 0.42\% for the vapor pressure and saturated liquid density, respectively, which represents a clear improvement over other existing SAFT-based group contribution approaches. The use of Mie potentials to describe the group-group interaction is shown to allow accurate simultaneous descriptions of the fluid-phase behavior and second-order thermodynamic derivative properties of the pure fluids based on a single set of group parameters. Furthermore, the application of the perturbation expansion to third order for the description of the reference monomeric fluid improves the predictions of the theory for the fluid-phase behavior of pure components in the near-critical region. The predictive capabilities of the approach stem from its formulation within a group-contribution formalism: predictions of the fluid-phase behavior and thermodynamic derivative properties of compounds not included in the development of group parameters are demonstrated. The performance of the theory is also critically assessed with predictions of the fluid-phase behavior (vapor-liquid and liquid-liquid equilibria) and excess thermodynamic properties of a variety of binary mixtures, including polymer solutions, where very good agreement with the experimental data is seen, without the need for adjustable mixture parameters. © 2014 AIP Publishing LLC.},
	number = {5},
	journal = {J. Chem. Phys.},
	author = {Papaioannou, Vasileios and Lafitte, Thomas and Avendaño, Carlos and Adjiman, Claire S. and Jackson, George and Müller, Erich A. and Galindo, Amparo},
	year = {2014},
	pages = {054107},
}

@incollection{lemmon_thermophysical_2020,
	address = {Gaithersburg MD},
	title = {Thermophysical {Properties} of {Fluid} {Systems}},
	booktitle = {{NIST} {Chemistry} {WebBook}, {NIST} {Standard} {Reference} {Database} {Number} 69,},
	publisher = {National Institute of Standards and Technology},
	author = {Lemmon, E. W. and McLinden, M. O. and Friend, D. G.},
	year = {2020},
	doi = {10.18434/T4D303},
	note = {Section: Thermophys},
}

@article{kontogeorgis_equation_1996,
	title = {An equation of state for associating fluids},
	volume = {35},
	issn = {08885885},
	doi = {10.1021/ie9600203},
	abstract = {An equation of state (EoS) suitable for describing associating fluids is presented. The equation combines the simplicity of a cubic equation of state (the Soave-Redlich-Kwong), which is used for the physical part and the theoretical background of the perturbation theory employed for the chemical (or association) part. The resulting EoS (Cubic Plus Association) is not cubic with respect to volume and contains five pure compound parameters which are determined using vapor pressures and saturated liquid densities. Excellent correlations of both vapor pressures and saturated liquid volumes are obtained for primary-alcohols (from methanol up to 1-tridecanol), phenol, tert-butyl alcohol, triethylene glycol, and water. Moreover, excellent prediction of saturated liquid volumes may be obtained from parameters which have been estimated by regressing only vapor pressures. Finally, we suggest a method for reducing the number of adjustable parameters for alcohols to three while maintaining the good correlation of vapor pressures and saturated liquid volumes. We investigate the possibility of using the homomorph approach for estimating the EoS parameters and explain the problems observed. The estimated pure compound parameters have been tested in the prediction of second virial coefficients with satisfactory results.},
	number = {11},
	journal = {Ind. Eng. Chem. Res.},
	author = {Kontogeorgis, Georgios M. and Voutsas, Epaminondas C. and Yakoumis, Iakovos V. and Tassios, Dimitrios P.},
	year = {1996},
	pages = {4310--4318},
}

@article{klamt_conductor-like_1995,
	title = {Conductor-like {Screening} {Model} for {Real} {Solvents}: {A} {New} {Approach} to the {Quantitative} {Calculation} of {Solvation} {Phenomena}},
	volume = {99},
	issn = {0022-3654},
	url = {https://pubs.acs.org/doi/abs/10.1021/j100007a062},
	doi = {10.1021/j100007a062},
	number = {7},
	journal = {J. Phys. Chem.},
	author = {Klamt, Andreas},
	month = feb,
	year = {1995},
	pages = {2224--2235},
}

@article{klamt_cosmo_1993,
	title = {{COSMO}: a new approach to dielectric screening in solvents with explicit expressions for the screening energy and its gradient},
	issn = {0300-9580},
	url = {http://xlink.rsc.org/?DOI=P29930000799},
	doi = {10.1039/P29930000799},
	number = {5},
	journal = {J. Chem. Soc., Perkin Trans. 2},
	author = {Klamt, A. and Schüürmann, G.},
	year = {1993},
	pages = {799--805},
}

@article{joback_estimation_1987,
	title = {Estimation of {Pure}-{Component} {Properties} from {Group}-{Contributions}},
	volume = {57},
	issn = {15635201},
	doi = {10.1080/00986448708960487},
	abstract = {Simple group-contribution methods are proposed to estimate eleven important physical properties of pure materials. A common set of structural groups was employed. High accuracy is not claimed, but the proposed methods are often as accurate as or more accurate than techniques in common use today. © 1987, Taylor \& Francis Group, LLC. All rights reserved.},
	number = {1-6},
	journal = {Chem. Eng. Commun.},
	author = {Joback, K. G. and Reid, R. C.},
	year = {1987},
	keywords = {Viscosity, critical properties, estimation methods, group contributions, ideal gas},
	pages = {233--243},
}

@article{inguva_continuum-scale_2021,
	title = {Continuum-scale modelling of polymer blends using the {Cahn}–{Hilliard} equation: transport and thermodynamics},
	volume = {17},
	copyright = {All rights reserved},
	issn = {1744-683X, 1744-6848},
	shorttitle = {Continuum-scale modelling of polymer blends using the {Cahn}–{Hilliard} equation},
	url = {http://xlink.rsc.org/?DOI=D1SM00272D},
	doi = {10.1039/D1SM00272D},
	abstract = {This review explores the physical features of the Cahn–Hilliard equation and how various thermodynamic models can be incorporated to study mixtures such as polymer blends.
          , 
            The Cahn–Hilliard equation is commonly used to study multi-component soft systems such as polymer blends at continuum scales. We first systematically explore various features of the equation system, which give rise to a deep connection between transport and thermodynamics-specifically that the Gibbs free energy of mixing function is central to formulating a well-posed model. Accordingly, we explore how thermodynamic models from three broad classes of approach (lattice-based, activity-based and perturbation methods) can be incorporated within the Cahn–Hilliard equation and examine how they impact the numerical solution for two model polymer blends, noting that although the analysis presented here is focused on binary mixtures, it is readily extensible to multi-component mixtures. It is observed that, although the predicted liquid–liquid interfacial tension is quite strongly affected, the choice of thermodynamic model has little influence on the development of the morphology.},
	language = {en},
	number = {23},
	urldate = {2021-09-27},
	journal = {Soft Matter},
	author = {Inguva, Pavan K. and Walker, Pierre J. and Yew, Hon Wa and Zhu, Kezheng and Haslam, Andrew J. and Matar, Omar K.},
	year = {2021},
	pages = {5645--5665},
}

@article{huang_equation_1991,
	title = {Equation of {State} for {Small}, {Large}, {Polydisperse}, and {Associating} {Molecules}: {Extension} to {Fluid} {Mixtures}},
	volume = {30},
	issn = {15205045},
	doi = {10.1021/ie00056a050},
	abstract = {Statistical associating fluid theory (SAFT) has been extended to mixtures using rigorous statistical mechanical expressions for the hard-sphere, chain, and association terms. In contrast to previous equations of state, only the dispersion term requires mixing rules (averaging equations for SAFT parameters). We use two approaches to deriving the mixing rules, a van der Waals one-fluid approximation (vdW1) rooted in conformal solution theory and a volume-fraction (vf) approximation similar to group-contribution equations of state. We test these approaches on 60 phase equilibrium data sets for asymmetric (small + large) and associating binaries. While both sets of mixing rules, vdW1 and vf, are found to be adequate away from the critical region, the vf predictions are found to be more accurate near the critical region. © 1991, American Chemical Society. All rights reserved.},
	number = {8},
	journal = {Ind. Eng. Chem. Res.},
	author = {Huang, Stanley H. and Radosz, Maciej},
	year = {1991},
	pages = {1994--2005},
}

@article{huang_equation_1990,
	title = {Equation of {State} for {Small}, {Large}, {Polydisperse}, and {Associating} {Molecules}},
	volume = {29},
	issn = {15205045},
	doi = {10.1021/ie00107a014},
	abstract = {Statistical Associating Fluid Theory (SAFT) has been extended to many real, molecular, and macromolecular fluids, such as chain, aromatic, and chlorinated hydrocarbons, ethers, alkanols (aliphatic alcohols), carboxylic acids, esters, ketones, amines, and polymers, having molar mass up to 100000. The key result of this work is an accurate and physically sound equation of state for predicting density, vapor pressure, and other fluid properties. Practical calculations require three nonspecific parameters: segment number, segment volume, and segment-segment interaction energy (segment energy for short). For chain molecules, the segment volume and segment energy are found to be nearly constant upon increasing the molar mass, while the segment number is found to be a linear function of molar mass. As a result, this equation of state represents a useful, predictive correlation for many compounds, such as polymers, where no extensive experimental data are available and where parameters have to be estimated based on molar mass and chemical structure only. Specific interactions, such as hydrogen bonding, are characterized by two association parameters, the association energy and volume, characteristic of each site-site pair. These parameters, having well-defined physical meaning, control the bond strength and hence the degree of association. © 1990, American Chemical Society. All rights reserved.},
	number = {11},
	journal = {Ind. Eng. Chem. Res.},
	author = {Huang, Stanley H. and Radosz, Maciej},
	year = {1990},
	pages = {2284--2294},
}

@article{gil-villegas_statistical_1997,
	title = {Statistical associating fluid theory for chain molecules with attractive potentials of variable range},
	volume = {106},
	issn = {0021-9606},
	url = {http://aip.scitation.org/doi/10.1063/1.473101},
	doi = {10.1063/1.473101},
	number = {10},
	journal = {J. Chem. Phys.},
	author = {Gil-Villegas, Alejandro and Galindo, Amparo and Whitehead, Paul J. and Mills, Stuart J. and Jackson, George and Burgess, Andrew N.},
	month = mar,
	year = {1997},
	pages = {4168--4186},
}



@article{bell_pure_2014,
	title = {Pure and {Pseudo}-pure {Fluid} {Thermophysical} {Property} {Evaluation} and the {Open}-{Source} {Thermophysical} {Property} {Library} {CoolProp}},
	volume = {53},
	issn = {0888-5885},
	url = {https://pubs.acs.org/doi/10.1021/ie4033999},
	doi = {10.1021/ie4033999},
	number = {6},
	journal = {Ind. Eng. Chem. Res.},
	author = {Bell, Ian H. and Wronski, Jorrit and Quoilin, Sylvain and Lemort, Vincent},
	month = feb,
	year = {2014},
	pages = {2498--2508},
}

@article{aasen_equation_2020,
	title = {Equation of state and force fields for {Feynman}-{Hibbs}-corrected {Mie} fluids. {II}. {Application} to mixtures of helium, neon, hydrogen, and deuterium},
	volume = {152},
	issn = {00219606},
	doi = {10.1063/1.5136079},
	abstract = {We extend the statistical associating fluid theory of quantum corrected Mie potentials (SAFT-VRQ Mie), previously developed for pure fluids [Aasen et al., J. Chem. Phys. 151, 064508 (2019)], to fluid mixtures. In this model, particles interact via Mie potentials with Feynman-Hibbs quantum corrections of first order (Mie-FH1) or second order (Mie-FH2). This is done using a third-order Barker-Henderson expansion of the Helmholtz energy from a non-additive hard-sphere reference system. We survey existing experimental measurements and ab initio calculations of thermodynamic properties of mixtures of neon, helium, deuterium, and hydrogen and use them to optimize the Mie-FH1 and Mie-FH2 force fields for binary interactions. Simulations employing the optimized force fields are shown to follow the experimental results closely over the entire phase envelopes. SAFT-VRQ Mie reproduces results from simulations employing these force fields, with the exception of near-critical states for mixtures containing helium. This breakdown is explained in terms of the extremely low dispersive energy of helium and the challenges inherent in current implementations of the Barker-Henderson expansion for mixtures. The interaction parameters of two cubic equations of state (Soave-Redlich-Kwong and Peng-Robinson) are also fitted to experiments and used as performance benchmarks. There are large gaps in the ranges and properties that have been experimentally measured for these systems, making the force fields presented especially useful.},
	number = {7},
	journal = {J. Chem. Phys.},
	author = {Aasen, Ailo and Hammer, Morten and Müller, Erich A. and Wilhelmsen, Øivind},
	month = feb,
	year = {2020},
	pmid = {32087642},
	note = {Publisher: American Institute of Physics Inc.},
	pages = {074507},
}

@article{aasen_equation_2019,
	title = {Equation of state and force fields for {Feynman}-{Hibbs}-corrected {Mie} fluids. {I}. {Application} to pure helium, neon, hydrogen, and deuterium},
	volume = {151},
	issn = {00219606},
	doi = {10.1063/1.5111364},
	abstract = {We present a perturbation theory that combines the use of a third-order Barker-Henderson expansion of the Helmholtz energy with Mie-potentials that include first- (Mie-FH1) and second-order (Mie-FH2) Feynman-Hibbs quantum corrections. The resulting equation of state, the statistical associating fluid theory for Mie potentials of variable range corrected for quantum effects (SAFT-VRQ-Mie), is compared to molecular simulations and is seen to reproduce the thermodynamic properties of generic Mie-FH1 and Mie-FH2 fluids accurately. SAFT-VRQ Mie is exploited to obtain optimal parameters for the intermolecular potentials of neon, helium, deuterium, ortho-, para-, and normal-hydrogen for the Mie-FH1 and Mie-FH2 formulations. For helium, hydrogen, and deuterium, the use of either the first- or second-order corrections yields significantly higher accuracy in the representation of supercritical densities, heat capacities, and speed of sounds when compared to classical Mie fluids, although the Mie-FH2 is slightly more accurate than Mie-FH1 for supercritical properties. The Mie-FH1 potential is recommended for most of the fluids since it yields a more accurate representation of the pure-component phase equilibria and extrapolates better to low temperatures. Notwithstanding, for helium, where the quantum effects are largest, we find that none of the potentials give an accurate representation of the entire phase envelope, and its thermodynamic properties are represented accurately only at temperatures above 20 K. Overall, supercritical heat capacities are well represented, with some deviations from experiments seen in the liquid phase region for helium and hydrogen.},
	number = {6},
	journal = {J. Chem. Phys.},
	author = {Aasen, Ailo and Hammer, Morten and Ervik, Åsmund and Müller, Erich A. and Wilhelmsen, Øivind},
	month = aug,
	year = {2019},
	note = {Publisher: American Institute of Physics Inc.},
	pages = {064508},
}

@book{kontogeorgis_thermodynamic_2010,
	address = {West Sussex},
	edition = {1st},
	title = {Thermodynamic {Models} for {Industrial} {Applications}: {From} {Classical} and {Advanced} {Mixing} {Rules} to {Association} {Theories}},
	isbn = {978-0-470-74753-7},
	abstract = {Using an applications perspective Thermodynamic Models for Industrial Applications provides a unified framework for the development of various thermodynamic models, ranging from the classical models to some of the most advanced ones. Among these are the Cubic Plus Association Equation of State (CPA EoS) and the Perturbed Chain Statistical Association Fluid Theory (PC-SAFT). These two advanced models are already in widespread use in industry and academia, especially within the oil and gas, chemical and polymer industries. Presenting both classical models such as the Cubic Equations of State and more advanced models such as the CPA, this book provides the critical starting point for choosing the most appropriate calculation method for accurate process simulations. Written by two of the developers of these models, Thermodynamic Models for Industrial Applications emphasizes model selection and model development and includes a useful "which model for which application" guide. It also covers industrial requirements as well as discusses the challenges of thermodynamics in the 21st Century.},
	publisher = {Wiley},
	author = {Kontogeorgis, Georgios M. and Folas, Georgios K.},
	year = {2010},
	doi = {10.1002/9780470747537},
	note = {Publication Title: Thermodynamic Models for Industrial Applications: From Classical and Advanced Mixing Rules to Association Theories},
	keywords = {ISBN-13: 9780470697269},
}

@article{hendriks_industrial_2010,
	title = {Industrial {Requirements} for {Thermodynamics} and {Transport} {Properties}},
	volume = {49},
	issn = {0888-5885},
	url = {https://pubs.acs.org/doi/10.1021/ie101231b},
	doi = {10.1021/ie101231b},
	abstract = {This paper reports the results of an investigation of industrial requirements for thermodynamic and transport properties carried out during the years 2019-2020. It is a follow-up of a similar investigation performed and published 10 years ago by the Working Party (WP) of Thermodynamics and Transport Properties of European Federation of Chemical Engineering (EFCE).1 The main goal was to investigate the advances in this area over the past 10 years, to identify the limitations that still exist, and to propose future R\&D directions that will address the industrial needs. An updated questionnaire, with two new categories, namely, digitalization and comparison to previous survey/changes over the past 10 years, was sent to a broad number of experts in companies with a diverse activity spectrum, in oil and gas, chemicals, pharmaceuticals/biotechnology, food, chemical/ mechanical engineering, consultancy, and power generation, among others, and in software suppliers and contract research laboratories. Very comprehensive answers were received by 37 companies, mostly from Europe (operating globally), but answers were also provided by companies in the USA and Japan. The response rate was about 60\%, compared to 47\% in the year 2010. The paper is written in such a way that both the majority and minority points of view are presented, and although the discussion is focused on needs and challenges, the benefits of thermodynamics and success stories are also reported. The results of the survey are thematically structured and cover changes, challenges, and further needs for a number of areas of interest such as data, models, systems, properties, and computational aspects (molecular simulation, algorithms and standards, and digitalization). Education and collaboration are discussed and recommendations on the future research activities are also outlined. In addition, a few initiatives, books, and reviews published in the past decade are briefly discussed. It is a long paper and, to provide the reader with a more complete understanding of the survey, many (anonymous) quotations (indicated with "." and italics) from the industrial colleagues who have participated in the survey are provided. To help disseminate the specific information of interest only to particular industrial sectors, the paper has been written in such a way that the individual sections can also be read independently of each other.},
	number = {22},
	journal = {Ind. Eng. Chem. Res.},
	author = {Hendriks, Eric and Kontogeorgis, Georgios M. and Dohrn, Ralf and de Hemptinne, Jean-Charles and Economou, Ioannis G. and Žilnik, Ljudmila Fele and Vesovic, Velisa},
	month = nov,
	year = {2010},
	pages = {11131--11141},
}

@article{voutsas_universal_2004,
	title = {Universal mixing rule for cubic equations of state applicable to symmetric and asymmetric systems: {Results} with the {Peng}-{Robinson} equation of state},
	volume = {43},
	issn = {08885885},
	doi = {10.1021/ie049580p},
	abstract = {A mixing rule for cubic equations of state (CEoS) applicable to all types of system asymmetries-referred to hereafter as the universal mixing rule (UMR)-is proposed. For the cohesion parameter of the CEoS, the mixing rule involves the Staverman-Guggenheim part of the combinatorial term and the residual term of the original UNIFAC Gibbs free energy expression. For the covolume parameter of the CEoS, the quadratic concentration-dependent mixing rule is used with the combining rule for the cross parameter bij = [1/2(bi1/2 + bj1/2)]2. This UMR is applied to the volume-translated and modified version of the Peng-Robinson equation of state of Magoulas and Tassios (Fluid Phase Equilib. 1990, 56, 119), leading to what is referred to as the UMR-PR model. Very satisfactory results are obtained using the existing interaction parameters of the original UNIFAC model for vapor-liquid equilibrium predictions at low and high pressures for a wide range of system asymmetries including mixtures containing polymers. Satisfactory liquid-liquid equilibrium predictions are also obtained with the UMR-PR model.},
	number = {19},
	journal = {Ind. Eng. Chem. Res.},
	author = {Voutsas, Epaminondas and Magoulas, Kostis and Tassios, Dimitrios},
	year = {2004},
	pages = {6238--6246},
}

@article{bell_benchmark_2020,
	title = {A {Benchmark} {Open}-{Source} {Implementation} of {COSMO}-{SAC}},
	volume = {16},
	issn = {15499626},
	doi = {10.1021/acs.jctc.9b01016},
	abstract = {The COSMO-SAC modeling approach has found wide application in science as well as in a range of industries due to its good predictive capabilities. While other models for liquid phases, as for example UNIFAC, are in general more accurate than COSMO-SAC, these models typically contain many adjustable parameters and can be limited in their applicability. In contrast, the COSMO-SAC model only contains a few universal parameters and subdivides the molecular surface area into charged segments that interact with each other. In recent years, additional improvements to the construction of the sigma profiles and evaluation of activity coefficients have been made. In this work, we present a comprehensive description of how to postprocess the results of a COSMO calculation through to the evaluation of thermodynamic properties. We also assembled a large database of COSMO files, consisting of 2261 compounds, freely available to academic and noncommercial users. We especially focus on the documentation of the implementation and provide the optimized source code in C++, wrappers in Python, and sample sigma profiles calculated from each approach, as well as tests and validation results. The misunderstandings in the literature relating to COSMO-SAC are described and corrected. The computational efficiency of the implementation is demonstrated.},
	number = {4},
	journal = {J. Chem. Theory Comput.},
	author = {Bell, Ian H. and Mickoleit, Erik and Hsieh, Chieh Ming and Lin, Shiang Tai and Vrabec, Jadran and Breitkopf, Cornelia and Jäger, Andreas},
	year = {2020},
	pmid = {32059112},
	pages = {2635--2646},
}

@article{lin_priori_2002,
	title = {A priori phase equilibrium prediction from a segment contribution solvation model},
	volume = {41},
	issn = {08885885},
	doi = {10.1021/ie001047w},
	abstract = {An activity coefficient model using molecular solvation based on the COSMO-RS method is proposed. In this model, quantum mechanical COSMO calculations are performed to obtain the screening charges for molecules in a perfect conductor. A statistical mechanical model that considers molecules to be a collection of surface segments is developed for the calculation of segment activity coefficients using these screening charges. Activity coefficients for molecules are then obtained by summing the contributions of the segments. This model requires only a single radius for each atom in the COSMO solvation calculations, one universal parameter to discern hydrogen-bond acceptors and donors, and two universal parameters to determine segment interactions. This is a significantly fewer number of parameters for phase equilibrium calculations than group contribution methods such as the UNIFAC (168 parameters) and modified UNIFAC (612 parameters) models. The resulting completely a priori prediction method results in absolute average deviations of 0.03 in vapor-phase mole fractions and 9\% in total pressure for vapor-liquid equilibrium predictions of 243 binary mixtures and root-mean-square deviations of the octanol/water partition coefficient log KOW, infinite dilution activity coefficients ln γ∞ in water, and in hexane for 64 compounds of 0.48, 1.65, and 0.50, respectively. This model is general and applicable for the a priori prediction of the phase behavior of most compounds, though admittedly it is less accurate than group contribution and other methods with many more parameters whose values have been obtained by regressing large amounts of data.},
	number = {5},
	journal = {Ind. Eng. Chem. Res.},
	author = {Lin, Shiang Tai and Sandler, Stanley I.},
	year = {2002},
	pages = {899--913},
}

@article{blas_thermodynamic_1997,
	title = {Thermodynamic behaviour of homonuclear and heteronuclear {Lennard}-{Jones} chains with association sites from simulation and theory},
	volume = {92},
	issn = {0026-8976},
	url = {https://www.tandfonline.com/doi/full/10.1080/002689797170707},
	doi = {10.1080/002689797170707},
	abstract = {Monte Carlo simulation and theoretical results are presented for mixtures of associating and non-associating Lennard-Jones chains. The molecular model accounts explicitly for repulsive, dispersive, chain, and association interactions. A modified statistical associating fluid theory for Lennard-Jones chains is used to compare with the NPT and Gibbs ensemble Monte Carlo simulation results. The equation is extended to describe heteronuclear Lennard-Jones chains, and results are compared with those obtained by Monte Carlo simulations. The influence of several variables, such as chain length, segment size and dispersive energy, polydispersity, etc., on the supercritical properties and the phase equilibria behaviour of these systems is discussed here. The theory seems to predict more accurately the behaviour of long chains rather than of those of intermediate length, due to the approximations made in the radial distribution function of the fluid. © 1997 Taylor \& Francis Ltd.},
	number = {1},
	journal = {Mol. Phys.},
	author = {Blas, Felipe J. and Vega, Lourdes F.},
	month = sep,
	year = {1997},
	pages = {135--150},
}

@article{chaparro_phasepy_2020,
	title = {Phasepy: {A} {Python} based framework for fluid phase equilibria and interfacial properties computation},
	volume = {41},
	issn = {0192-8651},
	url = {https://onlinelibrary.wiley.com/doi/10.1002/jcc.26405},
	doi = {10.1002/jcc.26405},
	number = {29},
	journal = {J. Comput. Chem.},
	author = {Chaparro, Gustavo and Mejía, Andrés},
	month = nov,
	year = {2020},
	pages = {2504--2526},
}

@article{huron_new_1979,
	title = {New mixing rules in simple equations of state for representing vapour-liquid equilibria of strongly non-ideal mixtures},
	volume = {3},
	issn = {03783812},
	url = {https://linkinghub.elsevier.com/retrieve/pii/0378381279800011},
	doi = {10.1016/0378-3812(79)80001-1},
	number = {4},
	journal = {Fluid Phase Equilib.},
	author = {Huron, Marie-José and Vidal, Jean},
	month = jan,
	year = {1979},
	pages = {255--271},
}

@article{mi_equation_2002,
	title = {Equation of state extended from {SAFT} with improved results for polar fluids across the critical point},
	volume = {201},
	issn = {03783812},
	doi = {10.1016/S0378-3812(02)00093-6},
	abstract = {An equation of state (EOS) extended from statistical associating fluid theory (SAFT) has been proposed recently to describe the thermodynamic properties of non-polar fluids across the critical point (CP) (Fluid Phase Equilib. 186 (2001) 165). In this work, this EOS is modified further to describe the thermodynamic properties of polar fluids across the CP by taking into account the dipole-dipole interaction. The dipole-dipole term proposed by Twu and Gubbins (Chem. Eng. Sci. 33 (1978) 863, 879) is used in this work in which the effective dipole moment is approximated as a liner function of density (Ind. Eng. Chem. Res. 35 (1996) 4727). We call this series of EOS with improved results across the CP as SAFT-CP. The new EOS that contains the dipole-dipole term includes five parameters for each polar fluid: the segment number m, the segment non-spherical parameter α, the segment volume v00, the segment interaction parameter u0/k and adjustable parameter c for effective dipole moment. Twelve polar fluids including hydrogen sulfide, ammonia, chloromethane, 1,1-difluoroethane, 1,1,1-trifluoroethane, 1,1,1,2-tetrafluoroethane, diethyl ether, ethyl acetate, acetone, 2-butanone, 2-pentanone, and 2-heptanone are used as examples. Polar fluids with associating sites are not included in this work, such as water and alkanols. The SAFT-CP EOS reproduces the saturated pressure and liquid density date with an average absolute derivation (AAD) of about 1\%. Critical temperatures, pressures and densities are calculated with the AAD less than 2\%. In the one-phase region including supercritical region, the SAFT-CP represents the experimental values of density with an AAD of about 2\%. The comparison of the calculated critical exponent β with the experimental one for ethyl ether shows the improvement in the region of temperature approximately up to (TC-2)K. Copyright © 2002 Elsevier Science B.V.},
	number = {2},
	journal = {Fluid Phase Equilib.},
	author = {Mi, J. G. and Chen, J. and Gao, G. H. and Fei, W. Y.},
	year = {2002},
	keywords = {Critical point, Equation of state, Polar fluids, SAFT-CP, Vapor-liquid equilibrium},
	pages = {295--307},
}

@article{mccabe_predicting_1998,
	title = {Predicting the high-pressure phase equilibria of binary mixtures of perfluoro-n-alkanes + n-alkanes using the {SAFT}-{VR} approach},
	volume = {102},
	issn = {15206106},
	doi = {10.1021/jp982331s},
	abstract = {The phase behavior of perfluoro-(n)-alkane + (n)-alkane binary mixtures is of particular interest given their unexpected large positive deviations from Raoult's law. Binary mixtures of perfluoromethane + (n)-alkanes from methane to heptane are studied here, illustrating the continuous change in phase behavior from type II to type III that these systems exhibit. Some symmetrical systems that display heteroazeotropy are also examined. Using the statistical associating fluid theory for potentials of variable attractive range (SAFT-VR),we predict the high-pressure phase diagram for each binary mixture studied. The perfluoro-n-alkane and n-alkane molecules are treated as attractive spherical segments tangentially bonded together to form chains. We use simple empirical relationships between the number of carbon atoms and the number of segments in each chain. The attractive interactions are included as a square-well potential of depth ϵ and range λ. The pure component parameters are obtained by fitting to experimental vapor pressure and saturated liquid density data from the triple to the critical point. These optimized parameters are rescaled by the respective experimental critical points and used to determine the critical lines and phase behavior of the mixtures. The critical lines predicted by SAFT-VR for the perfluoro-n-alkane + n-alkane mixtures are in excellent agreement with the experimental data and improve significantly the results obtained with the simpler SAFT-HS approach, where the attractive interactions are treated at the mean-field level. This is particularly gratifying as the unlike dispersion interaction between the perfluoroalkane and alkane segments is obtained from a single mixture (perfluorobutane + n-butane) and then transferred to the other systems.},
	number = {41},
	journal = {J. Phys. Chem. B},
	author = {McCabe, Clare and Galindo, Amparo and Gil-Villegas, Alejandro and Jackson, George},
	year = {1998},
	pages = {8060--8069},
}

@article{ma_comparison_2018,
	title = {A {Comparison} of {Automatic} {Differentiation} and {Continuous} {Sensitivity} {Analysis} for {Derivatives} of {Differential} {Equation} {Solutions}},
	url = {http://arxiv.org/abs/1812.01892},
	doi = {arXiv:1812.01892},
	abstract = {Derivatives of differential equation solutions are commonly for parameter estimation, fitting neural differential equations, and as model diagnostics. However, with a litany of choices and a Cartesian product of potential methods, it can be difficult for practitioners to understand which method is likely to be the most effective on their particular application. In this manuscript we investigate the performance characteristics of Discrete Local Sensitivity Analysis implemented via Automatic Differentiation (DSAAD) against continuous adjoint sensitivity analysis. Non-stiff and stiff biological and pharmacometric models, including a PDE discretization, are used to quantify the performance of sensitivity analysis methods. Our benchmarks show that on small systems of ODEs (approximately \${\textless}100\$ parameters+ODEs), forward-mode DSAAD is more efficient than both reverse-mode and continuous forward/adjoint sensitivity analysis. The scalability of continuous adjoint methods is shown to be more efficient than discrete adjoints and forward methods after crossing this size range. These comparative studies demonstrate a trade-off between memory usage and performance in the continuous adjoint methods that should be considered when choosing the technique, while numerically unstable backsolve techniques from the machine learning literature are demonstrated as unsuitable for most scientific models. The performance of adjoint methods is shown to be heavily tied to the reverse-mode AD method, with tape-based AD methods shown to be 2 orders of magnitude slower on nonlinear partial differential equations than static AD techniques. These results also demonstrate the applicability of DSAAD to differential-algebraic equations, delay differential equations, and hybrid differential equation systems, showcasing an ease of implementation advantage for DSAAD approaches.},
	journal = {arXiv:1812.01892},
	author = {Ma, Yingbo and Dixit, Vaibhav and Innes, Mike and Guo, Xingjian and Rackauckas, Christopher},
	month = dec,
	year = {2018},
	note = {\_eprint: 1812.01892},
}

@article{li_statistical_2003,
	title = {the {Statistical} {Associating} {Fluid} {Theory} {Equation} of {State}},
	author = {Li, Xiao-sen and Englezos, Peter},
	year = {2003},
	note = {ISBN: 1604822600},
	pages = {4953--4961},
}

@article{tihic_application_2009,
	title = {Application of {sPC}-{SAFT} and group contribution {sPC}-{SAFT} to polymer systems-{Capabilities} and limitations},
	volume = {281},
	issn = {03783812},
	doi = {10.1016/j.fluid.2009.04.002},
	abstract = {A group contribution (GC) version of the simplified Perturbed-Chain Statistical Associating Fluid Theory (sPC-SAFT) Equation of State is proposed in a previous work [A. Tihic, G.M. Kontogeorgis, N. von Solms, M.L. Michelsen, L. Constantinou, Ind. Eng. Chem. Res. 47 (2008) 5092-5101]. The reported predictive capability of the model demonstrates satisfactory description of the fluid behaviour of several polymer systems, including both vapour-liquid equilibria and liquid-liquid equilibria. This work continues the systematic study on phase behaviour of polymer systems with the two versions of the sPC-SAFT model, with and without GC. The reported results contribute to a better understanding of the applicability of the sPC-SAFT model to binary polymer mixtures, and identify both models as good predictive tools for several industrial applications. Limitations are also identified and discussed. © 2009 Elsevier B.V. All rights reserved.},
	number = {1},
	journal = {Fluid Phase Equilib.},
	author = {Tihic, Amra and von Solms, Nicolas and Michelsen, Michael L. and Kontogeorgis, Georgios M. and Constantinou, Leonidas},
	year = {2009},
	keywords = {Equation of State, PC-SAFT, Phase equilibria, Polymers},
	pages = {70--77},
}

@article{haslam_expanding_2020,
	title = {Expanding the {Applications} of the {SAFT}-γ{Mie} {Group}-{Contribution} {Equation} of {State}: {Prediction} of {Thermodynamic} {Properties} and {Phase} {Behavior} of {Mixtures}},
	volume = {65},
	issn = {15205134},
	doi = {10.1021/acs.jced.0c00746},
	abstract = {We present the latest developments in thermodynamic modeling using the SAFT-γMie group-contribution equation of state. The group database is updated, featuring now 58 groups; this expanded database incorporates new parameters for interactions between both like and unlike groups. This provides the capability to treat mixtures including alcohols, ethers, ketones, carboxylic acids, and acetates, amines, aromatic and cyclic compounds, electrolytes, inorganic acids, and some common solvents, such as water and acetone. A discussion is provided relating to the assignment of the groups, including some secondary groups that are introduced for multifunctional molecules to capture the influence of molecular polarization effects on the thermodynamic properties. Performance of the SAFT-γMie approach is illustrated for a wide variety of systems, highlighting its use in describing solid-liquid as well as vapor-liquid and liquid-liquid equilibria.},
	number = {12},
	journal = {J. Chem. Eng. Data},
	author = {Haslam, Andrew J. and González-Pérez, Alfonso and Di Lecce, Silvia and Khalit, Siti H. and Perdomo, Felipe A. and Kournopoulos, Spiros and Kohns, Maximilian and Lindeboom, Tom and Wehbe, Malak and Febra, Sara and Jackson, George and Adjiman, Claire S. and Galindo, Amparo},
	year = {2020},
	pages = {5862--5890},
}

@article{rehner_application_2021,
	title = {Application of {Generalized} ({Hyper}-) {Dual} {Numbers} in {Equation} of {State} {Modeling}},
	volume = {3},
	issn = {2673-2718},
	url = {https://www.frontiersin.org/articles/10.3389/fceng.2021.758090/full},
	doi = {10.3389/fceng.2021.758090},
	abstract = {The calculation of derivatives is ubiquitous in science and engineering. In thermodynamics, in particular, state properties can be expressed as derivatives of thermodynamic potentials. The manual differentiation of complex models can be tedious and error-prone. In this work, we revisit dual and hyper-dual numbers for the calculation of exact derivatives and show generalizations to higher order derivatives and derivatives with respect to vector quantities. The methods described in this paper are accompanied by an open source Rust implementation with Python bindings. Applications of the generalized (hyper-) dual numbers are given in the context of equation of state modeling and the calculation of critical points.},
	journal = {Front. Chem. Eng.},
	author = {Rehner, Philipp and Bauer, Gernot},
	month = oct,
	year = {2021},
}

@article{lemmon_thermodynamic_2009,
	title = {Thermodynamic properties of propane. {III}. {A} reference equation of state for temperatures from the melting line to 650 {K} and pressures up to 1000 {MPa}},
	volume = {54},
	issn = {00219568},
	doi = {10.1021/je900217v},
	abstract = {An equation of state is presented for the thermodynamic properties of propane that is valid for temperatures from the triple point temperature (85.525 K) to 650 K and for pressures up to 1000 MPa. The formulation can be used for the calculation of all thermodynamic properties, including density, heat capacity, speed of sound, energy, and saturation properties. Comparisons to available experimental data are given that establish the accuracy of calculated properties. The approximate uncertainties of properties calculated with the new equation are 0.01 \% to 0.03 \% in density below 350 K, 0.5 \% in heat capacities, 0.03 \% in the speed of sound between (260 and 420) K, and 0.02 \% in vapor pressure above 180 K. Deviations in the critical region are higher for all properties except vapor pressure. © 2009 American Chemical Society.},
	number = {12},
	journal = {J. Chem. Eng. Data},
	author = {Lemmon, Eric W. and McLinden, Mark O. and Wagner, Wolfgang},
	year = {2009},
	pages = {3141--3180},
}

@inproceedings{van_der_waals_equation_1910,
	title = {The {Equation} of {State} for {Gases} and {Liquids}},
	booktitle = {Nobel {Lecture}},
	author = {van der Waals, Johannes Diderik},
	year = {1910},
}

@misc{bell_thermo_nodate,
	title = {Thermo: {Chemical} properties component of {Chemical} {Engineering} {Design} {Library} ({ChEDL})},
	url = {https://github.com/CalebBell/thermo},
	urldate = {2022-03-15},
	author = {Bell, Caleb and {Contributors}},
}

@article{reamer_phase_1962,
	title = {Phase {Equilibria} in {Hydrocarbon} {Systems}. {Volumetric} and {Phase} {Behavior} of the {Ethane}-n-{Decane} {System}.},
	volume = {7},
	issn = {0021-9568},
	url = {https://pubs.acs.org/doi/abs/10.1021/je60013a001},
	doi = {10.1021/je60013a001},
	number = {2},
	journal = {J. Chem. Eng. Data},
	author = {Reamer, H. H. and Sage, B. H.},
	month = apr,
	year = {1962},
	pages = {161--168},
}

@book{michelsen_thermodynamic_2007,
	address = {Holte},
	edition = {2nd},
	title = {Thermodynamic {Modelling}: {Fundamentals} and {Computational} {Aspects}},
	isbn = {87-989961-3-4},
	url = {http://www.tie-tech.com/products/publications/more.php?id=32_0_1_0_M13},
	abstract = {With this book the authors provide a solid framework for developing efficient and robust algorithms for calculation of phase equilibrium of non-ideal mixtures as related to the design and operation of complex processes in the chemical and petroleum industry. Starting from classical thermodynamics, the reader is introduced to the various steps involved in calculating thermodynamic properties and their implication in state of the art phase equilibrium calculation methods, all in a clear and well organized succession. The material presented in this book is suitable for advanced graduate-level courses. It will also be an essential reference in the industry for scientific and engineering development of efficient computational tools for multicomponent multiphase mixtures.},
	publisher = {Tie-Line Publications},
	author = {Michelsen, ML and Mollerup, J},
	year = {2007},
}

@article{kolafa_lennard-jones_1994,
	title = {The {Lennard}-{Jones} fluid: an accurate analytic and theoretically-based equation of state},
	volume = {100},
	issn = {03783812},
	doi = {10.1016/0378-3812(94)80001-4},
	abstract = {A new analytic equation of state for the Lennard-Jones fluid is proposed. The equation is based on a perturbed virial expansion with a theoretically defined temperature-dependent reference hard sphere term. The expansion is written for the Helmholtz free energy which guarantees the thermodynamic consistency of the pressure and internal energy. The equation covers much wider range of temperatures (up to seven times the critical temperature) than existing equations and is significantly more accurate and has less parameters than the best equation available to date, the modified Benedict-Webb-Rubin equation due to Johnson, Zollweg, and Gubbins (1993, Mol. Phys. 78: 591-618). As a side-product, highly accurate explicit analytic correlations of the hard sphere diameters, as given by both the hybrid Barker-Henderson and Weeks-Chandler-Andersen theories, have been obtained. Computer simulation data to be regressed by the equation have been compiled from several sources and critically assessed. It has been shown that many literature data for state points with a large compressibility are subject to large systematic finite-size errors. Additional simulations on a series of systems of different sizes have been therefore performed to facilitate the extrapolation to the thermodynamic limit in the region close to the critical point. © 1994.},
	number = {C},
	journal = {Fluid Phase Equilib.},
	author = {Kolafa, Jiří and Nezbeda, Ivo},
	year = {1994},
	keywords = {Lennard-Jones fluid, computer simulation, equation of state, molecular-thermodynamic reference, perturbed hard spheres, perturbed virial expansion, theory},
	pages = {1--34},
}

@misc{noauthor_aspen_2016,
	title = {Aspen {Plus}},
	url = {https://www.aspentech.com/en/%0Aproducts/engineering/aspen-plus},
	urldate = {2022-03-15},
	publisher = {AspenTech},
	year = {2016},
}

@article{revels_forward-mode_2016,
	title = {Forward-{Mode} {Automatic} {Differentiation} in {Julia}},
	url = {http://arxiv.org/abs/1607.07892},
	abstract = {We present ForwardDiff, a Julia package for forward-mode automatic differentiation (AD) featuring performance competitive with low-level languages like C++. Unlike recently developed AD tools in other popular high-level languages such as Python and MATLAB, ForwardDiff takes advantage of just-in-time (JIT) compilation to transparently recompile AD-unaware user code, enabling efficient support for higher-order differentiation and differentiation using custom number types (including complex numbers). For gradient and Jacobian calculations, ForwardDiff provides a variant of vector-forward mode that avoids expensive heap allocation and makes better use of memory bandwidth than traditional vector mode. In our numerical experiments, we demonstrate that for nontrivially large dimensions, ForwardDiff's gradient computations can be faster than a reverse-mode implementation from the Python-based autograd package. We also illustrate how ForwardDiff is used effectively within JuMP, a modeling language for optimization. According to our usage statistics, 41 unique repositories on GitHub depend on ForwardDiff, with users from diverse fields such as astronomy, optimization, finite element analysis, and statistics. This document is an extended abstract that has been accepted for presentation at the AD2016 7th International Conference on Algorithmic Differentiation.},
	journal = {arXiv:1607.07892},
	author = {Revels, Jarrett and Lubin, Miles and Papamarkou, Theodore},
	month = jul,
	year = {2016},
	note = {\_eprint: 1607.07892},
}

@article{fu_simplified_1995,
	title = {A {Simplified} {SAFT} {Equation} of {State} for {Associating} {Compounds} and {Mixtures}},
	volume = {34},
	issn = {15205045},
	doi = {10.1021/ie00044a042},
	abstract = {A simplified statistical associating fluid theory (SAFT) equation of state is developed for associating and nonassociating compounds. The new equation of state has the same number of adjustable parameters as the original SAFT equation, but is simpler. For pure compounds, this equation of state can correlate the vapor pressure and liquid density with errors equal to those of the original SAFT equation. Both self-associating and cross-associating binary mixtures were used to test the simplified SAFT equation of state. With a single binary adjustable parameter, the new equation results in better correlations of vapor-liquid equilibria than the original SAFT equation for most mixtures. However, for some mixtures, both the original and simplified SAFT equations of state fail to provide a satisfactory description. The optimized binary parameter of the simplified SAFT equation of state is found to be linearly dependent on temperature for each mixture. Consequently, the binary parameter computed from several data sets can be used to accurately predict the vapor-liquid equilibrium at temperatures other than those for which experimental data are available. © 1995, American Chemical Society. All rights reserved.},
	number = {5},
	journal = {Ind. Eng. Chem. Res.},
	author = {Fu, Yuan Hao and Sandler, Stanley I.},
	year = {1995},
	pages = {1897--1909},
}

@article{walker_ab_nodate,
	title = {Ab initio development of generalized {Lennard}-{Jones} ({Mie}) force fields for predictions of thermodynamic properties in advanced molecular-based {SAFT} equations of state},
	journal = {J. Chem. Phys. (accepted)},
	author = {Walker, Pierre J. and Zhao, Tianpu and Haslam, Andrew J. and Jackson, George},
}

@article{fredenslund_computerized_1977,
	title = {Computerized {Design} of {Multicomponent} {Distillation} {Columns} {Using} the {UNIFAC} {Group} {Contribution} {Method} for {Calculation} of {Activity} {Coefficients}},
	volume = {16},
	issn = {01964305},
	doi = {10.1021/i260064a004},
	abstract = {The UNIFAC group-contribution method for estimating activity coefficients provides the process engineer with a rapid and reliable method for predicting equilibrium conditions required in distillation-column design. © 1977, American Chemical Society. All rights reserved.},
	number = {4},
	journal = {Ind. Eng. Chem. Process Des. Dev.},
	author = {Fredenslund, Aage and Gmehling, Jürgen and Michelsen, Michael L. and Rasmussen, Peter and Prausnitz, John M.},
	year = {1977},
	pages = {450--462},
}

@article{boukouvalas_prediction_1994,
	title = {Prediction of vapor-liquid equilibrium with the {LCVM} model: a linear combination of the {Vidal} and {Michelsen} mixing rules coupled with the original {UNIF}},
	volume = {92},
	issn = {03783812},
	url = {https://linkinghub.elsevier.com/retrieve/pii/037838129480043X},
	doi = {10.1016/0378-3812(94)80043-X},
	journal = {Fluid Phase Equilib.},
	author = {Boukouvalas, C. and Spiliotis, N. and Coutsikos, P. and Tzouvaras, N. and Tassios, D.},
	month = jan,
	year = {1994},
	pages = {75--106},
}

@article{kontogeorgis_multicomponent_1999,
	title = {Multicomponent phase equilibrium calculations for water-methanol-alkane mixtures},
	volume = {158-160},
	issn = {03783812},
	doi = {10.1016/s0378-3812(99)00060-6},
	abstract = {Prediction of phase equilibrium for multicomponent systems containing associating compounds (e.g., water and alcohols) is essential in a number of engineering applications (e.g., environmental technology, gas hydrate inhibition) and at the same time represents one of the most stringent tests for a thermodynamic model. Conventional models (e.g., cubic equations of state and excess Gibbs free energy models) provide rapid and\_ often reliable estimates of phase equilibrium in many cases but extension to multicomponent systems, especially those containing water is often troublesome. On the other hand, novel association equations of state perform considerably better but are slower compared to conventional models. Furthermore, the extension of several of them to cross-associating systems (e.g., water-alcohols) exhibits problems. In this work, the performance of two well-known conventional models (SRK and NRTL) is compared for multicomponent systems to a recently proposed association equation of state both in terms of accuracy of predictions and timing. The proposed model incorporates the Wertheim chemical association theory (employed previously in models such as SAFT) and the SRK equation. The model is applied in this work to multicomponent systems in such a way that the inclusion of the Wertheim theory does not give execution times much higher than conventional models. The model yields very satisfactory predictions of multicomponent equilibria for aqueous (both vapor-liquid and liquid-liquid equilibria) systems containing methanol, gases and hydrocarbons, which are moreover, as will be demonstrated in this work, considerably better compared to SRK and NRTL. © 1999 Elsevier Science B.V. All rights reserved.},
	journal = {Fluid Phase Equilib.},
	author = {Kontogeorgis, Georgios M. and Yakoumis, Iakovos V. and Meijer, Henk and Hendriks, Eric and Moorwood, Tony},
	year = {1999},
	keywords = {Alcohol, Association, Equation of state, Liquid-liquid equilibria, Multicomponent, Water},
	pages = {201--209},
}

@phdthesis{jorstad_equation_1993,
	type = {{PhD} {Thesis}},
	title = {Equation of {State} for {Hydrocarbons}},
	school = {University of Trondheim},
	author = {Jørstad, Oddvar},
	year = {1993},
	note = {Issue: December},
}

@article{bell_implementing_nodate,
	title = {Implementing an {Equation} of {State} {Without} {Derivatives}: teqp},
	journal = {Ind. Eng. Chem. Res. (submitted)},
	author = {Bell, Ian H. and Deiters, Ulrich K. and Leal, Allan M. M.},
}

@misc{noauthor_computer_nodate,
	title = {Computer {Calculations} for {Multicomponent} {Vapor}-{Liquid} and {Liquid}-{Liquid} {Equilibria} by {Prausnitz}, {J}. {Anderson}, {T}. {Grens}, {E}. {Eckert}, {C}. {Hsieh}, {R}. {OConnell}, {J}. (z-lib.org) (1).pdf},
}

@article{ott_excess_1993,
	title = {Excess volumes for (ethanol+water) at the temperatures (298.15 and 348.15) {K} and pressures (0.4, 5, and 15) {MPa} and at the temperature 323.15 {K} and pressures (5 and 15) {MPa}},
	volume = {25},
	issn = {00219614},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0021961483710293},
	doi = {10.1006/jcht.1993.1029},
	number = {2},
	journal = {J. Chem. Thermodyn.},
	author = {Ott, J.B. and Sipowska, J.T. and Gruszkiewicz, M.S. and Woolley, A.T.},
	month = feb,
	year = {1993},
	pages = {307--318},
}

@article{soave_equilibrium_1972,
	title = {Equilibrium constants from a modified {Redlich}-{Kwong} equation of state},
	volume = {27},
	issn = {00092509},
	url = {https://linkinghub.elsevier.com/retrieve/pii/0009250972800964},
	doi = {10.1016/0009-2509(72)80096-4},
	abstract = {A modified Redlich-Kwong equation of state is proposed. Vapor pressures of pure compounds can be closely reproduced by assuming the parameter a in the original equation to be temperature-dependent. With the introduction of the acentric factor as a third parameter, a generalized correlation for the modified parameter can be derived. It applies to all nonpolar compounds. With the application of the original generalized mixing rules, the proposed equation can be extended successfully to multicomponent-VLE calculations, for mixtures of nonpolar substances, with the exclusion of carbon dioxide. Less accurate results are obtained for hydrogen-containing mixtures. © 1972.},
	number = {6},
	journal = {Chem. Eng. Sci.},
	author = {Soave, Giorgio},
	month = jun,
	year = {1972},
	note = {Publisher: Pergamon Press},
	pages = {1197--1203},
}

@article{jones_critical_1930,
	title = {The critical solution temperature of the system methyl alcohol–cyclohexane as a means of detecting and estimating water in methyl alcohol},
	issn = {0368-1769},
	url = {http://xlink.rsc.org/?DOI=JR9300001316},
	doi = {10.1039/JR9300001316},
	journal = {J. Chem. Soc.},
	author = {Jones, David Charles and Amstell, Simon},
	year = {1930},
	pages = {1316--1323},
}

@article{karl_johnson_equation_1994,
	title = {Equation of state for {Leonard}-{Jones} chains},
	volume = {98},
	issn = {00223654},
	doi = {10.1021/j100076a028},
	abstract = {An equation of state for chains composed of tangent, freely jointed Lennard-Jones spheres is presented. The equation is based on a statistical mechanical description of polymerization that is based on Wertheim's theory of associating fluids. The Helmholtz free energy of a fluid of chains is expressed as the contribution from a monomeric reference fluid, which in this case is a fluid of Lennard-Jones spheres, plus a contribution due to bonding. The bonding term depends upon the number of monomers in a chain and the cavity correlation function of the reference fluid. We have performed molecular dynamics simulations of chain fluids composed of 2, 4, 12, 16, 18, 20, 50, and 100 spheres over the entire fluid density range at several temperatures and compared the results to the theory. The equation of state is found to be in good agreement with the simulation results, predicting pressures that are slightly too large overall. Internal energies are predicted well, except in the low-density region where the equation of state does not give the correct limiting value due to neglect of chain self-interaction. © 1994 American Chemical Society.},
	number = {25},
	journal = {J. Phys. Chem.},
	author = {Karl Johnson, J. and Müller, Erich A. and Gubbins, Keith E.},
	year = {1994},
	pages = {6413--6419},
}

@article{michelsen_modified_1990,
	title = {A modified {Huron}-{Vidal} mixing rule for cubic equations of state},
	volume = {60},
	issn = {03783812},
	url = {https://linkinghub.elsevier.com/retrieve/pii/037838129085053D},
	doi = {10.1016/0378-3812(90)85053-D},
	number = {1-2},
	journal = {Fluid Phase Equilib.},
	author = {Michelsen, Michael L.},
	month = oct,
	year = {1990},
	pages = {213--219},
}

@article{topliss_computational_1988,
	title = {Computational aspects of a non-cubic equation of state for phase-equilibrium calculations. {Effect} of density-dependent mixing rules},
	volume = {12},
	issn = {00981354},
	url = {https://linkinghub.elsevier.com/retrieve/pii/0098135488850671},
	doi = {10.1016/0098-1354(88)85067-1},
	number = {5},
	journal = {Computers \& Chemical Engineering},
	author = {Topliss, Robert J. and Dimitrelis, Dimitrios and Prausnitz, John M.},
	month = may,
	year = {1988},
	pages = {483--489},
}

@article{llovell_prediction_2006,
	title = {Prediction of thermodynamic derivative properties of pure fluids through the soft-{SAFT} equation of state},
	volume = {110},
	issn = {15206106},
	doi = {10.1021/jp0608022},
	abstract = {We present in this work the application of the soft-SAFT equation of state (EoS) to the calculation of some main derivative properties, including heat capacities, reduced bulk modulus, Joule-Thomson coefficient, and speed of sound. Calculations have been performed analytically through the derivation of a primary thermodynamic potential function. The application to the n-alkanes, n-alkenes, and 1-alkanols families has been done in a semipredictive manner, with the molecular parameters of the equation obtained from previous fitting to vapor-liquid equilibrium data of the same compounds. The equation is able to capture the typical extrema isothermal derivative properties exhibit with respect to density, providing quantitative agreement with experimental (or correlation) data in some cases. Results in the vicinity of the critical point are improved by adding a crossover treatment to take into account the long-range fluctuations present in this region. By taking advantage of the molecular nature of the equation, we have been able to separate and quantify the different contributions (reference fluid, chain, and association) to the total derivative properties. The association plays a predominant role in energetic properties, such as the heat capacities, while there is a competition between association and chain length as the chain length of the compound increases for volumetric properties, such as the isothermal compressibility. These results act in favor of the molecular-based equations, like soft-SAFT, as predictive tools for several applications. © 2006 American Chemical Society.},
	number = {23},
	journal = {J. Phys. Chem. B},
	author = {Llovell, Fèlix and Vega, Lourdes F.},
	year = {2006},
	pages = {11427--11437},
}

@article{deiters_precise_2021,
	title = {Precise {Numerical} {Differentiation} of {Thermodynamic} {Functions} with {Multicomplex} {Variables}},
	volume = {126},
	issn = {2165-7254},
	url = {https://nvlpubs.nist.gov/nistpubs/jres/126/jres.126.033.pdf},
	doi = {10.6028/jres.126.033},
	abstract = {The multicomplex finite-step method for numerical differentiation is an extension of the popular Squire–Trapp method, which uses complex arithmetics to compute first-order derivatives with almost machine precision. In contrast to this, the multicomplex method can be applied to higher-order derivatives. Furthermore, it can be applied to functions of more than one variable and obtain mixed derivatives. It is possible to compute various derivatives at the same time. This work demonstrates the numerical differentiation with multicomplex variables for some thermodynamic problems. The method can be easily implemented into existing computer programs, applied to equations of state of arbitrary complexity, and achieves almost machine precision for the derivatives. Alternative methods based on complex integration are discussed, too.},
	journal = {Journal of Research of the National Institute of Standards and Technology},
	author = {Deiters, Ulrich K. and Bell, Ian H.},
	month = nov,
	year = {2021},
	pages = {126033},
}

@book{wagner_international_2008,
	title = {International {Steam} {Tables}: {Properties} of {Water} and {Steam} {Based} on the {Industrial} {Formulation} of {IAPWS}-{IF97}},
	isbn = {978-3-540-21419-9},
	publisher = {Springer},
	author = {Wagner, Wolfgang and Kretzschmar, Hans-Joachim},
	editor = {Edition, Second},
	year = {2008},
}

@inproceedings{boston_proceedings_1980,
	address = {West Berlin},
	title = {Proceedings of the 2nd {International} {Conference} on {Phase} {Equilibria} and {Fluid} {Properties} in the {Chemical} {Process} {Industries}},
	author = {Boston, P.M. and Mathias, P.M.},
	year = {1980},
	pages = {823--849},
}

@article{yakoumis_vapor-liquid_1997,
	title = {Vapor-liquid equilibria for alcohol/hydrocarbon systems using the {CPA} {Equation} of {State}},
	volume = {130},
	issn = {03783812},
	doi = {10.1016/s0378-3812(96)03200-1},
	abstract = {The recently developed Cubic-Plus-Association Equation of State (CPA EoS) is extended in this study to binary systems containing one associating compound (alcohol) and an inert one (hydrocarbon). CPA combines the Soave-Redlich-Kwong (SRK) equation of state for the physical part with an association term based on perturbation theory. The classical van der Waals one-fluid mixing rules are used for the attractive and co-volume parameters, α and b, while the extension of the association term to mixtures is rigorous and does not require any mixing rules. Excellent correlation of Vapor-Liquid Equilibria (VLE) is obtained using a small value for the interaction parameter (kij) in the attractive term of the physical part of the equation of state even when it is temperature-independent. CPA yields much better results than SRK and its performance is similar to that of other association models, like the Anderko EoS. and the more complex SAFT and Simplified SAFT EoS. © 1997 Elsevier Science B.V.},
	number = {1-2},
	journal = {Fluid Phase Equilib.},
	author = {Yakoumis, Iakovos V. and Kontogeorgis, Georgios M. and Voutsas, Epaminondas C. and Tassios, Dimitrios P.},
	year = {1997},
	keywords = {Alcohols, Application, Association, Hydrocarbons, Vapor-liquid equilibria},
	pages = {31--47},
}

@article{hsieh_improvements_2010,
	title = {Improvements of {COSMO}-{SAC} for vapor-liquid and liquid-liquid equilibrium predictions},
	volume = {297},
	issn = {03783812},
	doi = {10.1016/j.fluid.2010.06.011},
	abstract = {The COSMO-SAC model has been revised for a better description of the nonideality of liquid mixtures, and thus more accurate predictions of both vapor-liquid equilibrium (VLE) and liquid-liquid equilibrium (LLE). Two major modifications are introduced. First, the electrostatic interaction parameter is made temperature-dependent, which is important in LLE predictions for non-hydrogen-bonding systems. Second, the variation in the strength of hydrogen-bonding interactions involving different types of functional groups is treated using separate sigma-profiles. The overall RMS error in LLE predictions of 278 binary mixtures (4281 data points) from the new model is 0.1047, which is 30\% lower than that from the original COSMO-SAC (0.1446), 10\% lower from that of UNIFAC-LLE (0.1161), and comparable to that from the modified UNIFAC model (0.1048). The accuracy in VLE predictions is also improved. The average deviation in total pressure at a fixed liquid composition is 6.54\% and the overall average deviation in vapor phase composition is 2.57\% for 1338 binary mixtures, compared to 7.25\% and 2.83\% from the original model. © 2010 Elsevier B.V.},
	number = {1},
	journal = {Fluid Phase Equilib.},
	author = {Hsieh, Chieh Ming and Sandler, Stanley I. and Lin, Shiang Tai},
	year = {2010},
	keywords = {COSMO-SAC, Liquid-liquid equilibria, Prediction, Solvation, Vapor-liquid equilibria},
	pages = {90--97},
}

@misc{keller_unitfuljl_2022,
	title = {Unitful.jl},
	url = {https://github.com/PainterQubits/Unitful.jl},
	urldate = {2022-03-15},
	author = {Keller, Andrew and {Contributors}},
	year = {2022},
}

@article{holderbaum_psrk_1991,
	title = {{PSRK}: {A} {Group} {Contribution} {Equation} of {State} {Based} on {UNIFAC}},
	volume = {70},
	issn = {03783812},
	doi = {10.1016/0378-3812(91)85038-V},
	abstract = {A group contribution equation of state called PSRK (Predictive Soave-Redlich-Kwong) which is based on the Soave-Redlich-Kwong equation (Soave, 1972) has been developed. It uses the UNIFAC method to calculate the mixture parameter a and includes all already existing UNIFAC parameters. This concept makes use of recent developments by Michelsen (1990b) and has the main advantage, that vapor-uquid-equilibria (VLB) can be predicted for a large number of systems without introducing new model parameters that must be fitted to experimental VLB-data. The PSRK equation of state can be used for VLB-predictions over a much larger temperature and pressure range than the UNIFAC γ-ϕsymbol-approach and is easily extended to mixtures containing supercritical compounds. Additional PSRK parameters, which allow the calculation of gas/gas and gas/alkane phase equilibria, are given in this paper. In addition to those mixtures covered by UNIFAC, phase equilibrium calculations may also include gases like CH4 C2H6, C3H6, c4H10, CO2, N2, H2 and CO. © 1991.},
	number = {2-3},
	journal = {Fluid Phase Equilib.},
	author = {Holderbaum, T. and Gmehling, J.},
	year = {1991},
	keywords = {PSRK, UNIFAC, group contribution equation of state, vapor liquid equilibria},
	pages = {251--265},
}

@article{diedrichs_prediction_2006,
	title = {Prediction of liquid heat capacities by the group contribution equation of state {VTPR}},
	volume = {248},
	issn = {03783812},
	doi = {10.1016/j.fluid.2006.07.009},
	abstract = {Liquid heat capacities of 33 pure compounds have been calculated using the group contribution equation of state VTPR (volume translated Peng-Robinson). Since the predicted heat capacities were not always in good agreement with the experimental data, systematic investigations were performed to improve the situation. Distinct improvements were obtained by fitting the Twu-α-parameters simultaneously to vapor pressure, enthalpy of vaporization and heat capacity data. © 2006 Elsevier B.V. All rights reserved.},
	number = {1},
	journal = {Fluid Phase Equilib.},
	author = {Diedrichs, Anja and Rarey, Jürgen and Gmehling, Jürgen},
	year = {2006},
	keywords = {Heat capacity, Prediction, VTPR, α-Function},
	pages = {56--69},
}

@book{baird_vapor_2019,
	title = {Vapor {Pressures}, {Densities}, and {PC}-{SAFT} {Parameters} for 11 {Bio}-compounds},
	volume = {40},
	isbn = {0-12-345678-9},
	url = {https://doi.org/10.1007/s10765-019-2570-9},
	abstract = {One major sustainable development goal is to produce chemicals and fuels from renewable resources, such as biomass, rather than from fossil fuels. A key part of this development is data on the properties of chemicals that appear in this bio-based supply chain. Many of the chemicals have yet to be studied thoroughly, and data on their properties is lacking. Here, we present new experimental data on the properties of 11 bio-compounds, along with PC-SAFT parameters for modeling their properties. The measured data includes vapor pressures, compressed densities, and refractive indexes. The 11 bio-compounds are tetrahydrofuran, 2-pentanone, furfural, 2-methoxy-4-methylphenol, 2-methylfuran, dihydrolevoglucosenone, cyclopentyl methyl ether, 2-sec-butylphenol, levoglucosenone, γ-valerolactone, and 2,6-dimethoxyphenol.},
	number = {11},
	publisher = {Springer US},
	author = {Baird, Zachariah Steven and Uusi-Kyyny, Petri and Pokki, Juha Pekka and Pedegert, Emilie and Alopaeus, Ville},
	year = {2019},
	doi = {10.1007/s10765-019-2570-9},
	note = {ISSN: 15729567
Publication Title: Int. J. Thermodyn.},
	keywords = {Bio-compounds, Density, PC-SAFT, Thermodynamic properties, Vapor pressure},
}

@article{horstmann_experimental_2000,
	title = {Experimental determination of the critical line for (carbon dioxide + ethane) and calculation of various thermodynamic properties for (carbon dioxide +n-alkane) using the {PSRK} model},
	volume = {32},
	issn = {00219614},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0021961400906116},
	doi = {10.1006/jcht.2000.0611},
	number = {4},
	journal = {J. Chem. Thermodyn.},
	author = {Horstmann, Sven and Fischer, Kai and Gmehling, Jürgen and Kolář, Petr},
	month = apr,
	year = {2000},
	pages = {451--464},
}

@article{taylor_molecular_1980,
	title = {Molecular {Physics}: {An} {International} {Journal} at the {Interface} {Between} {Chemistry} and {Physics}},
	number = {January 2014},
	author = {Taylor, Publisher},
	year = {1980},
	pages = {37--41},
}

@article{k_mogensen_optim_2018,
	title = {Optim: {A} mathematical optimization package for {Julia}},
	volume = {3},
	issn = {2475-9066},
	url = {http://joss.theoj.org/papers/10.21105/joss.00615},
	doi = {10.21105/joss.00615},
	number = {24},
	journal = {Journal of Open Source Software},
	author = {K Mogensen, Patrick and N Riseth, Asbjørn},
	month = apr,
	year = {2018},
	pages = {615},
}

@article{langenbach_cross-association_2012,
	title = {Cross-association of multi-component systems},
	volume = {110},
	issn = {0026-8976},
	url = {http://www.tandfonline.com/doi/abs/10.1080/00268976.2012.668963},
	doi = {10.1080/00268976.2012.668963},
	number = {11-12},
	journal = {Molecular Physics},
	author = {Langenbach, K. and Enders, S.},
	month = jun,
	year = {2012},
	pages = {1249--1260},
}

@article{thol_equation_2016,
	title = {Equation of {State} for the {Lennard}-{Jones} {Fluid}},
	volume = {45},
	issn = {0047-2689},
	url = {http://aip.scitation.org/doi/10.1063/1.4945000},
	doi = {10.1063/1.4945000},
	number = {2},
	journal = {Journal of Physical and Chemical Reference Data},
	author = {Thol, Monika and Rutkai, Gabor and Köster, Andreas and Lustig, Rolf and Span, Roland and Vrabec, Jadran},
	month = jun,
	year = {2016},
	pages = {023101},
}

@article{barr-david_vapor-liquid_1959,
	title = {Vapor-{Liquid} {Equilibrium} at {High} {Pressures}. {The} {Systems} {Ethanol}-{Water} and 2-{Propanol}-{Water}.},
	volume = {4},
	issn = {0021-9568},
	url = {https://pubs.acs.org/doi/abs/10.1021/je60002a003},
	doi = {10.1021/je60002a003},
	number = {2},
	journal = {J. Chem. Eng. Data},
	author = {Barr-David, Frank and Dodge, B. F.},
	month = apr,
	year = {1959},
	pages = {107--121},
}

@article{van_der_waals_molekulartheorie_1890,
	title = {Molekulartheorie eines {Körpers}, der aus zwei verschiedenen {Stoffen} besteht},
	volume = {5U},
	issn = {2196-7156},
	url = {https://www.degruyter.com/document/doi/10.1515/zpch-1890-0514/html},
	doi = {10.1515/zpch-1890-0514},
	number = {1},
	journal = {Zeitschrift für Physikalische Chemie},
	author = {van der Waals, J. D.},
	month = feb,
	year = {1890},
	pages = {133--173},
}

@article{rachford_procedure_1952,
	title = {Procedure for {Use} of {Electronic} {Digital} {Computers} in {Calculating} {Flash} {Vaporization} {Hydrocarbon} {Equilibrium}},
	volume = {4},
	issn = {0149-2136},
	url = {https://onepetro.org/JPT/article/4/10/19/162083/Procedure-for-Use-of-Electronic-Digital-Computers},
	doi = {10.2118/952327-G},
	number = {10},
	journal = {J. Pet. Technol.},
	author = {Rachford, H.H. and Rice, J.D.},
	month = oct,
	year = {1952},
	pages = {19--3},
}

@article{twu_new_1992,
	title = {A new cubic equation of state},
	volume = {75},
	issn = {03783812},
	url = {https://linkinghub.elsevier.com/retrieve/pii/037838129287007A},
	doi = {10.1016/0378-3812(92)87007-A},
	journal = {Fluid Phase Equilib.},
	author = {Twu, Chorng H. and Coon, John E. and Cunningham, John R.},
	month = aug,
	year = {1992},
	pages = {65--79},
}

@misc{rehner_feos_2022,
	title = {{FeOs} - {A} {Framework} for {Equations} of {State} and {Classical} {Density} {Functional} {Theory}},
	url = {https://github.com/feos-org/feos},
	urldate = {2022-03-15},
	author = {Rehner, Philipp and Bauer, Gernot},
	year = {2022},
}

@article{lymperiadis_group_2007,
	title = {A group contribution method for associating chain molecules based on the statistical associating fluid theory ({SAFT}- γ)},
	volume = {127},
	issn = {00219606},
	doi = {10.1063/1.2813894},
	abstract = {A predictive group-contribution statistical associating fluid theory (SAFT- γ) is developed by extending the molecular-based SAFT-VR equation of state [A. Gil-Villegas J. Chem. Phys. 106, 4168 (1997)] to treat heteronuclear molecules which are formed from fused segments of different types. Our models are thus a heteronuclear generalization of the standard models used within SAFT, comparable to the optimized potentials for the liquid state OPLS models commonly used in molecular simulation; an advantage of our SAFT- γ over simulation is that an algebraic description for the thermodynamic properties of the model molecules can be developed. In our SAFT- γ approach, each functional group in the molecule is modeled as a united-atom spherical (square-well) segment. The different groups are thus characterized by size (diameter), energy (well depth) and range parameters representing the dispersive interaction, and by shape factor parameters (which denote the extent to which each group contributes to the overall molecular properties). For associating groups a number of bonding sites are included on the segment: in this case the site types, the number of sites of each type, and the appropriate association energy and range parameters also have to be specified. A number of chemical families (n -alkanes, branched alkanes, n -alkylbenzenes, mono- and diunsaturated hydrocarbons, and n -alkan-1-ols) are treated in order to assess the quality of the SAFT- γ description of the vapor-liquid equilibria and to estimate the parameters of various functional groups. The group parameters for the functional groups present in these compounds (C H3, C H2, C H3 CH, ACH, ACC H2, C H2 , CH, and OH) together with the unlike energy parameters between groups of different types are obtained from an optimal description of the pure component phase equilibria. The approach is found to describe accurately the vapor-liquid equilibria with an overall \%AAD of 3.60\% for the vapor pressure and 0.86\% for the saturated liquid density. The fluid phase equilibria of some larger compounds comprising these groups, which are not included in the optimization database and some binary mixtures are examined to confirm the predictive capability of the SAFT- γ approach. A key advantage of our method is that the binary interaction parameters between groups can be estimated directly from an examination of pure components alone. This means that as a first approximation the fluid-phase equilibria of mixtures of compounds comprising the groups considered can be predicted without the need for any adjustment of the binary interaction parameters (which is common in other approaches). The special case of molecular models comprising tangentially bonded (all-atom and united-atom) segments is considered separately; we comment on the adequacy of such models in representing the properties of real molecules. © 2007 American Institute of Physics.},
	number = {23},
	journal = {J. Chem. Phys.},
	author = {Lymperiadis, Alexandros and Adjiman, Claire S. and Galindo, Amparo and Jackson, George},
	year = {2007},
}

@article{redlich_thermodynamics_1949,
	title = {On the {Thermodynamics} of {Solutions}. {V}. {An} {Equation} of {State}. {Fugacities} of {Gaseous} {Solutions}.},
	volume = {44},
	issn = {0009-2665},
	url = {https://pubs.acs.org/doi/abs/10.1021/cr60137a013},
	doi = {10.1021/cr60137a013},
	number = {1},
	journal = {Chem. Rev.},
	author = {Redlich, Otto and Kwong, J. N. S.},
	month = feb,
	year = {1949},
	pages = {233--244},
}

@article{haslam_introduction_2015,
	title = {An {Introduction} to {Statistical} {Thermodynamics} and its {Application} in {Equation}-of-{State} {Modelling} of {Fluids}},
	author = {Haslam, Andrew J},
	year = {2015},
	pages = {1--114},
}

@article{chen_modification_2002,
	title = {Modification of {PSRK} mixing rules and results for vapor-liquid equilibria, enthalpy of mixing and activity coefficients at infinite dilution},
	volume = {200},
	issn = {03783812},
	doi = {10.1016/S0378-3812(02)00048-1},
	abstract = {The predictive Soave-Redlich-Kwong (PSRK) equation of state (EOS) is a well-established method for the prediction of thermodynamic properties required in process simulation. But there are still some problems to be solved, e.g. the reliability for strong asymmetric mixtures of components which are very different in size. The following modifications are introduced in the PSRK mixing rules: the Flory-Huggins term in the mixing rule for the EOS parameter a, and the combinatorial part in the UNIFAC model are skipped simultaneously; a nonlinear mixing rule for the EOS parameter b, instead of the linear mixing rule, is proposed. With these two modifications better results are obtained for vapor-liquid equilibria and activity coefficients at infinite dilution for alkane-alkane systems, specially for asymmetric systems. In order to obtain better results for enthalpy of mixing, temperature-dependent parameters are used. Group interaction parameters have been fitted for several groups, and the results are compared with the Modified UNIFAC (Dortmund), and the PSRK methods. © 2002 Elsevier Science B.V. All rights reserved.},
	number = {2},
	journal = {Fluid Phase Equilib.},
	author = {Chen, Jian and Fischer, Kai and Gmehling, Jürgen},
	year = {2002},
	keywords = {Equation of state, Group contribution, Mixing rule, Theory},
	pages = {411--429},
}

@article{avila_thermodynamic_2002,
	title = {Thermodynamic {Properties} of {Synthetic} {Natural} {Gases}. 1. {Dew}-{Point} {Curves} of {Synthetic} {Natural} {Gases} and {Their} {Mixtures} with {Water} and {Methanol}. {Measurement} and {Correlation}},
	volume = {41},
	issn = {0888-5885},
	url = {https://pubs.acs.org/doi/10.1021/ie0110282},
	doi = {10.1021/ie0110282},
	abstract = {Dew points for two synthetic natural gas (SNG) mixtures between 1.2 × 105 and 81.8 × 105 Pa in the temperature range from 213.6 to 261.4 K, four SNG + water mixtures between 1.1 × 105 and 41.0 × 105 Pa and temperatures from 244.7 to 288.1 K, and four SNG + water + methanol mixtures between 1.1 × 10 5 and 20.7 × 105 Pa and temperatures from 247.6 to 288.6 K were experimentally determined. The experimental results obtained on the multicomponent systems were analyzed in terms of a predictive excess function-equation of state (EF-EOS) method, which reproduced experimental dew point temperature data with absolute average deviation (AAD) between 0.9 and 3. 1 K for the dry systems, from 0.0 to 1.6 K for the systems with water, and from 0.0 to 3.0 K for the systems with water and methanol. The experimental results obtained for synthetic natural gas (SNG) + water mixtures at pressure values higher than 5 × 105 Pa were also compared to a predictive equation of state (EOS) model. It reproduced experimental dew point temperature data within AAD between 1.8 and 5.3 K.},
	number = {15},
	journal = {Ind. Eng. Chem. Res.},
	author = {Avila, S. and Blanco, S. T. and Velasco, I. and Rauzy, E. and Otín, S.},
	month = jul,
	year = {2002},
	pages = {3714--3721},
}

@article{privat_are_2010,
	title = {Are safe results obtained when the {PC}-{SAFT} equation of state is applied to ordinary pure chemicals?},
	volume = {295},
	issn = {03783812},
	doi = {10.1016/j.fluid.2010.03.041},
	abstract = {The PC-SAFT equation of state is a very popular and promising model for fluids that employs a complicated pressure-explicit mathematical function (and can therefore not be solved analytically at a specified pressure and temperature, contrary to classical cubic equations). In this work, we demonstrate that in case of pure fluids, the PC-SAFT equation may exhibit up to five different volume roots whereas cubic equations give at the most three volume roots (and yet, only one or two volume roots have real significance). The consequence of this strongly atypical behaviour is the existence of two different fluid-fluid coexistence lines (the vapour-pressure curve and an additional liquid-liquid equilibrium curve) and two critical points for a same pure component, which is obviously physically inconsistent. In addition to nalkanes, nearly 60 very common pure components (branched alkanes, cycloalkanes, aromatics, esters, gases, and so on) were tested out and without any exception, we can claim that all of them exhibit this undesired behaviour. In addition, such similar phenomena (i.e. existence of more than three volume roots) may also arise with mixtures. From a computational point of view, most of the algorithms used for solving equations of state only search for three roots at the most and are thus likely to be inefficient when an equation of state gives more than three volume roots. To overcome this limitation, a simple procedure allowing to identify all the possible volume roots of an equation of state is proposed. © 2010 Elsevier B.V. All rights reserved.},
	number = {1},
	journal = {Fluid Phase Equilib.},
	author = {Privat, Romain and Gani, Rafiqul and Jaubert, Jean Noël},
	year = {2010},
	keywords = {Alkane, Artefact, Critical point, Density calculation, Equation of state, Inconsistent predictions, Liquid-liquid equilibrium, PC-SAFT, Pure-component parameters, Resolution of an equation of state, SRK, Vapour pressure},
	pages = {76--92},
}

@article{sadeqzadeh_development_2016,
	title = {The development of unlike induced association-site models to study the phase behaviour of aqueous mixtures comprising acetone, alkanes and alkyl carboxylic acids with the {SAFT}-γ {Mie} group contribution methodology},
	volume = {407},
	issn = {03783812},
	url = {http://dx.doi.org/10.1016/j.fluid.2015.07.047},
	doi = {10.1016/j.fluid.2015.07.047},
	abstract = {Providing accurate predictions of the thermodynamic properties of highly polar and hydrogen bonding compounds and their mixtures is challenging from a theoretical perspective. The combination of an equation of state (EoS) based on the statistical associating fluid theory (SAFT) with a group contribution (GC) methodology offers both accuracy and predictive capability for the thermodynamic properties of mixtures. In our current work, the SAFT-γ Mie equation of state is used to capture the underlying complexity of systems in which specific interactions (e.g. hydrogen bonding, dipolar interactions, chemical association) play an important role, by incorporating highly versatile association-site schemes to model mixtures in which unlike induced association interactions occur; this is done by assigning to the functional groups a number of association sites that are inactive in the pure fluid, but become active in certain mixtures. We refer to this type of association mechanism as "unlike induced" association and to the sites involved in this interaction as "unlike induced" association sites. The concept of unlike induced association sites is applied here to develop reliable SAFT-γ Mie group contribution models to describe the properties of acetone, alkyl carboxylic acids, and their mixtures with water and n-alkanes. The parameter table of available SAFT-γ Mie models is expanded to incorporate the corresponding group interaction parameters for acetone, which is treated as a molecular group, the carboxyl group COOH, and their unlike interaction group parameters with water, and the methyl CH3, methanediyl CH2, and methanetriyl CH alkyl groups. In particular, one unlike induced site is used with the acetone model to mediate hydrogen bonding of the acetone oxygen in mixtures containing hydrogen bond donors, and two pairs of unlike induced sites are included on the COOH group to mediate hydrogen bond formation in mixtures of carboxylic acids and hydrogen bond donors. The models developed allow for the successful description of the complex fluid-phase behaviour of the relevant binary and ternary mixtures, including accurate predictions of systems which have not been used to determine the model parameters.},
	journal = {Fluid Phase Equilib.},
	author = {Sadeqzadeh, Majid and Papaioannou, Vasileios and Dufal, Simon and Adjiman, Claire S. and Jackson, George and Galindo, Amparo},
	year = {2016},
	note = {Publisher: Elsevier B.V.},
	keywords = {Acetone, Carboxylic acid, Group contribution, N-Alkane, SAFT-γ Mie, Unlike induced association sites, Water},
	pages = {39--57},
}

@article{rackett_equation_1970,
	title = {Equation of state for saturated liquids},
	volume = {15},
	issn = {0021-9568},
	url = {https://pubs.acs.org/doi/abs/10.1021/je60047a012},
	doi = {10.1021/je60047a012},
	number = {4},
	journal = {J. Chem. Eng. Data},
	author = {Rackett, Harold G.},
	month = oct,
	year = {1970},
	pages = {514--517},
}

@article{souza_measurement_2018,
	title = {Measurement and modelling of the vapor–liquid equilibrium of ({CO2} + {CO}) at temperatures between (218.15 and 302.93) {K} at pressures up to 15 {MPa}},
	volume = {126},
	issn = {00219614},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0021961418303033},
	doi = {10.1016/j.jct.2018.06.022},
	journal = {J. Chem. Thermodyn.},
	author = {Souza, Lorena F.S. and Al Ghafri, Saif Z.S. and Trusler, J.P. Martin},
	month = nov,
	year = {2018},
	pages = {63--73},
}

@article{wong_theoretically_1992,
	title = {A theoretically correct mixing rule for cubic equations of state},
	volume = {38},
	issn = {0001-1541},
	url = {https://onlinelibrary.wiley.com/doi/10.1002/aic.690380505},
	doi = {10.1002/aic.690380505},
	number = {5},
	journal = {AIChE J.},
	author = {Wong, David Shan Hill and Sandler, Stanley I.},
	month = may,
	year = {1992},
	pages = {671--680},
}

@article{ahlers_development_2001,
	title = {Development of an universal group contribution equation of state. {Prediction} of liquid densities for pure compounds with a volume translated {Peng}-{Robinson} equation of state},
	volume = {191},
	issn = {03783812},
	doi = {10.1016/S0378-3812(01)00626-4},
	abstract = {With a view to the development of an universal group contribution equation of state, the Peng-Robinson (PR) equation of state (EOS) has been modified to obtain a better description of saturated liquid densities for the pure compounds. A simple improved volume translation together with a temperature dependent volume correction deliver an accurate representation of this property near and far from the critical point for polar and non-polar substances. The fitted parameters have been generalized as a function of the critical compressibility factor. The results are compared with the results of the original PR and the Soave-Redlich-Kwong (SRK) EOS. Copyright © 2001 Elsevier Science B.V.},
	number = {1-2},
	journal = {Fluid Phase Equilib.},
	author = {Ahlers, Jens and Gmehling, Jürgen},
	year = {2001},
	keywords = {Critical point, Density, Equation of state, Volume translation},
	pages = {177--188},
}

@article{abrams_statistical_1975,
	title = {Statistical thermodynamics of liquid mixtures: {A} new expression for the excess {Gibbs} energy of partly or completely miscible systems},
	volume = {21},
	issn = {15475905},
	doi = {10.1002/aic.690210115},
	abstract = {To obtain a semi‐theoretical equation for the excess Gibbs energy of a liquid mixture, Guggenheim's quasi‐chemical analysis is generalized through introduction of the local area fraction as the primary concentration variable. The resulting universal quasi‐chemical (UNIQUAC) equation uses only two adjustable parameters per binary. Extension to multicomponent systems requires no ternary (or higher) parameters. The UNIQUAC equation gives good representation of both vapor‐liquid and liquid‐liquid equilibria for binary and multicomponent mixtures containing a variety of nonelectrolyte components such as hydrocarbons, ketones, esters, amines, alcohols, nitriles, etc., and water. When well‐defined simplifying assumptions are introduced into the generalized quasi‐chemical treatment, the UNIQUAC equation reduces to any one of several well‐known equations for the excess Gibbs energy, including the Wilson, Margules, van Laar, and NRTL equations. The effects of molecular size and shape are introduced through structural parameters obtained from pure‐component data and through use of Staverman's combinatorial entropy as a boundary condition for athermal mixtures. The UNIQUAC equation, therefore, is applicable also to polymer solutions. Copyright © 1975 American Institute of Chemical Engineers},
	number = {1},
	journal = {AIChE J.},
	author = {Abrams, Denis S. and Prausnitz, John M.},
	year = {1975},
	pages = {116--128},
}

@article{llovell_phase_2007,
	title = {Phase equilibria, critical behavior and derivative properties of selected n-alkane/n-alkane and n-alkane/1-alkanol mixtures by the crossover soft-{SAFT} equation of state},
	volume = {41},
	issn = {08968446},
	doi = {10.1016/j.supflu.2006.10.001},
	abstract = {We present here results from the crossover soft-SAFT equation of state as applied to selected n-alkane/n-alkane and n-alkane/1-alkanol mixtures. The molecular parameters needed to apply the equation to experimental systems were obtained as a function of the molecular weight of the compounds, from published correlations. The fact that the equation takes into account the long range density and composition fluctuations appearing near the critical point enables it to predict with equal accuracy the behavior of the systems far from and close to the critical region. We have found that, for most of the mixtures investigated here, one size binary interaction parameter, with a fixed value for all systems, is enough to quantitatively predict the rich phase behavior shown by these mixtures, while for the case of very asymmetric mixtures, a second binary parameter, also independent of the thermodynamic conditions, is needed to quantitatively describe experimental data. Crossover soft-SAFT accurately reproduces transitions from type I to type V for the critical behavior of the methane/n-alkane and ethane/n-alkane homologous series. The equation also predicts in a quantitative manner the subcritical and critical behavior of the 1-propanol/n-hexane and ethanol/n-butane binary mixtures. Finally, we report speed of sounds of the mixture methane/n-butane and the heat capacities of the mixture 1-propanol/n-decane, in close agreement with experimental data. Results presented here encourage the development of molecular-based equations of state with a term taking into account the singular behavior in the near critical region, especially if one is searching for quantitative predictions in this region for further applications. © 2006 Elsevier B.V. All rights reserved.},
	number = {2},
	journal = {J. Supercrit. Fluids},
	author = {Llovell, Fèlix and Vega, Lourdes F.},
	year = {2007},
	keywords = {Critical region, Crossover term, Ethane/n-alkane mixtures, Methane/n-alkane mixtures, Second order derivative properties, Soft-SAFT equation, Type I to type V transition, n-Alkane/1-alkanol mixtures},
	pages = {204--216},
}

@article{jia_computation_2012,
	title = {Computation of liquid-vapor critical points for multi-component mixtures},
	volume = {15},
	issn = {13019724},
	doi = {10.5541/ijot.380},
	abstract = {Liquid-vapor critical point for a thermodynamic mixture is an important parameter for the design of mixture transportation and processing. The classical critical points model for the multicomponent mixture is based on the tangent plane distance in terms of the Helmholtz energy. In this work, we have applied the damped Newton-Raphson scheme to solve the model using the critical temperature, critical specific volume and change in mole fraction of each component as independent variables. According to numerical experiments, the convergence criteria, initial guesses of variables and damped factor formulation were determined. The method was tested on twenty five mixtures containing two to eleven components using the SRK and PR equation of state. Comparisons between the calculated critical parameters and experimental values illustrated the overall accuracy of the solution method is satisfactory. This method can solve all the variables simultaneously using the whole iteration, which is more reliable than the nested two-singe variable loops method proposed by Heidemann and Khalil. Thus it can be used for practical purposes of locating the liquid-vapor critical points of multi-component mixtures.},
	number = {3},
	journal = {Int. J. Thermodyn.},
	author = {Jia, Wenlong and Li, Changjun and Wu, Xia},
	year = {2012},
	keywords = {Damped newton-raphson method, Equation of state, Liquid-vapor critical points multicomponent mixtur, Mathematic model},
	pages = {149--156},
}

@article{wilhelmsen_thermodynamic_2017,
	title = {Thermodynamic {Modeling} with {Equations} of {State}: {Present} {Challenges} with {Established} {Methods}},
	volume = {56},
	issn = {15205045},
	doi = {10.1021/acs.iecr.7b00317},
	abstract = {Equations of state (EoS) are essential in the modeling of a wide range of industrial and natural processes. Desired qualities of EoS are accuracy, consistency, computational speed, robustness, and predictive ability outside of the domain where they have been fitted. In this work, we review present challenges associated with established models, and give suggestions on how to overcome them in the future. The most accurate EoS available, multiparameter EoS, have a second artificial Maxwell loop in the two-phase region that gives problems in phase-equilibrium calculations and excludes them from important applications such as treatment of interfacial phenomena with mass-based density functional theory. Suggestions are provided on how this can be improved. Cubic EoS are among the most computationally efficient EoS, but they often lack sufficient accuracy. We show that extended corresponding state EoS are capable of providing significantly more accurate single-phase predictions than cubic EoS with only a doubling of the computational time. In comparison, the computational time of multiparameter EoS can be orders of magnitude larger. For mixtures in the two-phase region, however, the accuracy of extended corresponding state EoS has a large potential for improvement. The molecular-based SAFT family of EoS is preferred when predictive ability is important, for example, for systems with strongly associating fluids or polymers where few experimental data are available. We discuss some of their benefits and present challenges. A discussion is presented on why predictive thermodynamic models for reactive mixtures such as CO2-NH3 and CO2-H2O-H2S must be developed in close combination with phase- and reaction equilibrium theory, regardless of the choice of EoS. After overcoming present challenges, a next-generation thermodynamic modeling framework holds the potential to improve the accuracy and predictive ability in a wide range of applications such as process optimization, computational fluid dynamics, treatment of interfacial phenomena, and processes with reactive mixtures.},
	number = {13},
	journal = {Ind. Eng. Chem. Res.},
	author = {Wilhelmsen, Øivind and Aasen, Ailo and Skaugen, Geir and Aursand, Peder and Austegard, Anders and Aursand, Eskil and Gjennestad, Magnus Aa and Lund, Halvor and Linga, Gaute and Hammer, Morten},
	year = {2017},
	pages = {3503--3515},
}

@article{renon_local_1968,
	title = {Local compositions in thermodynamic excess functions for liquid mixtures},
	volume = {14},
	issn = {15475905},
	doi = {10.1002/aic.690140124},
	abstract = {A critical discussion is given of the use of local compositions for representation of excess Gibbs energies of liquid mixtures. A new equation is derived, based on Scott's two‐liquid model and on an assumption of nonrandomness similar to that used by Wilson. For the same activity coefficients at infinite dilution, the Gibbs energy of mixing is calculated with the new equation as well as the equations of van Laar, Wilson, and Heil; these four equations give similar results for mixtures of moderate nonideality but they differ appreciably for strongly nonideal systems, especially for those with limited miscibility. The new equation contains a nonrandomness parameter α12 which makes it applicable to a large variety of mixtures. By proper selection of α12, the new equation gives an excellent representation of many types of liquid mixtures while other local composition equations appear to be limited to specific types. Consideration is given to prediction of ternary vapor‐liquid and ternary liquid‐liquid equilibria based on binary data alone. Copyright © 1968 American Institute of Chemical Engineers},
	number = {1},
	journal = {AIChE J.},
	author = {Renon, Henri and Prausnitz, J. M.},
	year = {1968},
	pages = {135--144},
}

@article{walsh_shock-wave_1957,
	title = {Shock-wave compressions of twenty-seven metals. equations of state of metals},
	volume = {108},
	issn = {0031899X},
	doi = {10.1103/PhysRev.108.196},
	abstract = {An explosive system is used to drive a strong shock wave into a plate of 24ST aluminum. This shock wave propagates through the 24ST aluminum into small test specimens which are in contact with the front surface of the plate. A photographic technique is used to measure velocities associated with the 24ST aluminum shock wave and with the shock wave in each specimen. The measured velocities are transformed, using the conservation relations, to pressure-compression points. Resulting pressure-compression curves are given for 27 metals. The range of data is different for each material but typically covers the pressure interval 150 to 400 kilobars; probable errors in reported experimental pressure-compression curves are 1 or 2\% in compression for a given pressure. The experimental curves, which consist thermodynamically of a known P, V, E locus for each material, are used to calculate a more complete high-pressure equation of state. This is done by means of a theoretical estimate of the volume variation of the Grüneisen ratio γ(V)=V(â{\textless})V. Calculated P, V, T states are listed for the various materials. For 24ST aluminum, quantities of application in shock-wave hydrodynamics are also tabulated. © 1957 The American Physical Society.},
	number = {2},
	journal = {Phys. Rev.},
	author = {Walsh, John M. and Rice, Melvin H. and McQueen, Robert G. and Yarger, Frederick L.},
	year = {1957},
	pages = {196--216},
}

@article{twu_new_1995,
	title = {A new generalized alpha function for a cubic equation of state {Part} 1. {Peng}-{Robinson} equation},
	volume = {105},
	issn = {03783812},
	doi = {10.1016/0378-3812(94)02601-V},
	abstract = {A generalized temperature and acentric factor dependent function of the attractive term, called the alpha function, of the Peng-Robinson cubic equation of state (PR CEOS) is developed. The approach in this work allows the alpha function to become a linear function of the acentric factor at a constant reduced temperature, not a fourth or sixth order function as suggested by Soave and other researchers. The advantage of a linear function in the acentric factor is obvious in the extrapolation of the alpha function to heavy hydrocarbons, petroleum fractions, and gas condensates. The new generalized alpha function, when used with the PR CEOS, allows the accurate reproduction of the vapor pressure data from the triple point to the critical point for hydrocarbons. The new CEOS provides much more reliable and accurate vapor pressure predictions for light as well as heavy hydrocarbons than the original PR equation. © 1995.},
	number = {1},
	journal = {Fluid Phase Equilib.},
	author = {Twu, Chorng H. and Coon, John E. and Cunningham, John R.},
	year = {1995},
	keywords = {Equations of state, Methods of calculation, Theory},
	pages = {49--59},
}

@article{mccabe_saft-vr_1999,
	title = {{SAFT}-{VR} modelling of the phase equilibrium of long-chain n-alkanes},
	volume = {1},
	issn = {14639076},
	doi = {10.1039/a808085b},
	abstract = {The statistical associating fluid theory for potentials of variable attractive range (SAFT-VR) has been used in the calculation of the phase equilibria for long-chain n-alkanes and their mixtures. We treat the molecules as chains formed from united-atom hard-sphere segments, with a square-well potential of variable attractive range to describe the dispersive forces. A empirical relationship derived in earlier work is used to determine the number of such segments in relation to the carbon number for each member of the homologous series. Simple linear relationships between the potential model parameters and molecular weight have been determined enabling predictions of the fluid phase equilibria of heavier n-alkane molecules for which no experimental data are available. This is illustrated by a comparison with simulation data from the literature for the coexisting densities of n- octatetracontane (C48H98). Additionally we have examined binary mixtures of methane + n-hexadecane (C16H34) and hexane + n-tetradecane (C14H30) with the SAFT-VR approach, using simple Lorentz-Berthelot combining rules to determine the unlike interaction parameters. This study will allow an extension of the SAFT-VR approach to polymeric systems.},
	number = {9},
	journal = {Phys. Chem. Chem. Phys.},
	author = {McCabe, Clare and Jackson, George},
	year = {1999},
	pages = {2057--2064},
}

@article{kraska_phase_1996,
	title = {Phase {Equilibria} {Calculations} with a {Modified} {SAFT} {Equation} of {State}. 2. {Binary} {Mixtures} of n-{Alkanes}, 1-{Alkanols}, and {Water}},
	volume = {35},
	issn = {08885885},
	doi = {10.1021/ie960233s},
	abstract = {The Lennard-Jones - statistical association fluid theory (LJ-SAFT) is applied to binary mixtures containing one self-associating and one nonassociating substance. The binary systems studied here are n-alkane/n-alkane, 1-alkanol/n-alkane, and water/n-alkane mixtures. For cases where the dipole-dipole term is needed, the influence of induction is also investigated. The results with LJ-SAFT exhibit better agreement with experimental data than SAFT. This improvement is due to the exchange of the hard-sphere reference system by the LJ reference system.},
	number = {12},
	journal = {Ind. Eng. Chem. Res.},
	author = {Kraska, Thomas and Gubbins, Keith E.},
	year = {1996},
	pages = {4738--4746},
}

@article{wilson_vapor-liquid_1964,
	title = {Vapor-{Liquid} {Equilibrium}. {XI}. {A} {New} {Expression} for the {Excess} {Free} {Energy} of {Mixing}},
	volume = {86},
	issn = {15205126},
	doi = {10.1021/ja01056a002},
	abstract = {An equation has been found which represents the excess free energy of mixing nonelectrolytes with two, or sometimes three, parameters for a binary mixture and no additional parameters for polycomponent systems. It is compared with the experimental values for several mixtures. The corresponding equations for the excess enthalpy and entropy of mixing are also derived. A semi theoretical interpretation is given. This equation should be particularly useful for large deviations from normality and for polycomponent mixtures. © 1964, American Chemical Society. All rights reserved.},
	number = {2},
	journal = {J. Am. Chem. Soc.},
	author = {Wilson, Grant M.},
	year = {1964},
	pages = {127--130},
}

@article{michelsen_robust_2006,
	title = {Robust and {Efficient} {Solution} {Procedures} for {Association} {Models}},
	volume = {45},
	issn = {0888-5885},
	url = {https://pubs.acs.org/doi/10.1021/ie060029x},
	doi = {10.1021/ie060029x},
	number = {25},
	journal = {Ind. Eng. Chem. Res.},
	author = {Michelsen, Michael L.},
	month = dec,
	year = {2006},
	pages = {8449--8453},
}

@article{twu_improved_1980,
	title = {Improved analytical representation of argon thermodynamic behavior},
	volume = {4},
	issn = {03783812},
	doi = {10.1016/0378-3812(80)80003-3},
	abstract = {The equation of state of Gosman and coworkers has been used extensively to calculate the thermodynamic properties of simple fluids. Gosman's equation of state, however, is inadequate when calculations are made (a) for liquids at low temperatures, (b) for fluids at very high temperatures and pressures, (c) for the derived thermodynamic properties such as enthalpy, entropy, etc., at low temperatures. One of the objectives of this work was to improve the equation of state and extend its use to lower temperatures and higher pressures. Based on perturbation theory using Pople's expansion for moderately anisotropic fluids, the equation of state accurately represents vapor pressures, densities and enthalpy departures of vapor, liquid, and fluid states as functions of three parameters (reduced temperature, reduced density and acentric factor) over the range Tr = 0.3 to 3.3 and Pr = 0 to 132 for simple fluids. The result is an improved analytical representation of these properties at low temperatures and high pressures for simple fluids. This equation of state should be useful for calculating reference system properties in perturbation equation of state studies. © 1980.},
	number = {1-2},
	journal = {Fluid Phase Equilib.},
	author = {Twu, C. H. and Lee, L. L. and Starling, K. E.},
	year = {1980},
	pages = {35--44},
}

@article{bamberger_high-pressure_2000,
	title = {High-pressure (vapor+liquid) equilibrium in binary mixtures of (carbon dioxide+water or acetic acid) at temperatures from 313 to 353 {K}},
	volume = {17},
	issn = {08968446},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0896844699000546},
	doi = {10.1016/S0896-8446(99)00054-6},
	number = {2},
	journal = {J. Supercrit. Fluids},
	author = {Bamberger, A. and Sieder, G. and Maurer, G.},
	month = apr,
	year = {2000},
	pages = {97--110},
}

@misc{leal_autodiff_2018,
	title = {autodiff, a modern, fast and expressive {C}++ library for automatic differentiation},
	url = {https://github.com/autodiff/autodiff/},
	urldate = {2022-03-15},
	author = {Leal, Allan M. M.},
	year = {2018},
}

@article{horstmann_psrk_2005,
	title = {{PSRK} group contribution equation of state: {Comprehensive} revision and extension {IV}, including critical constants and α-function parameters for 1000 components},
	volume = {227},
	issn = {03783812},
	doi = {10.1016/j.fluid.2004.11.002},
	abstract = {As a part of an ongoing process, the predictive Soave-Redlich-Kwong (PSRK) group contribution equation of state was extended by the introduction of additional structural groups (F 2, Cl 2, Br 2, HCN, NO 2, CF 4, O 3 and ClNO) and fitting of the corresponding group interaction parameters. Interaction parameters between already existing main groups were also optimized to the growing literature data base. Overall, 75 new parameter sets are given herein, and typical results are presented for various systems. For the sake of completeness, not only the group new interaction parameters but all available PSRK/UNIFAC interaction parameter sets (more than 900) are given as supplementary material. Moreover, the required pure component properties (critical properties, acentric factors, and Mathias-Copeman constants) were revised and are also included for about 1000 components. © 2004 Elsevier B.V. All rights reserved.},
	number = {2},
	journal = {Fluid Phase Equilib.},
	author = {Horstmann, Sven and Jab{\textbackslash}loniec, Anna and Krafczyk, Jörg and Fischer, Kai and Gmehling, Jürgen},
	year = {2005},
	keywords = {Equation of state, Group contribution, PSRK, UNIFAC, α-Function},
	pages = {157--164},
}

@article{djordjevic_mixing_2001,
	title = {Mixing rules for excess free energy models},
	volume = {66},
	issn = {03525139},
	doi = {10.2298/jsc0104213d},
	number = {4},
	journal = {J. Serb. Chem. Soc.},
	author = {Djordjević, Bojan D. and Kijevčanin, Mirjana Lj and Orlović, Jadranka P. and Šerbanović, Slobodan P.},
	year = {2001},
	keywords = {Correlation, Cubic equation of state, Excess molar properties, Mixing rule, Prediction, Vapour-liquid equilibria},
	pages = {213--236},
}

@book{robinson_characterization_1978,
	address = {Tulsa},
	title = {The characterization of the heptanes and heavier fractions for the {GPA} {Peng}-{Robinson} programs},
	publisher = {Gas Processors Association},
	author = {Robinson, Donald B. and Peng, Ding-Yu},
	year = {1978},
}

@article{cameretti_modeling_2008,
	title = {Modeling of aqueous amino acid and polypeptide solutions with {PC}-{SAFT}},
	volume = {47},
	issn = {02552701},
	doi = {10.1016/j.cep.2007.02.034},
	abstract = {Vapor pressures, liquid densities and solubilities of aqueous amino acid and oligopeptide solutions were modeled with an equation of state based on PC-SAFT. The amino acids glycine (Gly), alanine (Ala), serine (Ser), proline (Pro), and valine (Val) as well as the oligopeptides (Gly)n=1-5, and Ala(Gly)n=1-4 were considered. Five pure-component model parameters for each amino acid were fitted using experimental densities, vapor pressures, and solubility data. The oligopeptides were treated as co-polymers built up by the respective amino acids. Thus, no additional parameters had to be fitted for the prediction of densities and vapor-liquid behavior of their aqueous solutions besides the segment number. The model is able to excellently reproduce the experimental densities, vapor pressures and solubility data of aqueous amino acid and oligopeptide solutions. © 2007 Elsevier B.V. All rights reserved.},
	number = {6},
	journal = {Chem. Eng. Process.},
	author = {Cameretti, Luca F. and Sadowski, Gabriele},
	year = {2008},
	keywords = {Amino acid solutions, Density, Sol, Vapor pressure},
	pages = {1018--1025},
}

@article{stabnikov_equilibrium_1972,
	title = {On the {Equilibrium} in the {System} {Ethyl} {Alcohol} - {Water} at {Atmospheric} {Pressure}},
	volume = {15},
	journal = {Pishch. Promst. Kiev},
	author = {Stabnikov, V.N. and Matyushev, B.Z. and Protsyuk, T.B. and Yushchenko, N.M.},
	year = {1972},
	pages = {49--56},
}

@article{berberan-santos_van_2008,
	title = {The van der {Waals} equation: {Analytical} and approximate solutions},
	volume = {43},
	issn = {02599791},
	doi = {10.1007/s10910-007-9272-4},
	abstract = {The thermodynamic properties, enthalpy of vaporization, entropy, Helmholtz function, Gibbs function, but especially the heat capacity at constant volume of a van der Waals gas (and liquid) at the phase transition are examined in two different limit approximations. The first limit approximation is at the near-critical temperatures, i.e., for T/T c → 1, where T c is the critical temperature, the other limit approximation is at the near-zero temperatures, T→ 0. In these limits, the analytical equations for liquid and gas concentrations at saturated conditions were obtained. Although the heat capacities at constant volume of a van der Waals gas and liquid do not depend on the volume, they have different values and their change during the phase transition was calculated. It should be noticed that for real substances the equations obtained at the near-zero temperature are only valid for T {\textgreater} T triple point and T {\textgreater} T c , which means that found equations can be used only for substances with T triple point {\textgreater} T c . © 2007 Springer Science+Business Media, LLC.},
	number = {4},
	journal = {J. Math. Chem.},
	author = {Berberan-Santos, Mario N. and Bodunov, Evgeny N. and Pogliani, Lionello},
	year = {2008},
	keywords = {Critical temperature, Heat capacities, Phase transition, Thermodynamics, Van der Waals equation},
	pages = {1437--1457},
}

@article{chen_equation_2001,
	title = {Equation of state extended from {SAFT} with improved results for non-polar fluids across the critical point},
	volume = {186},
	issn = {03783812},
	doi = {10.1016/S0378-3812(01)00521-0},
	abstract = {Based on the thermodynamic perturbation theory of Wertheim, statistical associating fluid theory (SAFT) has became a successful equation of state for the description of thermodynamic properties of fluids, especially for systems including polymers. In recent years, different versions of SAFT have been developed based on square-well and Lennard-Jones reference fluids and improvements are achieved. In this paper SAFT is modified with two improvements in order to calculate the properties near the critical points of non-polar fluids. One improvement is the consideration of the segment shape in chain molecules using the hard convex body equation of state as the reference term and the relative expression for chain formation with the radial distribution function of hard convex body fluid is also included. The another improvement is the exclusion of the dispersion energy between intramolecular segments with a newly derived term based on the perturbation theory. The first improvement gives a better prediction of the critical points for one-segment non-spherical molecules and the second for chain molecules. The new equation of state includes four parameters for every non-polar fluid: the segment number m, the segment non-spherical parameter α, the segment volume v00 and the segment interaction parameter u0. The saturated pressures and saturated liquid densities up to the critical point can be calculated with average absolute deviations of 0.6 and 0.8\% for 44 non-polar fluids including n-alkanes, branched alkanes, cycloalkanes, alkenes, alkynes and aromatics. Critical temperatures, pressures and densities are calculated with the average absolute deviations of 0.2, 1.2 and 2.9\%. The new equation of state was used to predict such thermodynamic properties as PVT lines, and vaporization enthalpies. The prediction results are also in good agreement with experimental data from literature. Copyright © 2001 Elsevier Science B.V.},
	number = {1-2},
	journal = {Fluid Phase Equilib.},
	author = {Chen, J. and Mi, J. G.},
	year = {2001},
	keywords = {Critical properties, Equation of state, Non-polar fluids, SAFT},
	pages = {165--184},
}

@article{morch_measurement_2006,
	title = {Measurement and modeling of hydrocarbon dew points for five synthetic natural gas mixtures},
	volume = {239},
	issn = {03783812},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0378381205004541},
	doi = {10.1016/j.fluid.2005.11.010},
	number = {2},
	journal = {Fluid Phase Equilib.},
	author = {Mørch, Ø. and Nasrifar, Kh. and Bolland, O. and Solbraa, E. and Fredheim, A.O. and Gjertsen, L.H.},
	month = jan,
	year = {2006},
	pages = {138--145},
}

@article{thol_eos-lng_2019,
	title = {{EOS}-{LNG}: {A} {Fundamental} {Equation} of {State} for the {Calculation} of {Thermodynamic} {Properties} of {Liquefied} {Natural} {Gases}},
	volume = {48},
	issn = {0047-2689},
	url = {http://aip.scitation.org/doi/10.1063/1.5093800},
	doi = {10.1063/1.5093800},
	number = {3},
	journal = {Journal of Physical and Chemical Reference Data},
	author = {Thol, Monika and Richter, Markus and May, Eric F. and Lemmon, Eric W. and Span, Roland},
	month = sep,
	year = {2019},
	pages = {033102},
}

@incollection{bonilla-petriciolet_phase_2017,
	address = {Singapore},
	edition = {6},
	title = {Phase {Stability} and {Equilibrium} {Calculations} in {Reactive} {Systems} using {Differential} {Evolution} and {Tabu} {Search}},
	url = {http://www.worldscientific.com/doi/abs/10.1142/9789813207523_0007},
	booktitle = {Advances in {Process} {Systems} {Engineering}: {Stochastic} {Global} {Optimization}},
	publisher = {World Scientific},
	author = {Bonilla-Petriciolet, Adrián and Rangaiah, Gade Pandu and Segovia-Hernández, Juan Gabriel and Jaime-Leal, José Enrique},
	editor = {Rangaiah, Gade Pandu and Sharma, Shivom},
	month = jul,
	year = {2017},
	doi = {10.1142/9789813207523_0007},
	note = {Section: 7},
	pages = {413--463},
}

@article{gross_modeling_2002,
	title = {Modeling polymer systems using the perturbed-chain statistical associating fluid theory equation of state},
	volume = {41},
	issn = {08885885},
	doi = {10.1021/ie010449g},
	abstract = {The perturbed-chain statistical associating fluid theory (PC-SAFT) equation of state is applied to binary and ternary mixtures of polymers, solvents, and gases. The three pure-component parameters required for nonassociating molecules were identified for six polymer compounds. The phase equilibrium of polymer systems, which often involves high-pressure liquid-liquid mixtures as well as vapor-liquid mixtures at lower pressures, was investigated. Using a constant binary interaction parameter (kij), the PC-SAFT equation of state gives good correlations of the appropriate phase behavior over wide ranges of conditions. Comparisons to an earlier version of SAFT reveal an improvement of the proposed model.},
	number = {5},
	journal = {Ind. Eng. Chem. Res.},
	author = {Gross, Joachim and Sadowski, Gabriele},
	year = {2002},
	pages = {1084--1093},
}

@article{papaioannou_application_2016,
	title = {Application of the {SAFT}-γ {Mie} group contribution equation of state to fluids of relevance to the oil and gas industry},
	volume = {416},
	issn = {03783812},
	doi = {10.1016/j.fluid.2015.12.041},
	abstract = {The application of the SAFT-γ Mie group contribution approach [Papaioannou et al., J. Chem. Phys., 140 (2014) 054107] to the study of a range of systems of relevance to the oil and gas industry is presented. In particular we consider carbon dioxide, water, methanol, aromatics, alkanes, and their mixtures. Following a brief overview of the SAFT-γ Mie equation of state, a systematic methodology for the development of like and unlike group parameters relevant to the systems of interest is presented. The determination of group-group interactions entails a sequence of steps including: the selection of representative components and mixtures (in this instance carbon dioxide, water, methanol, aromatics, and alkanes); the definition of an appropriate set of groups to describe them; the collection of target experimental data used to estimate the group-group interactions; the determination of the group-group interaction parameters; and the assessment of the adequacy of the parameters and theoretical approach. The predictive capability of the SAFT-γ Mie group contribution approach is illustrated for a selection of mixtures, including representative examples of the simultaneous description of vapour-liquid and liquid-liquid equilibria, the densities of the coexisting phases, second derivative thermodynamic properties, and excess properties of mixing. Good quantitative agreement between the predictions and experimental data is achieved, even in the case of challenging mixtures comprising carbon dioxide and water, n-alkanes and water, and methanol and methane.},
	journal = {Fluid Phase Equilib.},
	author = {Papaioannou, Vasileios and Calado, Filipe and Lafitte, Thomas and Dufal, Simon and Sadeqzadeh, Majid and Jackson, George and Adjiman, Claire S. and Galindo, Amparo},
	year = {2016},
	keywords = {Fluid-phase behaviour, Group contribution methods, Oil and gas, SAFT, SAFT-VR},
	pages = {104--119},
}

@article{llovell_second-order_2006,
	title = {Second-order thermodynamic derivative properties of selected mixtures by the soft-{SAFT} equation of state},
	volume = {248},
	issn = {03783812},
	doi = {10.1016/j.fluid.2006.07.018},
	abstract = {We have discussed the capability of the soft-SAFT equation of state (EoS) to predict second order thermodynamic derivative properties of pure fluids in a recent paper [F. Llovell, L.F. Vega, J. Phys. Chem. B 110 (2006) 11427-11437]. The goal of this work is to extend these calculations to selected binary mixtures. The equation was applied in a semi-predictive manner: the pure component molecular parameters needed to apply soft-SAFT to experimental systems were obtained by fitting vapor-liquid equilibrium data and used, without further fitting, to calculate isochoric and isobaric heat capacities of selected alkane + n-alkane and n-alkane + 1-alkanol binary mixtures; isentropic compressibility coefficients and the speed of sound of selected n-alkane + 1-alkanol mixtures were calculated following the same procedure. We have used the crossover soft-SAFT equation which explicitly incorporates a renormalization group term in order to take into account the long range fluctuations appearing in the near critical region. Soft-SAFT was able to capture the qualitative behavior of the mixture properties studied, for a wide range of conditions, showing quantitative agreement with experimental data in some of the cases. As a further test to the equation, we have also calculated excess properties. The equation was able to capture the non-ideal behavior upon mixing experienced by these properties. This work shows the robustness of the molecular parameters and the equation to calculate properties not included in the fitting procedure, in a predictive manner. © 2006 Elsevier B.V. All rights reserved.},
	number = {2},
	journal = {Fluid Phase Equilib.},
	author = {Llovell, F. and Peters, C. J. and Vega, L. F.},
	year = {2006},
	keywords = {1-Alkanols, Binary mixtures, Crossover, Heat capacities, Isentropic compressibility, Second order derivative properties, Soft-SAFT, Speed of sound, n-Alkanes},
	pages = {115--122},
}

@phdthesis{van_der_waals_over_1873,
	type = {{PhD} {Thesis}},
	title = {Over de {Continuiteit} van den {Gas}- en {Vloeistoftoestand}},
	school = {University of Leiden},
	author = {van der Waals, Johannes Diderik},
	year = {1873},
}

@article{french_excess_1989,
	title = {Excess enthalpies of (acetone + water) at 278.15, 288.15, 298.15, 308.15, 318.15, and 323.15 {K}},
	volume = {21},
	issn = {00219614},
	url = {https://linkinghub.elsevier.com/retrieve/pii/0021961489900268},
	doi = {10.1016/0021-9614(89)90026-8},
	number = {8},
	journal = {J. Chem. Thermodyn.},
	author = {French, H.T},
	month = aug,
	year = {1989},
	pages = {801--809},
}

@article{marinichev_no_1965,
	title = {No {Title}},
	volume = {38},
	number = {7},
	journal = {J. Appl. Chem. USSR},
	author = {Marinichev, A.N. and Susarev, M.P.},
	year = {1965},
	pages = {1582--1584},
}

@article{muller_calculation_2020,
	title = {Calculation of thermodynamic equilibria with the predictive electrolyte model {COSMO}-{RS}-{ES}: {Improvements} for low permittivity systems},
	volume = {506},
	issn = {03783812},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0378381219304297},
	doi = {10.1016/j.fluid.2019.112368},
	journal = {Fluid Phase Equilib.},
	author = {Müller, Simon and González de Castilla, Andrés and Taeschler, Christoph and Klein, Andreas and Smirnova, Irina},
	month = feb,
	year = {2020},
	pages = {112368},
}

@article{clapeyron_memoire_1834,
	title = {Mémoire sur la {Puissance} {Motrice} de la {Chaleur}},
	volume = {XIV},
	journal = {J. Ec. Polytech. (Paris)},
	author = {Clapeyron, E.},
	year = {1834},
	pages = {153--90},
}

@article{kraska_phase_1996,
	title = {Phase {Equilibria} {Calculations} with a {Modified} {SAFT} {Equation} of {State}. 1. {Pure} {Alkanes}, {Alkanols}, and {Water}},
	volume = {35},
	issn = {08885885},
	doi = {10.1021/ie9602320},
	abstract = {The phase equilibria of the n-alkanes and the 1-alkanols have been calculated with the Lennard-Jones-SAFT (statistical association fluid theory) equation of state of Müller and Gubbins. This equation includes contributions from a dipole-dipole term, a modified association term, a chain term, and a Lennard-Jones term to account for monomer dispersion and overlap interactions. The influence of electrostatic forces due to the dipole moment has been investigated, and a simple treatment of the polarizability has been tested. It is shown by comparison with some sample calculations based on the renormalized perturbation theory that this approach is reasonable. The calculated phase equilibria are in good agreement with experimental data. The deviation between calculated and experimental data is significantly lower than for the original SAFT equation of state and a recently published chemical theory.},
	number = {12},
	journal = {Ind. Eng. Chem. Res.},
	author = {Kraska, Thomas and Gubbins, Keith E.},
	year = {1996},
	pages = {4727--4737},
}

@article{von_solms_computational_2003,
	title = {Computational and physical performance of a modified {PC}-{SAFT} equation of state for highly asymmetric and associating mixtures},
	volume = {42},
	issn = {08885885},
	doi = {10.1021/ie020753p},
	abstract = {Two modifications to perturbed-chain statistical associating fluid theory are proposed which simplify the calculation of phase-equilibrium properties for nonassociating and associating systems, polymers, and simple molecules without loss of accuracy. A simple linear extrapolation scheme is proposed to obtain parameters for linear alkanes up to polyethylene. It is shown that computing times are greatly reduced using these modifications and compare favorably with traditional equations of state for nonassociating and associating systems.},
	number = {5},
	journal = {Ind. Eng. Chem. Res.},
	author = {Von Solms, Nicolas and Michelsen, Michael L. and Kontogeorgis, Georgios M.},
	year = {2003},
	pages = {1098--1105},
}

@article{kunz_gerg-2008_2012,
	title = {The {GERG}-2008 wide-range equation of state for natural gases and other mixtures: {An} expansion of {GERG}-2004},
	volume = {57},
	issn = {00219568},
	doi = {10.1021/je300655b},
	abstract = {A new equation of state for the thermodynamic properties of natural gases, similar gases, and other mixtures, the GERG-2008 equation of state, is presented in this work. This equation is an expanded version of the GERG-2004 equation. GERG-2008 is explicit in the Helmholtz free energy as a function of density, temperature, and composition. The equation is based on 21 natural gas components: methane, nitrogen, carbon dioxide, ethane, propane, n-butane, isobutane, n-pentane, isopentane, n-hexane, n-heptane, n-octane, n-nonane, n-decane, hydrogen, oxygen, carbon monoxide, water, hydrogen sulfide, helium, and argon. Over the entire composition range, GERG-2008 covers the gas phase, liquid phase, supercritical region, and vapor-liquid equilibrium states for mixtures of these components. The normal range of validity of GERG-2008 includes temperatures from (90 to 450) K and pressures up to 35 MPa where the most accurate experimental data of the thermal and caloric properties are represented to within their accuracy. The extended validity range reaches from (60 to 700) K and up to 70 MPa. The given numerical information (including all of the sophisticated derivatives) enables the use of GERG-2008 for all of the various technical applications. Examples are processing, transportation through pipelines or by shipping, storage and liquefaction of natural gas, and processes to separate gas components. Comparisons with other equations of state, for example, AGA8-DC92 and Peng-Robinson equation (P-R), are also presented. GERG-2008 will be adopted as an ISO Standard (ISO 20765-2/3) for natural gases. © 2012 American Chemical Society.},
	number = {11},
	journal = {J. Chem. Eng. Data},
	author = {Kunz, O. and Wagner, W.},
	year = {2012},
	pages = {3032--3091},
}

@article{magoulas_thermophysical_1990,
	title = {Thermophysical properties of n-{Alkanes} from {C1} to {C20} and their prediction for higher ones},
	volume = {56},
	issn = {03783812},
	url = {https://linkinghub.elsevier.com/retrieve/pii/037838129085098U},
	doi = {10.1016/0378-3812(90)85098-U},
	journal = {Fluid Phase Equilib.},
	author = {Magoulas, Kostis and Tassios, Dimitrios},
	month = jan,
	year = {1990},
	pages = {119--140},
}

@article{bell_calculation_2017,
	title = {Calculation of critical points from {Helmholtz}-energy-explicit mixture models},
	volume = {433},
	issn = {03783812},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0378381216305349},
	doi = {10.1016/j.fluid.2016.10.030},
	journal = {Fluid Phase Equilib.},
	author = {Bell, Ian H. and Jäger, Andreas},
	month = feb,
	year = {2017},
	pages = {159--173},
}

@article{hsieh_considering_2014,
	title = {Considering the dispersive interactions in the {COSMO}-{SAC} model for more accurate predictions of fluid phase behavior},
	volume = {367},
	issn = {03783812},
	url = {http://dx.doi.org/10.1016/j.fluid.2014.01.032},
	doi = {10.1016/j.fluid.2014.01.032},
	abstract = {A term to consider the contribution of the dispersive interactions to the non-ideality of mixtures is introduced into the COSMO-SAC model on the basis of molecular simulation data from classical model force fields. This dispersion term is a one-constant Margules equation, where the constant is determined from the molecular dispersion parameter of the components. Furthermore, an atomic contribution method is proposed to calculate the dispersion parameter for a given molecule. For binary systems containing molecules consisting of C, H, N, O, F and Cl atoms, a total of 13 global parameters is introduced with the COSMO-SAC-dsp model. These parameters are obtained from regression to a large training set of binary vapor-liquid equilibrium (VLE) data from experiment. The overall deviations for VLE calculations on this training set are reduced by 25\% in terms of the vapor pressure and 12\% in terms of the vapor phase mole fraction. This dispersion term can provide a significant improvement for infinite dilution activity coefficient predictions, where the accuracy was increased by around 33\%. © 2014 Elsevier B.V.},
	journal = {Fluid Phase Equilib.},
	author = {Hsieh, Chieh Ming and Lin, Shiang Tai and Vrabec, Jadran},
	year = {2014},
	note = {Publisher: Elsevier B.V.},
	keywords = {COSMO-SAC, Dispersive interaction, Infinite dilution activity coefficient, Phase equilibria, Prediction},
	pages = {109--116},
}

@book{reid_properties_1987,
	address = {New York},
	edition = {4th},
	title = {The {Properties} of {Gases} and {Liquids}},
	publisher = {McGraw-Hill},
	author = {Reid, Robert C. and Prausnitz, John M. and Poling, Bruce E.},
	year = {1987},
	doi = {10.1063/1.3060771},
	note = {ISSN: 0031-9228},
}

@article{peneloux_consistent_1982,
	title = {A consistent correction for {Redlich}-{Kwong}-{Soave} volumes},
	volume = {8},
	issn = {03783812},
	url = {https://linkinghub.elsevier.com/retrieve/pii/0378381282800022},
	doi = {10.1016/0378-3812(82)80002-2},
	abstract = {If the volumetric and phase behaviour of a fluid mixture is calculated by means of an equation of state, certain translations along the volume axis may be effected that leave the predicted phase equilibrium conditions unchanged. This property may be exploited in the form at a consistent correction to improve volume estimations by the Redlich-Kwong-Soave method. Applications of this improved method to pure liquids, mixtures of liquids or gases, and petroleum fluids show that markedly superior volume estimations are obtained, except in the neighbourhood of the pure-component critical points; nonetheless, critical volumes for mixtures can be estimated correctly. © 1982.},
	number = {1},
	journal = {Fluid Phase Equilib.},
	author = {Péneloux, André and Rauzy, Evelyne and Fréze, Richard},
	month = jan,
	year = {1982},
	pages = {7--23},
}

@article{muller_equation_1995,
	title = {An {Equation} of {State} for {Water} from a {Simplified} {Intermolecular} {Potential}},
	volume = {34},
	issn = {15205045},
	doi = {10.1021/ie00037a055},
	abstract = {An equation of state for water is presented which accounts explicitly for repulsive, dispersive, multipolar, and association interactions. The thermodynamic properties are obtained from a simplified intermolecular potential by means of a perturbation theory, based on Wertheim's first-order theory for associating fluids, and make use of a Stockmayer (dipolar Lennard-Jones) reference fluid. The theory is tested rigorously by comparing to it to computer simulations. Theory and simulations are found to be in general good agreement. The parameters of the theory are fitted to the vapor-liquid coexistence conditions of water. Macroscopic properties, such as the phase diagram, the vapor pressure curve, and the energy of vaporization, and molecular properties, such as the fraction of monomelic species in the saturated liquid and bonding distributions, are reasonably well represented by the resulting equation of state. Some deficiencies of the model are pin pointed, and suggestions for the development of improved potential models and/or equations of state for water are made. © 1995, American Chemical Society. All rights reserved.},
	number = {10},
	journal = {Ind. Eng. Chem. Res.},
	author = {Müller, Erich A. and Gubbins, Keith E.},
	year = {1995},
	pages = {3662--3673},
}

@article{le_guennec_development_2016,
	title = {Development of the translated-consistent tc-{PR} and tc-{RK} cubic equations of state for a safe and accurate prediction of volumetric, energetic and saturation properties of pure compounds in the sub- and super-critical domains},
	volume = {429},
	issn = {03783812},
	doi = {10.1016/j.fluid.2016.09.003},
	abstract = {In this paper, translated and consistent versions of the Peng-Robinson (tc-PR) and Redlich-Kwong (tc-RK) cubic equations of state (CEoS) are developed. The adjective consistent means that the α-function used in such models passes the consistency test we recently developed and which guarantees safe extrapolation in the supercritical region and safe VLE calculation in multi-component systems. The adjective translated means that a volume translation aimed at exactly reproducing the experimental saturated liquid volume at a reduced temperature of 0.8 was used. The key conclusion of this paper is that the tc-PR EoS is certainly the safest and the most accurate 3-parameter cubic EoS ever published. Indeed the average deviations over roughly 1000 compounds belonging to different chemical families are: ΔPsat{\textless}1 \%, ΔvapH=ΔcP,Lsat=2\% and ΔvLsat(Tr{\textless}0.9)=2.3\%. In the case of a lack of experimental data to fit the 3 parameters of the α-function and to determine the value of the volume correction, the second part of this study aims at providing a generalized version of the tc-PR and tc-RK CEoS in which all parameters can be estimated from the mere knowledge of the acentric factor.},
	journal = {Fluid Phase Equilib.},
	author = {Le Guennec, Yohann and Privat, Romain and Jaubert, Jean Noël},
	year = {2016},
	keywords = {Consistent α-function, Equation of state, Peng-Robinson, Redlich-Kwong, Twu, Volume-translation},
	pages = {301--312},
}

@article{mollerup_unification_1998,
	title = {Unification of the two-parameter equation of state and the principle of corresponding states},
	volume = {148},
	issn = {03783812},
	doi = {10.1016/S0378-3812(98)00230-1},
	abstract = {A two-parameter equation of state is a two-parameter corresponding states model. A two-parameter corresponding states model is composed of two scale factor correlations and a reference fluid equation of state. In a two-parameter equation of state the reference equation of state is the two-parameter equation of state itself. If we retain the scale factor correlations derived from a two-parameter equation of state, but replace the two-parameter equation of state with a more accurate pure component equation of state for the reference fluid, we can improve the existing models of equilibrium properties without refitting any model parameters, and without imposing other restrictions as regards to species and mixing rules as already imposed by the two-parameter equation of state. The theory and procedure is outlined in the paper.},
	number = {1-2},
	journal = {Fluid Phase Equilib.},
	author = {Mollerup, Jørgen},
	year = {1998},
	keywords = {corresponding states, equation of state, thermodynamic models},
	pages = {1--19},
}

@article{ishihara_phase_1998,
	title = {Phase equilibrium properties of ethane+methanol system at 298.15 {K}},
	volume = {144},
	issn = {03783812},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0378381297002513},
	doi = {10.1016/S0378-3812(97)00251-3},
	number = {1-2},
	journal = {Fluid Phase Equilib.},
	author = {Ishihara, Katsuo and Tanaka, Hiroyuki and Kato, Masahiro},
	month = feb,
	year = {1998},
	pages = {131--136},
}

@article{yin_combined_1998,
	title = {Combined {Ab} {Initio} / {Empirical} {Approach} for {Optimization} of {LennardJones} {Parameters}},
	volume = {19},
	issn = {0192-8651},
	abstract = {Obtaining accurate LennardJones L-J parameters is a vital part of the optimization of empirical force fields due to their significant contribution to condensed-phase properties. We present a novel approach to optimize L-J parameters via the use of ab initio data on interactions between rare gas atoms and model compounds combined with the reproduction of experimental pure solvent properties. Relative values of ab initio minimum interaction energies and geometries between helium or neon and model compounds were used to optimize the relative magnitude of the L-J parameters. Absolute values of the L-J parameters were determined by reproducing experimental heats of vaporization and molecular volumes for pure solvents. Application of the approach was performed on methane, ethane, and propane. Free energies of aqueous solvation and butane pure solvent and aqueous solvation calculations were used to test the developed L-J parameters. The new alkane parameters are similar or improved as compared with current empirical force field parameters with respect to experimental pure solvent properties and free energies of aqueous solvation. Also included is a description of the internal portion of the force field},
	number = {3},
	journal = {J. Comput. Chem.},
	author = {Yin, Daxu and Mackerell, Alexander D},
	year = {1998},
	note = {ISBN: 3343481998
Publisher: John Wiley \& Sons, Inc},
	keywords = {CHARMM, helium, neon, parameters, parametrization},
}

@article{woon_gaussian_1994,
	title = {Gaussian basis sets for use in correlated molecular calculations. {IV}. {Calculation} of static electrical response properties},
	volume = {100},
	issn = {00219606},
	doi = {10.1063/1.466439},
	abstract = {An accurate description of the electrical properties of atoms and molecules is critical for quantitative predictions of the nonlinear properties of molecules and of long-range atomic and molecular interactions between both neutral and charged species. We report a systematic study of the basis sets required to obtain accurate correlated values for the static dipole (α1), quadrupole (α2), and octopole (α3) polarizabilities and the hyperpolarizability (γ) of the rare gas atoms He, Ne, and Ar. Several methods of correlation treatment were examined, including various orders of Moller-Plesset perturbation theory (MP2, MP3, MP4), coupled-cluster theory with and without perturbative treatment of triple excitations [CCSD, CCSD(T)], and singles and doubles configuration interaction (CISD). All of the basis sets considered here were constructed by adding even-tempered sets of diffuse functions to the correlation consistent basis sets of Dunning and co-workers. With multiply-augmented sets we find that the electrical properties of the rare gas atoms converge smoothly to values that are in excellent agreement with the available experimental data and/or previously computed results. As a further test of the basis sets presented here, the dipole polarizabilities of the F - and Cl- anions and of the HCl and N2 molecules are also reported. © 1994 American Institute of Physics.},
	number = {4},
	journal = {J. Chem. Phys.},
	author = {Woon, David E. and Dunning, Thorn H.},
	year = {1994},
	pages = {2975--2988},
}

@article{woon_gaussian_1993,
	title = {Gaussian basis sets for use in correlated molecular calculations. {III}. {The} atoms aluminum through argon},
	volume = {98},
	issn = {00219606},
	doi = {10.1063/1.464303},
	abstract = {Correlation consistent and augmented correlation consistent basis sets have been determined for the second row atoms aluminum through argon. The methodology, originally developed for the first row atoms [T. H. Dunning, Jr., J. Chem. Phys. 90, (1989)] is first applied to sulfur. The exponents for the polarization functions (dfgh) are systematically optimized for a correlated wave function (HF+1+2). The (sp) correlation functions are taken from the appropriate HF primitive sets; it is shown that these functions differ little from the optimum functions. Basis sets of double zeta [4s3p1d], triple zeta [5s4p2d1f], and quadruple zeta [6s5p3d2f1g] quality are defined. Each of these sets is then augmented with diffuse functions to better describe electron affinities and other molecular properties: s and p functions were obtained by optimization for the anion HF energy, while an additional polarization function for each symmetry present in the standard set was optimized for the anion HF+1+2 energy. The results for sulfur are then used to assist in determining double zeta, triple zeta, and quadruple zeta basis sets for the remainder of the second row of the p block. © 1993 American Institute of Physics.},
	number = {2},
	journal = {J. Chem. Phys.},
	author = {Woon, David E. and Dunning, Thom H.},
	year = {1993},
	pages = {1358--1371},
}

@article{wolbach_thermodynamics_1997,
	title = {Thermodynamics of {Hydrogen} {Bonding} from {Molecular} {Orbital} {Theory}: 1. {Water}},
	volume = {43},
	issn = {00011541},
	doi = {10.1002/aic.690430622},
	abstract = {To reduce the number of adjustable parameters that appear in the thermodynamic modeling of hydrogen-bonding fluids, the use of ab-initio molecular orbital calculations in the form of Hartree - Fock and density functional theories to compute thermodynamic properties are considered. In particular, the enthalpy and entropy changes on hydrogen bonding for water are computed. The theory, the computational methods and the basis sets used, as well as the results for water, are discussed. The results obtained are compared with those of others and with experimental estimates from the literature to determine the validity of the methods that are then used in this extended study. The results obtained here are also used to examine the validity of mixture group contribution methods for hydrogen-bonding mixtures, to develop simple estimation procedures for model parameters, and to reduce the number of calculations such as those described that need to be done.},
	number = {6},
	journal = {AIChE J.},
	author = {Wolbach, Jeffrey P. and Sandler, Stanley I.},
	year = {1997},
	pages = {1589--1596},
}

@article{wolbach_using_1997,
	title = {Using {Molecular} {Orbital} {Calculations} to {Describe} the {Phase} {Behavior} of {Hydrogen}-{Bonding} {Fluids}},
	volume = {36},
	issn = {08885885},
	doi = {10.1021/ie9607255},
	abstract = {We have used Hartree-Fock theory and density functional theory to compute the enthalpy and entropy changes of dimerization for water, methanol, and the family of carboxylic acids. These results are used in a physical equation of state, the statistical associating fluid theory (SAFT), in order to model the phase behavior of these hydrogen-bonding compounds. A procedure has been developed to relate the calculated enthalpy and entropy changes to the association parameters in SAFT using only low-pressure data, as well as to relate molar volumes from molecular orbital calculations to the segment size and chain length parameters in SAFT. By doing so, the SAFT model is reduced to a three-parameter equation of state for associating fluids. The modified equation of state is shown to be as accurate as the original SAFT model for correlating pure-component vapor-liquid equilibrium data with fewer adjustable parameters.},
	number = {10},
	journal = {Ind. Eng. Chem. Res.},
	author = {Wolbach, Jeffrey P. and Sandler, Stanley I.},
	year = {1997},
	pages = {4041--4051},
}

@article{wilson_gaussian_1999,
	title = {Gaussian basis sets for use in correlated molecular calculations. {IX}. {The} atoms gallium through krypton},
	volume = {110},
	issn = {00219606},
	doi = {10.1063/1.478678},
	abstract = {Valence correlation consistent and augmented correlation consistent basis sets have been determined for the third row, main group atoms gallium through krypton. The methodology, originally developed for the first row atoms, was first applied to the selenium atom, resulting in the expected natural groupings of correlation functions (although higher angular momentum functions tend to be relatively more important for the third row atoms as they were for the second row atoms). After testing the generality of the conclusions for the gallium atom, the procedure was used to generate correlation consistent basis sets for all of the atoms gallium through krypton. The correlation consistent basis sets for the third row main group atoms are as follows: cc-pVDZ: (14s11p6d)/[5s4p2d]; cc-PVTZ: (20s13p9d1f)/[6s5p3d1f]; cc-pVQZ: (21s16p12d2f1g)/[7s6p4d2f1g]; cc-pV5Z: (26s17p13d3f2g1h)/[8s7p5d3f2g1h]. Augmented sets were obtained by adding diffuse functions to the above sets (one for each angular momentum present in the set), with the exponents of the additional functions optimized in calculations on the atomic anions. Test calculations on the atoms as well as selected molecules with the new basis sets show good convergence to an apparent complete basis set limit. © 1999 American Institute of Physics.},
	number = {16},
	journal = {J. Chem. Phys.},
	author = {Wilson, Angela K. and Woon, David E. and Peterson, Kirk A. and Dunning, Thorn H.},
	month = apr,
	year = {1999},
	note = {Publisher: American Institute of Physics Inc.},
	pages = {7667--7676},
}

@article{wennmohs_comparative_2008,
	title = {A comparative study of single reference correlation methods of the coupled-pair type},
	volume = {343},
	issn = {03010104},
	doi = {10.1016/j.chemphys.2007.07.001},
	abstract = {Several variants of coupled electron pair type approximations are compared with respect to their accuracy in the prediction of bond distances, harmonic vibrational frequencies and anharmonic corrections for a range of closed-shell diatomic molecules. In the first part of the paper the coupled-electron pair (CEPA) methods (CEPA/1,2,3) are discussed. Extensions of these methods allow the derivation of the correlation energy from the stationarization of a correlation energy functional (CPF/1,2,3 methods). All methods are formulated as diagonally dressed configuration-interaction with single- and double-excitations (CISD) eigenvalue problems. Averaging the diagonal shifts of the CPF methods in various ways lead to the ACPF and AQCC methods. Several small modifications of the shifts for the single excitations are proposed that enhance the stability of the methods (NCPF/1,2,3, NCEPA/1,2,3, NACPF). The reduced shifts are justified by linear response arguments. The implementation of the methods for a closed-shell ground state is described. In the application part, we first tested the size-consistency, exactness for two-electron systems and unitary invariance of the methods. Extensive numerical studies with polarized quadruple-ζ basis sets are employed to test the accuracy of the coupled pair approaches relative to the more elaborate quadratic CI (QCISD) and coupled-cluster (CCSD and CCSD(T)) approaches. Not surprisingly, the CCSD(T) method is the most accurate approach on average. However, the proposed NCPF/1 variant led to even smaller average errors for bond distances (∼0.2 pm relative to ∼0.3 pm for CCSD(T)) while predicting still accurate harmonic frequencies (av. Error ∼25 cm-1 for NCPF/1, ∼8 cm-1 for CCSD(T) and ∼45 cm-1 for CCSD). All coupled pair methods are more accurate than present day DFT approaches (BP86, B3LYP). The exception is the recently proposed double-hybrid B2PLYP functional that approaches the coupled pair performance. Some more difficult copper containing diatomics are treated as well (CuH, CuF, CuCl and Cu2). We discuss why we believe that the coupled-pair approaches (and in particular the proposed NCPF/1 variant) are attractive for large-scale chemical applications. © 2007 Elsevier B.V. All rights reserved.},
	number = {2-3},
	journal = {Chem. Phys.},
	author = {Wennmohs, Frank and Neese, Frank},
	month = jan,
	year = {2008},
	keywords = {Configuration interaction, Coupled cluster approximation, Coupled pair approximation, Electron correlation},
	pages = {217--230},
}

@article{weigend_efficient_2002,
	title = {Efficient use of the correlation consistent basis sets in resolution of the identity {MP2} calculations},
	volume = {116},
	issn = {00219606},
	doi = {10.1063/1.1445115},
	number = {8},
	journal = {J. Chem. Phys.},
	author = {Weigend, Florian and Köhn, Andreas and Hättig, Christof},
	month = feb,
	year = {2002},
	pages = {3175--3183},
}

@article{wang_three-body_2006,
	title = {Three-body interactions and solid-liquid phase equilibria: {Application} of a molecular dynamics algorithm},
	volume = {74},
	issn = {15393755},
	doi = {10.1103/PhysRevE.74.031203},
	abstract = {The effect of three-body interactions on the solid-liquid phase boundaries of argon, krypton, and xenon is investigated via a novel technique that combines both nonequilibrium and equilibrium molecular dynamics. The simulations involve the evaluation of two- and three-body forces using accurate two-body and three-body intermolecular potentials. The effect of three-body interactions is to substantially increase the coexistence pressure and to lower the densities of liquid and solid phases. Comparison with experiment indicates that three-body interactions are required to accurately determine the total pressure. In contrast to vapor-liquid phase equilibria, the relative contribution of three-body interactions to the freezing pressure exceeds the contribution of two-body interactions at all temperatures. © 2006 The American Physical Society.},
	number = {3},
	journal = {Phys. Rev. E},
	author = {Wang, Liping and Sadus, Richard J.},
	year = {2006},
	pages = {1--5},
}

@article{wang_relationships_2006,
	title = {Relationships between three-body and two-body interactions in fluids and solids},
	volume = {125},
	issn = {00219606},
	doi = {10.1063/1.2353117},
	abstract = {Molecular dynamics data are reported for two-body and three-body interactions in noble gases at densities covering the gas, liquid, and solid phases. The data indicate that simple relationships exist between three- and two-body interactions in both fluid and solid phases. The relationship for liquids has a simple density dependence with only one external parameter. In contrast, the solid phase relationship depends both on density and on the square of density and requires the evaluation of two parameters. The relationships are tested for both system-size and temperature dependences. The values of the relationship parameters are only sensitive to system size when a small number of atoms are involved. For 500 or more atoms, they remain nearly constant. The relationships are valid for both subcritical and slightly supercritical temperatures. A practical benefit of the relationships is that they enable the use of two-body intermolecular potentials for the prediction of the properties of real systems without the computational expense of three-body calculations.© 2006 American Institute of Physics.},
	number = {14},
	journal = {J. Chem. Phys.},
	author = {Wang, Liping and Sadus, Richard J.},
	year = {2006},
	pages = {1--6},
}

@article{virtanen_scipy_2020,
	title = {{SciPy} 1.0: fundamental algorithms for scientific computing in {Python}},
	volume = {17},
	issn = {1548-7091},
	url = {http://www.nature.com/articles/s41592-019-0686-2},
	doi = {10.1038/s41592-019-0686-2},
	number = {3},
	journal = {Nat. Methods},
	author = {Virtanen, Pauli and Gommers, Ralf and Oliphant, Travis E. and Haberland, Matt and Reddy, Tyler and Cournapeau, David and Burovski, Evgeni and Peterson, Pearu and Weckesser, Warren and Bright, Jonathan and van der Walt, Stéfan J. and Brett, Matthew and Wilson, Joshua and Millman, K. Jarrod and Mayorov, Nikolay and Nelson, Andrew R. J. and Jones, Eric and Kern, Robert and Larson, Eric and Carey, C J and Polat, Ilhan and Feng, Yu and Moore, Eric W. and VanderPlas, Jake and Laxalde, Denis and Perktold, Josef and Cimrman, Robert and Henriksen, Ian and Quintero, E. A. and Harris, Charles R. and Archibald, Anne M. and Ribeiro, Antônio H. and Pedregosa, Fabian and van Mulbregt, Paul},
	month = mar,
	year = {2020},
	pages = {261--272},
}

@article{wang_effect_2006,
	title = {Effect of three-body interactions on the vapor-liquid phase equilibria of binary fluid mixtures},
	volume = {125},
	issn = {00219606},
	doi = {10.1063/1.2275309},
	abstract = {Gibbs-Duhem Monte Carlo simulations are reported for the vapor-liquid phase coexistence of binary argon+krypton mixtures at different temperatures. The calculations employ accurate two-body potentials in addition to contributions from three-body dispersion interactions resulting from third-order triple-dipole interactions. A comparison is made with experiment that illustrates the role of three-body interactions on the phase envelope. In all cases the simulations represent genuine predictions with input parameters obtained independently from sources other than phase equilibria data. Two-body interactions alone are insufficient to adequately describe vapor-liquid coexistence. In contrast, the addition of three-body interactions results in very good agreement with experiment. In addition to the exact calculation of three-body interactions, calculations are reported with an approximate formula for three-body interactions, which also yields good results. © 2006 American Institute of Physics.},
	number = {6},
	journal = {J. Chem. Phys.},
	author = {Wang, Liping and Sadus, Richard J.},
	year = {2006},
}

@misc{walker_orca_saft_2020,
	title = {{ORCA}\_SAFT},
	url = {https://github.com/pw0908/ORCA_SAFT},
	author = {Walker, Pierre J. and Zhao, Tianpu},
	year = {2020},
}

@article{von_muller_surface_2013,
	title = {Surface tension calculations by means of a {PCP}-{SAFT}-{DFT} formalism using equation of state parameters from quantum mechanics},
	volume = {356},
	issn = {03783812},
	doi = {10.1016/j.fluid.2013.07.005},
	abstract = {In the present work, we investigate if surface tensions of pure vapour-liquid systems can be determined predictively without the necessity of parameters adjusted to experimental data. In order to achieve this, we combine a so-called PCP-SAFT-DFT (perturbed-chain polar-statistical associating fluid theory-density functional theory) formalism with quantum mechanically obtained equation of state (EOS) parameters. We present results for some classes of non- and moderately polar substances (alkanes, ethers, aromates). For these compounds, the results are in good agreement with experimental data given that the critical point is estimated sufficiently accurate by means of the predicted EOS parameters. © 2013 Elsevier B.V.},
	journal = {Fluid Phase Equilib.},
	author = {von Müller, Alexander and Leonhard, Kai},
	month = oct,
	year = {2013},
	keywords = {Classical density functional theory, Equation of state, Statistical associating fluid theory, Surface tension},
	pages = {96--101},
}

@article{umer_efficient_2015,
	title = {Efficient yet accurate approximations for ab initio calculations of alcohol cluster thermochemistry},
	volume = {143},
	issn = {00219606},
	doi = {10.1063/1.4936406},
	abstract = {We have calculated the binding enthalpies and entropies of gas phase alcohol clusters from ethanol to 1-decanol. In addition to the monomers, we have investigated dimers, tetramers, and pentamers. Geometries have been obtained at the B3LYP/TZVP level and single point energy calculations have been performed with the Resolution of the Identity-MP2 (RIMP2) method and basis set limit extrapolation using aug-cc-pVTZ and aug-cc-pVQZ basis sets. Thermochemistry is calculated with decoupled hindered rotor treatment for large amplitude motions. The results show three points: First, it is more accurate to transfer the rigid-rotor harmonic oscillator entropies from propanol to longer alcohols than to compute them with an ultra-fine grid and tight geometry convergence criteria. Second, the computational effort can be reduced considerably by using dimerization energies of longer alcohols at density functional theory (B3LYP) level plus a RIMP2 correction obtained from 1-propanol. This approximation yields results almost with the same accuracy as RIMP2 - both methods differ for 1-decanol only 0.4 kJ/mol. Third, the entropy of dimerization including the hindered rotation contribution is converged at 1-propanol with respect to chain length. This allows for a transfer of hindered rotation contributions from smaller alcohols to longer ones which reduces the required computational and man power considerably.},
	number = {21},
	journal = {J. Chem. Phys.},
	author = {Umer, Muhammad and Kopp, Wassja A. and Leonhard, Kai},
	month = dec,
	year = {2015},
	note = {Publisher: American Institute of Physics Inc.},
}

@article{umer_pc-saft_2014,
	title = {{PC}-{SAFT} parameters from ab initio calculations},
	volume = {362},
	issn = {03783812},
	url = {http://dx.doi.org/10.1016/j.fluid.2013.08.037},
	doi = {10.1016/j.fluid.2013.08.037},
	abstract = {We use highly accurate ab initio calculations of binding enthalpies and entropies of gas phase clusters of alcohols to demonstrate how they can be used to obtain association parameters for PC-SAFT. The thermochemical results demonstrate that cooperativity effects and state dependent cluster distributions cause a strongly varying average enthalpy and entropy per bond as function of temperature and density for alcohols. In contrast to this, the two association parameters of PC-SAFT lead to density independent bond enthalpy and entropy and are thus effective parameters. Therefore, we choose to compute the cluster distribution at a universal state point and show that the thus obtained association parameters can be used to reduce the number of adjustable parameters from 5 to 3 with only a marginal loss of accuracy for most of the studied systems, and even an estimation of thermodynamic properties without adjusted parameters is possible. The ab initio calculations suggest that the 2B association scheme is more appropriate for 1-alkanols than the 3B one. © 2013 Elsevier B.V.},
	journal = {Fluid Phase Equilib.},
	author = {Umer, Muhammad and Albers, Katja and Sadowski, Gabriele and Leonhard, Kai},
	year = {2014},
	note = {Publisher: Elsevier B.V.},
	keywords = {Ab initio, Association, Predictive, SAFT},
	pages = {41--50},
}

@article{tsourtis_parameterization_2017,
	title = {Parameterization of {Coarse}-grained {Molecular} {Interactions} through {Potential} of {Mean} {Force} {Calculations} and {Cluster} {Expansion} {Techniques}: {Supplementary} {Material}},
	url = {www.mdpi.com/journal/entropy},
	doi = {10.3390/},
	abstract = {In this report, we present the model we used in the paper and show how to construct effective Coarse Grained (CG) potentials through atomistic simulations, using only a small number of atoms. The numerical algorithm is applied for the construction of CG potentials involving 2-and 3-body interactions; however, our proposed methodology is quite general and, in principle can be extended even for higher order terms. Then, we use the obtained effective potentials in CG level simulations and compare the results (specific observables) with the corresponding atomistic (projected to the Coarse level) simulations, in order to assess the efficiency and accuracy of our findings. 1. The model In more detail, we consider N molecules of CH 4 and we denote by ¯ q ≡ ¯ q 1 ,. .. , ¯ q N the positions of the N many carbons and by q i ≡ q i,1 ,. .. , q i,4 the positions of the 4 hydrogens that correspond to the i th carbon. We have two types of interactions, namely the bonded with (many body) interaction potential V b and the non-bonded with pair interaction potential V nb. The latter are of Lennard-Jones (LJ) type between all possibilities: C − C, C − H and H − H (with different coefficients), i.e., V nb = V CC + V CH + V HH. In the model used here the non-bonded interactions within the same CH 4 molecule are excluded. The microscopic canonical partition function is given by Z CH 4 = 1 N! Λ N d ¯ q (1 4!) N Λ 4N N ∏ i=1 dq i e −β(∑ N i=1 V b (¯ q i ,q i)+V nb (¯ q,q 1 ,...,q N)) , (1) where V nb is a pair potential of all possible pairs among ¯ q, q 1 ,. .. , q N , all of LJ type (eventually with different parameters). Note also that since only the 4 particles of H are indistinguishable, we have introduced the factor 1/4! for each molecule. We are interested in computing the effective Hamiltonian when only the centers of mass of the N many molecules are prescribed. Hence, let us introduce a map T : Λ 5 → Λ which gives the center of},
	journal = {Entropy},
	author = {Tsourtis, Anastasios and Harmandaris, Vagelis and Tsagkarogiannis, Dimitrios},
	year = {2017},
}

@article{trejos_semiclassical_2012,
	title = {Semiclassical approach to model quantum fluids using the statistical associating fluid theory for systems with potentials of variable range},
	volume = {136},
	issn = {00219606},
	doi = {10.1063/1.4712299},
	abstract = {Thermodynamic properties of quantum fluids are described using an extended version of the statistical associating fluid theory for potentials of variable range (SAFT-VR) that takes into account quantum corrections to the Helmholtz free energy A, based on the Wentzel-Kramers-Brillouin approximation. We present the theoretical background of this approach (SAFT-VRQ), considering two different cases depending on the continuous or discontinuous nature of the particles pair interaction. For the case of continuous potentials, we demonstrate that the standard Wigner-Kirkwood theory for quantum fluids can be derived from the de Broglie-Bohm formalism for quantum mechanics that can be incorporated within the Barker and Henderson perturbation theory for liquids in a straightforward way. When the particles interact via a discontinuous pair potential, the SAFT-VR method can be combined with the perturbation theory developed by Singh and Sinha [J. Chem. Phys. 67, 3645 (1977); Singh and Sinha J. Chem. Phys. 68, 562 (1978)]. We present an analytical expression for the first-order quantum perturbation term for a square-well potential, and the theory is applied to model thermodynamic properties of hydrogen, deuterium, neon, and helium-4. Vapor-liquid equilibrium, liquid and vapor densities, isochoric and isobaric heat capacities, Joule-Thomson coefficients and inversion curves are predicted accurately with respect to experimental data. We find that quantum corrections are important for the global behavior of properties of these fluids and not only for the low-temperature regime. Predictions obtained for hydrogen compare very favorably with respect to cubic equations of state. © 2012 American Institute of Physics.},
	number = {18},
	journal = {J. Chem. Phys.},
	author = {Trejos, Víctor M. and Gil-Villegas, Alejandro},
	year = {2012},
}

@techreport{tsuzuki_intermolecular_1998,
	title = {Intermolecular interaction potentials of methane and ethylene dimers calculated with the {Møller}-{Plesset}, coupled cluster and density functional methods},
	abstract = {Intermolecular interaction potentials of methane and ethylene dimers were calculated by the Hartree-Fock, Møller-Ples-Ž. set, coupled cluster and density functional methods. The CCSD T electron correlation energies were close to the Ž. Ž. MP4 SDTQ ones. The MP2 and MP3 energies were not largely different from the MP4 SDTQ ones. On the other hand the Ž. CCSD and MP4 SDQ methods largely underestimated the electron correlation energies. Dispersion interaction was not covered by the density functional methods using the BLYP, BPW91 and B3LYP functionals. These functionals also had defects in the evaluation of the repulsion interactions. q},
	author = {Tsuzuki, Seiji and Uchimaru, Tadafumi and Tanabe, Kazutoshi},
	year = {1998},
	note = {Publication Title: Chem. Phys. Lett.
Volume: 287},
	pages = {202--208},
}

@article{szczesniak_intermolecular_1990,
	title = {Intermolecular potential of the methane dimer and trimer},
	volume = {93},
	issn = {00219606},
	doi = {10.1063/1.458757},
	abstract = {The Heitler-London (HL) exchange energy is responsible for the anisotropy of the pair potential in methane. The equilibrium dimer structure is that which minimizes steric repulsion between hydrogens belonging to opposite subsystems. Dispersion energy, which represents a dominating attractive contribution, displays an orientation dependence which is the mirror image of that for HL exchange. The three-body correction to the pair potential is a superposition of HL and second-order exchange nonadditivities combined with the Axilrod-Teller dispersion nonadditivity. A great deal of cancellation between these terms results in near additivity of methane interactions in the long and intermediate regions. © 1990 American Institute of Physics.},
	number = {6},
	journal = {J. Chem. Phys.},
	author = {Szczȩśniak, M. M. and Cha{\textbackslash}lasiński, G. and Cybulski, S. M. and Scheiner, S.},
	year = {1990},
	pages = {4243--4253},
}

@misc{szabo_modern_1996,
	title = {Modern {Quantum} {Chemistry}: {Introduction} to {Advanced} {Electronic} {Structure} {Theory}},
	abstract = {Graduate-level text explains modern in-depth approaches to the calculation of the electronic structure and properties of molecules. Hartree-Fock approximation, electron pair approximation, much more. Largely self-contained, only prerequisite is solid course in physical chemistry. Over 150 exercises. 1989 edition.},
	author = {Szabo, A and Ostlund, N L},
	year = {1996},
}

@article{stoychev_automatic_2017,
	title = {Automatic {Generation} of {Auxiliary} {Basis} {Sets}},
	volume = {13},
	issn = {15499626},
	doi = {10.1021/acs.jctc.6b01041},
	abstract = {A procedure was developed to automatically generate auxiliary basis sets (ABSs) for use with the resolution of the identity (RI) approximation, starting from a given orbital basis set (OBS). The goal is to provide an accurate and universal solution for cases where no optimized ABSs are available. In this context, “universal” is understood as the ability of the ABS to be used for Coulomb, exchange, and correlation energy fitting. The generation scheme (denoted AutoAux) works by spanning the product space of the OBS using an even-tempered expansion for each atom in the system. The performance of AutoAux in conjunction with different OBSs [def2-SVP, def2-TZVP, def2-QZVPP, and cc-pwCVnZ (n = D, T, Q, 5)] has been evaluated for elements from H to Rn and compared to existing predefined ABSs. Due to the requirements of simplicity and universality, the generated ABSs are larger than the optimized ones but lead to similar errors in MP2 total energies (on the order of 10-5 to 10-4 Eh/atom).},
	number = {2},
	journal = {J. Chem. Theory Comput.},
	author = {Stoychev, Georgi L. and Auer, Alexander A. and Neese, Frank},
	month = feb,
	year = {2017},
	pmid = {28005364},
	note = {Publisher: American Chemical Society},
	pages = {554--562},
}

@article{skjold-jorgensen_vapor-liquid_1979,
	title = {Vapor-{Liquid} {Equilibria} by {UNIFAC} {Group} {Contribution}. {Revision} and {Extension}},
	volume = {18},
	issn = {01964305},
	doi = {10.1021/i260072a024},
	abstract = {The UNIFAC group contribution method for estimating liquid phase activity coefficients is widely used for phase equilibrium calculations. The accuracy and the range of applicability of the method is determined by the available number of reliable group parameters. New parameters are reported for eight different groups not previously covered by UNIFAC, and some of the previously published parameters have been revised based on new experimental vapor-liquid equilibrium data. The definition of the alcohol group has been modified making UNIFAC easier to use and more reliable for alcohol containing mixtures. © 1979, American Chemical Society. All rights reserved.},
	number = {4},
	journal = {Ind. Eng. Chem. Process Des. Dev.},
	author = {Skjold-Jørgensen, Steen and Kolbe, Bärbel and Gmehling, Jürgen and Rasmussen, Peter},
	year = {1979},
	pages = {714--722},
}

@article{sheldon_chapter_2006,
	title = {Chapter 7 {The} derivation of size parameters for the {SAFT}-{VR} equation of state from quantum mechanical calculations},
	volume = {22},
	issn = {15707946},
	doi = {10.1016/S1570-7946(06)80009-X},
	number = {C},
	journal = {Comput.-Aided Chem. Eng.},
	author = {Sheldon, T. J. and Giner, B. and Adjiman, C. S. and Galindo, A. and Jackson, G. and Jacquemin, D. and Wathelet, V. and Perpète, E. A.},
	year = {2006},
	pages = {143--159},
}

@article{smith_approximate_1970,
	title = {Approximate evaluation of the second-{Order} term in the perturbation theory of fluids},
	volume = {53},
	issn = {00219606},
	doi = {10.1063/1.1674017},
	abstract = {The second-order term in the free energy, A2, as given by the Barker-Henderson perturbation theory is considered for the square-well and 6:12 potentials. The second-order term is written in terms of integrals of the distribution functions of the unperturbed hard-sphere system. If the superposition approximation is used for the third- and fourth-order distribution functions, these integrals may be evaluated fairly easily and values for A 2 may be obtained. Comparison of these values with either the exact second-order term Monte Carlo calculations of the exact second-order term gives exact agreement for the lattice gas, fairly good agreement for the square-well potential, and good agreement for the 6:12 potential.},
	number = {2},
	journal = {J. Chem. Phys.},
	author = {Smith, W. R. and Henderson, D. and Barker, J. A.},
	year = {1970},
	pages = {508--515},
}

@article{schoen_liquid_1986,
	title = {Liquid {CH4}, liquid {CF4} and the partially miscible liquid mixture {CH4}/{CF4}: {A} molecular dynamics study based on both a spherically symmetric and a four-centre lennard-jones potential model},
	volume = {58},
	issn = {13623028},
	doi = {10.1080/00268978600101511},
	abstract = {The partially miscible liquid mixture CH4/CF4 was simulated using molecular dynamics calculations based on one-centre Lennard-Jones (LJ) potential functions and four-centre LJ potentials. The calculations with the latter potential model were performed with a fully vectorized molecular dynamics program exploiting constraints for the solution of the equations of motion for the molecules. The simulated static and dynamic properties of both the mixtures and the pure liquids are reasonably comparable with those of the real systems. Particularly, the phase separation of the mixture occurs in the range where it is observable in the real CH4/CF4 mixture. Given the limited test of the present study, both potential models are equally suitable for the simulation of this non-ideal mixture, where the unlike interaction parameters are chosen as proposed in [1]. However, while the spherically symmetric potential gives better pressures, the four sites potential model is preferable for the dynamic quantities in comparison with experiment. This is in good agreement with earlier simulation studies on other molecular systems. © 1986 Taylor \& Francis Group, LLC.},
	number = {4},
	journal = {Mol. Phys.},
	author = {Schoen, M. and Hoheisel, C. and Beyer, O.},
	year = {1986},
	pages = {699--709},
}

@article{schneider_decomposition_2016,
	title = {Decomposition of {Intermolecular} {Interaction} {Energies} within the {Local} {Pair} {Natural} {Orbital} {Coupled} {Cluster} {Framework}},
	volume = {12},
	issn = {15499626},
	doi = {10.1021/acs.jctc.6b00523},
	abstract = {The local coupled cluster method DLPNO-CCSD(T) allows calculations on systems containing hundreds of atoms to be performed while typically reproducing canonical CCSD(T) energies with chemical accuracy. In this work, we present a scheme for decomposing the DLPNO-CCSD(T) interaction energy between two molecules into physical meaningful contributions, providing a quantification of the most important components of the chemical interaction. The method, called Local Energy Decomposition (LED), is straightforward and requires negligible additional computing time. Both the Hartree-Fock and the correlation energy are decomposed into contributions from localized or pairs of localized occupied orbitals. Assigning these localized orbitals to fragments allows one to differentiate between intra- and intermolecular contributions to the interaction energy. Accordingly, the interaction energy can be decomposed into electronic promotion, electrostatic, exchange, dynamic charge polarization, and dispersion contributions. The LED scheme is applied to a number of test cases ranging from weakly, dispersively bound complexes to systems with strong ionic interactions. The dependence of the results on the one-particle basis set and various technical aspects, such as the localization scheme, are carefully studied in order to ensure that the results do not suffer from technical artifacts. A numerical comparison between the DLPNO-CCSD(T)/LED and the popular symmetry adapted perturbation theory (DFT-SAPT) is made, and the limitations of the proposed scheme are discussed.},
	number = {10},
	journal = {J. Chem. Theory Comput.},
	author = {Schneider, Wolfgang B. and Bistoni, Giovanni and Sparta, Manuel and Saitow, Masaaki and Riplinger, Christoph and Auer, Alexander A. and Neese, Frank},
	year = {2016},
	pages = {4778--4792},
}

@article{rowlinson_dipole_1958,
	title = {Dipole interactions in fluids and fluid mixtures},
	volume = {1},
	issn = {13623028},
	doi = {10.1080/00268975800100501},
	number = {4},
	journal = {Mol. Phys.},
	author = {Rowlinson, J. S.},
	year = {1958},
	pages = {414--415},
}

@article{riplinger_natural_2013,
	title = {Natural triple excitations in local coupled cluster calculations with pair natural orbitals},
	volume = {139},
	issn = {00219606},
	doi = {10.1063/1.4821834},
	abstract = {In this work, the extension of the previously developed domain based local pair-natural orbital (DLPNO) based singles- and doubles coupled cluster (DLPNO-CCSD) method to perturbatively include connected triple excitations is reported. The development is based on the concept of triples-natural orbitals that span the joint space of the three pair natural orbital (PNO) spaces of the three electron pairs that are involved in the calculation of a given triple-excitation contribution. The truncation error is very smooth and can be significantly reduced through extrapolation to the zero threshold. However, the extrapolation procedure does not improve relative energies. The overall computational effort of the method is asymptotically linear with the system size O(N). Actual linear scaling has been confirmed in test calculations on alkane chains. The accuracy of the DLPNO-CCSD(T) approximation relative to semicanonical CCSD(T0) is comparable to the previously developed DLPNO-CCSD method relative to canonical CCSD. Relative energies are predicted with an average error of approximately 0.5 kcal/mol for a challenging test set of medium sized organic molecules. The triples correction typically adds 30\%-50\% to the overall computation time. Thus, very large systems can be treated on the basis of the current implementation. In addition to the linear C 150H302 (452 atoms, {\textgreater}8800 basis functions) we demonstrate the first CCSD(T) level calculation on an entire protein, Crambin with 644 atoms, and more than 6400 basis functions. © 2013 AIP Publishing LLC.},
	number = {13},
	journal = {J. Chem. Phys.},
	author = {Riplinger, Christoph and Sandhoefer, Barbara and Hansen, Andreas and Neese, Frank},
	year = {2013},
	pmid = {24116546},
	pages = {134101},
}

@article{ravipati_investigation_2019,
	title = {An investigation of free-energy-averaged (coarse-grained) potentials for fluid adsorption on heterogeneous solid surfaces},
	volume = {21},
	issn = {14639076},
	doi = {10.1039/c9cp02601k},
	abstract = {Coarse-grained, two-body fluid-solid potentials provide a simple way to describe the interaction between a fluid molecule and a solid in adsorption theories, and also a means to reduce the computational expense in molecular simulations, compared to those employing full atomistic detail. Here we investigate the applicability of a recently proposed mapping procedure to obtain free-energy-averaged (FEA) fluid-solid interactions for fluids on various heterogeneous surfaces. Methane and graphite are chosen as the fluid and the solid, respectively, and the surface graphene layer is modified to create chemical and geometrical heterogeneities; for the latter surfaces, the FEA mapping is appropriately modified to account for vacancies. Adsorption isotherms and fluid density profiles are obtained by performing grand canonical Monte Carlo (GCMC) simulations for explicit-solid and FEA-potential representations, and are compared to gain insights about the applicability and limitations of the FEA potentials. For solids with homogeneous and chemically heterogeneous surfaces, adsorption isotherms and density profiles obtained using FEA potentials are in good agreement with those obtained using an explicit-solid representation. For surfaces containing vacancies, isotherms and density profiles obtained using the unmodified FEA potential differ significantly from their explicit-surface analogues. When using the FEA potential obtained with the modified mapping procedure some deviations are still seen at very high pressure, however, at low to moderate pressures, agreement is, once again, good.},
	number = {46},
	journal = {Phys. Chem. Chem. Phys.},
	author = {Ravipati, Srikanth and Galindo, Amparo and Jackson, George and Haslam, Andrew J.},
	year = {2019},
	pmid = {31538169},
	note = {Publisher: Royal Society of Chemistry},
	pages = {25558--25568},
}

@misc{pse_process_2020,
	title = {Process {Systems} {Enterprise}, {gPROMS}},
	url = {www.psenterprise.com/products/gproms},
	urldate = {2020-10-13},
	author = {{PSE}},
	year = {2020},
}

@article{pothoczki_structure_2015,
	title = {Structure of {Neat} {Liquids} {Consisting} of ({Perfect} and {Nearly}) {Tetrahedral} {Molecules}},
	volume = {115},
	issn = {15206890},
	doi = {10.1021/acs.chemrev.5b00308},
	number = {24},
	journal = {Chem. Rev.},
	author = {Pothoczki, Szilvia and Temleitner, László and Pusztai, László},
	year = {2015},
	note = {Publisher: American Chemical Society},
	pages = {13308--13361},
}

@article{platts_estimation_2000,
	title = {Estimation of {Molecular} {Linear} {Free} {Energy} {Relationship} {Descriptors} by a {Group} {Contribution} {Approach}. 2. {Prediction} of {Partition} {Coefficients}},
	volume = {40},
	issn = {00952338},
	doi = {10.1021/ci990427t},
	abstract = {A previously published method for the prediction of molecular linear free energy relationship descriptors is tested against experimentally determined partition coefficients in various solvent systems. Sets of partition data between water and octanol, cyclohexane, and chloroform were taken from the literature. For each set of partition data used, r2 values ranged from 0.8 to 0.9 and RMS errors from 0.7 to 1.0 log unit, comparable to errors obtained with previously published models for octanol-water partition. Modified solvation equations for water-octanol and water-cyclohexane partition are presented, and their implications discussed. The possibility of applying the current approach to a wide range of solvation and transport properties is put forward.},
	number = {1},
	journal = {J. Chem. Inf. Model.},
	author = {Platts, James A. and Abraham, Michael H. and Butina, Darko and Hersey, Anne},
	year = {2000},
	pages = {71--80},
}

@article{peters_development_2012,
	title = {Development of a group contribution method for polymers within the {PC}-{SAFT} model},
	volume = {324},
	issn = {03783812},
	url = {http://dx.doi.org/10.1016/j.fluid.2012.03.009},
	doi = {10.1016/j.fluid.2012.03.009},
	abstract = {Based on the PC-SAFT equation of state (EOS) a group contribution method (GCM) for polymers is developed to describe thermodynamic properties of the pure polymers as well as binary (co-)polymer/solvent liquid-liquid phase equilibria (LLE). The polymer parameters are obtained from group contributions by applying simple arithmetic and geometric mixing rules. Polymer classes of poly(olefines), poly(acrylates) as well as poly(methacrylates) are considered leading to the parameter set for five specific groups CH 3, {\textgreater}CH 2, {\textgreater}(CH) and {\textgreater}C{\textless} as well as the (CO)O group. The modeling approach is applied to pure polymer density and binary LLE data. Modeling results using the GCM polymer parameters are found to be in good agreement with experimental literature data. © 2012 Elsevier B.V.},
	journal = {Fluid Phase Equilib.},
	author = {Peters, Felix T. and Laube, Franziska S. and Sadowski, Gabriele},
	year = {2012},
	note = {Publisher: Elsevier B.V.},
	keywords = {Group contribution method, Liquid density, Liquid-liquid phase equilibrium, PC-SAFT, Polymer},
	pages = {70--79},
}

@article{pas_energy_2010,
	title = {Energy {Curves} for {Heavy} {Rare} {Gas} {Dimers} : and},
	volume = {2102},
	number = {April 2003},
	author = {Pas, Petr},
	year = {2010},
}

@article{pollock_systematic_2008,
	title = {Systematic approaches to the development of thermodynamic models for associating fluids and their mixtures},
	volume = {2008},
	number = {July},
	author = {Pollock, Michaela},
	year = {2008},
}

@article{pinski_analytical_2019,
	title = {Analytical gradient for the domain-based local pair natural orbital second order {Møller}-{Plesset} perturbation theory method ({DLPNO}-{MP2})},
	volume = {150},
	issn = {00219606},
	doi = {10.1063/1.5086544},
	abstract = {Building upon our previously published work [P. Pinski and F. Neese, J. Chem. Phys. 148, 031101 (2018)], we derive the formally complete analytical gradient for the domain-based local pair natural orbital second order Møller-Plesset (MP2) perturbation theory method. Extensive testing of geometry optimizations shows that the deviations from resolution of the identity-based MP2 structures are small. Covalent bond lengths are reproduced to within 0.1 pm, whereas errors in interatomic distances between noncovalently interacting system parts do not exceed 1\% with default truncation thresholds and 0.3\% with tight thresholds. Moreover, we introduce a procedure to circumvent instabilities of the gradient caused by singular coupled-perturbed localization equations, as they occur for some symmetric systems with continuously degenerate localized orbitals. The largest system for which a geometry optimization was completed is a host-guest complex with over 200 atoms and more than 4000 basis functions (triple-zeta basis). The most demanding single-point gradient calculation was performed for the small protein crambin containing 644 atoms and over 12 000 basis functions.},
	number = {16},
	journal = {J. Chem. Phys.},
	author = {Pinski, Peter and Neese, Frank},
	month = apr,
	year = {2019},
	pmid = {31042903},
	note = {Publisher: American Institute of Physics Inc.},
	pages = {164102},
}

@article{peters_extension_2013,
	title = {Extension of the {PC}-{SAFT} based group contribution method for polymers to aromatic, oxygen- and silicon-based polymers},
	volume = {339},
	issn = {03783812},
	url = {http://dx.doi.org/10.1016/j.fluid.2012.11.031},
	doi = {10.1016/j.fluid.2012.11.031},
	abstract = {A PC-SAFT group contribution method (GCM) for polymers developed earlier [10] is extended to aromatic, oxygen- and silicon-based (co-)polymers. Polymer parameters are determined using group contributions and applying simple arithmetic and geometric combination rules. Group contributions for six new groups are identified and parameterized: {\textgreater}CHAr, {\textgreater}CAr, O, {\textgreater}CO, OH and {\textgreater}Si{\textless}. The parameterization method is applied to liquid density and binary liquid-liquid equilibria and vapor-liquid equilibria as well as to excess enthalpies of polymers containing aromatic, oxygen- and silicon-containing monomer units in an extended spectrum of nonpolar, polar and associating solvents. Modeling results using both, GCM and fitted polymer parameters, show equally-good agreement with experimental data. © 2012 Elsevier B.V.},
	journal = {Fluid Phase Equilib.},
	author = {Peters, Felix T. and Herhut, Marcel and Sadowski, Gabriele},
	year = {2013},
	note = {Publisher: Elsevier B.V.},
	keywords = {Group contribution method, Liquid density, PC-SAFT, Phase equilibrium, Polymers},
	pages = {89--104},
}

@article{paricaud_general_2006,
	title = {A general perturbation approach for equation of state development: {Applications} to simple fluids, ab initio potentials, and fullerenes},
	volume = {124},
	issn = {00219606},
	doi = {10.1063/1.2181979},
	abstract = {A new perturbation scheme based on the Barker-Henderson perturbation theory [J. Chem. Phys. 47, 4714 (1967)] is proposed to predict the thermodynamic properties of spherical molecules. Accurate predictions of second virial coefficients and vapor-liquid coexistence properties are obtained for a large variety of potential functions (square well, Yukawa, Sutherland, Lennard-Jones, Buckingham, Girifalco). New Gibbs ensemble Monte Carlo simulations of the generalized exp- m Buckingham potential are reported. An extension of the perturbation approach to mixtures is proposed, and excellent predictions of vapor-liquid equilibria are obtained for Lennard-Jones mixtures. The perturbation scheme can be applied to complex potential functions fitted to ab initio data to predict the properties of real molecules such as neon. The new approach can also be used as an auxiliary tool in molecular simulation studies, to efficiently optimize an intermolecular potential on macroscopic properties or match force fields based on different potential functions. © 2006 American Institute of Physics.},
	number = {15},
	journal = {J. Chem. Phys.},
	author = {Paricaud, Patrice},
	year = {2006},
	pages = {154505},
}

@article{pahl_importance_2009,
	title = {The importance of accurate interaction potentials in the melting of argon nanoclusters},
	volume = {109},
	issn = {00207608},
	doi = {10.1002/qua.21976},
	abstract = {The melting temperatures of argon clusters ArN (N = 13, 55, 147, 309, 561, and 923) and of bulk argon have been obtained from exchange Monte Carlo simulations and are compared using different two-body interaction potentials, namely the standard Lennard-Jones (LJ), Aziz and extended Lennard-Jones (ELJ) potentials. The latter potential has many advantages: while maintaining the computational efficiency of the commonly used LJ potential, it is as accurate as the Aziz potential but the computer time scales more favorably with increasing cluster size. By applying the ELJ form and extrapolating the cluster data to the infinite system, we are able to extract the melting point of argon already in good agreement with experimental measurements. By considering the additional Axilrod-Teller three-body contribution as well, we calculate a melting temperature of ℡Jmelt = 84.7 K compared to the experimental value of Texpmelt = 83.85 K, whereas the LJ potential underestimates the melting point by more than 7 K. Thus melting temperatures within 1 K accuracy are now feasible. © 2009 Wiley Periodicals, Inc.},
	number = {9},
	journal = {Int. J. Quantum Chem.},
	author = {Pahl, E. and Calvo, F. and Schwerdtfeger, P.},
	year = {2009},
	keywords = {Melting, Monte Carlo simulation, Rare gas cluster},
	pages = {1812--1819},
}

@article{papadopoulos_approach_2020,
	title = {An approach for simultaneous computer-aided molecular design with holistic sustainability assessment: {Application} to phase-change {CO2} capture solvents},
	volume = {135},
	issn = {00981354},
	doi = {10.1016/j.compchemeng.2020.106769},
	abstract = {We propose an approach for the simultaneous consideration of a holistic sustainability assessment framework in computer-aided molecular design (CAMD). The framework supports the assessment of life cycle (LCA) and safety, hazard and environmental (EHS) impacts from cradle-to-gate of chemicals designed through CAMD. It enables the calculation of a total of 11 sustainability-related indicators, aggregating several impact categories. A lack of models and data gaps in property prediction are addressed through a data mining approach which deploys on-line similarity assessment against existing molecules. The LCA and EHS assessment are conducted simultaneously with CAMD or after CAMD to assess the designed solvents. A case study is presented on the design of phase-change solvents for chemisorption-based post-combustion CO2 capture. The proposed approach identifies verifiably useful phase-change solvents that exhibit favourable performance trade-offs compared to a reference CO2 capture solvent. The on-line use in CAMD of sustainability criteria favours the design of hydroxyl-containing solvents.},
	journal = {Comput. Chem. Eng.},
	author = {Papadopoulos, Athanasios I. and Shavalieva, Gulnara and Papadokonstantakis, Stavros and Seferlis, Panos and Perdomo, Felipe A. and Galindo, Amparo and Jackson, George and Adjiman, Claire S.},
	year = {2020},
	note = {Publisher: Elsevier Ltd},
	keywords = {CO2 capture, Computer-aided molecular design, Solvents, Sustainability assessment},
	pages = {106769},
}

@article{pai_ab_2014,
	title = {Ab initio potential energy surface for methane and carbon dioxide and application to vapor-liquid coexistence},
	volume = {141},
	issn = {00219606},
	doi = {10.1063/1.4891983},
	abstract = {A six-dimensional intermolecular potential energy surface for a rigid methane (CH4) and carbon dioxide (CO2) dimer was developed from the counterpoise-corrected supermolecular approach at the CCSD(T) level of theory. A total of 466 grid points distributed to 46 orientations were calculated from the complete basis set limit extrapolation based on up to aug-cc-pVQZ basis set. A modified site-site pair potential function was proposed for rapid representation of the high level ab initio calculations. A nonadditive three-body interaction was represented by the Axilrod-Teller-Muto expression for mixtures with the polarizability and the London dispersion constant of each molecule. Second to fourth virial coefficients of CH 4 and CO2 mixtures were calculated using both the Mayer sampling Monte Carlo method and the present potential functions. The virial equation of state derived from these coefficients was used to predict the pVT values and showed good agreement with experimental data below 200 bar at 300 K. The vapor-liquid coexistence curves of pure CH4, CO2 and their mixtures were presented with the aid of Gibbs ensemble Monte Carlo simulations. The predicted tie lines agreed with the experimental data within the uncertainties up to near the critical point. © 2014 AIP Publishing LLC.},
	number = {6},
	journal = {J. Chem. Phys.},
	author = {Pai, Sung Jin and Bae, Young Chan},
	month = aug,
	year = {2014},
	note = {Publisher: American Institute of Physics Inc.},
}

@article{pack_first_1982,
	title = {First quantum corrections to second virial coefficients for anisotropic interactions: {Simple}, corrected formula},
	volume = {78},
	issn = {00219606},
	doi = {10.1063/1.444762},
	abstract = {A simple formula for the first quantum correction to the second virial coefficient, valid for the interaction of any like or unlike combination of atoms, diatomics, spherical top, or symmetric top molecules is given. It is found that the commonly used formulas of Wang Chang contain an error that omits an anisotropic contribution. The sizes of the different contributions to the quantum correction are discussed. As examples, calculations for He-SF6 and He-CO2 are reported. © 1983 American Institute of Physics.},
	number = {12},
	journal = {J. Chem. Phys.},
	author = {Pack, Russell T.},
	year = {1982},
	pages = {7217--7222},
}

@article{oboyle_open_2011,
	title = {Open {Babel}: {An} {Open} chemical toolbox},
	volume = {3},
	issn = {17582946},
	doi = {10.1186/1758-2946-3-33},
	abstract = {Background: A frequent problem in computational modeling is the interconversion of chemical structures between different formats. While standard interchange formats exist (for example, Chemical Markup Language) and de facto standards have arisen (for example, SMILES format), the need to interconvert formats is a continuing problem due to the multitude of different application areas for chemistry data, differences in the data stored by different formats (0D versus 3D, for example), and competition between software along with a lack of vendorneutral formats. Results: We discuss, for the first time, Open Babel, an open-source chemical toolbox that speaks the many languages of chemical data. Open Babel version 2.3 interconverts over 110 formats. The need to represent such a wide variety of chemical and molecular data requires a library that implements a wide range of cheminformatics algorithms, from partial charge assignment and aromaticity detection, to bond order perception and canonicalization. We detail the implementation of Open Babel, describe key advances in the 2.3 release, and outline a variety of uses both in terms of software products and scientific research, including applications far beyond simple format interconversion. Conclusions: Open Babel presents a solution to the proliferation of multiple chemical file formats. In addition, it provides a variety of useful utilities from conformer searching and 2D depiction, to filtering, batch conversion, and substructure and similarity searching. For developers, it can be used as a programming library to handle chemical data in areas such as organic chemistry, drug design, materials science, and computational chemistry. It is freely available under an open-source license from http://openbabel.org. © 2011 O'Boyle et al; licensee Chemistry Central Ltd.},
	number = {10},
	journal = {J. Cheminf.},
	author = {O'Boyle, Noel M. and Banck, Michael and James, Craig A. and Morley, Chris and Vandermeersch, Tim and Hutchison, Geoffrey R.},
	month = oct,
	year = {2011},
	pmid = {21982300},
	pages = {33},
}

@article{neese_orca_2020,
	title = {The {ORCA} quantum chemistry program package},
	volume = {152},
	issn = {10897690},
	doi = {10.1063/5.0004608},
	abstract = {In this contribution to the special software-centered issue, the ORCA program package is described. We start with a short historical perspective of how the project began and go on to discuss its current feature set. ORCA has grown into a rather comprehensive general-purpose package for theoretical research in all areas of chemistry and many neighboring disciplines such as materials sciences and biochemistry. ORCA features density functional theory, a range of wavefunction based correlation methods, semi-empirical methods, and even force-field methods. A range of solvation and embedding models is featured as well as a complete intrinsic to ORCA quantum mechanics/molecular mechanics engine. A specialty of ORCA always has been a focus on transition metals and spectroscopy as well as a focus on applicability of the implemented methods to "real-life" chemical applications involving systems with a few hundred atoms. In addition to being efficient, user friendly, and, to the largest extent possible, platform independent, ORCA features a number of methods that are either unique to ORCA or have been first implemented in the course of the ORCA development. Next to a range of spectroscopic and magnetic properties, the linear- or low-order single- and multi-reference local correlation methods based on pair natural orbitals (domain based local pair natural orbital methods) should be mentioned here. Consequently, ORCA is a widely used program in various areas of chemistry and spectroscopy with a current user base of over 22 000 registered users in academic research and in industry.},
	number = {22},
	journal = {J. Chem. Phys.},
	author = {Neese, Frank and Wennmohs, Frank and Becker, Ute and Riplinger, Christoph},
	month = jun,
	year = {2020},
	pmid = {32534543},
	note = {Publisher: NLM (Medline)},
	pages = {224108},
}

@article{neese_orca_2012,
	title = {The {ORCA} program system},
	volume = {2},
	issn = {17590876},
	doi = {10.1002/wcms.81},
	abstract = {ORCA is a general-purpose quantum chemistry program package that features virtually all modern electronic structure methods (density functional theory, many-body perturbation and coupled cluster theories, and multireference and semiempirical methods). It is designed with the aim of generality, extendibility, efficiency, and user friendliness. Its main field of application is larger molecules, transition metal complexes, and their spectroscopic properties. ORCA uses standard Gaussian basis functions and is fully parallelized. The article provides an overview of its current possibilities and documents its efficiency. © 2011 John Wiley \& Sons, Ltd.},
	number = {1},
	journal = {Wiley Interdiscip. Rev.: Comput. Mol. Sci.},
	author = {Neese, Frank},
	month = jan,
	year = {2012},
	pages = {73--78},
}

@article{neese_software_2018,
	title = {Software update: the {ORCA} program system, version 4.0},
	volume = {8},
	issn = {17590884},
	doi = {10.1002/wcms.1327},
	abstract = {This short update provides an overview of the capabilities that have been added to the ORCA electronic structure package (version 4.0) since publication of the first article in 2012. WIREs Comput Mol Sci 2018, 8:e1327. doi: 10.1002/wcms.1327. This article is categorized under: Electronic Structure Theory {\textgreater} Ab Initio Electronic Structure Methods Electronic Structure Theory {\textgreater} Density Functional Theory Software {\textgreater} Quantum Chemistry.},
	number = {1},
	journal = {Wiley Interdiscip. Rev.: Comput. Mol. Sci.},
	author = {Neese, Frank},
	year = {2018},
	note = {Publisher: Blackwell Publishing Inc.},
	pages = {e1327},
}

@article{nasrabad_computational_2006,
	title = {Computational studies on thermodynamic properties, effective diameters, and free volume of argon using an ab initio potential},
	volume = {125},
	issn = {00219606},
	doi = {10.1063/1.2338310},
	abstract = {A quantum mechanical derived ab initio interaction potential for the argon dimer was tested in molecular simulations to reproduce the thermophysical properties of the vapor-liquid phase equilibria using the Gibbs ensemble Monte Carlo simulations as well as the liquid and supercritical equation of state using the NVT Monte Carlo simulations. The ab initio interaction potential was taken from the literature. A recently developed theory [R. Laghaei et al., J. Chem. Phys. 124, 154502 (2006)] was used to compute the effective diameters of argon in fluid phases and the results were subsequently applied in the generic van der Waals theory to compute the free volume of argon. The calculated densities of the coexisting phases, the vapor pressure, and the equation of state show excellent agreement with experimental values. The effective diameters and free volumes of argon are given over a wide range of densities and temperatures. An empirical formula was used to fit the effective diameters as a function of density and temperature. The computed free volume will be used in future investigations to calculate the transport properties of argon. © 2006 American Institute of Physics.},
	number = {8},
	journal = {J. Chem. Phys.},
	author = {Nasrabad, Afshin Eskandari and Laghaei, Rozita},
	year = {2006},
}

@article{neese_orca_2019,
	title = {{ORCA} {Version} 4.2.1 {Manual}},
	author = {Neese, Frank and Wennmohs, Frank and Aravena, Daniel and Atanasov, Michael and Becker, Ute and Bistoni, Giovanni and Bykov, Dmytro and Chilkuri, Vijay G and Datta, Dipayan and Kumar Dutta, Achintya and Ganyushin, Dmitry and Garcia, Miquel and Guo, Yang and Hansen, Andreas and Helmich-Paris, Benjamin and Huntington, Lee and Izsák, Róbert and Kollmar, Christian and Kossmann, Simone and Krupička, Martin and Lang, Lucas and Lenk, Dagmar and Liakos, Dimitrios G and Manganas, Dimitrios and Pantazis, Dimitrios A and Petrenko, Taras and Pinski, Peter and Reimann, Christoph and Retegan, Marius and Riplinger, Christoph and Risthaus, Tobias and Roemelt, Michael and Saitow, Masaaki and Sandhöfer, Barbara and Schapiro, Igor and Sivalingam, Kantharuban and De Souza, Bernardo and Stoychev, Georgi and Van Den Heuvel, Willem and Wezisla, Boris and Kállay, Mihály and Grimme, Stefan and Valeev, Edward and Chan, Garnet and Pittner, Jiri and Brehm, Martin and Goerigk, Lars and Vilhjálmuråsgeirsson, Vilhjálmur and Schneider, Wolfgang},
	year = {2019},
}

@article{marcelli_link_2000,
	title = {A link between the two-body and three-body interaction energies of fluids from molecular simulation},
	volume = {112},
	issn = {00219606},
	doi = {10.1063/1.481199},
	abstract = {Molecular simulation data are reported that indicate that there is a simple empirical relationship between two-body and three-body interaction energies. The significance of this relationship is that three-body interactions can be estimated accurately from two-body interactions without incurring the computational penalty of three-body calculations. The relationship is tested by performing Gibbs ensemble simulations for the vapor-liquid equilibria of argon. The results are in good agreement with calculations that explicitly evaluate all three-body interactions. © 2000 American Institute of Physics.},
	number = {14},
	journal = {J. Chem. Phys.},
	author = {Marcelli, Gianluca and Sadus, Richard J.},
	year = {2000},
	pages = {6382--6385},
}

@article{mccabe_application_2004,
	title = {Application of crossover theory to the {SAFT}-{VR} equation of state: {SAFT}-{VRX} for pure fluids},
	volume = {43},
	issn = {08885885},
	doi = {10.1021/ie034288n},
	abstract = {The molecular-based SAFT equation of state has proven to be very versatile in the prediction of fluid phase equilibria. However, in common with all analytic equations of state, SAFT exhibits classical behavior in the critical region rather than the nonanalytical, singular behavior seen in real fluids. As a result, accurate agreement over the whole phase diagram cannot be obtained and must be localized to either the critical or subcritical regions. To overcome this problem, we have combined the SAFT-VR equation of state with a crossover technique developed by Kiselev (Kiselev, S. B. Fluid Phase Equilib. 1998, 147, 7) to obtain the SAFT-VRX equation. We have applied SAFT-VRX to both associating and nonassociating pure fluids. Results are presented for n-alkanes, water, and carbon dioxide. Furthermore, by fitting to the phase diagram and PVT behavior for a small number of n-alkanes, we have developed simple expressions for the potential model parameters for the n-alkane homologous series. These prescriptions enable the accurate prediction of the thermodynamic properties, including the phase diagram, of n-alkanes without additional fitting to experimental data. Additionally, by combining density functional theory with SAFT-VRX we predict the surface tension of both low and high molecular weight n-alkanes.},
	number = {11},
	journal = {Ind. Eng. Chem. Res.},
	author = {McCabe, Clare and Kiselev, Sergei B.},
	year = {2004},
	pages = {2839--2851},
}

@article{llovell_thermodynamic_2004,
	title = {Thermodynamic properties of {Lennard}-{Jones} chain molecules: {Renormalization}-group corrections to a modified statistical associating fluid theory},
	volume = {121},
	issn = {00219606},
	doi = {10.1063/1.1809112},
	abstract = {A modified version of the statistical associating fluid theory (SAFT), the so-called soft-SAFT equation of state (EOS), has been extended by a crossover treatment to take into account the long density fluctuations encountered when the critical region is approached. The procedure, based on White's work from the renormalization group theory [Fluid Phase Equilibria 75, 53 (1992); L. W. Salvino and J. A. White, J. Chem. Phys. 96, 4559 (1992)], is implemented in terms of recursion relations where the density fluctuations are successively incorporated. The crossover soft-SAFT equation provides the correct nonclassical critical exponents when approaching the critical point, and reduces to the original soft-SAFT equation far from the critical region. The accuracy of the global equation is tested by direct comparison with molecular simulation results of Lennard-Jones chains, obtaining very good agreement and clear improvements compared to the original soft-SAFT EOS. Excellent agreement with vapor-liquid equilibrium experimental data inside and outside the critical region for the n-alkane series is also obtained. We provide a set of transferable molecular parameters for this family, unique for the whole range of thermodynamic properties. © 2004 American Institute of Physics.},
	number = {21},
	journal = {J. Chem. Phys.},
	author = {Llovell, Fèlix and Pàmies, Josep C. and Vega, Lourdes F.},
	month = dec,
	year = {2004},
	pages = {10715--10724},
}

@article{liakos_is_2015,
	title = {Is {It} {Possible} to {Obtain} {Coupled} {Cluster} {Quality} {Energies} at near {Density} {Functional} {Theory} {Cost}? {Domain}-{Based} {Local} {Pair} {Natural} {Orbital} {Coupled} {Cluster} vs {Modern} {Density} {Functional} {Theory}},
	volume = {11},
	issn = {15499626},
	doi = {10.1021/acs.jctc.5b00359},
	abstract = {The recently developed domain-based local pair natural orbital coupled cluster theory with single, double, and perturbative triple excitations (DLPNO-CCSD(T)) delivers results that are closely approaching those of the parent canonical coupled cluster method at a small fraction of the computational cost. A recent extended benchmark study established that, depending on the three main truncation thresholds, it is possible to approach the canonical CCSD(T) results within 1 kJ (default setting, TightPNO), 1 kcal/mol (default setting, NormalPNO), and 2-3 kcal (default setting, LoosePNO). Although thresholds for calculations with TightPNO are 2-4 times slower than those based on NormalPNO thresholds, they are still many orders of magnitude faster than canonical CCSD(T) calculations, even for small and medium sized molecules where there is little locality. The computational effort for the coupled cluster step scales nearly linearly with system size. Since, in many instances, the coupled cluster step in DLPNO-CCSD(T) is cheaper or at least not much more expensive than the preceding Hartree-Fock calculation, it is useful to compare the method against modern density functional theory (DFT), which requires an effort comparable to that of Hartree-Fock theory (at least if Hartree-Fock exchange is part of the functional definition). Double hybrid density functionals (DHDF's) even require a MP2-like step. The purpose of this article is to evaluate the cost vs accuracy ratio of DLPNO-CCSD(T) against modern DFT (including the PBE, B3LYP, M06-2X, B2PLYP, and B2GP-PLYP functionals and, where applicable, their van der Waals corrected counterparts). To eliminate any possible bias in favor of DLPNO-CCSD(T), we have chosen established benchmark sets that were specifically proposed for evaluating DFT functionals. It is demonstrated that DLPNO-CCSD(T) with any of the three default thresholds is more accurate than any of the DFT functionals. Furthermore, using the aug-cc-pVTZ basis set and the LoosePNO default settings, DLPNO-CCSD(T) is only about 1.2 times slower than B3LYP. With NormalPNO thresholds, DLPNO-CCSD(T) is about a factor of 2 slower than B3LYP and shows a mean absolute deviation of less than 1 kcal/mol to the reference values for the four different data sets used. Our conclusion is that coupled cluster energies can indeed be obtained at near DFT cost.},
	number = {9},
	journal = {J. Chem. Theory Comput.},
	author = {Liakos, Dimitrios G. and Neese, Frank},
	month = sep,
	year = {2015},
	pmid = {26575901},
	note = {Publisher: American Chemical Society},
	pages = {4054--4063},
}

@article{llovell_incorporating_2015,
	title = {Incorporating critical divergence of isochoric heat capacity into the soft-{SAFT} equation of state},
	volume = {61},
	issn = {00011541},
	doi = {10.1002/aic.14911},
	number = {9},
	journal = {AIChE J.},
	author = {Llovell, Fèlix and Vega, Lourdes F. and Anisimov, Mikhail A. and Sengers, Jan V.},
	month = sep,
	year = {2015},
	pages = {3073--3080},
}

@article{liakos_exploring_2015,
	title = {Exploring the accuracy limits of local pair natural orbital coupled-cluster theory},
	volume = {11},
	issn = {15499626},
	doi = {10.1021/ct501129s},
	abstract = {The domain based local pair natural orbital coupled cluster method with single-, double-, and perturbative triple excitations (DLPNO-CCSD(T)) is an efficient quantum chemical method that allows for coupled cluster calculations on molecules with hundreds of atoms. Because coupled-cluster theory is the method of choice if high-accuracy is needed, DLPNO-CCSD(T) is very promising for large-scale chemical application. However, the various approximations that have to be introduced in order to reach near linear scaling also introduce limited deviations from the canonical results. In the present work, we investigate how far the accuracy of the DLPNO-CCSD(T) method can be pushed for chemical applications. We also address the question at which additional computational cost improvements, relative to the previously established default scheme, come. To answer these questions, a series of benchmark sets covering a broad range of quantum chemical applications including reaction energies, hydrogen bonds, and other noncovalent interactions, conformer energies, and a prototype organometallic problem were selected. An accuracy of 1 kcal/mol or better can readily be obtained for all data sets using the default truncation scheme, which corresponds to the stated goal of the original implementation. Tightening of the three thresholds that control DLPNO leads to mean absolute errors and standard deviations from the canonical results of less than 0.25 kcal/mol ({\textless}1 kJ/mol). The price one has then to pay is an increased computational time by a factor close to 3. The applicability of the method is shown to be independent of the nature of the reaction. On the basis of the careful analysis of the results, three different sets of truncation thresholds (termed LoosePNO, NormalPNO, and TightPNO) have been chosen for black box use of DLPNO-CCSD(T). This will allow users of the method to optimally balance performance and accuracy.},
	number = {4},
	journal = {J. Chem. Theory Comput.},
	author = {Liakos, Dimitrios G. and Sparta, Manuel and Kesharwani, Manoj K. and Martin, Jan M. L. and Neese, Frank},
	month = apr,
	year = {2015},
	note = {Publisher: American Chemical Society},
	pages = {1525--1539},
}

@book{levine_quantum_2013,
	edition = {7},
	title = {Quantum {Chemistry}},
	publisher = {Pearson},
	author = {Levine, Ira N.},
	year = {2013},
}

@article{kendall_electron_1992,
	title = {Electron affinities of the first-row atoms revisited. {Systematic} basis sets and wave functions},
	volume = {96},
	issn = {00219606},
	doi = {10.1063/1.462569},
	abstract = {The calculation of accurate electron affinities (EAs) of atomic or molecular species is one of the most challenging tasks in quantum chemistry. We describe a reliable procedure for calculating the electron affinity of an atom and present results for hydrogen, boron, carbon, oxygen, and fluorine (hydrogen is included for completeness). This procedure involves the use of the recently proposed correlation-consistent basis sets augmented with functions to describe the more diffuse character of the atomic anion coupled with a straightforward, uniform expansion of the reference space for multireference singles and doubles configuration-interaction (MRSD-CI) calculations. Comparison with previous results and with corresponding full CI calculations are given. The most accurate EAs obtained from the MRSD-CI calculations are (with experimental values in parentheses) hydrogen 0.740 eV (0.754), boron 0.258 (0.277), carbon 1.245 (1.263), oxygen 1.384 (1.461), and fluorine 3.337 (3.401 ). The EAs obtained from the MR-SDCI calculations differ by less than 0.03 eV from those predicted by the full CI calculations. © 1992 American Institute of Physics.},
	number = {9},
	journal = {J. Chem. Phys.},
	author = {Kendall, Rick A. and Dunning, Thom H. and Harrison, Robert J.},
	year = {1992},
	pages = {6796--6806},
}

@article{kubicki_quantum_2019,
	title = {Quantum mechanical modeling of the vibrational spectra of minerals with a focus on clays},
	volume = {9},
	issn = {2075163X},
	doi = {10.3390/min9030141},
	abstract = {We present an overview of how to use quantum mechanical calculations to predict vibrational frequencies of molecules and materials such as clays and silicates. Other methods of estimating vibrational frequencies are mentioned, such as classical molecular dynamics simulations; references are given for additional information on these approaches. Herein, we discuss basic vibrational theory, calculating Raman and infrared intensities, steps for creating realistic models, and applications to spectroscopy, thermodynamics, and isotopic fractionation. There are a wide variety of programs and methods that can be employed to model vibrational spectra, but this work focuses on hybrid density functional theory (DFT) approaches. Many of the principles are the same when used in other programs and DFT methods, so a novice can benefit from simple examples that illustrate key points to consider when modeling vibrational spectra. Other methods and programs are listed to give the beginner a starting point for exploring and choosing which approach will be best for a given problem. The modeler should also be aware of the numerous analytical methods available for obtaining information on vibrations of atoms in molecules and materials. In addition to traditional infrared and Raman spectroscopy, sum-frequency generation (SFG) and inelastic neutron scattering (INS) are also excellent techniques for obtaining vibrational frequency information in certain circumstances.},
	number = {3},
	journal = {Minerals},
	author = {Kubicki, James D. and Watts, Heath D.},
	year = {2019},
	keywords = {Clays, Computational chemistry, Density functional theory (DFT), Infrared spectroscopy, Minerals, Raman spectroscopy, Vibrational frequencies},
}

@article{kournopoulos_molecular_2022,
	title = {Molecular theory of the static dielectric constant of dipolar fluids},
	journal = {J. Chem. Phys. (accepted)},
	author = {Kournopoulos, S. and Haslam, A. J. and Jackson, G. and Galindo, A. and Schoen, M.},
	year = {2022},
}

@article{kossmann_comparison_2009,
	title = {Comparison of two efficient approximate {Hartee}-{Fock} approaches},
	volume = {481},
	issn = {00092614},
	doi = {10.1016/j.cplett.2009.09.073},
	abstract = {The efficiency of two approximate Hartree-Fock approaches was benchmarked. Weigend's RI-JK algorithm is compared to the recently developed RIJCOSX technique in terms of accuracy and total wall clock times. Both methods reproduce the canonical results within the chemical accuracy of ∼kcal mol-1. RI-JK turns out to be more robust than RIJCOSX due to an overall positive error in the total energies. However, RIJCOSX outperforms RI-JK regarding speed-ups for the largest (gly)8 chain and maintains comparable accuracy. © 2009 Elsevier B.V. All rights reserved.},
	number = {4-6},
	journal = {Chem. Phys. Lett.},
	author = {Kossmann, Simone and Neese, Frank},
	year = {2009},
	pages = {240--243},
}

@article{kazepidis_optimal_2019,
	title = {Optimal design of post combustion {CO2} capture processes based on phase-change solvents},
	volume = {46},
	issn = {15707946},
	doi = {10.1016/B978-0-12-818634-3.50078-3},
	abstract = {The current work addresses the investigation of phase-change solvents behaviour during the design of post-combustion CO2 capture processes. The use of phase-change solvents leads to energetic gains due to their lower regeneration energy demands. The latter are enhanced in this work by the consideration of systematic structural and operating modifications imposed on a reference absorption/desorption flowsheet. Such modifications are realized with the help of a rigorous and flexible model that can represent the phase-change behaviour and includes stream redistribution options that aim to enhance the main process driving forces. An aqueous N-methylcyclohexylamine (MCA) solution is employed in an effort to exploit the solvent's phase separation behaviour towards the reduction of the total process cost and energy requirements.},
	journal = {Comput.-Aided Chem. Eng.},
	author = {Kazepidis, Panagiotis and Papadopoulos, Athanasios I. and Seferlis, P. and Perdomo, Felipe A. and Galindo, Amparo and Jackson, George and Adjiman, Claire S.},
	year = {2019},
	note = {ISBN: 9780128186343},
	keywords = {CO2 capture, MCA, N-methylcyclohexylamine, optimal design, phase change solvents},
	pages = {463--468},
}

@article{jager_ab_2009,
	title = {Ab initio pair potential energy curve for the argon atom pair and thermophysical properties of the dilute argon gas. {I}. {Argon}-argon interatomic potential and rovibrational spectra},
	volume = {107},
	issn = {00268976},
	doi = {10.1080/00268970903213305},
	abstract = {An argon-argon interatomic potential energy curve was derived from quantum-mechanical ab initio calculations using basis sets of up to d-aug-cc-pV(6+d)Z quality supplemented with bond functions and ab initio methods up to CCSDT(Q). In addition, corrections for relativistic effects were determined. An analytical potential function was fitted to the ab initio values and utilised to compute the rovibrational spectrum. The quality of the interatomic potential function was tested by comparison of the calculated spectrum with experimental ones and those derived from other potentials of the literature. In a following paper the new interatomic potential is used to determine selected thermophysical properties of argon by means of quantum-statistical mechanics and the corresponding kinetic theory considering two-body and three-body interactions.},
	number = {20},
	journal = {Mol. Phys.},
	author = {Jäger, Benjamin and Hellmann, Robert and Bich, Eckard and Vogel, Eckhard},
	year = {2009},
	keywords = {Argon ab initio pair potential, Argon analytical potential function, Rovibrational spectra},
	pages = {2181--2188},
}

@article{jager_state---art_2016,
	title = {State-of-the-art ab initio potential energy curve for the krypton atom pair and thermophysical properties of dilute krypton gas},
	volume = {144},
	issn = {00219606},
	doi = {10.1063/1.4943959},
	abstract = {A new reference krypton-krypton interatomic potential energy curve was developed by means of quantum-chemical ab initio calculations for 36 interatomic separations. Highly accurate values for the interaction energies at the complete basis set limit were obtained using the coupled-cluster method with single, double, and perturbative triple excitations as well as t-aug-cc-pV5Z and t-aug-cc-pV6Z basis sets including mid-bond functions, with the 6Z basis set being newly constructed for this study. Higher orders of coupled-cluster terms were considered in a successive scheme up to full quadruple excitations. Core-core and core-valence correlation effects were included. Furthermore, relativistic effects were studied not only at a scalar relativistic level using second-order direct perturbation theory, but also utilizing full four-component and Gaunt-effect computations. An analytical pair potential function was fitted to the interaction energies, which is characterized by a depth of 200.88 K with an estimated standard uncertainty of 0.51 K. Thermophysical properties of low-density krypton were calculated for temperatures up to 5000 K. Second and third virial coefficients were obtained from statistical thermodynamics. Viscosity and thermal conductivity as well as the self-diffusion coefficient were computed using the kinetic theory of gases. The theoretical results are compared with experimental data and with results for other pair potential functions from the literature, especially with those calculated from the recently developed ab initio potential of Waldrop et al. [J. Chem. Phys. 142, 204307 (2015)]. Highly accurate experimental viscosity data indicate that both the present ab initio pair potential and the one of Waldrop et al. can be regarded as reference potentials, even though the quantum-chemical methods and basis sets differ. However, the uncertainties of the present potential and of the derived properties are estimated to be considerably lower.},
	number = {11},
	journal = {J. Chem. Phys.},
	author = {Jäger, Benjamin and Hellmann, Robert and Bich, Eckard and Vogel, Eckhard},
	month = mar,
	year = {2016},
	note = {Publisher: American Institute of Physics Inc.},
	pages = {114304},
}

@article{jager_ab_2011,
	title = {Ab initio virial equation of state for argon using a new nonadditive three-body potential},
	volume = {135},
	issn = {00219606},
	doi = {10.1063/1.3627151},
	abstract = {An ab initio nonadditive three-body potential for argon has been developed using quantum-chemical calculations at the CCSD(T) and CCSDT levels of theory. Applying this potential together with a recent ab initio pair potential from the literature, the third and fourth to seventh pressure virial coefficients of argon were computed by standard numerical integration and the Mayer-sampling Monte Carlo method, respectively, for a wide temperature range. All calculated virial coefficients were fitted separately as polynomials in temperature. The results for the third virial coefficient agree with values evaluated directly from experimental data and with those computed for other nonadditive three-body potentials. We also redetermined the second and third virial coefficients from the best experimental pT data utilizing the computed higher virial coefficients as constraints. Thus, a significantly closer agreement of the calculated third virial coefficients with the experimental data was achieved. For different orders of the virial expansion, pT data have been calculated and compared with results from high quality measurements in the gaseous and supercritical region. The theoretically predicted pressures are within the very small experimental errors of ±0.02\% for p ≤ 12 MPa in the supercritical region near room temperature, whereas for subcritical temperatures the deviations increase up to +0.3\%. The computed pressure at the critical density and temperature is about 1.3\% below the experimental value. At pressures between 200 MPa and 1000 MPa and at 373 K, the calculated values deviate by 1 to 9 from the experimental results. © 2011 American Institute of Physics.},
	number = {8},
	journal = {J. Chem. Phys.},
	author = {Jäger, Benjamin and Hellmann, Robert and Bich, Eckard and Vogel, Eckhard},
	month = aug,
	year = {2011},
}

@book{israelachvili_intermolecular_2011,
	title = {Intermolecular and {Surface} {Forces}},
	isbn = {978-0-12-375182-9},
	publisher = {Academic Press},
	author = {Israelachvili, Jacob N.},
	year = {2011},
	doi = {10.1016/C2009-0-21560-1},
}

@article{hudson_intermolecular_1959,
	title = {Intermolecular {Forces} {Between} {Unlike}},
	volume = {56},
	number = {2},
	journal = {Trans. Faraday Soc.},
	author = {Hudson, G.H. and McCoubrey, J.},
	year = {1959},
	pages = {761--766},
}

@article{hellmann_ab_2011,
	title = {Ab initio intermolecular potential energy surface and thermophysical properties of hydrogen sulfide},
	volume = {13},
	issn = {1463-9076},
	url = {http://xlink.rsc.org/?DOI=c1cp20873j},
	doi = {10.1039/c1cp20873j},
	number = {30},
	journal = {Phys. Chem. Chem. Phys.},
	author = {Hellmann, Robert and Bich, Eckard and Vogel, Eckhard and Vesovic, Velisa},
	year = {2011},
	pages = {13749},
}

@article{hellmann_ab_2008,
	title = {Ab initio intermolecular potential energy surface and second pressure virial coefficients of methane},
	volume = {128},
	issn = {00219606},
	doi = {10.1063/1.2932103},
	abstract = {A six-dimensional potential energy hypersurface (PES) for two interacting rigid methane molecules was determined from high-level quantum-mechanical ab initio computations. A total of 272 points for 17 different angular orientations on the PES were calculated utilizing the counterpoise-corrected supermolecular approach at the CCSD(T) level of theory with basis sets of aug-cc-pVTZ and aug-cc-pVQZ qualities. The calculated interaction energies were extrapolated to the complete basis set limit. An analytical site-site potential function with nine sites per methane molecule was fitted to the interaction energies. In addition, a semiempirical correction to the analytical potential function was introduced to take into account the effects of zero-point vibrations. This correction includes adjustments of the dispersion coefficients and of a single-parameter within the fit to the measured values of the second virial coefficient B (T) at room temperature. Quantitative agreement was then obtained with the measured B values over the whole temperature range of the measurements. The calculated B values should definitely be more reliable at very low temperatures (T{\textless}150 K) than values extrapolated using the currently recommended equation of state. © 2008 American Institute of Physics.},
	number = {21},
	journal = {J. Chem. Phys.},
	author = {Hellmann, Robert and Bich, Eckard and Vogel, Eckhard},
	year = {2008},
	pages = {214303},
}

@article{hellmann_intermolecular_2014,
	title = {Intermolecular potential energy surface and thermophysical properties of the {CH} 4 –{N} 2 system},
	volume = {141},
	issn = {0021-9606},
	url = {http://aip.scitation.org/doi/10.1063/1.4902807},
	doi = {10.1063/1.4902807},
	number = {22},
	journal = {J. Chem. Phys.},
	author = {Hellmann, Robert and Bich, Eckard and Vogel, Eckhard and Vesovic, Velisa},
	month = dec,
	year = {2014},
	pages = {224301},
}

@article{haslam_prediction_2008,
	title = {Prediction of binary intermolecular potential parameters for use in modelling fluid mixtures},
	volume = {266},
	issn = {03783812},
	doi = {10.1016/j.fluid.2008.02.004},
	abstract = {We show how to extend the Hudson-McCoubrey combining rules, which were derived assuming the Lennard-Jones potential, for use with intermolecular potentials that are not of Lennard-Jones form. In particular, we illustrate the method by deriving combining rules for use with the square-well intermolecular potential. We show how these combining rules may be applied for equations of state such as the statistical associating fluid theory (SAFT), and that they perform at least as well as, and usually far better than, the standard Lorentz-Berthelot rules for all mixtures of simple molecules that we have considered. Liquid-liquid-equilibrium as well as vapour-liquid-equilibrium data are demonstrated to be important in judging the quality of combining rules. A methodology for the inclusion of the effect of polar interactions in our combining rules is suggested, however the success for these systems is mixed. The theory provides an excellent description of the thermodynamic properties of water vapour + methane and rationalises recent, apparently contradictory, models of the mixture of carbon dioxide + water, however the approach is less successful for mixtures such as carbon monoxide + hydrogen sulphide. This indicates that further work is still required for reliable prediction of binary-interaction parameters in mixtures of polar molecules. © 2008 Elsevier B.V. All rights reserved.},
	number = {1-2},
	journal = {Fluid Phase Equilib.},
	author = {Haslam, Andrew J. and Galindo, Amparo and Jackson, George},
	year = {2008},
	keywords = {Combining rules, Mixture fluid phase equilibria, Unlike intermolecular-potential parameters},
	pages = {105--128},
}

@article{hellmann_ab_2007,
	title = {Ab initio potential energy curve for the helium atom pair and thermophysical properties of dilute helium gas. {I}. {Helium}-helium interatomic potential},
	volume = {105},
	issn = {00268976},
	doi = {10.1080/00268970701730096},
	abstract = {A helium-helium interatomic potential energy curve was determined from quantum-mechanical ab initio calculations. Very large atom-centred basis sets including a newly developed d-aug-cc-pV8Z basis set supplemented with bond functions and ab initio methods up to full CI were applied. The aug-cc-pV7Z basis set of Gdanitz (J. Chem. Phys. 113, 5145 (2000)) was modified to be more consistent with the aug-cc-pV5Z and aug-cc-pV6Z basis sets. The diagonal Born-Oppenheimer corrections as well as corrections for relativistic effects were also calculated. A new analytical representation of the interatomic potential energy was fitted to the ab initio calculated values. In a following paper this potential model will be used in the framework of quantum-statistical mechanics and of the corresponding kinetic theory to calculate the most important thermophysical properties of helium governed by two-body and three-body interactions.},
	number = {23-24},
	journal = {Mol. Phys.},
	author = {Hellmann, Robert and Bich, Eckard and Vogel, Eckhard},
	month = dec,
	year = {2007},
	keywords = {Ab initio, Computational chemistry, Electronic structure, Helium pair potential, Quantum chemistry},
	pages = {3013--3023},
}

@article{hellmann_ab_2008-1,
	title = {Ab initio potential energy curve for the neon atom pair and thermophysical properties of the dilute neon gas. {I}. {Neon}–neon interatomic potential and rovibrational spectra},
	volume = {106},
	issn = {0026-8976},
	url = {http://www.tandfonline.com/doi/abs/10.1080/00268970701843147},
	doi = {10.1080/00268970701843147},
	number = {1},
	journal = {Mol. Phys.},
	author = {Hellmann, Robert and Bich, Eckard and Vogel, Eckhard},
	month = jan,
	year = {2008},
	pages = {133--140},
}

@article{hellmann_ab_2014,
	title = {Ab initio potential energy surface for the carbon dioxide molecule pair and thermophysical properties of dilute carbon dioxide gas},
	volume = {613},
	issn = {00092614},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0009261414007325},
	doi = {10.1016/j.cplett.2014.08.057},
	journal = {Chem. Phys. Lett.},
	author = {Hellmann, Robert},
	month = oct,
	year = {2014},
	pages = {133--138},
}

@article{hellmann_nonadditive_2017,
	title = {Nonadditive three-body potential and third to eighth virial coefficients of carbon dioxide},
	volume = {146},
	issn = {00219606},
	doi = {10.1063/1.4974995},
	abstract = {A new nonadditive three-body interaction potential for carbon dioxide was determined from supermolecular ab initio calculations up to the coupled cluster with single, double, and perturbative triple excitations [CCSD(T)] level of theory for 9401 configurations. A physically motivated analytical function with terms for describing nonadditive dispersion, induction, and exchange contributions was fitted to the calculated nonadditive three-body interaction energies. For the 7996 configurations with a total interaction energy of less than 3000 K, the mean absolute error of the analytical function is 0.32 K. The new nonadditive three-body potential was applied together with a previously published pair potential [R. Hellmann, Chem. Phys. Lett. 613, 133 (2014)] to calculate the third to seventh virial coefficients of CO2 at subcritical and supercritical temperatures up to 2000 K. The eighth virial coefficient was also calculated, but using only the pair potential and only at temperatures from 600 K to 2000 K because of the enormous computational costs. A simple analytical function was fitted individually to the calculated values of each virial coefficient, including previously determined values of the second virial coefficient, to obtain an analytical virial equation of state (VEOS). For densities at which the VEOS is converged, the agreement in pressure with the reference EOS of Span and Wagner [J. Phys. Chem. Ref. Data 25, 1509 (1996)] is mostly within ±0.5\%. However, for temperatures above about 700 K, much larger deviations occur at higher densities, which we ascribe mainly to deficiencies of the reference EOS due to the lack of accurate data for these experimentally difficult conditions.},
	number = {5},
	journal = {J. Chem. Phys.},
	author = {Hellmann, Robert},
	month = feb,
	year = {2017},
	pmid = {28178823},
	note = {Publisher: American Institute of Physics Inc.},
	pages = {054302},
}

@article{hattig_optimization_2005,
	title = {Optimization of auxiliary basis sets for {RI}-{MP2} and {RI}-{CC2} calculations: {Core}-valence and quintuple-ζ basis sets for {H} to {Ar} and {QZVPP} basis sets for {Li} to {Kr}},
	volume = {7},
	issn = {14639076},
	doi = {10.1039/b415208e},
	abstract = {An implementation of analytic basis set gradients is reported for the optimization of auxiliary basis sets in resolution-of-the-identity second-order Møller-Plesset perturbation theory (RI-MP2) and approximate coupled-cluster singles-and-doubles (RI-CC2) calculations. The analytic basis set gradients are applied in the optimization of auxiliary basis sets for a number of large one-electron orbital basis sets which provide correlation energies close to the basis set limit: the core-valence basis sets cc-pwCVXZ (B-Ne, Al-Ar) with X = D, T, Q, 5, the quintuple-ζ basis sets cc-pV5Z (H-Ar) and cc-pV(5 + d)Z (Al-Ar) and the doubly-polarized valence quadruple-ζ basis sets QZVPP for Li-Kr. The quality of the optimized auxiliary basis sets is evaluated for several test sets with small and medium sized molecules.},
	number = {1},
	journal = {Phys. Chem. Chem. Phys.},
	author = {Hättig, Christof},
	month = jan,
	year = {2005},
	pages = {59--66},
}

@article{hellmann_cross_2016,
	title = {Cross second virial coefficients and dilute gas transport properties of the ({CH} 4 + {CO} 2 ), ({CH} 4 + {H} 2 {S}), and ({H} 2 {S} + {CO} 2 ) systems from accurate intermolecular potential energy surfaces},
	volume = {102},
	issn = {00219614},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0021961416301793},
	doi = {10.1016/j.jct.2016.07.034},
	journal = {J. Chem. Thermodyn.},
	author = {Hellmann, Robert and Bich, Eckard and Vesovic, Velisa},
	month = nov,
	year = {2016},
	pages = {429--441},
}

@article{hellmann_reference_2018,
	title = {Reference {Values} for the {Second} {Virial} {Coefficient} and {Three} {Dilute} {Gas} {Transport} {Properties} of {Ethane} from a {State}-of-the-{Art} {Intermolecular} {Potential} {Energy} {Surface}},
	volume = {63},
	issn = {0021-9568},
	url = {https://pubs.acs.org/doi/10.1021/acs.jced.7b01069},
	doi = {10.1021/acs.jced.7b01069},
	number = {2},
	journal = {J. Chem. Eng. Data},
	author = {Hellmann, Robert},
	month = feb,
	year = {2018},
	pages = {470--481},
}

@article{hellmann_intermolecular_2017,
	title = {Intermolecular potential energy surface and thermophysical properties of propane},
	volume = {146},
	issn = {0021-9606},
	url = {http://aip.scitation.org/doi/10.1063/1.4978412},
	doi = {10.1063/1.4978412},
	number = {11},
	journal = {J. Chem. Phys.},
	author = {Hellmann, Robert},
	month = mar,
	year = {2017},
	pages = {114304},
}

@article{hellmann_ab_2013,
	title = {Ab initio potential energy surface for the nitrogen molecule pair and thermophysical properties of nitrogen gas},
	volume = {111},
	issn = {0026-8976},
	url = {http://www.tandfonline.com/doi/abs/10.1080/00268976.2012.726379},
	doi = {10.1080/00268976.2012.726379},
	number = {3},
	journal = {Mol. Phys.},
	author = {Hellmann, Robert},
	month = feb,
	year = {2013},
	pages = {387--401},
}

@article{hattig_auxiliary_2012,
	title = {Auxiliary basis sets for density-fitted correlated wavefunction calculations: {Weighted} core-valence and {ECP} basis sets for post-d elements},
	volume = {14},
	issn = {14639076},
	doi = {10.1039/c2cp40400a},
	abstract = {We report optimised auxiliary basis sets for the resolution-of-the-identity (or density-fitting) approximation of two-electron integrals in second-order Moller-Plesset perturbation theory (MP2) and similar electronic structure calculations with correlation-consistent basis sets for the post-d elements Ga-Kr, In-Xe, and Tl-Rn. The auxiliary basis sets are optimised such that the density-fitting error is negligible compared to the one-electron basis set error. To check to which extent this criterion is fulfilled we estimated for a test set of 80 molecules the basis set limit of the correlation energy at the MP2 level and evaluated the remaining density-fitting and the one-electron basis set errors. The resulting auxiliary basis sets are only 2-6 times larger than the corresponding one-electron basis sets and lead in MP2 calculations to speed-ups of the integral evaluation by one to three orders of magnitude. The density-fitting errors in the correlation energy are at least hundred times smaller than the one-electron basis set error, i.e. in the order of only 1-100 μH per atom. © the Owner Societies 2012.},
	number = {18},
	journal = {Phys. Chem. Chem. Phys.},
	author = {Hättig, Christof and Schmitz, Gunnar and Koßmann, Jörg},
	month = may,
	year = {2012},
	pages = {6549--6555},
}

@article{habenschuss_x-ray_1981,
	title = {X-ray diffraction study and models of liquid methane at 92 {K}},
	volume = {74},
	issn = {00219606},
	doi = {10.1063/1.441706},
	abstract = {New x-ray diffraction data for liquid methane near the triple point are presented. The data are analyzed using molecular scattering factors for methane which permit extraction of the carbon-carbon structure and correlation functions. Several site-site pair potentials are used with the reference interaction site model (RISM) to predict the structure and correlation functions for a dense methane-like fluid, and these are compared to the structure and correlation functions derived from the diffraction study. In addition, the accuracy of RISM is assessed by comparison with published computer simulation calculations on methane. Our results indicate that although the RISM distribution functions for "tetrahedral" molecules such as methane hae some physically unrealistic features, they compare well with molecular dynamics results. Site-site interaction potentials give an adequate description of liquid methane, provided that attractive forces are included in the potential. Although methane molecules are "seen" by x rays as spherically symmetric, orientational correlations between pairs of neighboring molecules are clearly present in the liquid near the triple point. © 1981 American Institute of Physics.},
	number = {9},
	journal = {J. Chem. Phys.},
	author = {Habenschuss, Anton and Johnson, Elijah and Narten, A. H.},
	year = {1981},
	pages = {5234--5241},
}

@article{guzman_third_2007,
	title = {Third virial coefficient of nonpolar gases from accurate binary potentials and ternary forces},
	volume = {40},
	issn = {09534075},
	doi = {10.1088/0953-4075/40/20/002},
	abstract = {An explicit model for the third virial coefficient C(T) is presented, based on accurate binary interactions plus three-body forces; its predictions are compared to experimental data for 15 fluids (argon, krypton, xenon, nitrogen, oxygen, fluorine, carbon monoxide, carbon dioxide, perfluoromethane, methane, ethene, ethane, propane, n-butane, and n-pentane). Three-body interactions are represented by the Axilrod-Teller-Muto (ATM) triple-dipole potential, while the binary potential profile is systematically varied using approximate non-conformal (ANC) potentials. Non-conformality affects significantly both two- and three-body contributions to C(T). A formula for C(T) of ANC+ATM systems is obtained in terms of all interaction parameters; the three-body contribution is proportional to the parameter ν of the ATM potential while its temperature dependence is proportional to that of a reference fluid (argon). The ANC+ATM model reproduces C(T) within experimental error for most of the fluids considered, with a small negative deviation in some cases, which may be ascribed to the need of a complement to the ATM term. © 2007 IOP Publishing Ltd.},
	number = {20},
	journal = {J. Phys. B: At. Mol. Phys. B: Atomic, Molecular and Optical Physics},
	author = {Guzmán, Orlando and del Río, Fernando},
	year = {2007},
	pages = {3989--4003},
}

@article{gopinath_outer_2016,
	title = {Outer approximation algorithm with physical domain reduction for computer‐aided molecular and separation process design},
	volume = {62},
	issn = {0001-1541},
	url = {https://onlinelibrary.wiley.com/doi/10.1002/aic.15411},
	doi = {10.1002/aic.15411},
	abstract = {superhydrophobic surfaces can be used to reduce the minimum voltage and to increase the maximum speed under certain conditions, but there are some harmful side-effects. First of all, the electrostatic pressure can push water into the surface pores, which hinders actuation. The phenomenon can also be treated as a vertical electrowetting effect. Another drawback is that the use of superhydrophobic surfaces makes actuation more critical to the properties of the liquid. For example, actuation of biological buffer solutions was not successful. For these reasons, it is concluded that it is more beneficial to use a smooth surface with low hysteresis than a superhydrophobic surface in droplet actuation. Electrostatic droplet actuation is a potential method for manipulating liquid on a microscopic scale, but there is still work to do. This work contains a detailed examination of the droplet actuation mechanism, and trapping of charges in the solid-liquid interface is found to be the most severe problem that needs to be solved.},
	number = {9},
	journal = {AIChE J.},
	author = {Gopinath, Smitha and Jackson, George and Galindo, Amparo and Adjiman, Claire S.},
	month = sep,
	year = {2016},
	pmid = {23641116},
	note = {ISBN: 9513862380
\_eprint: 0201037v1},
	keywords = {Electrostatic droplet actuation, Electrowetting, Lab-on-a-chip, MEMS, Microfluidics, Superhydrophobic surfaces},
	pages = {3484--3504},
}

@article{gopinath_feasibility-based_2016,
	title = {A feasibility-based algorithm for {Computer} {Aided} {Molecular} and {Process} {Design} of solvent-based separation systems},
	volume = {38},
	issn = {15707946},
	url = {http://dx.doi.org/10.1016/B978-0-444-63428-3.50017-5},
	doi = {10.1016/B978-0-444-63428-3.50017-5},
	abstract = {Computer-aided molecular and product design (CAMPD) can in principle be used to find simultaneously the optimal conditions in separation processes and the structure of the optimal solvents. In many cases, however, the solution of CAMPD problems is challenging. In this paper, we propose a solution approach for the CAMPD of solvent-based separation systems in which implicit constraints on phase behaviour in process models are used to test the feasibility of the process and solvent domains. The tests not only eliminate infeasible molecules from the search space but also infeasible combinations of solvent molecules and process conditions. The tests also provide bounds for the optimization of the process model (primal problem) for each solvent, facilitating numerical solution. This is demonstrated on a prototypical natural gas purification process.},
	number = {1999},
	journal = {Comput.-Aided Chem. Eng.},
	author = {Gopinath, Smitha and Galindo, Amparo and Jackson, George and Adjiman, Claire S.},
	year = {2016},
	note = {ISBN: 9780444634283
Publisher: Elsevier Masson SAS},
	keywords = {CAMPD, CO2 capture, MINLP, solvent},
	pages = {73--78},
}

@article{grimme_consistent_2010,
	title = {A consistent and accurate ab initio parametrization of density functional dispersion correction ({DFT}-{D}) for the 94 elements {H}-{Pu}},
	volume = {132},
	issn = {00219606},
	doi = {10.1063/1.3382344},
	abstract = {The method of dispersion correction as an add-on to standard Kohn-Sham density functional theory (DFT-D) has been refined regarding higher accuracy, broader range of applicability, and less empiricism. The main new ingredients are atom-pairwise specific dispersion coefficients and cutoff radii that are both computed from first principles. The coefficients for new eighth-order dispersion terms are computed using established recursion relations. System (geometry) dependent information is used for the first time in a DFT-D type approach by employing the new concept of fractional coordination numbers (CN). They are used to interpolate between dispersion coefficients of atoms in different chemical environments. The method only requires adjustment of two global parameters for each density functional, is asymptotically exact for a gas of weakly interacting neutral atoms, and easily allows the computation of atomic forces. Three-body nonadditivity terms are considered. The method has been assessed on standard benchmark sets for inter- and intramolecular noncovalent interactions with a particular emphasis on a consistent description of light and heavy element systems. The mean absolute deviations for the S22 benchmark set of noncovalent interactions for 11 standard density functionals decrease by 15\%-40\% compared to the previous (already accurate) DFT-D version. Spectacular improvements are found for a tripeptide-folding model and all tested metallic systems. The rectification of the long-range behavior and the use of more accurate C6 coefficients also lead to a much better description of large (infinite) systems as shown for graphene sheets and the adsorption of benzene on an Ag(111) surface. For graphene it is found that the inclusion of three-body terms substantially (by about 10\%) weakens the interlayer binding. We propose the revised DFT-D method as a general tool for the computation of the dispersion energy in molecules and solids of any kind with DFT and related (low-cost) electronic structure methods for large systems. © 2010 American Institute of Physics.},
	number = {15},
	journal = {J. Chem. Phys.},
	author = {Grimme, Stefan and Antony, Jens and Ehrlich, Stephan and Krieg, Helge},
	month = apr,
	year = {2010},
	pmid = {20423165},
	pages = {154104},
}

@book{feynman_quantum_1965,
	address = {New York},
	title = {Quantum mechanics and path integrals},
	publisher = {McGraw-Hill},
	author = {Feynman, Richard P and Hibbs, Albert R},
	year = {1965},
}

@article{fermeglia_novel_1999,
	title = {A novel approach to thermophysical properties prediction for chloro- fluoro-hydrocarbons},
	volume = {166},
	issn = {03783812},
	doi = {10.1016/S0378-3812(99)00295-2},
	abstract = {In this paper we present a new procedure, based on quantum/molecular (QM/MM) mechanics and molecular dynamics (MD) computer simulations, for estimating the Perturbed Hard Sphere Chain Theory (PHSCT) equation of state (EOS) parameters of a set of 14 alternative chloro-fluoro-hydrocarbons (CFH) of industrial relevance and to predict their thermophysical properties and PVT behavior. Force field and quantum-mechanical techniques were employed in molecular modeling and for the calculation of geometrical and chemico- physical parameters. The Connolly surface algorithm, corrected for quantum- mechanical effects, was used in the evaluation of molecular surfaces and volumes. From these data, the parameters of the PHSCT EOS, V* and A*, were obtained. The third parameter, E*, was calculated from extensive MD simulations under NPT conditions. The new, original method proposed in this work gives good results, is relatively inexpensive, is absolutely general and can be applied in principle to any EOS, provided the parameters have a physical meaning. The tuning of the energetic parameter to a generated data set accounts for the degree of empiricism introduced at a certain stage in the development of any EOS.},
	number = {1},
	journal = {Fluid Phase Equilib.},
	author = {Fermeglia, Maurizio and Pricl, Sabrina},
	year = {1999},
	keywords = {Equation of state, Molecular dynamics, Molecular simulation, Refrigerants, Thermophysical properties, Vapor-liquid equilibria},
	pages = {21--37},
}

@article{fermeglia_thermodynamic_1997,
	title = {Thermodynamic properties of pure hydrofluorocarbons by a perturbed hard-sphere-chain equation of state},
	volume = {52},
	issn = {00092509},
	doi = {10.1016/S0009-2509(96)00503-9},
	abstract = {This paper deals with the evaluation of thermodynamic properties of pure hydro-fluorocarbons. A perturbed-hard-sphere-chain equation of state was adapted to these compounds and tested on a large database of refrigerants and hydrocarbons, with reference to both volumetric and equilibrium properties. The ability of the proposed model to reproduce experimental values is discussed and comparison with that of the PHCT equation of state is presented. The model contains three parameters, which are only slightly correlated with one another. Expressions for predicting the parameter values as a function of molecular quantities are proposed. The results obtained show that the proposed model can be reliably used for calculation of pure properties of refrigerants, starting from the Bondi volume and surface area values, plus a single vapour pressure value. The results are promising in view of application to mixtures of refrigerants and long-chain hydrocarbons. In this respect, the paper can be regarded as a necessary step toward the prediction of the mixture behaviour of refrigerants and the effect of the presence of the lubricant oil in the mixture.},
	number = {9},
	journal = {Chem. Eng. Sci.},
	author = {Fermeglia, Maurizio and Bertucco, Alberto and Patrizioi, Damiano},
	year = {1997},
	keywords = {Refrigerant, equation of state, perturbation theory, thermodynamics},
	pages = {1517--1527},
}

@article{gibbons_quantum_1968,
	title = {Quantum deviations from the principle of corresponding states},
	volume = {72},
	issn = {00223654},
	doi = {10.1021/j100853a053},
	abstract = {An extension to the principle of corresponding states in terms of reduction by molecular constants is suggested which permits the calculation of consistent thermodynamic properties for simple molecules where quantum effects are important in the gas phase. The method correlates differences among the reduced properties of Ar, Ne, and 4He with the reduced de Broglie wavelength. The thermodynamic properties of Ne, nH2, and 3He are calculated from empirical equations for Ar, Ne, and 4He. The agreement with experimental data is good for the prediction of the properties of Ne and nH2 but is less good for the properties of 3He. The method fails for the liquid and critical regions of the phase diagram.},
	number = {7},
	journal = {J. Phys. Chem.},
	author = {Gibbons, R. M.},
	year = {1968},
	pages = {2567--2575},
}

@article{gao_reaction_2016,
	title = {Reaction {Mechanism} {Generator}: {Automatic} construction of chemical kinetic mechanisms},
	volume = {203},
	issn = {00104655},
	url = {http://dx.doi.org/10.1016/j.cpc.2016.02.013},
	doi = {10.1016/j.cpc.2016.02.013},
	abstract = {Reaction Mechanism Generator (RMG) constructs kinetic models composed of elementary chemical reaction steps using a general understanding of how molecules react. Species thermochemistry is estimated through Benson group additivity and reaction rate coefficients are estimated using a database of known rate rules and reaction templates. At its core, RMG relies on two fundamental data structures: graphs and trees. Graphs are used to represent chemical structures, and trees are used to represent thermodynamic and kinetic data. Models are generated using a rate-based algorithm which excludes species from the model based on reaction fluxes. RMG can generate reaction mechanisms for species involving carbon, hydrogen, oxygen, sulfur, and nitrogen. It also has capabilities for estimating transport and solvation properties, and it automatically computes pressure-dependent rate coefficients and identifies chemically-activated reaction paths. RMG is an object-oriented program written in Python, which provides a stable, robust programming architecture for developing an extensible and modular code base with a large suite of unit tests. Computationally intensive functions are cythonized for speed improvements. Program summary Program title: RMG Catalogue identifier: AEZW-v1-0 Program summary URL:http://cpc.cs.qub.ac.uk/summaries/AEZW-v1-0.html Program obtainable from: CPC Program Library, Queen's University, Belfast, N. Ireland Licensing provisions: MIT/X11 License No. of lines in distributed program, including test data, etc.: 958681 No. of bytes in distributed program, including test data, etc.: 9495441 Distribution format: tar.gz Programming language: Python. Computer: Windows, Ubuntu, and Mac OS computers with relevant compilers. Operating system: Unix/Linux/Windows. RAM: 1 GB minimum, 16 GB or more for larger simulations Classification: 16.12. External routines: RDKit, Open Babel, DASSL, DASPK, DQED, NumPy, SciPy Nature of problem: Automatic generation of chemical kinetic mechanisms for molecules containing C, H, O, S, and N. Solution method: Rate-based algorithm adds most important species and reactions to a model, with rate constants derived from rate rules and other parameters estimated via group additivity methods. Additional comments: The RMG software package also includes CanTherm, a tool for computing the thermodynamic properties of chemical species and both high-pressure-limit and pressure-dependent rate coefficients for chemical reactions using results from quantum chemical calculations. CanTherm is compatible with a variety of ab initio quantum chemistry software programs, including but not limited to Gaussian, MOPAC, QChem, and MOLPRO. Running time: From 30 s for the simplest molecules, to up to several weeks, depending on the size of the molecule and the conditions of the reaction system chosen.},
	journal = {Comput. Phys. Commun.},
	author = {Gao, Connie W. and Allen, Joshua W. and Green, William H. and West, Richard H.},
	year = {2016},
	note = {Publisher: Elsevier B.V.},
	keywords = {Automatic reaction mechanism generation, Chemical kinetics, Combustion, Rate-based algorithm},
	pages = {212--225},
}

@article{forte_effective_2014,
	title = {Effective coarse-grained solid-fluid potentials and their application to model adsorption of fluids on heterogeneous surfaces},
	volume = {16},
	issn = {14639076},
	doi = {10.1039/c4cp00670d},
	abstract = {The use of effective fluid-surface potentials, in which the full positional dependence is replaced by a dependence only on the distance from the surface of the solid, is common practice as a route to reduce the complexity of evaluating adsorption of fluids on substrates. Conceptually this is equivalent to replacing the detailed description of the discrete molecular nature by a coarse-grained description in which the solid is represented by a continuous (structureless) surface. These effective fluid-surface potentials are essential in the development of theories for surface adsorption, and they provide a means to reduce the computational cost associated with the molecular simulation of the system. The main purpose of the present contribution is to emphasise the necessity of using an adequate averaging procedure to obtain effective fluid-surface potentials. A simple unweighted average of the configurational energy is commonly employed, resulting in effective potentials that are temperature independent. We describe here a procedure to develop free-energy-averaged effective fluid-surface potentials retaining the important temperature dependence of the coarse-grained interaction between the particle and the surface. Although the approach is general in nature, we assess the merits of free-energy-averaged potentials for the adsorption of methane on graphene and graphite, making appropriate comparisons with the description obtained with the more traditional temperature-independent potentials. Additionally, we develop effective fluid-surface potentials for crystalline faces of monolayer and multilayer homogeneous and heterogeneous fcc lattices based on the Lennard-Jones (12-6) pair potential, and compute the corresponding adsorption isotherms of Lennard-Jones fluids on these surfaces using Grand Canonical Monte Carlo (GCMC) simulations. The adequacy of the two different options to obtain effective fluid-surface potentials (a free-energy-based versus a simple unweighted average) is compared critically. It is shown here that the higher the heterogeneity of the surface the less adequate simple unweighted averages are to describe the adsorption behaviour in comparison to free-energy averages. © the Partner Organisations 2014.},
	number = {36},
	journal = {Phys. Chem. Chem. Phys.},
	author = {Forte, Esther and Haslam, Andrew J. and Jackson, George and Müller, Erich A.},
	year = {2014},
	pages = {19165--19180},
}

@techreport{fiuidmech_new_1973,
	title = {A {New} {Two}-{Constant} {Equation} of {State}},
	abstract = {The development of a new two-constant equation of state in which the attractive pressure term of the semiem-pirical van der Waals equation has been modified is outlined. Examples of the use of the equation for predicting the vapor pressure and volumetric behavior of singie-component systems, and the phase behavior and volu-metric behavior of binary, ternary, and multicomponent systems are given. The proposed equation combines simplicity and accuracy. It performs as well as or better than the Soave-Redlich-Kwong equation in all cases tested and shows its greatest advantages in the prediction of liquid phase densities.},
	author = {FIuidMech, J and Berg, H J and D, Robb I and Co, J and Sci, Ioidlnterface and K, LaMer V and Peng, Ding-Yu and Robinson, Donald B},
	year = {1973},
	note = {Publication Title: Ind. fng. Chem.. Fundam
Volume: 19},
	pages = {1469},
}

@article{espindola-heredia_optimized_2009,
	title = {Optimized equation of the state of the square-well fluid of variable range based on a fourth-order free-energy expansion},
	volume = {130},
	issn = {00219606},
	doi = {10.1063/1.3054361},
	abstract = {The free energy of square-well (SW) systems of hard-core diameter σ with ranges 1≤λ≤3 is expanded in a perturbation series. This interval covers most ranges of interest, from short-ranged SW fluids (λ≃1.2) used in modeling colloids to long ranges (λ≃3) where the van der Waals classic approximation holds. The first four terms are evaluated by means of extensive Monte Carlo simulations. The calculations are corrected for the thermodynamic limit and care is taken to evaluate and to control the various sources of error. The results for the first two terms in the series confirm well-known independent results but have an increased estimated accuracy and cover a wider set of well ranges. The results for the third- and fourth-order terms are novel. The free-energy expansion for systems with short and intermediate ranges, 1≤λ≤2, is seen to have properties similar to those of systems with longer ranges, 2≤λ≤3. An equation of state (EOS) is built to represent the free-energy data. The thermodynamics given by this EOS, confronted against independent computer simulations, is shown to predict accurately the internal energy, pressure, specific heat, and chemical potential of the SW fluids considered and for densities 0≤ρ 3 ≤0.9 including subcritical temperatures. This fourth-order theory is estimated to be accurate except for a small region at high density, ρ 3 ≈0.9, and low temperature where terms of still higher order might be needed. © 2009 American Institute of Physics.},
	number = {2},
	journal = {J. Chem. Phys.},
	author = {Espíndola-Heredia, Rodolfo and Del Río, Fernando and Malijevsky, Anatol},
	year = {2009},
	note = {Publisher: American Institute of Physics Inc.},
}

@article{ervik_bottled_2016,
	title = {Bottled {SAFT}: {A} {Web} {App} {Providing} {SAFT}-γ {Mie} {Force} {Field} {Parameters} for {Thousands} of {Molecular} {Fluids}},
	volume = {56},
	issn = {15205142},
	doi = {10.1021/acs.jcim.6b00149},
	abstract = {Coarse-grained molecular simulation has become a popular tool for modeling simple and complex fluids alike. The defining aspects of a coarse grained model are the force field parameters, which must be determined for each particular fluid. Because the number of molecular fluids of interest in nature and in engineering processes is immense, constructing force field parameter tables by individually fitting to experimental data is a futile task. A step toward solving this challenge was taken recently by Mejía et al., who proposed a correlation that provides SAFT-γ Mie force field parameters for a fluid provided one knows the critical temperature, the acentric factor and a liquid density, all relatively accessible properties. Building on this, we have applied the correlation to more than 6000 fluids, and constructed a web application, called "Bottled SAFT", which makes this data set easily searchable by CAS number, name or chemical formula. Alternatively, the application allows the user to calculate parameters for components not present in the database. Once the intermolecular potential has been found through Bottled SAFT, code snippets are provided for simulating the desired substance using the "raaSAFT" framework, which leverages established molecular dynamics codes to run the simulations. The code underlying the web application is written in Python using the Flask microframework; this allows us to provide a modern high-performance web app while also making use of the scientific libraries available in Python. Bottled SAFT aims at taking the complexity out of obtaining force field parameters for a wide range of molecular fluids, and facilitates setting up and running coarse-grained molecular simulations. The web application is freely available at http://www.bottledsaft.org. The underlying source code is available on Bitbucket under a permissive license.},
	number = {9},
	journal = {J. Chem. Inf. Model.},
	author = {Ervik, Asmund and Mejía, Andrés and Müller, Erich A.},
	year = {2016},
	pmid = {27556884},
	pages = {1609--1614},
}

@article{dunning_gaussian_1989,
	title = {Gaussian basis sets for use in correlated molecular calculations. {I}. {The} atoms boron through neon and hydrogen},
	volume = {90},
	issn = {00219606},
	doi = {10.1063/1.456153},
	abstract = {In the past, basis sets for use in correlated molecular calculations have largely been taken from single configuration calculations. Recently, Almlöf, Taylor, and co-workers have found that basis sets of natural orbitals derived from correlated atomic calculations (ANOs) provide an excellent description of molecular correlation effects. We report here a careful study of correlation effects in the oxygen atom, establishing that compact sets of primitive Gaussian functions effectively and efficiently describe correlation effects if the exponents of the functions are optimized in atomic correlated calculations, although the primitive (sp) functions for describing correlation effects can be taken from atomic Hartree-Fock calculations if the appropriate primitive set is used. Test calculations on oxygen-containing molecules indicate that these primitive basis sets describe molecular correlation effects as well as the ANO sets of Almlöf and Taylor. Guided by the calculations on oxygen, basis sets for use in correlated atomic and molecular calculations were developed for all of the first row atoms from boron through neon and for hydrogen. As in the oxygen atom calculations, it was found that the incremental energy lowerings due to the addition of correlating functions fall into distinct groups. This leads to the concept of correlation consistent basis sets, i.e., sets which include all functions in a given group as well as all functions in any higher groups. Correlation consistent sets are given for all of the atoms considered. The most accurate sets determined in this way, [5s4p3d2f1g], consistently yield 99\% of the correlation energy obtained with the corresponding ANO sets, even though the latter contains 50\% more primitive functions and twice as many primitive polarization functions. It is estimated that this set yields 94\%-97\% of the total (HF + 1 + 2) correlation energy for the atoms neon through boron. © 1989 American Institute of Physics.},
	number = {2},
	journal = {J. Chem. Phys.},
	author = {Dunning, Thom H.},
	year = {1989},
	pages = {1007--1023},
}

@phdthesis{dufal_development_2013,
	type = {{PhD} {Thesis}},
	title = {Development and application of advanced thermodynamic molecular description for complex reservoir fluids containing carbon dioxide and brines},
	abstract = {This thesis contains a study of the thermodynamic properties of complex reservoir fluids. The focus of this work is the development of an equation of state and molecular models to describe the phase behaviour of the different components of the reservoir fluids that may be encountered in the context of CO2 injection into geological formations suitable for storage, e.g., saline aquifers or depleted hydrocarbon reservoirs, together with that of mixtures of these components that may be encountered. The major constituents of these reservoir fluids are the injected gas (CO2, which may contain some impurities), alkanes and various other hydrocarbons from natural gas or crude oil, water and salts. The first task is to ensure that the method selected (the SAFT-VR Mie equation of state) to model those fluids can provide an accurate description of the simplest of the fluids encountered, CO2 and hydrocarbons. A crucial aspect of this concerns a detailed examination of the procedure for searching the highly degenerate model-parameter space to obtain the best models for each fluid. The suitability of the method is also assessed by studying other simple fluids, as a means to test the range of validity of the models developed. Once the method has been validated for a wide range of relatively simple fluids, the next step is to study more-complex fluids including, in particular, water. Water is ubiquitous in the systems of interest but is a notoriously difficult fluid to model accurately using simple models of the sort that are tractable for use in the context of equation-of-state modelling. The provision of a good model of water underpins a large part of the work and is accomplished only as a result of further development of the theory upon which the equation of state is based, involving not only its statistical-mechanical foundation but also lengthy numerical procedures to isolate the most physically reasonable application of the theory. Bearing in mind its simplicity, the resulting model for water, within the context of the refined theory, provides for a remarkably good representation of the thermodynamic properties of water and forms a highlight of the thesis. The remaining part of the work is the development of a framework in which to treat the ionic components of reservoir fluids. Following the implementation of a standard method to treat electrolyte solutions, the main goal of the thesis is achieved with the modelling of the phase equilibria of CO2-brine systems, demonstrating that the proposed method is a suitable tool for the study of complex reservoir fluids containing carbon dioxide and brines.},
	school = {Imperial College London},
	author = {Dufal, Simon},
	year = {2013},
}

@article{doran_multipole_1974,
	title = {The multipole long-range ({Van} der {Waals}) interaction coefficients for neon, argon, krypton and xenon},
	volume = {7},
	issn = {00223700},
	doi = {10.1088/0022-3700/7/5/006},
	abstract = {The dipole-dipole, dipole-quadrupole, dipole-octupole, quadrupole- quadrupole, dipole-dipole-dipole, dipole-dipole-quadrupole, dipole-quadrupole- quadrupole, quadrupole-quadrupole-quadrupole and dipole-dipole-octupole longe range interaction coefficients for neon, argon, krypton and xenon are calculated by time dependent Brueckner-Goldstone perturbation theory.},
	number = {5},
	journal = {J. Phys. B: At. Mol. Phys.},
	author = {Doran, M. B.},
	year = {1974},
	pages = {558--569},
}

@article{del_rio_analytical_2013,
	title = {Analytical equation of state with three-body forces: {Application} to noble gases},
	volume = {139},
	issn = {0021-9606},
	url = {http://aip.scitation.org/doi/10.1063/1.4829055},
	doi = {10.1063/1.4829055},
	number = {18},
	journal = {J. Chem. Phys.},
	author = {del Río, Fernando and Díaz-Herrera, Enrique and Guzmán, Orlando and Moreno-Razo, José Antonio and Ramos, J. Eloy},
	month = nov,
	year = {2013},
	pages = {184503},
}

@article{deiters_fully_2019,
	title = {Fully a priori prediction of the vapor-liquid equilibria of {Ar}, {Kr}, and {Xe} from ab initio two-body plus three-body interatomic potentials},
	volume = {151},
	issn = {00219606},
	doi = {10.1063/1.5109052},
	abstract = {Fully a priori predictions are reported for the vapor-liquid equilibria (VLE) properties of Ar, Kr, and Xe using molecular simulation techniques and recently developed ab initio two-body interatomic potentials. Simulation data are reported at temperatures from near the triple point to close to the critical point. The two-body ab initio potentials exaggerate the size of the experimental VLE temperature-density envelope, overestimating the critical temperature and underestimating the vapor pressure. These deficiencies can be partially rectified by the addition of a density-dependent three-body term. At many temperatures, the ab initio + three-body simulations for Kr and Xe predict the vapor pressure to an accuracy that is close to experimental uncertainty. The predicted VLE coexisting densities for Xe almost match experimental data. The improvement with experiment is also reflected in more accurate enthalpies of vaporization. The fully a priori predictions for all of the VLE properties of either Kr or Xe are noticeably superior to simulations using the Lennard-Jones potential.},
	number = {3},
	journal = {J. Chem. Phys.},
	author = {Deiters, Ulrich K. and Sadus, Richard J.},
	month = jul,
	year = {2019},
	pmid = {31325952},
	note = {Publisher: American Institute of Physics Inc.},
	pages = {034509},
}

@article{deiters_two-body_2019,
	title = {Two-body interatomic potentials for {He}, {Ne}, {Ar}, {Kr}, and {Xe} from ab initio data},
	volume = {150},
	issn = {00219606},
	doi = {10.1063/1.5085420},
	abstract = {A new method is reported for developing accurate two-body interatomic potentials from existing ab initio data. The method avoids the computational complexity of alternative methods without sacrificing accuracy. Two-body potentials are developed for He, Ne, Ar, Kr, and Xe, which accurately reproduce the potential energy at all inter-atomic separations. Monte Carlo simulations of the pressure, radial distribution function, and isochoric heat capacity using the simplified potential indicate that the results are in very close, and sometimes almost indistinguishable, agreement with more complicated current state-of-the-art two-body potentials.},
	number = {13},
	journal = {J. Chem. Phys.},
	author = {Deiters, Ulrich K. and Sadus, Richard J.},
	month = apr,
	year = {2019},
	pmid = {30954035},
	note = {Publisher: American Institute of Physics Inc.},
	pages = {134504},
}

@article{crusius_ab_2015,
	title = {Ab initio intermolecular potential energy surface and thermophysical properties of nitrous oxide},
	volume = {142},
	issn = {0021-9606},
	url = {http://aip.scitation.org/doi/10.1063/1.4922830},
	doi = {10.1063/1.4922830},
	number = {24},
	journal = {J. Chem. Phys.},
	author = {Crusius, Johann-Philipp and Hellmann, Robert and Hassel, Egon and Bich, Eckard},
	month = jun,
	year = {2015},
	pages = {244307},
}

@article{crusius_intermolecular_2014,
	title = {Intermolecular potential energy surface and thermophysical properties of ethylene oxide},
	volume = {141},
	issn = {0021-9606},
	url = {http://aip.scitation.org/doi/10.1063/1.4899074},
	doi = {10.1063/1.4899074},
	number = {16},
	journal = {J. Chem. Phys.},
	author = {Crusius, Johann-Philipp and Hellmann, Robert and Hassel, Egon and Bich, Eckard},
	month = oct,
	year = {2014},
	pages = {164322},
}

@article{cripwell_accounting_2019,
	title = {Accounting for cross association in non-self-associating species using a physically consistent {SAFT}-{VR} {Mie} approach},
	volume = {483},
	issn = {03783812},
	url = {https://doi.org/10.1016/j.fluid.2018.11.003},
	doi = {10.1016/j.fluid.2018.11.003},
	abstract = {This work presents a formalised, physically consistent approach to account for cross association in the SAFT framework. The focus of the approach was to account for solvation of non-self-associating components, using members of the ketone and ether functional groups as model components. Physical consistency is captured by only considering a single negative site in these components, with the association mechanisms termed the “N scheme” as a result. An accurate polar parameter set is a prerequisite for the approach, where polar and dispersion interactions are already accounted for in pure component properties and those of mixtures where solvation is absent. Using SAFT-VR Mie-GV as the example framework, the approach considers the discretisation of the two association parameters, and it applies the resulting matrix of parameter sets to mixture VLE data for the ketone or ether with alcohols in the C2 to C4 range. Analysis of the resulting AAD contour plots demonstrate that the use of average solvation parameters for each functional groups are appropriate, rather than component-specific parameters, and they offer excellent pure predictions for alcohol mixtures and good predictions for aqueous mixtures. As a final test, the approach was applied to chloroform, considering a single positive site and using the proposed parameterisation method. The resulting “P scheme” for chloroform, in conjunction with the N scheme for acetone, yields excellent predictions for the quintessential chloroform/acetone mixture and emphasises the suitability and predictive strength of the approach.},
	journal = {Fluid Phase Equilib.},
	author = {Cripwell, Jamie T. and Kruger, Francois J. and Burger, Andries J.},
	year = {2019},
	note = {Publisher: Elsevier Ltd},
	keywords = {Chloroform, Cross association, Ether, Hydrogen bonding, Ketone, Polar, Polar SAFT, SAFT-VR Mie, Solvation, Vapour-liquid equilibria},
	pages = {1--13},
}

@article{constantinou_new_1994,
	title = {New group contribution method for estimating properties of pure compounds},
	volume = {40},
	issn = {15475905},
	doi = {10.1002/aic.690401011},
	abstract = {A new group contribution method for the estimation of properties of pure organic compounds is presented. Estimation is performed at two levels: the basic level uses contributions from first‐order groups, while the next higher level uses a small set of second‐order groups having the first‐order groups as building blocks. Thus, the method provides both a first‐order approximation (first‐order group contributions) and a more accurate second‐order prediction (first‐ and second‐order group contributions). This article discusses methods for prediction of normal boiling point, normal melting point, critical pressure, critical temperature, critical volume, standard enthalpy of vaporization at 298 K, standard Gibbs energy, and standard enthalpy of formation at 298 K. The predictions are based exclusively on the molecular structure of the compound, and the method is able to distinguish among isomers. Compared to the currently‐used methods, this technique demonstrates significant improvements in accuracy and applicability. Copyright © 1994 American Institute of Chemical Engineers},
	number = {10},
	journal = {AIChE J.},
	author = {Constantinou, Leonidas and Gani, Rafiqul},
	year = {1994},
	pages = {1697--1710},
}

@article{de_boer_quantum_1948,
	title = {Quantum theory of condensed permanent gases {I} the law of corresponding states},
	volume = {14},
	issn = {00318914},
	doi = {10.1016/0031-8914(48)90032-9},
	abstract = {It is shown in a quite general way, that the equation of states of the noble gases, H2, D2 and N2 can be written in a reduced form, in which the thermodynamic quantities T, P, V, etc. are expressed in "molecular units", i.e. units obtained from the characteristics parameters of the intermolecular field. In general the reduced equation of states contains a parameter A*, containing also h and the mass of the molecules, which measures essentially the influence of quantum mechanics on the phenomenon considered. Only when classical statistics can be applied and A* = 0, the reduced equation of states implies the law of corresponding states in its classical form. The reduction with molecular units is applied to the condensed phase of the substances mentioned above to study experimentally the thermodynamical properties as a function of A* and to obtain in this way information on the influence of quantum theory on these phenomena. © 1948.},
	number = {2-3},
	journal = {Physica},
	author = {De Boer, J.},
	year = {1948},
	pages = {139--148},
}

@techreport{castillot_three-body_1981,
	title = {Three-{Body} {Potential} {Energy} {Terms} for {Methane} {Trimers}},
	abstract = {An SCF LCAO MO calculation on the methane-methane-methane system is presented, in order to analyze the deviation from pairwise additivity of the interaction energy. Three-body terms are shown to be remarkably similar to those of noble gas trimers both in magnitude and in their dependence on the geometrical arrangements of the three molecules.},
	author = {Castillot, S and Les, A},
	year = {1981},
	note = {Publication Title: INTERNATIONAL JOURNAL OF QUANTUM CHEMISTRY
Volume: XIX},
	pages = {637--648},
}

@article{chao_molecular_2009,
	title = {Molecular dynamics simulations of fluid methane properties using {Ab} {Initio} intermolecular interaction potentials},
	volume = {30},
	issn = {01928651},
	doi = {10.1002/jcc.21185},
	abstract = {Intermolecular interaction energy data for the methane dimer have been calculated at a spectroscopic accuracy and employed to construct an ab initio potential energy surface (PES) for molecular dynamics (MD) simulations of fluid methane properties. The full potential curves of the methane dimer at 12 symmetric conformations were calculated by the supermolecule counterpoise-corrected second-order Møller-Plesset (MP2) perturbation theory. Single-point coupled cluster with single and double and perturbative triple excitations [CCSD(T)] calculations were also carried out to calibrate the MP2 potentials. We employed Pople's medium size basis sets [up to 6-31111G(3df, 3pd)] and Dunning's correlation consistent basis sets (cc-pVXZ and aug-cc-pVXZ, X 5 D, T, Q). For each conformer, the intermolecular carbon-carbon separation was sampled in a step 0.1 Å for a range of 3-9 Å, resulting in a total of 732 configuration points calculated. The MP2 binding curves display significant anisotropy with respect to the relative orientations of the dimer. The potential curves at the complete basis set (CBS) limit were estimated using well-established analytical extrapolation schemes. A 4-site potential model with sites located at the hydrogen atoms was used to fit the ab initio potential data. This model stems from a hydrogen-hydrogen repulsion mechanism to explain the stability of the dimer structure. MD simulations using the ab initio PES show quantitative agreements on both the atom-wise radial distribution functions and the self-diffusion coefficients over a wide range of experimental conditions. © 2008 Wiley Periodicals, Inc.},
	number = {12},
	journal = {J. Comput. Chem.},
	author = {Chao, Shih Wei and Li, Arvin Huang Te and Chao, Sheng D.},
	month = sep,
	year = {2009},
	pmid = {19090563},
	keywords = {Ab initio intermolecular potential energy surface, Fluid methane, Methane dimer, Molecular dynamics simulation, Radial distribution function, Self-diffusion coefficient},
	pages = {1839--1849},
}

@article{boys_calculation_1970,
	title = {The calculation of small molecular interactions by the differences of separate total energies. {Some} procedures with reduced errors},
	volume = {19},
	issn = {13623028},
	doi = {10.1080/00268977000101561},
	abstract = {A new direct difference method for the computation of molecular interactions has been based on a bivariational transcorrelated treatment, together with special methods for the balancing of other errors. It appears that these new features can give a strong reduction in the error of the interaction energy, and they seem to be particularly suitable for computations in the important region near the minimum energy. It has been generally accepted that this problem is dominated by unresolved difficulties and the relation of the new methods to these apparent difficulties is analysed here. © 1970 Molecular Physics.},
	number = {4},
	journal = {Mol. Phys.},
	author = {Boys, S. F. and Bernardi, F.},
	year = {1970},
	pages = {553--566},
}

@article{bistoni_finding_2020,
	title = {Finding chemical concepts in the {Hilbert} space: {Coupled} cluster analyses of noncovalent interactions},
	volume = {10},
	issn = {17590884},
	doi = {10.1002/wcms.1442},
	abstract = {Noncovalent interactions (NCIs) play a major role in essentially all fields of chemical research. Energy decomposition analysis (EDA) schemes provide in-depth insights into their nature by decomposing interaction energies into additive contributions, such as electrostatics, polarization, and London dispersion. Although modern local variants of the “gold standard” coupled-cluster singles and doubles method plus perturbative triples (CCSD(T)) have made it possible to accurately quantify NCIs for relatively large systems, extracting chemically meaningful energy terms from such high level electronic structure calculations has been a long lasting challenge in computational chemistry. This review describes basic principles, interpretative aspects and applications of recently developed coupled cluster-based EDAs for the analysis of NCIs. The focus is on computationally efficient methods for systems with a few hundred atoms, for example, the recently introduced local energy decomposition analysis. In order to draw connections between different interpretative frameworks, these schemes are compared with other popular approaches for the quantification and analysis of NCIs, such as Symmetry Adapted Perturbation Theory and supermolecular EDAs based on mean-field as well as correlated approaches. Strengths and limitations of the various techniques are discussed. This article is characterized under: Electronic Structure Theory {\textgreater} Ab Initio Electronic Structure Methods Structure and Mechanism {\textgreater} Molecular Structures.},
	number = {3},
	journal = {Wiley Interdiscip. Rev.: Comput. Mol. Sci.},
	author = {Bistoni, Giovanni},
	month = may,
	year = {2020},
	note = {Publisher: Blackwell Publishing Inc.},
	keywords = {London dispersion, coupled cluster, energy decomposition analysis, local correlation, local energy decomposition},
	pages = {e1442},
}

@article{bich_ab_2007,
	title = {Ab initio potential energy curve for the helium atom pair and thermophysical properties of the dilute helium gas. {II}. {Thermophysical} standard values for low-density helium},
	volume = {105},
	issn = {0026-8976},
	url = {http://www.tandfonline.com/doi/abs/10.1080/00268970701744584},
	doi = {10.1080/00268970701744584},
	number = {23-24},
	journal = {Mol. Phys.},
	author = {Bich, Eckard and Hellmann, Robert and Vogel, Eckhard},
	month = dec,
	year = {2007},
	pages = {3035--3049},
}

@article{berntsen_algorithm_1991,
	title = {Algorithm 698: {DCUHRE}: {An} {Adaptive} {Multidimensional} {Integration} {Routine} for a {Vector} of {Integrals}},
	volume = {17},
	number = {4},
	journal = {ACM Trans. Math. Softw.},
	author = {Berntsen, Jarle and Espelid, Terje O and Genz, Alan},
	year = {1991},
	pages = {452--456},
}

@book{bender_advanced_1999,
	address = {New York, NY},
	title = {Advanced {Mathematical} {Methods} for {Scientists} and {Engineers} {I}},
	isbn = {978-1-4419-3187-0},
	publisher = {Springer New York},
	author = {Bender, Carl M. and Orszag, Steven A.},
	year = {1999},
	doi = {10.1007/978-1-4757-3069-2},
}

@article{barker_perturbation_1967,
	title = {Perturbation theory and equation of state for fluids. {II}. {A} successful theory of liquids},
	volume = {47},
	issn = {00219606},
	doi = {10.1063/1.1701689},
	abstract = {The perturbation theory previously shown to give good results for the equation of state of a square-well fluid at liquid densities and temperatures is applied to more realistic potentials with soft repulsion, in particular the 6:12 potential. For an arbitrary potential function a modified potential is defined involving three parameters, namely a hard-sphere diameter, an inverse-steepness parameter for the repulsive region, and a depth parameter for the attractive region. When the latter parameters are zero, the modified potential becomes the hard-sphere potential; when they are one, it becomes the original potential. The configuration integral is expanded in a double-power series in the inverse-steepness and depth parameters, the hard-sphere diameter being chosen so that the first-order term in the inverse-steepness parameter is zero. The first-order term in the depth parameter is evaluated essentially exactly and the second-order term approximately: other second-order terms and all higher-order terms are neglected. The resulting equation of state is in good agreement with molecular dynamics, Monte Carlo results, and experimental data for argon at all temperatures and densities relevant for fluids.},
	number = {11},
	journal = {J. Chem. Phys.},
	author = {Barker, J. A. and Henderson, D.},
	year = {1967},
	pages = {4714--4721},
}

@article{barker_liquid_1971,
	title = {Liquid argon: {Monte} carlo and molecular dynamics calculations},
	volume = {21},
	issn = {13623028},
	doi = {10.1080/00268977100101821},
	abstract = {Thermodynamic properties of liquid argon are calculated by Monte Carlo and molecular dynamics techniques, using accurate pair-potential functions determined from the properties of solid and gaseous argon, together with the Axilrod-Teller three-body interaction. Satisfactory techniques for evaluating three-body contributions to thermodynamic properties without excessive requirements of computer time are described. Quantum corrections are included. Agreement with experiment is excellent: the best pair and triplet potentials give an excellent description of the properties of solid, gaseous and liquid argon. © 1971 Molecular physics.},
	number = {4},
	journal = {Mol. Phys.},
	author = {Barker, J. A. and Fisher, R. A. and Watts, R. O.},
	year = {1971},
	pages = {657--673},
}

@techreport{barker_what_nodate,
	title = {What is "liquid" ? {Understanding} the states of n-iatter},
	author = {Barker, J A and Henderson, D},
}

@article{axilrod_interaction_1943,
	title = {Interaction of the van der {Waals} {Type} {Between} {Three} {Atoms}},
	volume = {11},
	issn = {0021-9606},
	url = {http://aip.scitation.org/doi/10.1063/1.1723844},
	doi = {10.1063/1.1723844},
	number = {6},
	journal = {J. Chem. Phys.},
	author = {Axilrod, B. M. and Teller, E.},
	month = jun,
	year = {1943},
	pages = {299--300},
}

@article{altun_hfld_2019,
	title = {{HFLD}: {A} {Nonempirical} {London} {Dispersion}-{Corrected} {Hartree}-{Fock} {Method} for the {Quantification} and {Analysis} of {Noncovalent} {Interaction} {Energies} of {Large} {Molecular} {Systems} †},
	volume = {15},
	issn = {15499626},
	doi = {10.1021/acs.jctc.9b00425},
	abstract = {A nonempirical quantum mechanical method for the efficient and accurate quantification and analysis of intermolecular interactions is presented and tested on existing benchmark sets. The leading idea here is to focus on the intermolecular part of the correlation energy that contains the all-important London dispersion (LD) interaction. To keep the cost of the method low, essentially at the level of a Hartree-Fock (HF) calculation, the intramolecular part of the correlation energy is neglected. We also neglect the nondispersive parts of the intermolecular correlation energy. This scheme that we denote as Hartree-Fock plus London dispersion (HFLD) can be readily realized on the basis of the recently reported multilevel implementation of the domain-based local pair natural orbital coupled-cluster (DLPNO-CC) theory in conjunction with the well-established local energy decomposition (LED) analysis. The accuracy and efficiency of the HFLD method are evaluated on rare gas dimers, on the S66 and L7 benchmark sets of noncovalent interactions, and on an additional set (LP14) consisting of bulky Lewis pairs held together by intermolecular interactions of various strengths, with interaction energies ranging from -8 to -107 kcal/mol. It is first shown that the LD energy calculated with this approach is essentially identical to that obtained from the full DLPNO-CCSD(T)/LED calculation, with a mean absolute error of 0.2 kcal/mol on the S66 benchmark set. Moreover, in terms of the overall interaction energies, the HFLD method shows an efficiency that is comparable to that of the HF method, while retaining an accuracy between that of the DLPNO-CCSD and DLPNO-CCSD(T) schemes. Since the underlying DLPNO-CCSD method is linear scaling with respect to the system size, the HFLD approach also does not lead to new bottlenecks for large systems. As an illustrative example of its efficiency, the HFLD scheme was applied to the interaction between the substrate and the residues in the active site of the cyclohexanone monooxygenase enzyme. The excellent cost/performance ratio indicates that the HFLD method opens new avenues for the accurate calculation and analysis of noncovalent interaction energies in large molecular systems.},
	number = {11},
	journal = {J. Chem. Theory Comput.},
	author = {Altun, Ahmet and Neese, Frank and Bistoni, Giovanni},
	year = {2019},
	pmid = {31538779},
	pages = {5894--5907},
}

@article{avendano_saft-_2011,
	title = {{SAFT}-γ force field for the simulation of molecular fluids. 1. {A} single-site coarse grained model of carbon dioxide},
	volume = {115},
	issn = {15205207},
	doi = {10.1021/jp204908d},
	abstract = {An application of the "top-down" concept for the development of accurate coarse-grained intermolecular potentials of complex fluids is presented. With the more common "bottom-up" procedure, coarse-grained models are constructed from a suitable simplification of a detailed atomistic representation, and small adjustments to the intermolecular parameters are made by comparison with limited experimental data where necessary. In contrast, in the top-down approach, a molecular-based equation of state is used to obtain an effective coarse-grained intermolecular potential that reproduces the macroscopic experimental thermophysical properties over a wide range of conditions. These coarse-grained intermolecular potentials can then be used in conventional molecular simulation to obtain properties (such as structure or dynamics) that are not directly accessible from the equation of state or at extreme conditions where the theory is expected to fail. To demonstrate our procedure, a coarse-grained model for carbon dioxide (CO2) is obtained from a recent implementation of the statistical associating fluid theory of variable range (SAFT-VR) employing a Mie (generalized Lennard-Jones) potential; the parameters of this single-site Mie model of CO2 are estimated by optimizing the equation of state's description of the experimental vapor-pressure and saturated liquid density data. This approach is only viable because of the excellent agreement of the SAFT-VR Mie EoS with simulation data. Our single-site SAFT-γ coarse-grained model for CO2 is used in Monte Carlo molecular simulation to assess the adequacy of the description of the fluid-phase behavior and properties that were not used to develop the potential model such as the enthalpy of vaporization, interfacial tension, density profiles, supercritical densities, and second-derivative thermodynamic properties (thermal expansivity, isothermal compressibility, heat capacity, Joule-Thompson coefficient, and speed of sound). The accuracy of the description with the single-site SAFT-γ model of CO2 is found to be of similar quality to that of more sophisticated intermolecular potentials such as a six-site (three LJ centers and three charged sites) all-atom model. The SAFT-γ top-down approach to coarse-graining resolves a key challenge with coarse-graining techniques: the provision of a direct robust link between the microscopic and macroscopic scales. © 2011 American Chemical Society.},
	number = {38},
	journal = {J. Phys. Chem. B},
	author = {Avendaño, Carlos and Lafitte, Thomas and Galindo, Amparo and Adjiman, Claire S. and Jackson, George and Müller, Erich A.},
	year = {2011},
	pages = {11154--11169},
}

@article{altun_local_2019,
	title = {Local {Energy} {Decomposition} of {Open}-{Shell} {Molecular} {Systems} in the {Domain}-{Based} {Local} {Pair} {Natural} {Orbital} {Coupled} {Cluster} {Framework}},
	volume = {15},
	issn = {15499626},
	doi = {10.1021/acs.jctc.8b01145},
	abstract = {Local energy decomposition (LED) analysis decomposes the interaction energy between two fragments calculated at the domain-based local pair natural orbital CCSD(T) (DLPNO-CCSD(T)) level of theory into a series of chemically meaningful contributions and has found widespread applications in the study of noncovalent interactions. Herein, an extension of this scheme that allows for the analysis of interaction energies of open-shell molecular systems calculated at the UHF-DLPNO-CCSD(T) level is presented. The new scheme is illustrated through applications to the CH 2 ···X (X = He, Ne, Ar, Kr, and water) and heme···CO interactions in the low-lying singlet and triplet spin states. The results are used to discuss the mechanism that governs the change in the singlet-triplet energy gap of methylene and heme upon adduct formation.},
	number = {3},
	journal = {J. Chem. Theory Comput.},
	author = {Altun, Ahmet and Saitow, Masaaki and Neese, Frank and Bistoni, Giovanni},
	year = {2019},
	pmid = {30702888},
	pages = {1616--1632},
}

@article{altun_effect_2019,
	title = {Effect of {Electron} {Correlation} on {Intermolecular} {Interactions}: {A} {Pair} {Natural} {Orbitals} {Coupled} {Cluster} {Based} {Local} {Energy} {Decomposition} {Study}},
	volume = {15},
	issn = {15499626},
	doi = {10.1021/acs.jctc.8b00915},
	abstract = {The development of post-Hartree-Fock (post-HF) energy decomposition schemes that are able to decompose the HF and correlation components of the interaction energy into chemically meaningful contributions is a very active field of research. One of the challenges is to provide a clear-cut quantification to the elusive London dispersion component of the intermolecular interaction. London dispersion is well-known to be a pure correlation effect, and as such it is not properly described by mean field theories. In this context, we have recently developed the local energy decomposition (LED) analysis, which provides a chemically meaningful decomposition of the interaction energy between two or more fragments computed at the domain-based local pair natural orbitals coupled cluster (DLPNO-CCSD(T)) level of theory. In this work, this scheme is used in conjunction with other interpretation tools to study a series of molecular adducts held together by intermolecular interactions of different natures. The HF and correlation components of the interaction energy are thus decomposed into a series of chemically meaningful contributions. Emphasis is placed on discussing the physical effects associated with the inclusion of electron correlation. It is found that four distinct physical effects can contribute to the magnitude of the correlation part of intermolecular binding energies (Eint C ): (i) London dispersion, (ii) the correlation correction to the reference induction energy, (iii) the correlation correction to the electron sharing process, and (iv) the correlation correction to the permanent electrostatics. As expected, the largest contribution to the correlation binding energy of neutral, apolar molecules is London dispersion, as in the argon dimer case. In contrast, the correction for the HF induction energy dominates Eint C in systems in which an apolar molecule interacts with charged or strongly polar species, as in Ar-Li + . This effect has its origin in the systematic underestimation of polarizabilities at the HF level of theory. For similar reasons, electron sharing largely contributes to the correlation binding energy of covalently bound molecules, as in the beryllium dimer case. Finally, the correction for HF permanent electrostatics significantly contributes to Eint C in molecules with strong dipoles, such as water and hydrogen fluoride dimers. This effect originates from the characteristic overestimation of dipole moments at the HF level of theory, leading in some cases to positive Eint C values. Our results are apparently in contrast to the widely accepted view that Eint C is typically dominated by London dispersion, at least, in the strongly interacting region. Clearly, post-HF energy decomposition schemes are very powerful tools to analyze, categorize, and understand the various contributions to the intermolecular interaction energy. Hopefully, this will eventually lead to insights that are helpful in designing systems with tailored properties. All analysis tools presented in this work will be available free of charge in the next release of the ORCA program package.},
	number = {1},
	journal = {J. Chem. Theory Comput.},
	author = {Altun, Ahmet and Neese, Frank and Bistoni, Giovanni},
	month = jan,
	year = {2019},
	pmid = {30495957},
	note = {Publisher: American Chemical Society},
	pages = {215--228},
}

@article{pikal_theory_1971,
	title = {Theory of the {Onsager} transport coefficients lij and {Rij} for electrolyte solutions},
	volume = {75},
	issn = {0022-3654, 1541-5740},
	url = {https://pubs.acs.org/doi/10.1021/j100689a016},
	doi = {10.1021/j100689a016},
	language = {en},
	number = {20},
	urldate = {2022-05-05},
	journal = {The Journal of Physical Chemistry},
	author = {Pikal, Michael J.},
	month = sep,
	year = {1971},
	pages = {3124--3134},
}

@article{li_taking_2014,
	title = {Taking into {Account} the {Ion}-{Induced} {Dipole} {Interaction} in the {Nonbonded} {Model} of {Ions}},
	volume = {10},
	issn = {1549-9618, 1549-9626},
	url = {https://pubs.acs.org/doi/10.1021/ct400751u},
	doi = {10.1021/ct400751u},
	abstract = {Metal ions exist in almost half of the proteins in the protein databank, and they serve as structural, electron-transfer, and catalytic elements in the metabolic processes of organisms. Molecular dynamics (MD) simulation is a powerful tool that provides information about biomolecular systems at the atomic level. Coupled with the growth in computing power, algorithms like the particle mesh Ewald (PME) method have become the accepted standard when dealing with long-range interactions in MD simulations. The nonbonded model of metal ions consists of an electrostatic plus 12−6 Lennard-Jones (LJ) potential and is used largely because of its speed relative to more accurate models. In previous work we found that ideal parameters do not exist that reproduce several experimental properties for M(II) ions simultaneously using the nonbonded model coupled with the PME method due to the underestimation of metal ion-ligand interactions. Via a consideration of the nature of the nonbonded model, we proposed that the observed error largely arises from overlooking charge-induced dipole interactions. The electrostatic plus 12−6 LJ potential model works reasonably well for neutral systems but does struggle with more highly charged systems. In the present work we designed and parametrized a new nonbonded model for metal ions by adding a 1/r4 term to the 12−6 model. We call it the 12−6−4 LJ-type nonbonded model due to its mathematical construction. Parameters were determined for 16 +2 metal ions for the TIP3P, SPC/ E, and TIP4PEW water models. The ﬁnal parameters reproduce the experimental hydration free energies (HFE), ion-oxygen distances (IOD) in the ﬁrst solvation shell, and coordination numbers (CN) accurately for most of the metal ions investigated. Preliminary tests on MgCl2 at diﬀerent concentrations in aqueous solution and Mg2+−nucleic acid systems show reasonable results suggesting that the present parameters can work in mixed systems. The 12−6−4 LJ-type nonbonded model is readily adopted into standard force ﬁelds like AMBER, CHARMM, and OPLS-AA with only a modest computational overhead. The new nonbonded model does not consider charge-transfer eﬀects explicitly and, hence, may not be suitable for the simulation of systems where charge-transfer eﬀects play a decisive role.},
	language = {en},
	number = {1},
	urldate = {2022-05-04},
	journal = {Journal of Chemical Theory and Computation},
	author = {Li, Pengfei and Merz, Kenneth M.},
	month = jan,
	year = {2014},
	pages = {289--297},
}

@article{li_parameterization_2015,
	title = {Parameterization of {Highly} {Charged} {Metal} {Ions} {Using} the 12-6-4 {LJ}-{Type} {Nonbonded} {Model} in {Explicit} {Water}},
	volume = {119},
	issn = {1520-6106, 1520-5207},
	url = {https://pubs.acs.org/doi/10.1021/jp505875v},
	doi = {10.1021/jp505875v},
	abstract = {Highly charged metal ions act as catalytic centers and structural elements in a broad range of chemical complexes. The nonbonded model for metal ions is extensively used in molecular simulations due to its simple form, computational speed, and transferability. We have proposed and parametrized a 12-6-4 LJ (Lennard-Jones)-type nonbonded model for divalent metal ions in previous work, which showed a marked improvement over the 12-6 LJ nonbonded model. In the present study, by treating the experimental hydration free energies and ion−oxygen distances of the ﬁrst solvation shell as targets for our parametrization, we evaluated 12-6 LJ parameters for 18 M(III) and 6 M(IV) metal ions for three widely used water models (TIP3P, SPC/E, and TIP4PEW). As expected, the interaction energy underestimation of the 12-6 LJ nonbonded model increases dramatically for the highly charged metal ions. We then parametrized the 12-6-4 LJ-type nonbonded model for these metal ions with the three water models. The ﬁnal parameters reproduced the target values with good accuracy, which is consistent with our previous experience using this potential. Finally, tests were performed on a protein system, and the obtained results validate the transferability of these nonbonded model parameters.},
	language = {en},
	number = {3},
	urldate = {2022-05-04},
	journal = {The Journal of Physical Chemistry B},
	author = {Li, Pengfei and Song, Lin Frank and Merz, Kenneth M.},
	month = jan,
	year = {2015},
	pages = {883--895},
}

@article{pereira_impact_2014,
	title = {On the impact of using volume as an independent variable for the solution of {P} – {T} fluid-phase equilibrium with equations of state},
	volume = {71},
	issn = {00981354},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0098135414001884},
	doi = {10.1016/j.compchemeng.2014.06.009},
	language = {en},
	urldate = {2022-04-25},
	journal = {Computers \& Chemical Engineering},
	author = {Pereira, Frances E. and Galindo, Amparo and Jackson, George and Adjiman, Claire S.},
	month = dec,
	year = {2014},
	pages = {67--76},
}

@article{cheng_accelerating_2015,
	title = {Accelerating {Electrolyte} {Discovery} for {Energy} {Storage} with {High}-{Throughput} {Screening}},
	volume = {6},
	issn = {1948-7185, 1948-7185},
	url = {https://pubs.acs.org/doi/10.1021/jz502319n},
	doi = {10.1021/jz502319n},
	abstract = {Computational screening techniques have been found to be an eﬀective alternative to the trial and error of experimentation for discovery of new materials. With increased interest in development of advanced electrical energy storage systems, it is essential to ﬁnd new electrolytes that function eﬀectively. This Perspective reviews various methods for screening electrolytes and then describes a hierarchical computational scheme to screen multiple properties of advanced electrical energy storage electrolytes using highthroughput quantum chemical calculations. The approach eﬀectively down-selects a large pool of candidates based on successive property evaluation. As an example, results of screening are presented for redox potentials, solvation energies, and structural changes of ∼1400 organic molecules for nonaqueous redox ﬂow batteries. Importantly, on the basis of high-throughput screening, in silico design of suitable candidate molecules for synthesis and electrochemical testing can be achieved. We anticipate that the computational approach described in this Perspective coupled with experimentation will have a signiﬁcant role to play in the discovery of materials for future energy needs.},
	language = {en},
	number = {2},
	urldate = {2022-04-18},
	journal = {The Journal of Physical Chemistry Letters},
	author = {Cheng, Lei and Assary, Rajeev S. and Qu, Xiaohui and Jain, Anubhav and Ong, Shyue Ping and Rajput, Nav Nidhi and Persson, Kristin and Curtiss, Larry A.},
	month = jan,
	year = {2015},
	pages = {283--291},
}

@article{fedorov_ionic_2014,
	title = {Ionic {Liquids} at {Electrified} {Interfaces}},
	volume = {114},
	issn = {0009-2665, 1520-6890},
	url = {https://pubs.acs.org/doi/10.1021/cr400374x},
	doi = {10.1021/cr400374x},
	language = {en},
	number = {5},
	urldate = {2022-04-18},
	journal = {Chemical Reviews},
	author = {Fedorov, Maxim V. and Kornyshev, Alexei A.},
	month = mar,
	year = {2014},
	pages = {2978--3036},
}

@article{zhang_review_2006,
	title = {A review on electrolyte additives for lithium-ion batteries},
	volume = {162},
	issn = {03787753},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0378775306017538},
	doi = {10.1016/j.jpowsour.2006.07.074},
	abstract = {This paper reviews electrolyte additives used in Li-ion batteries. According to their functions, the additives can be divided into these categories: (1) solid electrolyte interface (SEI) forming improver, (2) cathode protection agent, (3) LiPF6 salt stabilizer, (4) safety protection agent, (5) Li deposition improver, and (6) other agents such as solvation enhancer, Al corrosion inhibitor, and wetting agent. The function and mechanism of each category additives are generally described and discussed.},
	language = {en},
	number = {2},
	urldate = {2022-04-18},
	journal = {Journal of Power Sources},
	author = {Zhang, Sheng Shui},
	month = nov,
	year = {2006},
	pages = {1379--1394},
}

@article{silva_revisiting_2020,
	title = {Revisiting {Ionic} {Liquid} {Structure}-{Property} {Relationship}: {A} {Critical} {Analysis}},
	volume = {21},
	issn = {1422-0067},
	shorttitle = {Revisiting {Ionic} {Liquid} {Structure}-{Property} {Relationship}},
	url = {https://www.mdpi.com/1422-0067/21/20/7745},
	doi = {10.3390/ijms21207745},
	abstract = {In the llast ffeew yyeeaars, iioonic lliiqquids ((ILs) hhave bbeen tthe ffooccus ooff eexxtteennsive studies concerning the relationship betweenn ssttrruuccttuurreeaannddpprrooppeerrttiieessaannddhhoowwtthhisisimimppaacctstsththeeiriraapppplilciacatitoionn. D. Desepsipteitea alalragregenunmumbebrerofofstsutuddieise,s,sesevverearlaltotoppicicssrreemmaaininccoonnttrroovveerrssiaialloorr nnoott fullyy answered, such aass: the existence of iioonnppaaiirrss,,ththeecoconncecpept tofofrfereeevovloulmume aenadndthetheeffeeﬀctecotf owfawteartaenr danitds imtspimlicpalticoantsioinsthine tmheodmuoladtiuolnatoiofnILosfpIhLysspichoychsiecmocihcaelmpircoapl eprrtioepse. rIntieths.isIpnatpheirs, pwaepper,eswenetparecrsietnictaal rcervitieicwalorfesvtiaetwe-ooffsthtaet-ea-rotfl-ittheer-aaturtrleitreergaaturdreinrgegstarrudcitnugres–trpurcotpuerert–ypreolpaetirotynsrheliaptioofnIsLhsi,pwoefrIeL-se,xwame irnee-eaxnaamlyintiecaalntahleyotricieasl tohnetohreiesstrouncthueres–tpruroctpuerret–ypcroorprelratytiocnosrraenladtipornesseanntdnperwespeenrtsnpewctipvesrsbpaescetdivoens bthaeseedxiostnintghedeaxtais.tTinhge dinattear.rTelhaetiionntebrreetlwateieon btreatnwsepeonrtrpanrospoertipesro(pveisrctioesit(yv,isdcoifsfiutys,iodniﬀ, ucsoinodnu, cotinvdituyc)tiovfitIyL) osftrIuLcstutrruectaunrde afrnede fvroeleuvmoeluamreeaanrealaynseadlyasenddadnidscduisssceudssaetda amt oalmecoulleacrulleavrelle.vInel.adIndiatdiodnit,iwone, dweemdoenmstornatsetrhaotewhtohwe tahneaalynsailsyosifsmoficmroicsrcoospciocpfiecafteuarteusre(ps a(prtairctuiclaurllayrluysuinsigngNNMMR-Rd-edreirvievdedddataata) )ccaannbbeeuusseeddttooeexxplain and predicctt macroossccooppiicc pprrooppeerrttiieess,, rreeaacchhiinngg nneeww ppeerrssppeeccttiivveess oonn tthhee prooppeerrttiieess aanndd appliiccaattiioonn of ILs.},
	language = {en},
	number = {20},
	urldate = {2022-03-09},
	journal = {International Journal of Molecular Sciences},
	author = {Silva, Wagner and Zanatta, Marcileia and Ferreira, Ana Sofia and Corvo, Marta C. and Cabrita, Eurico J.},
	month = oct,
	year = {2020},
	pages = {7745},
}

@article{marcus_ion_2006,
	title = {Ion {Pairing}},
	volume = {106},
	issn = {0009-2665, 1520-6890},
	url = {https://pubs.acs.org/doi/10.1021/cr040087x},
	doi = {10.1021/cr040087x},
	language = {en},
	number = {11},
	urldate = {2022-03-09},
	journal = {Chemical Reviews},
	author = {Marcus, Yizhak and Hefter, Glenn},
	month = nov,
	year = {2006},
	pages = {4585--4621},
}

@article{macfarlane_concept_2009,
	title = {On the concept of ionicity in ionic liquids},
	volume = {11},
	issn = {1463-9076, 1463-9084},
	url = {http://xlink.rsc.org/?DOI=b900201d},
	doi = {10.1039/b900201d},
	language = {en},
	number = {25},
	urldate = {2022-03-09},
	journal = {Physical Chemistry Chemical Physics},
	author = {MacFarlane, Douglas R. and Forsyth, Maria and Izgorodina, Ekaterina I. and Abbott, Andrew P. and Annat, Gary and Fraser, Kevin},
	year = {2009},
	pages = {4962},
}

@article{zhang_direct_2015,
	title = {Direct {Correlation} between {Ionic} {Liquid} {Transport} {Properties} and {Ion} {Pair} {Lifetimes}: {A} {Molecular} {Dynamics} {Study}},
	volume = {6},
	issn = {1948-7185, 1948-7185},
	shorttitle = {Direct {Correlation} between {Ionic} {Liquid} {Transport} {Properties} and {Ion} {Pair} {Lifetimes}},
	url = {https://pubs.acs.org/doi/10.1021/acs.jpclett.5b00003},
	doi = {10.1021/acs.jpclett.5b00003},
	abstract = {Self-diﬀusivities as a function of temperature were computed for 29 diﬀerent ionic liquids (ILs) covering a wide variety of cation and anion classes. Ideal ionic conductivities (σNE) were estimated from the self-diﬀusivities via the Nernst− Einstein relation. The ion pair (IP) lifetimes (τIP) and ion cage (IC) lifetimes (τIC) of each IL were also computed. A linear relationship between the calculated self-diﬀusivities and the inverse of IP or IC lifetimes was observed. A similar inverse linear relationship was also observed for ideal ionic conductivity. These relationships were found to be independent of temperature and the nature of the IL. These observations connect macroscopic dynamic properties with local atomic-level motions and strongly suggest that the dynamics of ILs are governed by a universal IP or IC forming and breaking mechanism. Thus, in order to design an ionic liquid with enhanced dynamics, one should consider how to minimize IP or IC lifetimes.},
	language = {en},
	number = {4},
	urldate = {2022-03-09},
	journal = {The Journal of Physical Chemistry Letters},
	author = {Zhang, Yong and Maginn, Edward J.},
	month = feb,
	year = {2015},
	pages = {700--705},
}

@article{avni_conductivity_2022,
	title = {Conductivity of {Concentrated} {Electrolytes}},
	volume = {128},
	issn = {0031-9007, 1079-7114},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.128.098002},
	doi = {10.1103/PhysRevLett.128.098002},
	language = {en},
	number = {9},
	urldate = {2022-03-06},
	journal = {Physical Review Letters},
	author = {Avni, Yael and Adar, Ram M. and Andelman, David and Orland, Henri},
	month = mar,
	year = {2022},
	pages = {098002},
}

@article{harris_comment_2018,
	title = {Comment on “{Ionic} {Conductivity}, {Diffusion} {Coefficients}, and {Degree} of {Dissociation} in {Lithium} {Electrolytes}, {Ionic} {Liquids}, and {Hydrogel} {Polyelectrolytes}”},
	volume = {122},
	issn = {1520-6106, 1520-5207},
	url = {https://pubs.acs.org/doi/10.1021/acs.jpcb.8b08610},
	doi = {10.1021/acs.jpcb.8b08610},
	language = {en},
	number = {48},
	urldate = {2022-03-06},
	journal = {The Journal of Physical Chemistry B},
	author = {Harris, Kenneth R.},
	month = dec,
	year = {2018},
	pages = {10964--10967},
}

@article{mcdaniel_ion_2018,
	title = {Ion {Correlation} and {Collective} {Dynamics} in {BMIM}/{BF} $_{\textrm{4}}$ -{Based} {Organic} {Electrolytes}: {From} {Dilute} {Solutions} to the {Ionic} {Liquid} {Limit}},
	volume = {122},
	issn = {1520-6106, 1520-5207},
	shorttitle = {Ion {Correlation} and {Collective} {Dynamics} in {BMIM}/{BF} $_{\textrm{4}}$ -{Based} {Organic} {Electrolytes}},
	url = {https://pubs.acs.org/doi/10.1021/acs.jpcb.8b04886},
	doi = {10.1021/acs.jpcb.8b04886},
	abstract = {Quantifying ion association and collective dynamical processes in organic electrolytes is essential for fundamental property interpretation and optimization for electrochemical applications. The extent of ion correlation depends on both the ion concentration and dielectric strength of the solvent; ions may be largely uncorrelated in suﬃciently high-dielectric solvents at low concentration, but properties of concentrated electrolytes are dictated by correlated and collective ion processes. In this work, we utilize molecular dynamics simulations to characterize ion association and collective ion dynamics in organic electrolytes composed of binary mixtures of 1-butyl-3-methylimidazolium tetraﬂuoroborate [BMIM+][BF4−] and 1,2-dichloroethane, acetone, acetonitrile, and water solvents. We illustrate diﬀerent physical regimes of characteristically distinct ion correlations for the systematic range of electrolyte concentrations and solvent dielectric strengths. Dilute electrolytes composed of low-dielectric solvents exhibit signiﬁcant counterion correlation in the form of ion pairing and clustering driven by both weak screening and relatively low solvation energies. This regime is characterized by enhanced ion coordination numbers and near equality of cation and anion diﬀusion coeﬃcients, despite the signiﬁcantly diﬀerent ion sizes. In contrast, ion correlation in highly concentrated electrolytes is dominated by the anti-correlated motion of both like-charge and opposite-charge ions, approaching neat ionic liquid behavior. We show that the cross-over of these correlation regimes is clearly illuminated by quantifying the fractional self and distinct contributions to the net ionic conductivity. For organic electrolytes composed of low-dielectric solvents, we conclude that signiﬁcant ion correlation exists at all concentrations but the nature of the correlation changes markedly from the dilute electrolyte to the pure ionic liquid limit.},
	language = {en},
	number = {28},
	urldate = {2022-03-06},
	journal = {The Journal of Physical Chemistry B},
	author = {McDaniel, Jesse G. and Son, Chang Yun},
	month = jul,
	year = {2018},
	pages = {7154--7169},
}

@article{ardhra_effect_2022,
	title = {Effect of {Concentration} and {Temperature} on the {Structure} and {Ion} {Transport} in {Diglyme}-{Based} {Sodium}-{Ion} {Electrolyte}},
	issn = {1520-6106, 1520-5207},
	url = {https://pubs.acs.org/doi/10.1021/acs.jpcb.2c00557},
	doi = {10.1021/acs.jpcb.2c00557},
	language = {en},
	urldate = {2022-03-06},
	journal = {The Journal of Physical Chemistry B},
	author = {Ardhra, Shylendran and Prakash, Prabhat and Siva Dev, Rabin and Venkatnathan, Arun},
	month = mar,
	year = {2022},
	pages = {acs.jpcb.2c00557},
}

@article{kivela_effect_2022,
	title = {Effect of {Water} on a {Hydrophobic} {Deep} {Eutectic} {Solvent}},
	volume = {126},
	issn = {1520-6106, 1520-5207},
	url = {https://pubs.acs.org/doi/10.1021/acs.jpcb.1c08170},
	doi = {10.1021/acs.jpcb.1c08170},
	abstract = {Deep eutectic solvents (DESs) formed by hydrogen bond donors and acceptors are a promising new class of solvents. Both hydrophilic and hydrophobic binary DESs readily absorb water, making them ternary mixtures, and a small water content is always inevitable under ambient conditions. We present a thorough study of a typical hydrophobic DES formed by a 1:2 mole ratio of tetrabutyl ammonium chloride and decanoic acid, focusing on the eﬀects of a low water content caused by absorbed water vapor, using multinuclear NMR techniques, molecular modeling, and several other physicochemical techniques. Already very low water contents cause dynamic nanoscale phase segregation, reduce solvent viscosity and fragility, increase self-diﬀusion coeﬃcients and conductivity, and enhance local dynamics. Water interferes with the hydrogen-bonding network between the chloride ions and carboxylic acid groups by solvating them, which enhances carboxylic acid self-correlation and ion pair formation between tetrabutyl ammonium and chloride. Simulations show that the component molar ratio can be varied, with an eﬀect on the internal structure. The water-induced changes in the physical properties are beneﬁcial for most prospective applications but water creates an acidic aqueous nanophase with a high halide ion concentration, which may have chemically adverse eﬀects.},
	language = {en},
	number = {2},
	urldate = {2022-03-06},
	journal = {The Journal of Physical Chemistry B},
	author = {Kivelä, Henri and Salomäki, Mikko and Vainikka, Petteri and Mäkilä, Ermei and Poletti, Fabrizio and Ruggeri, Stefano and Terzi, Fabio and Lukkari, Jukka},
	month = jan,
	year = {2022},
	pages = {513--527},
}

@article{zhang_salting-out_2016,
	title = {Salting-{Out} and {Salting}-{In} of {Polyelectrolyte} {Solutions}: {A} {Liquid}-{State} {Theory} {Study}},
	volume = {49},
	issn = {0024-9297, 1520-5835},
	shorttitle = {Salting-{Out} and {Salting}-{In} of {Polyelectrolyte} {Solutions}},
	url = {https://pubs.acs.org/doi/10.1021/acs.macromol.6b02160},
	doi = {10.1021/acs.macromol.6b02160},
	abstract = {We study the phase behavior of polyelectrolyte (PE) solutions with salt using a simple liquid-state (LS) theory. This LS theory accounts for hard-core excluded volume repulsion by the Boublik−Mansoori−Carnahan− Starling−Leland equation of state, electrostatic correlation by the mean-spherical approximation, and chain connectivity by the ﬁrst-order thermodynamic perturbation theory. We predict a closed-loop binodal curve in the PE concentration-salt concentration phase diagram when the Bjerrum length is smaller than the critical Bjerrum length in salt-free PE solution. The phase-separated region shrinks with decreasing Bjerrum length, and disappears below a critical Bjerrum length. These results are qualitatively consistent with experiments, but cannot be captured by the Voorn−Overbeek theory. On the basis of the closed-loop binodal curve and the lever rule, we predict three scenarios of salting-out and salting-in phenomena with addition of monovalent salt into an initially salt-free PE solution. The Galvani potentialthe electric potential diﬀerence between the coexisting phasesis found to depend nonmonotonically on the overall salt concentration in some PE concentration range, which is related to the partition of the co-ions in the coexisting phases. Free energy analysis suggests that phase separation is driven by a gain in the electrostatic energy, at the expense of a large translational entropy penalty, due to signiﬁcant counterion accumulation in the PE-rich phase.},
	language = {en},
	number = {24},
	urldate = {2022-02-24},
	journal = {Macromolecules},
	author = {Zhang, Pengfei and Alsaifi, Nayef M. and Wu, Jianzhong and Wang, Zhen-Gang},
	month = dec,
	year = {2016},
	pages = {9720--9730},
}

@article{murata_microscopic_2015,
	title = {Microscopic identification of the order parameter governing liquid–liquid transition in a molecular liquid},
	volume = {112},
	issn = {0027-8424, 1091-6490},
	url = {http://www.pnas.org/lookup/doi/10.1073/pnas.1501149112},
	doi = {10.1073/pnas.1501149112},
	abstract = {A liquid–liquid transition (LLT) in a single-component substance is an unconventional phase transition from one liquid to another. LLT has recently attracted considerable attention because of its fundamental importance in our understanding of the liquid state. To access the order parameter governing LLT from a microscopic viewpoint, here we follow the structural evolution during the LLT of an organic molecular liquid, triphenyl phosphite (TPP), by time-resolved small- and wide-angle X-ray scattering measurements. We find that locally favored clusters, whose characteristic size is a few nanometers, are spontaneously formed and their number density monotonically increases during LLT. This strongly suggests that the order parameter of LLT is the number density of locally favored structures and of nonconserved nature. We also show that the locally favored structures are distinct from the crystal structure and these two types of orderings compete with each other. Thus, our study not only experimentally identifies the structural order parameter governing LLT, but also may settle a long-standing debate on the nature of the transition in TPP, i.e., whether the transition is LLT or merely microcrystal formation.},
	language = {en},
	number = {19},
	urldate = {2022-02-24},
	journal = {Proceedings of the National Academy of Sciences},
	author = {Murata, Ken-ichiro and Tanaka, Hajime},
	month = may,
	year = {2015},
	pages = {5956--5961},
}

@article{tanaka_bond_2012,
	title = {Bond orientational order in liquids: {Towards} a unified description of water-like anomalies, liquid-liquid transition, glass transition, and crystallization: {Bond} orientational order in liquids},
	volume = {35},
	issn = {1292-8941, 1292-895X},
	shorttitle = {Bond orientational order in liquids},
	url = {http://link.springer.com/10.1140/epje/i2012-12113-y},
	doi = {10.1140/epje/i2012-12113-y},
	abstract = {There are at least three fundamental states of matter, depending upon temperature and pressure: gas, liquid, and solid (crystal). These states are separated by ﬁrst-order phase transitions between them. In both gas and liquid phases a complete translational and rotational symmetry exist, whereas in a solid phase both symmetries are broken. In intermediate phases between liquid and solid, which include liquid crystal and plastic crystal phases, only one of the two symmetries is preserved. Among the fundamental states of matter, the liquid state is the most poorly understood. We argue that it is crucial for a better understanding of liquids to recognize that a liquid generally has the tendency to have a local structural order and its presence is intrinsic and universal to any liquid. Such structural ordering is a consequence of many-body correlations, more speciﬁcally, bond angle correlations, which we believe are crucial for the description of the liquid state. We show that this physical picture may naturally explain diﬃcult unsolved problems associated with the liquid state, such as anomalies of water-type liquids (water, Si, Ge, . . . ), liquid-liquid transition, liquid-glass transition, crystallization and quasicrystal formation, in a uniﬁed manner. In other words, we need a new order parameter representing a low local free-energy conﬁguration, which is a bond orientational order parameter in many cases, in addition to a density order parameter for the physical description of these phenomena. Here we review our two-order-parameter model of liquid and consider how transient local structural ordering is linked to all of the above-mentioned phenomena. The relationship between these phenomena is also discussed.},
	language = {en},
	number = {10},
	urldate = {2022-02-24},
	journal = {The European Physical Journal E},
	author = {Tanaka, Hajime},
	month = oct,
	year = {2012},
	pages = {113},
}

@article{kobayashi_reversibility_2016,
	title = {The reversibility and first-order nature of liquid–liquid transition in a molecular liquid},
	volume = {7},
	issn = {2041-1723},
	url = {http://www.nature.com/articles/ncomms13438},
	doi = {10.1038/ncomms13438},
	language = {en},
	number = {1},
	urldate = {2022-02-24},
	journal = {Nature Communications},
	author = {Kobayashi, Mika and Tanaka, Hajime},
	month = dec,
	year = {2016},
	pages = {13438},
}

@article{zhang_supernatant_nodate,
	title = {The {Supernatant} {Phase} in {Polyelectrolyte} {Complex} {Coacervation}: {Cluster} {Formation}, {Binodal}, and {Nucleation}},
	language = {en},
	author = {Zhang, Pengfei and Wang, Zhen-Gang},
	pages = {47},
}

@article{zhang_interfacial_2021,
	title = {Interfacial {Structure} and {Tension} of {Polyelectrolyte} {Complex} {Coacervates}},
	volume = {54},
	issn = {0024-9297, 1520-5835},
	url = {https://pubs.acs.org/doi/10.1021/acs.macromol.1c01809},
	doi = {10.1021/acs.macromol.1c01809},
	abstract = {We develop a simple inhomogeneous mean-ﬁeld theory to study the interfacial structure and tension of polyelectrolyte complex coacervates in equilibrium with a supernatant solution. Our theory treats the electrostatic correlation by combining the Debye−Hückel theory with the ﬁrst-order thermodynamic perturbation theory within the local density approximation, and incorporates the conformation entropy contribution for both polyions using Lifshitz’s ground-state dominance approximation. Using this theory, we systematically examine the interfacial properties of both symmetric and concentrationasymmetric coacervates. The interfacial tension γ is generally rather low, on the order of 1 mN/m or less. For asymmetric coacervates, an intricate electric double layer forms in the interfacial region, which can even contain several oscillations under certain conditions. The interfacial tension generally decreases with increasing the stoichiometric asymmetry, the added-salt concentration, and the initial polymer concentration of the mixture. We further ﬁnd that the interfacial tension can be quantitatively related to the degree of phase separation S, where S is the Euclidean distance in composition between the two coexisting phases. In particular, we ﬁnd that γ as a function of S for diﬀerent concentration asymmetries collapses approximately to two master curves, which merge together and follow γ ∼ S3 for small S.},
	language = {en},
	number = {23},
	urldate = {2022-02-24},
	journal = {Macromolecules},
	author = {Zhang, Pengfei and Wang, Zhen-Gang},
	month = dec,
	year = {2021},
	pages = {10994--11007},
}

@article{harris_evidence_2021,
	title = {Evidence of a liquid–liquid transition in a glass-forming ionic liquid},
	volume = {118},
	issn = {0027-8424, 1091-6490},
	url = {http://www.pnas.org/lookup/doi/10.1073/pnas.2020878118},
	doi = {10.1073/pnas.2020878118},
	abstract = {A liquid–liquid transition (LLT) is a transformation from one liquid to another through a first-order transition. The LLT is fundamental to the understanding of the liquid state and has been reported in a few materials such as silicon, phosphorus, triphenyl phosphite, and water. Furthermore, it has been suggested that the unique properties of materials such as water, which is critical for life on the planet, are linked to the existence of the LLT. However, the experimental evidence for the existence of an LLT in many molecular liquids remains controversial, due to the prevalence and high propensity of the materials to crystallize. Here, we show evidence of an LLT in a glass-forming trihexyltetradecylphosphonium borohydride ionic liquid that shows no tendency to crystallize under normal laboratory conditions. We observe a step-like increase in the static dielectric permittivity at the transition. Furthermore, the sizes of nonpolar local domains and ion-coordination numbers deduced from wide-angle X-ray scattering also change abruptly at the LLT. We independently corroborate these changes in local organization using Raman spectroscopy. The experimental access to the evolution of local order and structural dynamics across a liquid–liquid transition opens up unprecedented possibilities to understand the nature of the liquid state.},
	language = {en},
	number = {11},
	urldate = {2022-02-09},
	journal = {Proceedings of the National Academy of Sciences},
	author = {Harris, Matthew A. and Kinsey, Thomas and Wagle, Durgesh V. and Baker, Gary A. and Sangoro, Joshua},
	month = mar,
	year = {2021},
	pages = {e2020878118},
}

@article{harris_relations_2010,
	title = {Relations between the {Fractional} {Stokes}−{Einstein} and {Nernst}−{Einstein} {Equations} and {Velocity} {Correlation} {Coefficients} in {Ionic} {Liquids} and {Molten} {Salts}},
	volume = {114},
	issn = {1520-6106, 1520-5207},
	url = {https://pubs.acs.org/doi/10.1021/jp102687r},
	doi = {10.1021/jp102687r},
	language = {en},
	number = {29},
	urldate = {2022-02-02},
	journal = {The Journal of Physical Chemistry B},
	author = {Harris, Kenneth R.},
	month = jul,
	year = {2010},
	pages = {9572--9577},
}

@article{harris_can_2016,
	title = {Can the {Transport} {Properties} of {Molten} {Salts} and {Ionic} {Liquids} {Be} {Used} {To} {Determine} {Ion} {Association}?},
	volume = {120},
	issn = {1520-6106, 1520-5207},
	url = {https://pubs.acs.org/doi/10.1021/acs.jpcb.6b08381},
	doi = {10.1021/acs.jpcb.6b08381},
	abstract = {There have long been arguments supporting the concept of ion association in molten salts and ionic liquids, largely based on diﬀerences between the conductivity and that predicted from self-diﬀusion coeﬃcients by the Nernst−Einstein equation for noninteracting ions. It is known from molecular dynamics simulations that even simple models based on charged hard spheres show such a diﬀerence due to the (anti)-correlation of ion motions. Formally this is expressed as a diﬀerence between the velocity crosscorrelation coeﬃcient of the oppositely charged ions and the mean of those for the two like-charged ions. This article examines molten salt and ionic liquid transport property data, comparing simple and model associated salts (ZnCl2, PbCl2, and TlCl) including weakly dissociated molecular liquids (H2O, HCOOH, H2SO4). Analysis employing Laity resistance coeﬃcients (rij) shows that the common ion-association rationalization is ﬂawed, consistent with recent direct measurements of the degree of ionicity in ionic liquid chlorides and with theoretical studies. However, the protic ionic liquids [PyrOMe][BF4] and [DBUH][CH3SO3] have larger than usual NE deviation parameters ({\textgreater}0.5), and large negative like-ion rii, analogous to those of ZnCl2. Structural, spectroscopic, and theoretical studies are suggested to determine whether these are indeed genuine examples of association.},
	language = {en},
	number = {47},
	urldate = {2022-02-02},
	journal = {The Journal of Physical Chemistry B},
	author = {Harris, Kenneth R.},
	month = dec,
	year = {2016},
	pages = {12135--12147},
}

@article{raju_aqueous_2009,
	title = {Aqueous {Solution} of [bmim][{PF} $_{\textrm{6}}$ ]: {Ion} and {Solvent} {Effects} on {Structure} and {Dynamics}},
	volume = {113},
	issn = {1520-6106, 1520-5207},
	shorttitle = {Aqueous {Solution} of [bmim][{PF} $_{\textrm{6}}$ ]},
	url = {https://pubs.acs.org/doi/10.1021/jp8111777},
	doi = {10.1021/jp8111777},
	language = {en},
	number = {14},
	urldate = {2022-02-02},
	journal = {The Journal of Physical Chemistry B},
	author = {Raju, S. G. and Balasubramanian, S.},
	month = apr,
	year = {2009},
	pages = {4799--4806},
}

@article{bester-rogac_mobility_2016,
	title = {Mobility and association of ions in aqueous solutions: the case of imidazolium based ionic liquids},
	volume = {18},
	issn = {1463-9076, 1463-9084},
	shorttitle = {Mobility and association of ions in aqueous solutions},
	url = {http://xlink.rsc.org/?DOI=C6CP05010G},
	doi = {10.1039/C6CP05010G},
	abstract = {Combining MD simulations and RISM calculations with experiments, we demonstrated that the interionic interactions of investigated ILs as model 1,1 electrolytes in water solutions are weak but evidently dependent on the molecular structure.
          , 
            The mobility and the mechanism of ion pairing of 1,1 electrolytes in aqueous solutions were investigated systematically on nine imidazolium based ionic liquids (ILs) from 1-methylimidazolium chloride, [MIM][Cl], to 1-dodecyl-3-methylimidazolium chloride, [1,3-DoMIM][Cl], with two isomers 1,2-dimethylimidazolium chloride, [1,2-MMIM][Cl], and 1,3-dimethylimidazolium chloride, [1,3-MMIM][Cl]. Molecular dynamics (MD) simulations, statistical mechanics calculations in the framework of the integral equation theory using one-dimensional (1D-) and three-dimensional (3D-) reference interaction site model (RISM) approaches as well as conductivity measurements were applied. From experiment and MD simulations it was found that the mobility/diffusion coefficients of cations in the limit of infinite dilution decrease with an increasing length of the cation alkyl chain, but not linearly. The aggregation tendency of cations with long alkyl chains at higher IL concentrations impedes their diffusivity. Binding free energies of imidazolium cations with the chloride anion estimated by RISM calculations, MD simulations and experiments reveal that the association of investigated ILs as model 1,1 electrolytes in water solutions is weak but evidently dependent on the molecular structure (alkyl chain length), which also strongly affects the mobility of cations.},
	language = {en},
	number = {41},
	urldate = {2022-02-02},
	journal = {Physical Chemistry Chemical Physics},
	author = {Bešter-Rogač, Marija and Fedotova, Marina V. and Kruchinin, Sergey E. and Klähn, Marco},
	year = {2016},
	pages = {28594--28605},
}

@article{doherty_revisiting_2017,
	title = {Revisiting {OPLS} {Force} {Field} {Parameters} for {Ionic} {Liquid} {Simulations}},
	volume = {13},
	issn = {1549-9618, 1549-9626},
	url = {https://pubs.acs.org/doi/10.1021/acs.jctc.7b00520},
	doi = {10.1021/acs.jctc.7b00520},
	abstract = {Our OPLS-2009IL force ﬁeld parameters (J. Chem. Theory Comput. 2009, 5, 1038−1050) were originally developed and tested on 68 unique ionic liquids featuring the 1-alkyl-3-methylimidazolium [RMIM], N-alkylpyridinium [RPyr], and choline cations. Experimental validation was limited to densities and a few, largely conﬂicting, heat of vaporization (ΔHvap) values reported in the literature at the time. Owing to the use of Monte Carlo as our sampling technique, it was also not possible to investigate the reproduction of dynamics. The [RMIM] OPLS-2009IL parameters have been revisited in this work and adapted for use in molecular dynamics (MD) simulations. In addition, new OPLS-AA parameters have been developed for multiple anions, i.e., AlCl4−, BF4−, Br−, Cl−, NO3−, PF6−, acetate, benzoate bis(pentaﬂuoroethylsulfonyl)amide, bis(triﬂuoroethylsulfonyl)amide, dicyanamide, formate, methylsulfate, perchlorate, propanoate, thiocyanate, tricyanomethanide, and triﬂuoromethanesulfonate. The computed solvent densities, heats of vaporization, viscosities, diﬀusion coeﬃcients, heat capacities, surface tensions, and other relevant solvent data compared favorably with experiment. A charge scaling of ±0.8 e was also investigated as a means to mimic polarization and charge transfer eﬀects. The 0.8-scaling led to signiﬁcant improvements for ΔHvap, surface tension, and self-diﬀusivity; however, a concern when scaling charges is the potential degradation of local intermolecular interactions at short ranges. Radial distribution functions (RDFs) were used to examine cation−anion interactions when employing 0.8*OPLS-2009IL and the scaled force ﬁeld accurately reproduced RDFs from ab initio MD simulations.},
	language = {en},
	number = {12},
	urldate = {2022-02-02},
	journal = {Journal of Chemical Theory and Computation},
	author = {Doherty, Brian and Zhong, Xiang and Gathiaka, Symon and Li, Bin and Acevedo, Orlando},
	month = dec,
	year = {2017},
	pages = {6131--6145},
}

@article{bhargava_refined_2007,
	title = {Refined potential model for atomistic simulations of ionic liquid [bmim][{PF6}]},
	volume = {127},
	issn = {0021-9606, 1089-7690},
	url = {http://aip.scitation.org/doi/10.1063/1.2772268},
	doi = {10.1063/1.2772268},
	language = {en},
	number = {11},
	urldate = {2022-02-02},
	journal = {The Journal of Chemical Physics},
	author = {Bhargava, B. L. and Balasubramanian, S.},
	month = sep,
	year = {2007},
	pages = {114510},
}

@article{doherty_virtual_2018,
	title = {Virtual {Site} {OPLS} {Force} {Field} for {Imidazolium}-{Based} {Ionic} {Liquids}},
	volume = {122},
	issn = {1520-6106, 1520-5207},
	url = {https://pubs.acs.org/doi/10.1021/acs.jpcb.7b11996},
	doi = {10.1021/acs.jpcb.7b11996},
	abstract = {Molecular simulations of ionic liquids can provide deeper insight into the relationship between intermolecular interactions and macroscopic measurements for the solvents. However, many existing force ﬁelds have multiple shortcomings, including poor solvent dynamics, the underestimation of hydrogen-bonding strength, and errors in solvent interactions/organization. A new force ﬁeld, called optimized potentials for liquid simulation-ionic-liquid virtual site (OPLS-VSIL), has been developed for imidazolium-based ionic liquids featuring a novel topology incorporating a virtual site bisecting the nitrogen atoms that oﬄoads negative charge to inside the plane of the ring. Guided by free energy of hydration calculations, an empirically derived set of partial charges and nonbonded Lennard-Jones terms for both 1-alkyl-3-methylimidazolium and 11 diﬀerent anions provided accurate bulk-phase ionic-liquid properties and produced radial distribution functions nearly indistinguishable from ab initio molecular dynamics simulations. For example, overall mean absolute errors (MAEs) of 3.1−3.4\% were computed for the density, heat of vaporization, and viscosity of approximately 20 diﬀerent ion pair combinations. Additional physical properties, such as, self-diﬀusion coeﬃcients, heat capacity, and surface tension also gave signiﬁcant MAE improvements using OPLS-VSIL compared to the existing ﬁxed-charge ionic-liquid force ﬁelds. Local interactions, including cation−anion hydrogen bonding and π−π stacking between the imidazolium rings, were also accurately reproduced.},
	language = {en},
	number = {11},
	urldate = {2022-02-01},
	journal = {The Journal of Physical Chemistry B},
	author = {Doherty, Brian and Zhong, Xiang and Acevedo, Orlando},
	month = mar,
	year = {2018},
	pages = {2962--2974},
}

@article{bedrov_molecular_2019,
	title = {Molecular {Dynamics} {Simulations} of {Ionic} {Liquids} and {Electrolytes} {Using} {Polarizable} {Force} {Fields}},
	volume = {119},
	issn = {0009-2665, 1520-6890},
	url = {https://pubs.acs.org/doi/10.1021/acs.chemrev.8b00763},
	doi = {10.1021/acs.chemrev.8b00763},
	abstract = {Many applications in chemistry, biology, and energy storage/conversion research rely on molecular simulations to provide fundamental insight into structural and transport properties of materials with high ionic concentrations. Whether the system is comprised entirely of ions, like ionic liquids, or is a mixture of a polar solvent with a salt, e.g., liquid electrolytes for battery applications, the presence of ions in these materials results in strong local electric ﬁelds polarizing solvent molecules and large ions. To predict properties of such systems from molecular simulations often requires either explicit or mean-ﬁeld inclusion of the inﬂuence of polarization on electrostatic interactions. In this manuscript, we review the pros and cons of diﬀerent treatments of polarization ranging from the mean-ﬁeld approaches to the most popular explicit polarization models in molecular dynamics simulations of ionic materials. For each method, we discuss their advantages and disadvantages and emphasize key assumptions as well as their adjustable parameters. Strategies for the development of polarizable models are presented with a speciﬁc focus on extracting atomic polarizabilities. Finally, we compare simulations using polarizable and nonpolarizable models for several classes of ionic systems, discussing the underlying physics that each approach includes or ignores, implications for implementation and computational eﬃciency, and the accuracy of properties predicted by these methods compared to experiments.},
	language = {en},
	number = {13},
	urldate = {2022-02-01},
	journal = {Chemical Reviews},
	author = {Bedrov, Dmitry and Piquemal, Jean-Philip and Borodin, Oleg and MacKerell, Alexander D. and Roux, Benoît and Schröder, Christian},
	month = jul,
	year = {2019},
	pages = {7940--7995},
}

@article{carneiro_density_2014,
	title = {Density of {Mixtures} {Containing} {Sugars} and {Ionic} {Liquids}: {Experimental} {Data} and {PC}-{SAFT} {Modeling}},
	volume = {59},
	issn = {0021-9568, 1520-5134},
	shorttitle = {Density of {Mixtures} {Containing} {Sugars} and {Ionic} {Liquids}},
	url = {https://pubs.acs.org/doi/10.1021/je500079y},
	doi = {10.1021/je500079y},
	abstract = {The potential use of ionic liquids (ILs) for biomass and carbohydrate processing has been discovered in the past decade. Many advantages have been pointed out in their application for bioreﬁning purposes. The phase equilibria and volumetric properties of mixtures containing ILs and biomass-derived compounds such as sugars or sugar alcohols are relevant for process design. In this work, the density, at atmospheric pressure, of binary mixtures containing sugars (glucose and fructose) or sugar alcohols (xylitol and sorbitol) and ionic liquids (1-ethyl-3methylimidazolium ethylsulfate and Aliquat336) is presented within large temperature (278 K to 343 K) and composition ranges (up to sugar or sugar alcohol mass fraction of 0.30). The density data followed a bilinear trend with respect to temperature and composition. The data were therefore represented using planar regression with a very good accuracy, average relative deviation (ARD) {\textless} 0.1 \% in most of the cases. The perturbed-chain statistical association ﬂuid theory (PCSAFT) equation of state was applied to model solutions containing ILs. The pure-component parameters for Aliquat336 were ﬁtted to pure-IL density data. Applying temperature-dependent kij parameters, PC-SAFT allowed satisfactory modeling of the measured density data and literature solubility data of sugars and sugar alcohols in Aliquat336.},
	language = {en},
	number = {10},
	urldate = {2021-09-30},
	journal = {Journal of Chemical \& Engineering Data},
	author = {Carneiro, Aristides P. and Rodríguez, Oscar and Held, Christoph and Sadowski, Gabriele and A. Macedo, Eugénia},
	month = oct,
	year = {2014},
	pages = {2942--2954},
}

@article{chen_modeling_2012,
	title = {Modeling the {Solubility} of {Carbon} {Dioxide} in {Imidazolium}-{Based} {Ionic} {Liquids} with the {PC}-{SAFT} {Equation} of {State}},
	volume = {116},
	issn = {1520-6106, 1520-5207},
	url = {https://pubs.acs.org/doi/10.1021/jp309944t},
	doi = {10.1021/jp309944t},
	abstract = {The goal of this work was to check the ability of the PC-SAFT equation to represent the solubility of carbon dioxide (CO2) in ionic liquids. Parameters of pure imidazoliumbased ionic liquids were estimated using experimental densities over a large range of temperatures and then correlated with respect to the molecular weight and structure of the solvents. It was found that such a correlation is able to predict the density with high accuracy. The solubility of carbon dioxide in such ionic liquids was then studied. The binary interaction parameter kij needed for the representation of such binary systems was ﬁrst ﬁtted to experimental liquid−vapor equilibria data. In a second step, a correlation based on the group contribution concept was developed to determine this temperature-dependent parameter. The ability of the model to describe accurately carbon dioxide solubility in imidazolium-based ionic liquids is demonstrated.},
	language = {en},
	number = {49},
	urldate = {2021-09-30},
	journal = {The Journal of Physical Chemistry B},
	author = {Chen, Yushu and Mutelet, Fabrice and Jaubert, Jean-Noël},
	month = dec,
	year = {2012},
	pages = {14375--14388},
}

@article{mceldrew_theory_2020,
	title = {Theory of ion aggregation and gelation in super-concentrated electrolytes},
	volume = {152},
	issn = {0021-9606, 1089-7690},
	url = {http://aip.scitation.org/doi/10.1063/5.0006197},
	doi = {10.1063/5.0006197},
	abstract = {In concentrated electrolytes with asymmetric or irregular ions, such as ionic liquids and solvent-in-salt electrolytes, ion association is more complicated than simple ion-pairing. Large branched aggregates can form at significant concentrations at even moderate salt concentrations. When the extent of ion association reaches a certain threshold, a percolating ionic gel network can form spontaneously. Gelation is a phenomenon that is well known in polymer physics, but it is practically unstudied in concentrated electrolytes. However, despite this fact, the ion-pairing description is often applied to these systems for the sake of simplicity. In this work, drawing strongly from established theories in polymer physics, we develop a simple thermodynamic model of reversible ionic aggregation and gelation in concentrated electrolytes accounting for the competition between ion solvation and ion association. Our model describes, with the use of several phenomenological parameters, the populations of ionic clusters of different sizes as a function of salt concentration; it captures the onset of ionic gelation and also the post-gel partitioning of ions into the gel. We discuss the applicability of our model, as well as the implications of its predictions on thermodynamic, transport, and rheological properties.},
	language = {en},
	number = {23},
	urldate = {2022-01-22},
	journal = {The Journal of Chemical Physics},
	author = {McEldrew, Michael and Goodwin, Zachary A. H. and Bi, Sheng and Bazant, Martin Z. and Kornyshev, Alexei A.},
	month = jun,
	year = {2020},
	pages = {234506},
}

@article{fong_ion_2021,
	title = {Ion {Correlations} and {Their} {Impact} on {Transport} in {Polymer}-{Based} {Electrolytes}},
	volume = {54},
	issn = {0024-9297, 1520-5835},
	url = {https://pubs.acs.org/doi/10.1021/acs.macromol.0c02545},
	doi = {10.1021/acs.macromol.0c02545},
	abstract = {The development of next-generation polymer-based electrolytes for energy storage applications would greatly beneﬁt from a deeper understanding of transport phenomena in these systems. In this Perspective, we argue that the Onsager transport equations provide an intuitive but underutilized framework for analyzing transport in polymer-based electrolytes. Unlike the ubiquitous Stefan− Maxwell equations, the Onsager framework generates transport coeﬃcients with clear physical interpretation at the atomistic level and can be computed easily from molecular simulations using Green−Kubo relations. Herein we present an overview of the Onsager transport theory as it applies to polymer-based electrolytes and discuss its relation to experimentally measurable transport properties and the Stefan−Maxwell equations. Using case studies from recent computational work, we demonstrate how this framework can clarify nonintuitive phenomena such as negative cation transference number, anticorrelated cation−anion motion, and the dramatic failure of the Nernst−Einstein approximation. We discuss how insights from such analysis can inform design rules for improved systems.},
	language = {en},
	number = {6},
	urldate = {2022-01-22},
	journal = {Macromolecules},
	author = {Fong, Kara D. and Self, Julian and McCloskey, Bryan D. and Persson, Kristin A.},
	month = mar,
	year = {2021},
	pages = {2575--2591},
}

@article{lee_complex_2021,
	title = {Complex {Coacervation} of {Polymerized} {Ionic} {Liquids} in {Non}-aqueous {Solvents}},
	volume = {1},
	issn = {2694-2453, 2694-2453},
	url = {https://pubs.acs.org/doi/10.1021/acspolymersau.1c00017},
	doi = {10.1021/acspolymersau.1c00017},
	abstract = {Oppositely charged polymerized ionic liquids (PILs) were used to form complex coacervates in two diﬀerent organic solvents, 2,2,2-triﬂuoroethanol (TFE) and hexaﬂuoro-2propanol (HFIP), and the corresponding phase diagrams were constructed using UV−vis, NMR, and turbidity experiments. While previous studies on complex coacervates have focused almost exclusively on aqueous environments, the use of PILs in the current work enabled studies in solvents with substantially lower dielectric constants (27.0 for TFE, 16.7 for HFIP). The critical salt concentration required to induce complete miscibility was roughly 2-fold larger in HFIP compared with TFE, and two diﬀerent PIL complexes, solidlike precipitates and liquidlike coacervates, were found in both systems. This study provides insight into the eﬀects of low-dielectric-constant solvents on complex coacervation, which has not been widely studied because of the limited solubility of conventional polyelectrolytes in these media.},
	language = {en},
	number = {2},
	urldate = {2022-01-22},
	journal = {ACS Polymers Au},
	author = {Lee, Minjung and Perry, Sarah L. and Hayward, Ryan C.},
	month = oct,
	year = {2021},
	pages = {100--106},
}

@article{ylitalo_electrostatic_2021,
	title = {Electrostatic {Correlations} and {Temperature}-{Dependent} {Dielectric} {Constant} {Can} {Model} {LCST} in {Polyelectrolyte} {Complex} {Coacervation}},
	volume = {54},
	issn = {0024-9297, 1520-5835},
	url = {https://pubs.acs.org/doi/10.1021/acs.macromol.1c02000},
	doi = {10.1021/acs.macromol.1c02000},
	abstract = {The ability of polyelectrolytes to condense into a liquidlike, polyelectrolyte-rich phase out of a dilute supernatant phase through complex coacervation has led to fascinating phenomena, such as membraneless organelles and self-assembled capsules for drug delivery. Recent experiments have demonstrated that heating above a lower critical solution temperature (LCST) can drive complex coacervation. Here, we show that a coarsegrained model of electrostatic correlations is suﬃcient to model an LCST when accounting for the empirical decrease in the dielectric constant of the solvent upon heating. The predictions of the model agree qualitatively with experimental measurements of the compositions of the coexisting coacervate and supernatant phases. The model also achieves modest quantitative agreement with experiments, despite incorporating no other experimental parameters besides the dielectric constant and a ﬁtted length scale. This agreement underscores the important role that can be played by electrostatic correlations in driving complex coacervation above an LCST.},
	language = {en},
	number = {24},
	urldate = {2022-01-22},
	journal = {Macromolecules},
	author = {Ylitalo, Andrew S. and Balzer, Christopher and Zhang, Pengfei and Wang, Zhen-Gang},
	month = dec,
	year = {2021},
	pages = {11326--11337},
}

@article{li_influence_2019,
	title = {Influence of binary ionic liquid mixtures of [{BMIM}][{Cl}] and [{BMIM}][{BF4}] on isobaric vapor-liquid equilibrium of acetonitrile + water at atmospheric pressure},
	volume = {284},
	issn = {01677322},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0167732219301989},
	doi = {10.1016/j.molliq.2019.04.047},
	abstract = {The effects of ionic liquid mixtures on the phase behavior of azeotropic mixture of acetonitrile + water were presented through the experimental determinations of isobaric vapor-liquid equilibrium for acetonitrile + water + 1-butyl-3-methylimidazolium tetraﬂuoroborate ([BMIM][BF4]) and acetonitrile + water + 1-butyl-3methylimidazolium chloride ([Bmim][Cl]) + [BMIM][BF4] at atmospheric pressure (101.3 kPa). The mole ratios of [BMIM][Cl] to [BMIM][BF4] in the mixing ILs were ﬁxed at 2:1, 1:1 and 1:2, respectively. The results showed that [BMIM][BF4] was ineffective in breaking the azeotropy of acetonitrile and water, which whereas could be broken when [BMIM][Cl] reached a certain concentration in the mixing ILs. VLE data of ternary and quaternary mixtures were satisfactorily correlated and predicted with NRTL model and COSMO-SAC could give a reasonable prediction of VLE for the investigated mixtures. Additionally, the analysis of interactions among different molecules showed that the interactions between [BMIM][Cl] and water are strong while ones between [BMIM][BF4] and water weak.},
	language = {en},
	urldate = {2022-01-12},
	journal = {Journal of Molecular Liquids},
	author = {Li, Jinlong and Zhu, Hong and Peng, Changjun and Liu, Honglai},
	month = jun,
	year = {2019},
	pages = {675--681},
}

@article{bester-rogac_ion_2014,
	title = {Ion {Association} of {Imidazolium} {Ionic} {Liquids} in {Acetonitrile}},
	volume = {118},
	issn = {1520-6106, 1520-5207},
	url = {https://pubs.acs.org/doi/10.1021/jp412344a},
	doi = {10.1021/jp412344a},
	language = {en},
	number = {5},
	urldate = {2022-01-12},
	journal = {The Journal of Physical Chemistry B},
	author = {Bešter-Rogač, Marija and Stoppa, Alexander and Buchner, Richard},
	month = feb,
	year = {2014},
	pages = {1426--1435},
}

@article{nordness_characterization_2019,
	title = {Characterization of {Aqueous} 1-{Ethyl}-3-{Methylimidazolium} {Ionic} {Liquids} for {Calculation} of {Ion} {Dissociation}},
	volume = {123},
	issn = {1520-6106, 1520-5207},
	url = {https://pubs.acs.org/doi/10.1021/acs.jpcb.8b11892},
	doi = {10.1021/acs.jpcb.8b11892},
	abstract = {We employ precise measuring techniques to determine the densities, viscosities, and ionic conductivities of three aqueous 1-ethyl-3-methylimidazolium [emim]+ ionic liquid (IL) systems with minimal experimental uncertainty. We simultaneously present a novel method for estimating ion dissociation relying only on these three measurements and the estimated Stokes radii of the ions based on the Stokes−Einstein and Nernst−Einstein equations. Ion dissociation values are estimated across a range of IL concentrations, emphasizing dilute IL regions, using ionic radii calculated from widely used UNIQUAC and UNIFAC values. With these approximations and assuming the presence of only ion pairs, the ion dissociation of all three ILs reaches a minimum value at a water mole fraction of about 0.98. Upon further dilution with water, the ion dissociation increases as the system approaches inﬁnite dilution of the IL. We postulate that the apparent minimum in the ion dissociation is caused by the Stokes radii of the cation and anion increasing as the concentration becomes more dilute, due to the formation of ion triplets.},
	language = {en},
	number = {6},
	urldate = {2022-01-12},
	journal = {The Journal of Physical Chemistry B},
	author = {Nordness, Oscar and Simoni, Luke D. and Stadtherr, Mark A. and Brennecke, Joan F.},
	month = feb,
	year = {2019},
	pages = {1348--1358},
}

@article{lee_origin_2017,
	title = {The {Origin} of {Ion}-{Pairing} and {Redissociation} of {Ionic} {Liquid}},
	volume = {121},
	issn = {1520-6106, 1520-5207},
	url = {https://pubs.acs.org/doi/10.1021/acs.jpcb.7b01189},
	doi = {10.1021/acs.jpcb.7b01189},
	abstract = {We address the possible occurrence of a minimum extent of dissociation (α) of ionic liquid (IL) in IL−solvent mixtures. This phenomenon, known as the redissociation of IL, is responsible for many interesting composition-dependent properties in such mixtures. A thermodynamic model is developed to provide a semiquantitative prediction on the change of α with solvent concentration. It is found that the occurrence of minimum α coincides with the occurrence of a maximum in the mean activity coeﬃcient of dissociated ions, indicating better solvation of free, dissociated ions both with decreasing and increasing solvent concentration. The favorable solvation of free ions is found to change from long-range ion−solvent dielectric polarization to ion−ion-pair dielectric polarization with decreasing solvent concentration. Therefore, the composition dependence of the IL solution dielectric constants, determined from that of the ion-pair and the solvent, is found to be the most important factor for the presence of redissociation in IL solutions.},
	language = {en},
	number = {23},
	urldate = {2022-01-12},
	journal = {The Journal of Physical Chemistry B},
	author = {Lee, Bong-Seop and Lin, Shiang-Tai},
	month = jun,
	year = {2017},
	pages = {5818--5823},
}

@article{nordness_ion_2020,
	title = {Ion {Dissociation} in {Ionic} {Liquids} and {Ionic} {Liquid} {Solutions}},
	volume = {120},
	issn = {0009-2665, 1520-6890},
	url = {https://pubs.acs.org/doi/10.1021/acs.chemrev.0c00373},
	doi = {10.1021/acs.chemrev.0c00373},
	abstract = {The extent to which cations and anions in ionic liquids (ILs) and ionic liquid solutions are dissociated is of both fundamental scientiﬁc interest and practical importance because ion dissociation has been shown to impact viscosity, density, surface tension, volatility, solubility, chemical reactivity, and many other important chemical and physical properties. When mixed with solvents, ionic liquids provide the unique opportunity to investigate ion dissociation from inﬁnite dilution in the solvent to a completely solvent-free state, even at ambient conditions. The most common way to estimate ion dissociation in ILs and IL solutions is by comparing the molar conductivity determined from ionic conductivity measurements such as electrochemical impedance spectroscopy (EIS) (which measure the movement of only the charged, i.e., dissociated, ions) with the molar conductivity calculated from ion diﬀusivities measured by pulse ﬁeld gradient nuclear magnetic resonance spectroscopy (PFG-NMR, which gives movement of all of the ions). Because the NMR measurements are time-consuming, the number of ILs and IL solutions investigated by this method is relatively limited. We have shown that use of the Stokes−Einstein equation with estimates of the eﬀective ion Stokes radii allows ion dissociation to be calculated from easily measured density, viscosity, and ionic conductivity data (ρ, η, λ), which is readily available in the literature for a much larger number of pure ILs and IL solutions. Therefore, in this review, we present values of ion dissociation for ILs and IL solutions (aqueous and nonaqueous) determined by both the traditional molar conductivity/PFG-NMR method and the ρ, η, λ method. We explore the eﬀect of cation and anion alkyl chain length, structure, and interaction motifs of the cation and anion, temperature, and the strength of the solvent in IL solutions.},
	language = {en},
	number = {23},
	urldate = {2022-01-12},
	journal = {Chemical Reviews},
	author = {Nordness, Oscar and Brennecke, Joan F.},
	month = dec,
	year = {2020},
	pages = {12873--12902},
}

@article{de_sousa_liquid-liquid_2021,
	title = {Liquid-liquid equilibrium data for the ternary system based on ionic liquid + organic solvents + water at 298 {K} and atmospheric pressure applied in antidepressant partitioning},
	volume = {278},
	issn = {13835866},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S1383586621012405},
	doi = {10.1016/j.seppur.2021.119532},
	language = {en},
	urldate = {2022-01-12},
	journal = {Separation and Purification Technology},
	author = {de Sousa, Kênia Marcatti and Lima, Thailan Souza Pereira and de Souza, Ranyere Lucena and Nerli, Bibiana Beatriz and Pereira, Matheus M. and Soares, Cleide Mara Faria and Lima, Álvaro Silva},
	month = dec,
	year = {2021},
	pages = {119532},
}

@article{lin_modeling_2021,
	title = {Modeling dissociation of ionic liquids with electrolyte {NRTL} model},
	volume = {329},
	issn = {01677322},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0167732221002506},
	doi = {10.1016/j.molliq.2021.115524},
	abstract = {Dissociation of ionic liquids (ILs) is critical to electrochemical process performance by affecting ionic conductivity. Prior studies of thermodynamic modeling either assumed no dissociation or complete dissociation that were not consistent with experimental observations. This work presented an eNRTL model for three aqueous imidazolium-based IL systems: [Emim][EtSO4], [Emim][TFA], and [Emim][TfO]. The model accurately correlates the IL dissociation and VLE data in the entire concentration range from pure IL to inﬁnite dilution aqueous solution. The system non-ideality is dominated by the dissociation chemistry. Dissociation behavior is driven by strong short-range interaction of the molecular IL-water pair relative to the dissociated IL-water pair, consistent with prior studies indicating that molecular IL and water can form an energetically favorable complex. The interaction energy parameters calculated in this work qualitatively agrees with the hydrogen bonding ability of the anions previously reported. This work not only provides a model that well describes the IL dissociation but also demonstrates the physical signiﬁcance of eNRTL model.},
	language = {en},
	urldate = {2022-01-12},
	journal = {Journal of Molecular Liquids},
	author = {Lin, Yu-Jeng and Hossain, Nazir and Chen, Chau-Chyun},
	month = may,
	year = {2021},
	pages = {115524},
}

@article{gil-villegas_statistical_2001,
	title = {A statistical associating fluid theory for electrolyte solutions ({SAFT}-{VRE})},
	volume = {99},
	issn = {0026-8976, 1362-3028},
	url = {http://www.tandfonline.com/doi/abs/10.1080/00268970010018666},
	doi = {10.1080/00268970010018666},
	language = {en},
	number = {6},
	urldate = {2022-01-04},
	journal = {Molecular Physics},
	author = {Gil-Villegas, A. and Galindo, A. and Jackson, G.},
	month = mar,
	year = {2001},
	pages = {531--546},
}

@article{maribo-mogensen_modeling_2013,
	title = {Modeling of {Dielectric} {Properties} of {Complex} {Fluids} with an {Equation} of {State}},
	volume = {117},
	issn = {1520-6106, 1520-5207},
	url = {https://pubs.acs.org/doi/10.1021/jp310572q},
	doi = {10.1021/jp310572q},
	abstract = {The static permittivity is a key property for describing solutions containing polar and hydrogen bonding compounds. However, the precise relationship between the molecular and dielectric properties is not well-established. Here we show that the relative permittivity at zero frequency (static permittivity) can be modeled simultaneously with thermodynamic properties. The static permittivity is calculated from an extension of the framework developed by Onsager, Kirkwood, and Fröhlich to associating mixtures. The thermodynamic properties are calculated from the cubic-plusassociation (CPA) equation of state that includes the Wertheim association model as formulated in the statistical associating ﬂuid theory (SAFT) to account for hydrogen bonding molecules. We show that, by using a simple description of the geometry of the association, we may calculate the Kirkwood g-factor as a function of the probability of hydrogen bond formation. The results show that it is possible to predict the static permittivity of complex mixtures over wide temperature and pressure ranges from simple extensions of well-established theories simultaneously with the calculation of thermodynamic properties.},
	language = {en},
	number = {12},
	urldate = {2022-01-04},
	journal = {The Journal of Physical Chemistry B},
	author = {Maribo-Mogensen, Bjørn and Kontogeorgis, Georgios M. and Thomsen, Kaj},
	month = mar,
	year = {2013},
	pages = {3389--3397},
}

@article{maribo-mogensen_modeling_2013-1,
	title = {Modeling of {Dielectric} {Properties} of {Aqueous} {Salt} {Solutions} with an {Equation} of {State}},
	volume = {117},
	issn = {1520-6106, 1520-5207},
	url = {https://pubs.acs.org/doi/10.1021/jp403375t},
	doi = {10.1021/jp403375t},
	abstract = {The static permittivity is the most important physical property for thermodynamic models that account for the electrostatic interactions between ions. The measured static permittivity in mixtures containing electrolytes is reduced due to kinetic depolarization and reorientation of the dipoles in the electrical ﬁeld surrounding ions. Kinetic depolarization may explain 25−75\% of the observed decrease in the permittivity of solutions containing salts, but since this is a dynamic property, this eﬀect should not be included in the thermodynamic modeling of electrolytes. Kinetic depolarization has, however, been ignored in relation to thermodynamic modeling, and authors have either neglected the eﬀect of salts on permittivity or used empirical correlations ﬁtted to the measured static permittivity, leading to an overestimation of the reduction in the thermodynamic static permittivity. We present a new methodology for obtaining the static permittivity over wide ranges of temperatures, pressures, and compositions for use within an equation of state for mixed solvents containing salts. The static permittivity is calculated from a new extension of the framework developed by Onsager, Kirkwood, and Fröhlich to associating mixtures. Wertheim’s association model as formulated in the statistical associating ﬂuid theory is used to account for hydrogenbonding molecules and ion−solvent association. Finally, we compare the Debye−Hückel Helmholtz energy obtained using an empirical model with the new physical model and show that the empirical models may introduce unphysical behavior in the equation of state.},
	language = {en},
	number = {36},
	urldate = {2022-01-04},
	journal = {The Journal of Physical Chemistry B},
	author = {Maribo-Mogensen, Bjørn and Kontogeorgis, Georgios M. and Thomsen, Kaj},
	month = sep,
	year = {2013},
	pages = {10523--10533},
}

@article{zhuang_like_2021,
	title = {Like dissolves like: {A} first-principles theory for predicting liquid miscibility and mixture dielectric constant},
	volume = {7},
	issn = {2375-2548},
	shorttitle = {Like dissolves like},
	url = {https://www.science.org/doi/10.1126/sciadv.abe7275},
	doi = {10.1126/sciadv.abe7275},
	language = {en},
	number = {7},
	urldate = {2022-01-04},
	journal = {Science Advances},
	author = {Zhuang, Bilin and Ramanauskaite, Gabriele and Koa, Zhao Yuan and Wang, Zhen-Gang},
	month = feb,
	year = {2021},
	pages = {eabe7275},
}

@article{lee_unusual_2012,
	title = {Unusual {Lower} {Critical} {Solution} {Temperature} {Phase} {Behavior} of {Poly}(ethylene oxide) in {Ionic} {Liquids}},
	volume = {45},
	issn = {0024-9297, 1520-5835},
	url = {https://pubs.acs.org/doi/10.1021/ma300335p},
	doi = {10.1021/ma300335p},
	abstract = {We describe the LCST-type phase behavior of poly(ethylene oxide) (PEO) dissolved in imidazolium-based tetraﬂuoroborate ionic liquids (ILs). Phase diagrams were determined by a combination of small-angle neutron scattering (SANS) and cloud point (CP) measurements. Unlike typical LCST phase diagrams of polymer solutions, the PEO/IL phase diagram is either roughly symmetric with a critical composition near 50\% polymer or asymmetric with a critical composition shifted to an even higher concentration of PEO. As the molecular weight decreases from 20 500 to 4200 g/mol, the critical temperature (Tc) increases slightly (∼10 °C). However, a larger increase in Tc (27 °C) was observed as the molecular weight decreases from 4200 to 2100 g/mol, likely due to the increasing importance of hydrogen bonds between the −OH end groups of PEO and the ﬂuorine atoms of the anions. This inference is supported by the strong dependence of the phase diagram on the identity of the PEO end groups (hydroxy vs methoxy). Furthermore, replacing the most acidic proton of the imidazolium ring (in the C2 position) with a methyl group lowers the Tc and changes the shape of the phase diagram signiﬁcantly, suggesting that the hydrogen bonds between the H atoms on the C2 position of the imidazolium ring and the O atoms of PEO play an important role in determining the LCST phase behavior of this system.},
	language = {en},
	number = {8},
	urldate = {2021-10-13},
	journal = {Macromolecules},
	author = {Lee, Hau-Nan and Newell, Nakisha and Bai, Zhifeng and Lodge, Timothy P.},
	month = apr,
	year = {2012},
	pages = {3627--3633},
}

@article{stoychev_modeling_2009,
	title = {Modeling the {Phase} {Behavior} of {PEO}−{PPO}−{PEO} {Surfactants} in {Carbon} {Dioxide} {Using} the {PC}-{SAFT} {Equation} of {State}: {Application} to {Dry} {Decontamination} of {Solid} {Substrates}},
	volume = {54},
	issn = {0021-9568, 1520-5134},
	shorttitle = {Modeling the {Phase} {Behavior} of {PEO}−{PPO}−{PEO} {Surfactants} in {Carbon} {Dioxide} {Using} the {PC}-{SAFT} {Equation} of {State}},
	url = {https://pubs.acs.org/doi/10.1021/je800875k},
	doi = {10.1021/je800875k},
	language = {en},
	number = {5},
	urldate = {2021-10-12},
	journal = {Journal of Chemical \& Engineering Data},
	author = {Stoychev, Ivan and Galy, Julien and Fournel, Bruno and Lacroix-Desmazes, Patrick and Kleiner, Matthias and Sadowski, Gabriele},
	month = may,
	year = {2009},
	pages = {1551--1559},
}

@article{lee_lower_2010,
	title = {Lower {Critical} {Solution} {Temperature} ({LCST}) {Phase} {Behavior} of {Poly}(ethylene oxide) in {Ionic} {Liquids}},
	volume = {1},
	issn = {1948-7185, 1948-7185},
	url = {https://pubs.acs.org/doi/10.1021/jz100617t},
	doi = {10.1021/jz100617t},
	abstract = {We describe the LCST-type phase behavior of poly(ethylene oxide) (PEO) (M = 5000 and 20000) dissolved in 1,3-dialkylimidazolium tetrafluoroborate ionic liquids. The phase transition temperatures were identified using cloud point measurements. In these PEO/ionic liquid systems, liquid-liquid phase separation is observed in the temperature range from 130 to 170 °C. We report unusual temperature-composition phase diagrams in which the cloud point curves are strongly asymmetric, with the critical composition (wc) shifted to high concentrations of PEO. The critical temperature (Tc) and the critical composition (wc) of these systems are not a strong function of the molecular weight of PEO. In addition, the values of the LCST increase as the length of the alkyl chain in the imidazolium cation increases. By using ionic liquid blends as solvents, the LCSTs can be tuned by varying the mixing ratio of two ionic liquids.},
	language = {en},
	number = {13},
	urldate = {2021-09-30},
	journal = {The Journal of Physical Chemistry Letters},
	author = {Lee, Hau-Nan and Lodge, Timothy P.},
	month = jul,
	year = {2010},
	pages = {1962--1966},
}

@article{paduszynski_thermodynamic_2012,
	title = {Thermodynamic {Modeling} of {Ionic} {Liquid} {Systems}: {Development} and {Detailed} {Overview} of {Novel} {Methodology} {Based} on the {PC}-{SAFT}},
	volume = {116},
	issn = {1520-6106, 1520-5207},
	shorttitle = {Thermodynamic {Modeling} of {Ionic} {Liquid} {Systems}},
	url = {https://pubs.acs.org/doi/10.1021/jp3009207},
	doi = {10.1021/jp3009207},
	abstract = {We present the results of an extensive study on a novel approach of modeling ionic liquids (ILs) and their mixtures with molecular compounds, incorporating perturbed-chain statistical associating ﬂuid theory (PC-SAFT). PC-SAFT was used to calculate the thermodynamic properties of diﬀerent homologous series of ILs based on the bis(triﬂuormethylsulfonyl)imide anion ([NTf2]). First, pure ﬂuid parameters were obtained for each IL by means of ﬁtting the model predictions to experimental liquid densities over a broad range of temperature and pressure. The reliability and physical signiﬁcance of the parameters as well as the employed molecular scheme were tested by calculation of density, vapor pressure, and other properties of pure ILs (e.g., critical properties, normal boiling point). Additionally, the surface tension of pure ILs was calculated by coupling the PC-SAFT equation of state with density gradient theory (DGT). All correlated/predicted results were compared with literature experimental or simulation data. Afterward, we attempted to model various thermodynamic properties of some binary systems composed of IL and organic solvent or water. The properties under study were the binary vapor−liquid, liquid−liquid, and solid−liquid equilibria and the excess enthalpies of mixing. To calculate cross-interaction energies we used the standard combining rules of Lorentz−Berthelot, Kleiner−Sadowski, and Wolbach− Sandler. It was shown that incorporation of temperature-dependent binary corrections was required to obtain much more accurate results than in the case of conventional predictions. Binary corrections were adjusted to inﬁnite dilution activity coeﬃcients of a particular solute in a given IL determined experimentally or predicted by means of the modiﬁed UNIFAC (Dortmund) group contribution method. We concluded that the latter method allows accurate and reliable calculations of bulkphase properties in a totally predictive manner.},
	language = {en},
	number = {16},
	urldate = {2021-09-30},
	journal = {The Journal of Physical Chemistry B},
	author = {Paduszyński, Kamil and Domańska, Urszula},
	month = apr,
	year = {2012},
	pages = {5002--5018},
}

@article{carneiro_solubility_2013,
	title = {Solubility of {Sugars} and {Sugar} {Alcohols} in {Ionic} {Liquids}: {Measurement} and {PC}-{SAFT} {Modeling}},
	volume = {117},
	issn = {1520-6106, 1520-5207},
	shorttitle = {Solubility of {Sugars} and {Sugar} {Alcohols} in {Ionic} {Liquids}},
	url = {https://pubs.acs.org/doi/10.1021/jp404864c},
	doi = {10.1021/jp404864c},
	abstract = {Bioreﬁning processes using ionic liquids (ILs) require proper solubility data of biomass-based compounds in ILs, as well as an appropriate thermodynamic approach for the modeling of such data. Carbohydrates and their derivatives such as sugar alcohols represent a class of compounds that could play an important role in bioreﬁning. Thus, in this work, the pure IL density and solubility of xylitol and sorbitol in ﬁve diﬀerent ILs were measured between 288 and 339 K. The ILs under consideration were 1-ethyl-3-methylimidazolium dicyanamide, 1-butyl-3-methylimidazolium dicyanamide ([bmim][DCA]), Aliquat dicyanamide, trihexyltetradecylphosphonium dicyanamide, and 1-ethyl-3-methylimidazolium triﬂuoroacetate. Comparison with the literature data was performed, showing good agreement. With the exception of [bmim][DCA], the solubility of these sugar alcohols in the other ILs is presented for the ﬁrst time. The measured data as well as previously published solubility data of glucose and fructose in these ILs were modeled by means of PC-SAFT using a molecular-based associative approach for ILs. PC-SAFT was used in this work as it has shown to be applicable to model the solubility of xylitol and sorbitol in ILs (Paduszyński; et al. J. Phys. Chem. B 2013, 117, 7034−7046). For this purpose, three pure IL parameters were ﬁtted to pure IL densities, activity coeﬃcients of 1-propanol at inﬁnite dilution in ILs, and/or xylitol solubility in ILs. This approach allows accurate modeling of the pure IL data and the mixture data with only one binary interaction parameter kij between sugar and the IL or sugar alcohol and the IL. In cases where only the pure IL density and activity coeﬃcients of 1-propanol at inﬁnite dilution in ILs were used for the IL parameter estimation, the solubility of the sugars and sugar alcohols in the ILs could be predicted (kij = 0 between sugar and the IL or sugar alcohol and the IL) with reasonable accuracy.},
	language = {en},
	number = {34},
	urldate = {2021-09-30},
	journal = {The Journal of Physical Chemistry B},
	author = {Carneiro, Aristides P. and Held, Christoph and Rodríguez, Oscar and Sadowski, Gabriele and Macedo, Eugénia A.},
	month = aug,
	year = {2013},
	pages = {9980--9995},
}

@article{white_origins_2013,
	title = {Origins of {Unusual} {Phase} {Behavior} in {Polymer}/{Ionic} {Liquid} {Solutions}},
	volume = {46},
	issn = {0024-9297, 1520-5835},
	url = {https://pubs.acs.org/doi/10.1021/ma400710z},
	doi = {10.1021/ma400710z},
	abstract = {Recent experimental studies [Lee et al. Macromolecules 2012, 45, 3627−3633] on polymer/IL solutions of poly(ethylene oxide) (PEO) and 1-ethyl-3-methylimidazolium tetraﬂuoroborate ([EMIM][BF4]) show some striking trends in the phase boundaries. While most polymer solutions have critical compositions (ϕcrit) that are solvent-rich, these systems had phase diagrams that were either roughly symmetric (ϕcrit ≈ 50\%), or, in other related systems, had ϕcrit shifted even more toward polymer-rich compositions. In this work, we carry out a modeling investigation to probe the origins of this shift in the location of the critical composition. There appear to be two underlying sources: The ﬁrst is a signiﬁcantly stronger cohesive energy density, and lowered free volume, for the pure solvent component relative to the pure polymer component. This manifests itself as a “role reversal” in the pure component energetic parameters, compared to those of more typical polymer solutions. The resulting unfavorable entropic eﬀects in the mixture produce a coexistence curve shifted toward compositions that are richer in the component with the lower cohesive energy densityin this case the polymer component. The second factor is the aggregation of the ionic liquid component, eﬀectively reducing (and repositioning) the ideal contribution to the entropy of mixing relative to what would result if the IL were fully dispersed. Evidence for IL aggregation is discussed in the context of a simple model to predict aggregation in a dielectric continuum. In agreement with experiment, both of these factors (role reversal in energetics and IL aggregation) serve to shift the critical composition to the more polymer-rich side of the phase diagram compared to what is found for more typical polymer solutions.},
	language = {en},
	number = {14},
	urldate = {2021-09-30},
	journal = {Macromolecules},
	author = {White, Ronald P. and Lipson, Jane E. G.},
	month = jul,
	year = {2013},
	pages = {5714--5723},
}

@article{hoarfrost_lower_2013,
	title = {Lower {Critical} {Solution} {Temperature} {Phase} {Behavior} of {Poly}( \textit{n} -butyl methacrylate) in {Ionic} {Liquid} {Mixtures}},
	volume = {46},
	issn = {0024-9297, 1520-5835},
	url = {https://pubs.acs.org/doi/10.1021/ma401450w},
	doi = {10.1021/ma401450w},
	abstract = {Ionic liquids feature a combination of properties that make them very interesting solvents for polymers, but many questions remain regarding the thermodynamics of polymer/ionic liquid solutions. In this work, the lower-criticalsolution-temperature (LCST) phase behavior of poly(n-butyl methacrylate) (PnBMA) in mixtures of the ionic liquids 1butyl-3-methylimidazolium:bis(triﬂuoromethylsulfonyl)imide ([BMIm][TFSI]) and 1-ethyl-3-methylimidazolium:TFSI ([EMIm][TFSI]) is characterized by transmittance, light scattering, and small-angle neutron scattering measurements. Several relevant thermodynamic parameters are easily tuned by varying the ionic liquid composition. In particular, the cloud point, spinodal, and Θ temperatures are all found to increase linearly with [BMIm] content. The interaction parameters, χ, are determined as a function of temperature and concentration using three diﬀerent methods, and the results from each method are compared. The entropic and enthalpic components of the interaction parameter, χ, are also found to vary linearly with [BMIm] content in the ionic liquid, increasing and decreasing, respectively. The increase in the enthalpic driving force for mixing with increasing [BMIm] content dominates over the decrease in the entropic penalty for mixing, leading to improved solubility. This result is discussed in terms of molecular interactions and oriented solvation. This work characterizes the solution thermodynamics of one representative system in a very interesting class of polymer solutions, and provides insight into the molecular mechanisms underlying its LCST phase behavior.},
	language = {en},
	number = {23},
	urldate = {2021-09-30},
	journal = {Macromolecules},
	author = {Hoarfrost, Megan L. and He, Yanpu and Lodge, Timothy P.},
	month = dec,
	year = {2013},
	pages = {9464--9472},
}

@article{jung_phase_2020,
	title = {Phase {Behavior} of {Poly}(ethylene oxide) in {Room} {Temperature} {Ionic} {Liquids}: {A} {Molecular} {Simulation} and {Deep} {Neural} {Network} {Study}},
	volume = {124},
	issn = {1520-6106, 1520-5207},
	shorttitle = {Phase {Behavior} of {Poly}(ethylene oxide) in {Room} {Temperature} {Ionic} {Liquids}},
	url = {https://pubs.acs.org/doi/10.1021/acs.jpcb.0c06510},
	doi = {10.1021/acs.jpcb.0c06510},
	abstract = {The phase behavior of polymers in room temperature ionic liquids is a topic of considerable interest. In this work we study the phase diagram of poly(ethylene oxide) in four imidazolium ionic liquids (ILs) using molecular simulation. We develop united atom models for 1-butyl-2,3-dimethylimidazolium ([BMMIM]), 1-ethyl-2,3-dimethylimidazolium ([EMMIM]), and 1-ethyl-3-methylimidazolium ([EMIM]) in an analogous fashion to previously developed models for 1-butyl-3-methylimidazolium ([BMIM]) and tetraﬂuoroborate ([BF4]) using symmetry-adapted perturbation theory. At high temperatures we obtain the coexistence concentrations using an interface method where the polymer and IL are simulated in a large elongated box, and an interface between coexisting phases is formed. At lower temperatures we use a deep neural network (DNN) method. The input descriptors for the DNN are the cohesive energy of mixing, the volume change of mixing, and the coordination numbers between cation and polymer, all of which are obtained from simulations of mixed systems at a series of temperatures. The DNN is trained by using the phase-separated systems at high temperatures and a mixed phase at low temperatures. The method predicts a lower critical solution temperature which decreases as the alkyl chain length on the cation is decreased, consistent with experiment. The simulations show that methylation of the cation has little eﬀect on the phase diagram. This is in contrast to what is seen in experiments but could be because the polymer chains in the simulations are too short. At low temperatures the chains display two conformational motifs, namely a crown ether conformation and a ring conformation, each of which can wrap the chain around a single cation. This provides the entropic penalty for mixing and a reason for demixing as the temperature is raised. Such conformations might not be possible for longer chains. The combination of data-driven techniques and molecular simulation shows promise in the study of the phase behavior and physical properties of complex ﬂuids.},
	language = {en},
	number = {41},
	urldate = {2021-09-30},
	journal = {The Journal of Physical Chemistry B},
	author = {Jung, Hyuntae and Yethiraj, Arun},
	month = oct,
	year = {2020},
	pages = {9230--9238},
}

@article{gao_polarization_2021,
	title = {Polarization of ionic liquid and polymer and its implications for polymerized ionic liquids: {An} overview towards a new theory and simulation},
	issn = {2642-4150, 2642-4169},
	shorttitle = {Polarization of ionic liquid and polymer and its implications for polymerized ionic liquids},
	url = {https://onlinelibrary.wiley.com/doi/10.1002/pol.20210330},
	doi = {10.1002/pol.20210330},
	abstract = {Ionic liquid (IL)-containing polymers garner attention for electrochemical applications. This article overviews recent experimental and theoretical studies of polymer electrolytes that would be likely to cultivate new theoretical and computational frameworks for IL-containing polymers. The first two sections outline the uniqueness of ILs that differentiates them from inorganic salts in polymers and explore deviation from the concept of the metaphor “roomtemperature molten salt.” Such distinct properties include (1) large intrinsic dipole moment and electronic polarizability, (2) hydrogen bonding, (3) π-interactions, (4) a broad distribution of charges over the entire ion, and (5) the anisotropy of the ions. Moreover, the complexity of these properties substantially increases when the ions are polymerized. Indeed, their exceptional features would overcome the hurdle due to a trade-off between ionic conductivity and mechanical robustness in inorganic salt-doped polymers. Given these facts, the rest of the article focuses on emerging trends in the study of the dielectric response, phase separation, ion conductivity, and mechanical robustness of the polymer electrolytes, highlighting outstanding observations in experiments that may inspire existing theory and simulation. Our discussion also includes improving computational complexity for IL-containing polymers. To this end, recent machine learning studies that consider ILs and polymer liquids are presented.},
	language = {en},
	urldate = {2021-09-30},
	journal = {Journal of Polymer Science},
	author = {Gao, Tong and Itliong, Jester and Kumar, Sai Prashanth and Hjorth, Zackerie and Nakamura, Issei},
	month = aug,
	year = {2021},
	pages = {pol.20210330},
}

@article{li_salt-induced_2021,
	title = {Salt-{Induced} {Liquid}–{Liquid} {Phase} {Separation}: {Combined} {Experimental} and {Theoretical} {Investigation} of {Water}–{Acetonitrile}–{Salt} {Mixtures}},
	volume = {143},
	issn = {0002-7863, 1520-5126},
	shorttitle = {Salt-{Induced} {Liquid}–{Liquid} {Phase} {Separation}},
	url = {https://pubs.acs.org/doi/10.1021/jacs.0c09420},
	doi = {10.1021/jacs.0c09420},
	abstract = {Salt-induced liquid−liquid phase separation in liquid mixtures is a common phenomenon in nature and in various applications, such as in separation and extraction of chemicals. Here, we present results of a systematic investigation of the phase behaviors in water−acetonitrile−salt mixtures using a combination of experiment and theory. We obtain complete ternary phase diagrams for nine representative salts in water− acetonitrile mixtures by cloud point and component analysis. We construct a thermodynamic free energy model by accounting for the nonideal mixing of the liquids, ion hydration, electrostatic interactions, and Born energy. Our theory yields phase diagrams in good agreement with the experimental data. By comparing the contributions due to the electrostatic interaction, Born energy, and hydration, we ﬁnd that hydration is the main driving force for the liquid−liquid separation and is a major contributor to the speciﬁc ion eﬀects. Our theory highlights the important role of entropy in the hydration driving force. We discuss the implications of our ﬁndings in the context of salting-out assisted liquid−liquid extraction and make suggestions for selecting salt ions to optimize the separation performance.},
	language = {en},
	number = {2},
	urldate = {2021-09-30},
	journal = {Journal of the American Chemical Society},
	author = {Li, Minglun and Zhuang, Bilin and Lu, Yuyuan and An, Lijia and Wang, Zhen-Gang},
	month = jan,
	year = {2021},
	pages = {773--784},
}

@article{kjellander_multiple_2020,
	title = {A multiple decay-length extension of the {Debye}–{Hückel} theory: to achieve high accuracy also for concentrated solutions and explain under-screening in dilute symmetric electrolytes},
	volume = {22},
	issn = {1463-9076, 1463-9084},
	shorttitle = {A multiple decay-length extension of the {Debye}–{Hückel} theory},
	url = {http://xlink.rsc.org/?DOI=D0CP02742A},
	doi = {10.1039/D0CP02742A},
	abstract = {Very accurate pair distributions and thermodynamics of electrolytes from multiple Debye–Hückel-type decay components, which become oscillatory when appropriate.
          , 
            
              The Poisson–Boltzmann and Debye–Hückel approximations for the pair distributions and mean electrostatic potential in electrolytes predict that these entities have one single decay mode with a decay length equal to the Debye length 1/
              κ
              D
              , that is, they have a characteristic contribution that decays with distance
              r
              like e
              −κDr
              /
              r
              . However, in reality, electrolytes have several decay modes e
              −κr
              /
              r
              , e
              −κ′r
              /
              r etc.
              with different decay lengths, 1
              /κ
              , 1
              /κ
              ′
              etc.
              , that in general are different from the Debye length. As an illustration of the significance of multiple decay modes in electrolytes, the present work uses a very simple extension of the Debye–Hückel approximation with two decay lengths, which predicts oscillatory modes when appropriate. This approach gives very accurate results for radial distribution functions and thermodynamic properties of aqueous solutions of monovalent electrolytes for all concentrations investigated, including high ones. It is designed to satisfy necessary statistical mechanical conditions for the distributions. The effective dielectric permittivity of the electrolyte plays an important role in the theory and each mode has its own value of this entity. Electrolytes with high electrostatic coupling, like those with multivalent ions and/or with solvent of low dielectric constant, have decay lengths in dilute solutions that substantially deviate from the Debye length. It is shown that this is caused by nonlinear ion–ion correlation effects and the origin of under-screening,
              i.e.
              , 1/
              κ
              {\textgreater} 1/
              κ
              D
              , in dilute symmetric electrolytes is analyzed. The under-screening is accompanied by an increase in the effective dielectric permittivity that is also caused by these correlations. The theoretical results for the decay length are successfully compared with recent experimental data for simple electrolytes in various solvents. The paper includes background material on electrolyte theory and screening in order to be accessible for nonexperts in the field.},
	language = {en},
	number = {41},
	urldate = {2021-09-30},
	journal = {Physical Chemistry Chemical Physics},
	author = {Kjellander, Roland},
	year = {2020},
	pages = {23952--23985},
}

@article{huang_confinement_2018,
	title = {Confinement {Induced} {Dilution}: {Electrostatic} {Screening} {Length} {Anomaly} in {Concentrated} {Electrolytes} in {Confined} {Space}},
	volume = {122},
	issn = {1932-7447, 1932-7455},
	shorttitle = {Confinement {Induced} {Dilution}},
	url = {https://pubs.acs.org/doi/10.1021/acs.jpcc.7b11093},
	doi = {10.1021/acs.jpcc.7b11093},
	abstract = {For electrolytes conﬁned in nanoscale space, a growing body of experimental evidence suggests that the electrostatic screening length (or Debye length) increases with the electrolyte concentration in the concentrated regime (e.g., ionic liquids). This electrostatic screening length anomaly can be understood under the assumption of an eﬀectively dilute electrolyte due to massive ion-pairing, which, however, contradicts with the conventional wisdom that ionic liquids are highly dissociated, given the negative free energy of dissociation. To resolve this puzzle, a phenomenological theory is developed to understand ion-pair dissociation in electrolytes in conf ined space. Nanoconﬁnement suppresses lattice expansion upon ion-pair dissociation, shifting the eﬀective free energy of dissociation toward positive values, favoring massive ion-pairing, and rendering a long electrostatic screening length. The dependence of the electrostatic screening length on the temperature and the ionic size is discussed. It is of high priority to investigate the nanoconﬁnement eﬀect of the diﬀerential double-layer capacitance Cdl to further corroborate the conﬁnement induced dilution phenomenon.},
	language = {en},
	number = {6},
	urldate = {2021-09-30},
	journal = {The Journal of Physical Chemistry C},
	author = {Huang, Jun},
	month = feb,
	year = {2018},
	pages = {3428--3433},
}

@article{smith_electrostatic_2016,
	title = {The {Electrostatic} {Screening} {Length} in {Concentrated} {Electrolytes} {Increases} with {Concentration}},
	volume = {7},
	issn = {1948-7185, 1948-7185},
	url = {https://pubs.acs.org/doi/10.1021/acs.jpclett.6b00867},
	doi = {10.1021/acs.jpclett.6b00867},
	abstract = {According to classical electrolyte theories interactions in dilute (low ion density) electrolytes decay exponentially with distance, with the Debye screening length the characteristic length scale. This decay length decreases monotonically with increasing ion concentration due to eﬀective screening of charges over short distances. Thus, within the Debye model no long-range forces are expected in concentrated electrolytes. Here we reveal, using experimental detection of the interaction between two planar charged surfaces across a wide range of electrolytes, that beyond the dilute (Debye−Hückel) regime the screening length increases with increasing concentration. The screening lengths for all electrolytes studiedincluding aqueous NaCl solutions, ionic liquids diluted with propylene carbonate, and pure ionic liquidscollapse onto a single curve when scaled by the dielectric constant. This nonmonotonic variation of the screening length with concentration, and its generality across ionic liquids and aqueous salt solutions, demonstrates an important characteristic of concentrated electrolytes of substantial relevance from biology to energy storage.},
	language = {en},
	number = {12},
	urldate = {2021-09-30},
	journal = {The Journal of Physical Chemistry Letters},
	author = {Smith, Alexander M. and Lee, Alpha A. and Perkin, Susan},
	month = jun,
	year = {2016},
	pages = {2157--2163},
}

@article{inguva_introducing_2021,
	title = {Introducing students to research codes: {A} short course on solving partial differential equations in {Python}},
	volume = {36},
	copyright = {All rights reserved},
	issn = {17497728},
	shorttitle = {Introducing students to research codes},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S1749772821000117},
	doi = {10.1016/j.ece.2021.01.011},
	language = {en},
	urldate = {2021-09-27},
	journal = {Education for Chemical Engineers},
	author = {Inguva, Pavan and Bhute, Vijesh J. and Cheng, Thomas N.H. and Walker, Pierre J.},
	month = jul,
	year = {2021},
	pages = {1--11},
}

